Two beams are better than one: Enabling reliable and high throughput mmWave links

Millimeter-wave communication with high throughput and high reliability is poised to be a gamechanger for V2X and VR applications. However, mmWave links are notorious for low reliability since they suffer from frequent outages due to blockage and user mobility. We build mmReliable, a reliable mmWave system that implements multi-beamforming and user tracking to handle environmental vulnerabilities. It creates constructive multi-beam patterns and optimizes their angle, phase, and amplitude to maximize the signal strength at the receiver. Multi-beam links are reliable since they are resilient to occasional blockages of few constituent beams compared to a single-beam system. We implement mmReliable on a 28 GHz testbed with 400 MHz bandwidth, and a 64 element phased array supporting 5G NR waveforms. Rigorous indoor and outdoor experiments demonstrate that mmReliable achieves close to 100\% reliability providing 2.3x improvement in the throughput-reliability product than single-beam systems. This is an extended version of a paper published in Sigcomm'21.

==> Arxiv/1_intro_v10.tex <==
% !TEX root = main.tex
% main intro from Sigcomm original submission

\vspace{-0.15in}
\section{Introduction}\label{sec:intro}

5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, 
defined as the fraction of time during which the link does not suffer an outage~\cite{driscoll2017enabling,ji2018ultra}. 
%In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that 
can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and therefore suffers from severe outage due to blockage and user's mobility. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that human blockages always bring down the link to an outage, which
is detrimental for high-reliability applications~\cite{ji2018ultra}.

% For example, blockage can reduce the signal strength by 20 dB, leading to an outage (no connectivity) for an extended period of 500 ms~\cite{maccartney2017rapid}, which is detrimental for high-reliability applications \cite{ji2018ultra}.
%When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam.
% Sub-6 GHz WiFi achieves high data-rate using spatial multiplexing which is function of existence of diverse multi-path in environment . However, 
% therefore even without multiplexing it can achieve multi-Gbps
% ~\footnote{Note that WiFi achieves high data-rate using spatial multiplexing which is function of existence of  diverse multi-path in environment and mmWave uses high bandwidth to achieve the same, but only requires existence  of a path between transmitter and receiver.}. To achieve 
% High bandwidth and directional beams allow mmWave to achieve high data rates required for video streaming applications.
% However, the directional link is vulnerable to blockages, device rotation, and user's mobility. A mobile blocker can reduce the signal strength by 20 dB, leading to outage which can be for an extended period of 500 ms~\cite{maccartney2017rapid}. When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam. In outdoor scenarios beam misalignment issue aggravates, 
% mmWave network if used for V2X has to support up to 500 km/h mobility while maintaining high throughput, high reliability, and ultra-low latency, which is challenging to achieve.
% Traditionally, mmWave network is optimized to provide high throughput of the order of a multi-Gbps~\cite{CellularCap-Rap}, thanks to high bandwidth and directional beams to combat higher pathloss at mmWave frequencies. 
%  The mmWave link can also degrade due to beam misalignment caused by device rotation and user's mobility.

Ideally, we want to create a reliable mmWave link (a link without outage) that achieves high data-rate, and easy to deploy with upcoming 5G infrastructure. However, conventional mmWave design~\cite{ieee80211ad} centers on improving the link throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive,Xarray2020} and coverage~\cite{zhou2019robot,wei2017facilitating}, which ends up sacrificing the reliability requirement. The mmWave base station and the user tediously scan multiple beams to establish a directional link through \textit{beam training}. The beam training process is usually \textit{reactive}~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} which kicks in only after a significant degradation in link quality, leading to loss of connectivity and thereof reliability.
To improve reliability, some approaches are \textit{proactive}, that act before the link degrades by tracking the user with side-channel information from out-of-band LTE/WiFi~\cite{sur2017wifi,nitsche2015steering} or rely on external sensors. These solutions apart from not being ubiquitous and self-reliant, have limited accuracy ~\cite{haider2018listeer,zhou2018following,wei2017pose,va2015beam}. All these approaches make the system difficult to deploy and dependant on external information.
In contrast, our goal is to improve the inherent continuity and reliability of mmWave link and overall throughput without side-channel or external information.


% \textit{Long outage duration and high frequency of prolonged beam training reduce the reliability of mmWave link.}

% fast handover~\cite{sur2018towards} or joint transmission from multiple APs~\cite{zhang2018mmchoir}.

% Though most research focuses on reducing the beam training delay, the delay generally increases with the size of the phased array~\cite{abari2016millimeter,barati2016initial,hassanieh2018fast}. 
%Besides, the beam training process has to be triggered frequently to avoid the harmful consequences of blockage and the user's mobility.

% In this work, we ask, can we achieve high-reliability mmWave links?  Traditionally, mmWave work has focused on blockage mitigation and beam alignment procedures \cite{sur2016beamspy,hassanieh2018fast} intending to improve the link throughput, which inadvertently ends up relegating the reliability requirement, leading to prolonged outages. The mmWave AP and the user periodically scan multiple beams in their codebook to find the right directional beam, commonly known as \textit{beam training}. The beam training process has to be triggered more frequently to avoid the harmful consequences of blockage and the user's mobility and can last as long as 10 msec for a codebook of a large antenna array~\cite{ieee80211ad}. Furthermore, blockage/user mobility detection is usually reactive~\cite{feng2017dealing} and may kick in only after significant detrimental impact on link quality, leading to loss of reliability. Some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam to avoid signal degradation due to mobility, but at the cost of significantly lower throughput while still being susceptible to outage due to blockages. \textit{Long outage duration, high frequency of beam training, and long beam training delays reduce the reliability of mmWave link.}
% The beam training is conducted to recover from outage or initial beam training, . %for communication through a process commonly known as \textit{beam training}. Although beam training has been studied extensively \textcolor{red}{[cite]}, the beam training delay is of the order of the logarithm of number of beams in the codebook~\cite{dina}. The codebook size for a large phased array can be huge, and the training takes order of a few 10 ms, during which there is no communication.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/mmreliable_prototype_v2.pdf}
    \caption{\name utilizes beams with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beams}
    \label{fig:prototype}
    \vspace{-0.18in}
\end{figure}
% to take advantage of multi-path caused by strong reflectors in the environment to improve reliability. We get insights
% \textbf{\name's first design principle} is inspired from sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. To improve reliability, some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam as shown in Figure~\ref{fig:prototype}(a). However, a wide-beam suffers from significantly lower throughput and connectivity range while still being susceptible to outage due to blockages. In contrast, \name creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that are aligned towards LOS or strong reflected paths as shown in Figure~\ref{fig:prototype}(b). The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 



% In this paper, we present \name, which intends to create a reliable mmWave link, while maintaining high data rates. We get the insights from sub-6 GHz communication which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. 
% \name's first design principle is slightly counter-intuitive, where it creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that take advantage of multi-path caused by strong reflectors in the environment as shown in Figure~\ref{fig:prototype} (b). Beam splitting may reduce the range of connectivity, but provides reliability. 
% The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Notably, multi-beam provides an advantage in terms of range and throughput compared to a wide-beam since all the beams in a multi-beam pattern are aligned towards LOS or strong reflected paths. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

% Multi-lobe pattern has been used in MUTE and BounceNet ~\cite{jog2019many, ghasempour2018multi}.

% Theory work xxx needs channel by decoupling beam patterns which is challenging and time consuming [ACO, ]

In this paper, we introduce \name, a system which achieves both high-reliability and high-data-rate mmWave links, while being 5G NR compliant. \name is inspired by sub-6 GHz communication,  
% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
%\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.
%
%\textbf{\name's first design principle} is inspired by sub-6 GHz communication, 
which delivers high reliability and throughput, by exploiting multipath diversity from environmental reflections
% \cite{addmmwave citation as well here}. 
However, the same is not valid for traditional mmWave, which uses a single RF chain creating a single directional beam along the Line of Sight (LOS) or toward a strong reflector (NLOS). 
\name uses single RF chain to create custom beam patterns with multiple directional beam (\textit{multi-beam}) that are each aligned towards LOS and strong reflected paths, while keeping the Total Radiated Power (TRP) same as a single beam (FCC compliant), as shown in Fig.~\ref{fig:prototype}(b). 
The idea here is that probability of multiple beams simultaneously facing a blockage is low, reducing the possibility of link outage and increasing reliability. 

% \todo{no!!, you are performing constrcutive combining which is helping it improve SNR!! talk about constructive combining and then give the example, your techniques should be summarized here...} 

An obvious implication of splitting the single beam to a multi-beam is loss in power per beam to meet the total radiated power (TRP) constraint. The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver i.e. trading off throughput for reliability. Turns out we can break the trade-off, we observe that the received signal is the sum of multiple copies of the transmitted signal, one from every beam in a multi-beam as shown in Fig.~\ref{fig:prototype}(b). If we can ensure the multiple copies add up in the signal domain constructively (Section 3), then we can increase the received signal power, and thereof the SNR while not increasing the total radiated power. 
%

Let's take an intuitive example: consider a mmWave channel consisting of two paths; and two-beams are aligned along those two-channel paths as shown in Figure \ref{fig:prototype}(b). For simplicity, assume the path loss is unity for each path, and the phase of signal travelled for each path is the same. \name's transmitter splits the total power of $a^2$ equally into two beams with power $a^2/2$ on each beam, i.e., amplitude $a/\sqrt{2}$ on each beam, which propagates through the channel and is received at the omni-receiver. Since the phase align for both paths, the received signal adds in signal domain, i.e. total amplitude of the received signal $ a/\sqrt{2} + a/\sqrt{2} = \sqrt{2}a$. The received signal upon converting to SNR (signal-to-noise ratio) is proportional to $2a^2$. In contrast, a traditional mmWave single-beam link does not exploit the second path and would provide an SNR proportional to $a^2$, which is 3 dB lower compared to a multi-beam case, thereby mutli-beam throughput is better than single beam. We mathematically show that, if the beam directions, phase, power per beam of mutli-beam are chosen optimally, then multi-beam will always achieve SNR higher than single beam even in wireless channels with weak multi-path, while using same total radiated power. Achieving optimal beam parameters would be henceforth referred as \constructivemultibeam.

\review{The intro discusses a highly unrealistic scenario as one "for the sake of simplicity" where the two paths are equally strong. It is better that the authors be upfront that this scenario is not likely but it is there to demonstrate the utility of the system. I assume it is almost never the case that both beams are equally good.}
\newtodo{We will highlight the assumptions made in the example in the introduction section and also show how the paper addresses them.}
%that are weak under the assumption that one can achieve proper per beam power control and phase coherent constructive combining. Specifically, we extend this analysis and mathematically prove that with appropriate amplitude and phase per beam, one can achieve optimal constructive combining that maximizes the signal-to-noise ratio. 


% In the above simple example, we assumed a strong multi-path channel with similar gain as the direct path and aligned phase with the direct path at the receiver (constructive combining). However, 

%Continuously maintaining such a \textit{\constructivemultibeam} even with changing wireless channel can enable reliable, high-throughput links by harnessing environmental reflections without increasing the total radiated power. 
%we need to solve  while being 5G NR compliant, we need to overcome two key challenges: First, we need to develop a beam training procedure which can enable constructive combining 
A natural question how can we establish a \constructivemultibeam link, while being protocol compliant and low-overhead.
To achieve \constructivemultibeam, one needs to estimate the optimal beam directions, beam-phase, and power per beam. \name key insights is to decouple this problem into first finding beam directions and then estimating the per beam amplitude and phase control. \name builds a novel low-overhead algorithm, thatwhich first leverage standard 5G NR beam training or any existing improved beam training algorithm~\cite{jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560} to learns the direction of all the strong paths. With just two additional 5G NR lowest complexity probes (CSI-RS), it learns the optimal power per beam and phase to be applied to each beam.

After estimating \constructivemultibeam parameters, \name needs to create the mutli-beam with those properties. \name creates each beam with orthogonal beamforming vectors, allowing application of accurate phase and power per beam. The orthogonal beams is an important step to minimize cross-talk between beams and is essential in obtaining the desired constructive combining gains mentioned earlier. 

%\name develops a novel low-overhead algorithm to extract all optimal beam parameters while re-using the same protocol used for mm-wave beam training for creating single beam,  with just two additional probes which are 5G NR compliant. Note, \name algorithm also infers optimal power per beam and phase per beam as well beyond single traditional beam training algorithm (Section 3). 
%by exploring the intricacies of the 5G protocol, thereby developing a low-cost beam probing mechanism to estimate the beam parameters. 
%Extensive literature has optimized creating a single has a huge complexity and extensive literature has worked to optimize it, to create multi-beam this would grow exponentially.
%It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. 
%In contrast, 

%Finally, we implement the discussed multi-beam design steps on our phased array testbed and verify the robustness of our solution to quantization errors and other hardware non-idealities.



 %We mathematically show that our multi-beam patterns with optimized phase and amplitude are optimal and maximizes the SNR for any given wireless channel.


So far, we have explained how to establish an initial low-overhead \constructivemultibeam; the critical challenge is continuously maintaining it, as wireless channel changes due to blockage and mobility. Mobility adversely affects the established links by causing misalignment between transmit and receive beams, degrading both throughput and reliability. Link blockages could completely occlude one or more beams of a multi-beam. In contrast to a single-beam system where only one beam is misaligned, in a multi-beam system, all the beams get misaligned simultaneously due to mobility. Hence Multi-beam presents unique challenges and opportunities to handle mobility and blockage in mmWave links. 

\name builds a novel proactive constructive multi-beam tracking algorithm, which proactively re-aligns each of the beam parameters (per-beam direction, phase and amplitude) to continuously maintains the constructive nature. First, since the received signal is sum of signals from all beams, \name builds a novel super-resolution algorithm to estimate properties of each beam individually. Next, it uses the estimated per beam properties to infer the underlying cause of power loss i.e. blockage or mobility per beam, if any. Instead of waiting for beams to degrade, \name proactively optimizes each of the beam directions by jointly inferring the underlying cause, and achieves \constructivemultibeam. Since each measurements requires only two partial channel probes, the overhead remains low. This allows \name to achieve an elusive goal with mmWave links, which is to create and maintain reliable high throughput links, free from sporadic outages.
 

%Our key insight is that we can infer the user mobility dynamics by estimating how the wireless channel changes across all the beams. Thus, our solution handles multi-beam links by estimating each beam's channel response independently, which allows us to generate a proactive response to mobility dynamics.
%Hence, \name designs a super-resolution algorithm based on sinc interpolation to extract the per beam channel response from the observed combined channel response.
%After isolating the per beam channel, \name can associate the key parameters required to handle mobility, like the direction of user and path loss, to track the beams adaptively and prevent any further misalignments.

% Therefore the challenge is to estimate the user mobility dynamics affecting each beam's wireless channel.

% all the beams in multi beam pattern will get misaligned, and by observing the signal strength changes across multiple beams, we can tap into these correlations to enable a proactive response to the misalignments.
% However, this key step requires 
% per beam power from CIR, needs superreoslution
% In order to tap into these gains from multiple beams, we need to formulate novel tracking methods since the tracking problem is complicated with mutli-beams. 
% This is because \name needs to re-align all the multiple beams with power and phase control per beam depending upon blockage or mobility situations. Therefore, none of the prior work can be used, as it requires tracking multiple beams angle, phase and power tracking. \name builds a novel proactive approach to maintain and track power, phase and beam direction of each of the multiple beams. \name's approach is to track the effects of mobility or blockage per-beam in the background by simply leveraging passive measurements of the mmWave received signal, making \name self-reliant. \name uses a tracking algorithm to periodically re-align each beam of the multi-beam and adjust their phase and amplitude, even when there is no significant link degradation. For example, in the blockage case, \name reduces the power along the blocked beam long before the link is degraded, thus increasing the power along the unblocked beam and maintaining the link. Similarly, in the case of user mobility, it continually re-aligns the beam directed towards the user. Therefore, \name prevents links from falling into outages.
% , as demonstrated through a prototype in Figure \ref{fig:prototype_2}. 




% To realize per beam tracking on a practical system even under mobility or blockage, \name needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to identify the blockage or user movement (self-reliant). Specifically, it measures the rate of degradation of the signal strength and creates thresholds for blockage and user movement and depending upon the observed degradation of the signal strength, it pro-actively calls it out as blockage or user movement. Furthermore, under user movement or mobility, the general motion is complex and hard to track, making beam re-alignment difficult. 

% In contrast, \name's key contribution is to decouple the complex user movement into rotation and translation movement and track them individually. An important observation is that all the beams within multi-beam undergo the same amount of angular movement for the rotation case, while for the translation case, the beams undergo different motion. We leverage this observation to design an angular rotation based beam tracking algorithm. A natural question is how do we measure the angular rotation per beam. In order to measure angular rotation per beam, we use the rate of change of amplitude per beam and phased-array antenna response, to determine the amount of rotation per beam. In summary, \name designs a novel amplitude-based tracking algorithm to track each beam individually. It only needs to measure 100 $\mu$sec of the received amplitude per beam to make the measurement. \textcolor{blue}{Also, note that \name only measures the angle to the UE for tracking and doesnot require exact user location, thus, preserving user privacy.}

%Second, \name needs to react to blockage or user movement per beam. The reaction to blockage is to reduce the power on the blocked beam. In contrast, to react for user mobility is challenging, it needs to  and the power and the phase for constructive combining, which requires it to identify the user movement. 

%First, to identify whether a particular beam is blocked or mis-aligned due to mobility, 

% On a practical system, per beam tracking has to be performed even with user mobility and blockage. \name, therefore, needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to make this distinction. The challenge is that the received signal is a combination of all beams in the multi-beam due to a single receiver chain on the receiver (analog beamforming). A naive approach could be to use the received signal to measure the channel in time-domain and use the separation of different beams in time-of-flight to identify amplitude corresponding to each beam. However, the multiple beams can often have very close times-of-flight (ToF) and cannot be resolved even with the high-sampling rate of mmWave (2.5 ns resolution with 400 MHz). To accurately determine amplitude per beam, \name builds a super-resolution algorithm that leverages the relative time-of-flight information (between beams). \name's insight is that the relative time-of-flight remains constant across multiple packets between beams, and \name uses this insight to learn their amplitudes. Furthermore, the relative ToFs are easily acquired during the initial standard beam training phase, requiring no protocol changes to achieve the tracking algorithm. 

% Finally, an implicit assumption made while performing per-beam tracking is the ability to recover per-beam amplitude. 

\textbf{Evaluation:} We build a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array, which can support channels of up to 400 MHz. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 
We obtained NSF license to perform experiments at 28 GHz in our university area. We deploy \name in various indoor and outdoor scenarios. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 

\vspace{-12pt}
%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 

%The key insight to 

% first point is seperation between blockage vs mobility. 
%\name first leverages the multi-beam set up to identify any movement or blockage. Then, 

%While in case of mobility, \name estimates the change directly in each beam angle due to the mobility. Specifically, it leverages the multi-beams to jointly estimate the accurate tracking of the beam angle for each beam. \name's proactive beam alignment process is fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. 
%\textit{}  


 
 %\textcolor{blue}{ Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and relative ToF \textcolor{red}{[downplay relative ToF here?]}(relative to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.}
 
% \name's second design principle for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility, i.e., \name preemptively tracks the beam and refines it without any explicit beam training. The approach gradually tracks the effects of mobility and the environment in the background, even when link throughput is not significantly affected. The beams are then periodically aligned with the mobile user. Therefore, it prevents links from falling into outages, as demonstrated through a prototype in Figure~\ref{fig:prototype}(c). \name's beam refinement is very fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. \textit{In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.}  


% The design philosophy of \name is different from other approaches. While recent proposals relies on assistance from device positioning system~\cite{zhou2018following,wei2017pose,va2015beam}, out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, or light sensors~\cite{haider2018listeer}, \name is deployed without any additional hardware or sensor support. In a similar line of research, BeamSpy~\cite{sur2016beamspy} and Beam-forcast~\cite{zhou2017beam} provides a model-driven approach to handle blockage and mobility, respectively; however, they lack a unified framework to integrate both vulnerabilities. Above all, the literature focusses on improving the average throughput of the system over a long timescale. On the other hand, \name's design philosophy is to improve system reliability at a short millisecond timescale. 


% An important observation here is that individual beams in a multi-beam are affected differently by these effects. Blockage significantly reduces the power of the beam oriented toward it, rotation of the user causes an almost equal drop in power across all beams, and translation causes an unequal power drop across beams. In case of blockage, \name reduces the power along the blocked beam, while in case of mobility, \name estimates the angle of movement.

% When \name detects blockage of a beam, it reduces the power along that beam. 



% \name achieves its goal by first setting up a multi-beam mmWave link and then proactively maintaining it. 
% To realize multi-beam tracking on a practical system, \name needs to address the following additional challenges.

% \noindent
% \textbf{Challenge 1) Multi-beam set up:} The first challenge for \name is to establish a multi-beam communication link. These beams travel through different path and add up at the receiver, could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput.
% and ensure that the signal along multiple beams adds up constructively at the receiver.



% \noindent
% \textbf{Solution:} \name takes advantage of recent advances in antenna design that allows high resolution in digital phase and amplitude control (6 bit and 4-bit resp. in our system). We showed that multi-beam patterns could be created by a weighted average of complex phasers of individual beams within multi-beam. The weights, however, if not appropriately set, may cause the signal along multi-paths to add up destructively at the receiver. We introduce a co-phasing factor that adjusts the relative phase of beams in multi-beam setup and device a method to tune that factor with low probing overhead.

% \noindent
% \textbf{Challenge 2) Multi-path separability:} \name is built on tracking per-beam amplitude in a multi-beam setup. Per-beam tracking is challenging since the received signal is a combination of all beams in the multi-beam due to analog beamforming. 

% \noindent
% \textbf{Solution:}  \name's key insight is to use the relative ToF information for each beam to learn its amplitude. However, with multiple beams often the multiple paths can have very close ToF, and cannot be resolved even with 15 cm resolution (2 GHz bandwidth at 60 GHz) or 75 cm resolution (400 MHz bandwidth at 28 GHz). To accurately resolve the beams, we build a super-resolution algorithm that leverages the relative ToF information (between beams) learned during the initial training phase, to produce accurate amplitude information per beam. 

% We then use the variation in per-beam amplitude over time to identify movement/blockage and modify the multi-beam pattern to maintain a reliable link.



% \noindent
% \textbf{Challenge 3) Multi-path parameter estimation:} 
% Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. 

% \noindent
% \textbf{Solution:}
% We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and related ToF (related to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.

% however, these parameters are typically estimated individually which pose  the mapping of AoA, AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. 

% Prior work \cite{palacios2018adaptive} relies on a custom training process to estimate absolute channel response per antenna and then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. 

% A key challenge is to associate the AoA with the AoD of corresponding reflectors.

% \name requires the knowledge of reflector location, orientation, and reflectively. Prior work suggest to get it offline manually \cite{wei2017facilitating} but \name need to get them in real-time.


% \name uses initial beam training to infer the strongest multi-paths in the environment, their angles of departure (AoD, beam from the transmitter), angles of arrival (AoA, beam at the receiver) and relative times-of-flight (relative ToF for each strong multi-path). \name uses the AoA, AoD, and relative ToF to learn reflector orientations in the environment by a smart ToF based association algorithm; the orientation of reflectors are necessary for proactive learning. 

% This knowledge of the multi-path environment augmented with recent advancements in mmWave antennas (achieving 6-bit phase and 7-bit amplitude control per antenna) to create a multi-beam link facilitates proactive learning as described below.
% enhanced by multi-path effects at both the transmitter and receiver.







% \begin{comment}


% Turns out 5G NR o
% super-resolution algorithm to recover Recall that during the initial beam training, we can learn about all the strong multi-path, we 
% can also use the initial 
% \item \textit{}
%     Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.


%     A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
    
% A natural question how does \name uses multi-beam to mitigate blockage and track user under mobility, 
% how does it maintain reliable connectivity using multi-beam. 



% To achieve reliable connectivity using multi-beam, \name builds an algorithm to track each of the individual beam 
% in the multiple beam from transmitter to the receiver. The individual track 



% % tell them how individual beam tracking in multi-beam solves both the 


% Challenge 1: individual beam tracking 

% Challenge 2: amplitude level tracking 
% % multi-beam tracking

% % amplitude level tracking 

% % ToF based seperation to achieve amplitude. 

% % rotation and translation 

% to the receiver but also help to track the user trajectory. \name refines the beam pattern over time to keep 
% it aligned with the mobile user, thus creating a stable WiFi-like link 
% %\textcolor{red}{[Should we mention that \name approximates the omni-pattern of sub-6GHz WiFi for directional mmWave link?]}. 
% The beam refinement\footnote{We use the IEEE 802.11ad terminology of beam training and beam refinement 
% which is discussed in Section \ref{sec:motivation}} with a multi-lobe pattern requires scanning of a constant 
% number of beams (0.1 ms latency) as compared to the beam training process that requires scanning 100's of beams 
% in the codebook at both transceiver (10 ms latency). \name's time complexity is of the order of the number of lobes, 
% which is typically directed towards 2-3 strong reflectors due to channel sparsity.

% Multi-lobe beam patterns has been explored in literature \textcolor{red}{[Cite Agile-link]} to reduce the 
% beam training delay, however, for the first time, \name exploits the unseen opportunity to use multi-lobe 
% patterns during the data transmission phase to enhance the link reliability. 

% The key challenges for \name are as follows:
% \begin{itemize}
%     \item \textit{The blockage mitigation has to be proactive.} \name creates custom multi-lobe patterns that are aligned with the strong reflectors providing multipath diversity. While some paths may suffer blockage, alternate unblocked paths are immediately available. A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
%     \item \textit{Beam alignment requires accurate tracking of mobile user with minimal overhead.} Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.
% \end{itemize}

% \end{comment}


% Instead of using a fix codebook based design, we first estimate the multipath directions and implement multipath aware beam patterns.
% Note the code book might contain thousands of beam patterns but there are only a 2-3 multipaths due to channel sparsity.
% In a nutshell, we propose a paradigm shift for millimeter wave communication to design multipath aware beam patterns. Finding the right beam out of thousands of possible beam patterns is time-consuming, however, creating a beam pattern based on direction inference is tractable since there are only a few multipath directions. Tracking the multipath components can lead to a robust and reliable connection.



% To reestablish the link quality, beam training is performed 

% Blockage and mobility~\cite{sur201560} are the most challenging and fundamental problems for mmWave system. The current solutions are not adequate: too naive and does not take advantage of unique mmWave properties such as high bandwidth, channel sparsity, and unique shape of beam patterns. 

% Due to the availability of higher bandwidth in the mmWave frequency range, the mmWave RAN can achieve data rates of the order of a few Gbps~\cite{CellularCap-Rap}, suitable for the QoS requirements for augmented reality (AR) and virtual reality (VR) applications. However, due to high path loss at mmWave frequencies, the coverage of mmWave RAN is limited. To improve the rate and coverage of mmWave networks, phased array antennas are used to create directional beams. Hundreds of antennas can be packed in a small area thanks to a low wavelength (a few millimeters) at these high frequencies. The directional antennas put a unique challenge for mmWave networks to find an optimal beam pattern at the access point (AP) and the user equipment (UE). IEEE 802.11ad standards describe a beam training algorithm that is used periodically to search for a suitable beam pattern. The beam pattern selected during the beamtraining phase (see Figure \ref{fig:twophases}) is used throughout the data transmission phase. 
% Mmwave links are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by more than 20 dB~\cite{georgeFading}. 




%  \textcolor{red}{Ish: I am throwing random ideas in next few paragraphs which need to be placed and rewritten properly.}

% Standards: IEEE 802.11ad \cite{ieee80211ad}, 802.15.3c~\cite{ieee802153c},  802.11ay~\cite{ieee80211ay}






% mmWave links are inherently directional to combat high path loss at higher frequencies. These directional links are highly susceptible to beam misalignment due to user mobility compared to a wide sector-level beam. Therefore, most commercial devices \textcolor{red}{[cite]} does not use fine beam patterns to avoid the signal degradation due to mobility. On the other hand, we take advantage of the fine beam patterns to track the user and refine the beam pattern to always align with the mobile user. 





% \begin{itemize}
%     \item \textit{Sparse channel:} The mmwave channel is sparse, i.e., only the LOS and a few NLOS paths characterize the channel. Furthermore, mmWave uses analog beams to focus the transmit energy in specific directions by choosing a particular combination of phase and attenuation at each transmit antenna \textcolor{red}{Figure: analog architecture}. 
    
%  \textit{   Note that the multi-stream communication may suffer from destructive interference due to the combination of multipath signal of opposite phase arriving at the receiver. 
%     In case two paths are interfering destructively, they won't appear in the CIR and so we won't consider those paths. They can be detected by their different AOD/TOF.}
%     \item \textit{Known patterns:} The directivity gain of the phased array antenna is a deterministic function of the codebook and antenna spacing and is known \textit{a-priori}. 
%     \item \textit{Advanced hardware:} Recent advances in antenna design allows high resolution in digital phase and amplitude control (6 bit and 4 bit resp. in our system). Furthermore, the phased array can generate close to ideal beam patterns by following various antenna calibration processes \textcolor{red}{[cite]}. This capability to generate regular beam patterns allow us to perform accurate RSSI based beam tracking.
%     \item \textit{CSI:} The CSI is used for many sensing application such as localization and tracking, and is readily available on commercial WiFi devices such as Quantenna \textcolor{red}{[cite]}. We expect the same trend for commercial mmWave system. 
%     \item \textit{Wideband:} We utilize the CSI and high bandwidth available at mmWave frequencies to separate multipaths via power-delay profile. prior work on blockage mitigation and beam alignment are based on narrow-band channel model~\cite{sur2016beamspy,zhou2017beam} which does not resolve multipaths.
% \end{itemize}



% Our main contributions are summarized as follows:
% \begin{itemize}
% \item \todo{Main contribution and results}
%     % \item We leverage the initial beam training to estimate the multipath parameters \{AOD, AOA, TOF\} and achieve high reliability through custom multi-lobe beam patterns. We also analyse reliability-throughput tradeoff for mmWave networks.
%     % \item We track the multipath and design a beam refinement algorithm to establish a stable link even under high user mobility scenario.
% \end{itemize}

% However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. 


% Thus, an unblocked Line of Sight (LOS) link is highly desirable for mmWave systems. When a LOS link is blocked, strong Non-Line of Sight (NLOS) links may also be helpful in achieving high reliability. However, NLOS links can also be blocked by mobile blockers. A mobile human blocker can block a link %between User Equipment (UE) and Base Station (BS) 
% for approximately 500 ms~\cite{georgeFading}. 


% At high frequencies, the attenuation due to obstacles is significant. For instance, 


==> Arxiv/1_intro_v11.tex <==
% !TEX root = main.tex
% Useless arxiv it
\section{Introduction}\label{sec:intro}

5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, 
defined as the fraction of time during which the link does not suffer an outage~\cite{driscoll2017enabling,ji2018ultra}. 
%In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that 
can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and therefore suffers from severe outage due to blockage and user's mobility. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that human blockages always bring down the link to an outage, which
is detrimental for high-reliability applications~\cite{ji2018ultra}.

% For example, blockage can reduce the signal strength by 20 dB, leading to an outage (no connectivity) for an extended period of 500 ms~\cite{maccartney2017rapid}, which is detrimental for high-reliability applications \cite{ji2018ultra}.
%When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam.
% Sub-6 GHz WiFi achieves high data-rate using spatial multiplexing which is function of existence of diverse multi-path in environment . However, 
% therefore even without multiplexing it can achieve multi-Gbps
% ~\footnote{Note that WiFi achieves high data-rate using spatial multiplexing which is function of existence of  diverse multi-path in environment and mmWave uses high bandwidth to achieve the same, but only requires existence  of a path between transmitter and receiver.}. To achieve 
% High bandwidth and directional beams allow mmWave to achieve high data rates required for video streaming applications.
% However, the directional link is vulnerable to blockages, device rotation, and user's mobility. A mobile blocker can reduce the signal strength by 20 dB, leading to outage which can be for an extended period of 500 ms~\cite{maccartney2017rapid}. When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam. In outdoor scenarios beam misalignment issue aggravates, 
% mmWave network if used for V2X has to support up to 500 km/h mobility while maintaining high throughput, high reliability, and ultra-low latency, which is challenging to achieve.
% Traditionally, mmWave network is optimized to provide high throughput of the order of a multi-Gbps~\cite{CellularCap-Rap}, thanks to high bandwidth and directional beams to combat higher pathloss at mmWave frequencies. 
%  The mmWave link can also degrade due to beam misalignment caused by device rotation and user's mobility.

Ideally, we would like to create a reliable mmWave link (a link without outage) that achieves high data-rate, and easy to deploy with upcoming 5G infrastructure. However, conventional mmWave design~\cite{ieee80211ad} centers on improving the link throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive} and coverage~\cite{zhou2019robot,wei2017facilitating}, which inadvertently ends up relegating the reliability requirement. The mmWave base station and the user tediously scan multiple beams to establish a directional link through \textit{beam training}. The beam training process is usually \textit{reactive}~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} which kicks in only after a significant degradation in link quality, leading to loss of connectivity and thereof reliability.
There are a few \textit{proactive} approaches that act before the link degrades by tracking the user. These proactive approaches either require side-channel information from out-of-band LTE/WiFi~\cite{sur2017wifi,nitsche2015steering} or rely on external sensors. These solutions apart from not being ubiquitous and self-reliant, have limited accuracy 
% and are limited to indoor environments
~\cite{haider2018listeer,zhou2018following,wei2017pose,va2015beam}. All these approaches make the system difficult to deploy and dependant on external information or non-stand-alone access.
% \textcolor{blue}{Moreover, external sensors collect sensitive information such as user location, which pose a privacy concern.
In contrast, our goal is to improve the inherent continuity and reliability of mmWave link and overall throughput without side-channel or external information.% i.e., self-reliant and easy to deploy. 
% Above all, the existing literature focuses on improving the average throughput of the system over a longer timescale.
% In contrast, our goal is to improve system reliability at both shorter and longer timescales,
% without side-channel or external information i.e. a self-reliant and easy to deploy solution. 



% \textit{Long outage duration and high frequency of prolonged beam training reduce the reliability of mmWave link.}

% fast handover~\cite{sur2018towards} or joint transmission from multiple APs~\cite{zhang2018mmchoir}.

% Though most research focuses on reducing the beam training delay, the delay generally increases with the size of the phased array~\cite{abari2016millimeter,barati2016initial,hassanieh2018fast}. 
%Besides, the beam training process has to be triggered frequently to avoid the harmful consequences of blockage and the user's mobility.

% In this work, we ask, can we achieve high-reliability mmWave links?  Traditionally, mmWave work has focused on blockage mitigation and beam alignment procedures \cite{sur2016beamspy,hassanieh2018fast} intending to improve the link throughput, which inadvertently ends up relegating the reliability requirement, leading to prolonged outages. The mmWave AP and the user periodically scan multiple beams in their codebook to find the right directional beam, commonly known as \textit{beam training}. The beam training process has to be triggered more frequently to avoid the harmful consequences of blockage and the user's mobility and can last as long as 10 msec for a codebook of a large antenna array~\cite{ieee80211ad}. Furthermore, blockage/user mobility detection is usually reactive~\cite{feng2017dealing} and may kick in only after significant detrimental impact on link quality, leading to loss of reliability. Some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam to avoid signal degradation due to mobility, but at the cost of significantly lower throughput while still being susceptible to outage due to blockages. \textit{Long outage duration, high frequency of beam training, and long beam training delays reduce the reliability of mmWave link.}
% The beam training is conducted to recover from outage or initial beam training, . %for communication through a process commonly known as \textit{beam training}. Although beam training has been studied extensively \textcolor{red}{[cite]}, the beam training delay is of the order of the logarithm of number of beams in the codebook~\cite{dina}. The codebook size for a large phased array can be huge, and the training takes order of a few 10 ms, during which there is no communication.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.52\textwidth]{figures/mmReliable_prototype.pdf}
    \caption{Shows the Conventional mmWave on the left and \name on the right. \name utilizes beam patterns with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beam pattern. }
    \label{fig:prototype}
    \vspace{-0.1in}
\end{figure}
% to take advantage of multi-path caused by strong reflectors in the environment to improve reliability. We get insights
% \textbf{\name's first design principle} is inspired from sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. To improve reliability, some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam as shown in Figure~\ref{fig:prototype}(a). However, a wide-beam suffers from significantly lower throughput and connectivity range while still being susceptible to outage due to blockages. In contrast, \name creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that are aligned towards LOS or strong reflected paths as shown in Figure~\ref{fig:prototype}(b). The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 



% In this paper, we present \name, which intends to create a reliable mmWave link, while maintaining high data rates. We get the insights from sub-6 GHz communication which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. 
% \name's first design principle is slightly counter-intuitive, where it creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that take advantage of multi-path caused by strong reflectors in the environment as shown in Figure~\ref{fig:prototype} (b). Beam splitting may reduce the range of connectivity, but provides reliability. 
% The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Notably, multi-beam provides an advantage in terms of range and throughput compared to a wide-beam since all the beams in a multi-beam pattern are aligned towards LOS or strong reflected paths. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

% Multi-lobe pattern has been used in MUTE and BounceNet ~\cite{jog2019many, ghasempour2018multi}.

% Theory work xxx needs channel by decoupling beam patterns which is challenging and time consuming [ACO, ]

In this paper, we introduce \name, a system which achieves both high-reliability and high-data-rate mmWave links, while being 5G NR compliant. \name is inspired by sub-6 GHz communication,  
% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
%\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.
%
%\textbf{\name's first design principle} is inspired by sub-6 GHz communication, 
which delivers high reliability and throughput, by exploiting multipath diversity from environmental reflections\cite{addmmwave citation as well here please don't edit this file, edit v10}. 
However, the same is not valid for traditional mmWave, which uses a single directional beam along the Line of Sight (LOS) or toward a strong reflector (NLOS). 
\name creates and maintains custom beam patterns with multiple directional beams (\textit{multi-beam} for brevity) that are each aligned towards LOS and strong reflected paths, while keeping the Total Radiated Power (TRP) same as a single beam (FCC compliant), as shown in Fig.~\ref{fig:prototype}(b). 
The idea here is that probability of multiple beams simultaneously facing a blockage is low, reducing the possibility of link outage. 

An obvious implication of splitting the single beam to a multi-beam is loss in power per beam to meet the total radiated power (TRP) constraint. The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver i.e. trading off throughput for reliability. Turns out we can break the trade-off, we observe that the received signal is the sum of multiple copies of the transmitted signal, one from every beam in a multi-beam as shown in Fig.~\ref{fig:prototype}(b). If we can ensure the multiple copies add up in the signal domain constructively, then we can increase the received signal power, and thereof the SNR while not increasing the total radiated power. Thus, with constructive combing of multi-beams henceforth referred as \constructivemultibeam, we can ensure no loss in throughput. Continuously maintaining such a \textit{\constructivemultibeam} can enable reliable, high-throughput links by harnessing environmental reflections without increasing the total transmit power. 

The first requirement in the multi-beam framework is to establish such \constructivemultibeam with low-overhead while complying with existing protocols. A challenge on this front is the estimation of optimal beam directions to orient each beam. \name leverages the large body of prior work on beam-training~\cite{jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560} and obtains the strongest beamforming directions. The second challenge is to choose the optimal phase and amplitude on a per-beam basis. \name extracts these parameters using a two-probe channel estimation technique with low overhead. This technique is agnostic to the underlying beam-training method and fits into the 5G-NR framework.
 
After estimating \constructivemultibeam parameters, \name needs to create the mutli-beam with those properties. \name creates each beam with orthogonal beamforming vectors, which enables it to apply accurate phase and power per beam. The use of orthogonal beams is an important step to minimize cross-talk between beams and is essential in obtaining the desired constructive combining gains mentioned earlier. 
%Finally, we implement the discussed multi-beam design steps on our phased array testbed and verify the robustness of our solution to quantization errors and other hardware non-idealities.

So far, we have explained how to establish a low-overhead \constructivemultibeam. An added requirement now is to continuously maintain this \constructivemultibeam in a manner that is resilient to blockage and mobility. Mobility adversely affects the established links by causing misalignment between transmit and receive beams, degrading both throughput and reliability. Link blockages could completely occlude one or more beams of a multi-beam. In contrast to a single-beam system where only one beam gets misaligned, in a multi-beam system, all the beams get misaligned simultaneously due to user mobility. Hence Multi-beam presents a unique challenges and opportunities to handle mobility and blockage in mmWave links. 

\name builds a novel proactive constructive multi-beam tracking algorithm, which proactively re-aligns each of the beam parameters (per-beam direction, phase and amplitude) to continuously maintains the constructive nature. First, since the received signal is sum of signals from all beams, \name builds a novel super-resolution algorithm to estimate properties of each beam individually. Next, it uses the estimated per beam properties to infer the underlying cause of power loss i.e. blockage or mobility per beam, if any. Instead of waiting for beams to degrade, \name proactively optimizes each of the beam directions by jointly inferring the underlying cause, and achieves \constructivemultibeam. Since each measurements requires only two partial channel probes, the overhead remains low. This allows \name to achieve an elusive goal with mmWave links, which is to create and maintain reliable high throughput links, free from sporadic outages.
 

%Our key insight is that we can infer the user mobility dynamics by estimating how the wireless channel changes across all the beams. Thus, our solution handles multi-beam links by estimating each beam's channel response independently, which allows us to generate a proactive response to mobility dynamics.
%Hence, \name designs a super-resolution algorithm based on sinc interpolation to extract the per beam channel response from the observed combined channel response.
%After isolating the per beam channel, \name can associate the key parameters required to handle mobility, like the direction of user and path loss, to track the beams adaptively and prevent any further misalignments.

% Therefore the challenge is to estimate the user mobility dynamics affecting each beam's wireless channel.

% all the beams in multi beam pattern will get misaligned, and by observing the signal strength changes across multiple beams, we can tap into these correlations to enable a proactive response to the misalignments.
% However, this key step requires 
% per beam power from CIR, needs superreoslution
% In order to tap into these gains from multiple beams, we need to formulate novel tracking methods since the tracking problem is complicated with mutli-beams. 
% This is because \name needs to re-align all the multiple beams with power and phase control per beam depending upon blockage or mobility situations. Therefore, none of the prior work can be used, as it requires tracking multiple beams angle, phase and power tracking. \name builds a novel proactive approach to maintain and track power, phase and beam direction of each of the multiple beams. \name's approach is to track the effects of mobility or blockage per-beam in the background by simply leveraging passive measurements of the mmWave received signal, making \name self-reliant. \name uses a tracking algorithm to periodically re-align each beam of the multi-beam and adjust their phase and amplitude, even when there is no significant link degradation. For example, in the blockage case, \name reduces the power along the blocked beam long before the link is degraded, thus increasing the power along the unblocked beam and maintaining the link. Similarly, in the case of user mobility, it continually re-aligns the beam directed towards the user. Therefore, \name prevents links from falling into outages.
% , as demonstrated through a prototype in Figure \ref{fig:prototype_2}. 




% To realize per beam tracking on a practical system even under mobility or blockage, \name needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to identify the blockage or user movement (self-reliant). Specifically, it measures the rate of degradation of the signal strength and creates thresholds for blockage and user movement and depending upon the observed degradation of the signal strength, it pro-actively calls it out as blockage or user movement. Furthermore, under user movement or mobility, the general motion is complex and hard to track, making beam re-alignment difficult. 

% In contrast, \name's key contribution is to decouple the complex user movement into rotation and translation movement and track them individually. An important observation is that all the beams within multi-beam undergo the same amount of angular movement for the rotation case, while for the translation case, the beams undergo different motion. We leverage this observation to design an angular rotation based beam tracking algorithm. A natural question is how do we measure the angular rotation per beam. In order to measure angular rotation per beam, we use the rate of change of amplitude per beam and phased-array antenna response, to determine the amount of rotation per beam. In summary, \name designs a novel amplitude-based tracking algorithm to track each beam individually. It only needs to measure 100 $\mu$sec of the received amplitude per beam to make the measurement. \textcolor{blue}{Also, note that \name only measures the angle to the UE for tracking and doesnot require exact user location, thus, preserving user privacy.}

%Second, \name needs to react to blockage or user movement per beam. The reaction to blockage is to reduce the power on the blocked beam. In contrast, to react for user mobility is challenging, it needs to  and the power and the phase for constructive combining, which requires it to identify the user movement. 

%First, to identify whether a particular beam is blocked or mis-aligned due to mobility, 

% On a practical system, per beam tracking has to be performed even with user mobility and blockage. \name, therefore, needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to make this distinction. The challenge is that the received signal is a combination of all beams in the multi-beam due to a single receiver chain on the receiver (analog beamforming). A naive approach could be to use the received signal to measure the channel in time-domain and use the separation of different beams in time-of-flight to identify amplitude corresponding to each beam. However, the multiple beams can often have very close times-of-flight (ToF) and cannot be resolved even with the high-sampling rate of mmWave (2.5 ns resolution with 400 MHz). To accurately determine amplitude per beam, \name builds a super-resolution algorithm that leverages the relative time-of-flight information (between beams). \name's insight is that the relative time-of-flight remains constant across multiple packets between beams, and \name uses this insight to learn their amplitudes. Furthermore, the relative ToFs are easily acquired during the initial standard beam training phase, requiring no protocol changes to achieve the tracking algorithm. 

% Finally, an implicit assumption made while performing per-beam tracking is the ability to recover per-beam amplitude. 

\textbf{Evaluation:} We build a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array, which can support channels of up to 400 MHz. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 
We obtained NSF license to perform experiments at 28 GHz in our university area. We deploy \name in various indoor and outdoor scenarios. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 


%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 

%The key insight to 

% first point is seperation between blockage vs mobility. 
%\name first leverages the multi-beam set up to identify any movement or blockage. Then, 

%While in case of mobility, \name estimates the change directly in each beam angle due to the mobility. Specifically, it leverages the multi-beams to jointly estimate the accurate tracking of the beam angle for each beam. \name's proactive beam alignment process is fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. 
%\textit{}  


 
 %\textcolor{blue}{ Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and relative ToF \textcolor{red}{[downplay relative ToF here?]}(relative to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.}
 
% \name's second design principle for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility, i.e., \name preemptively tracks the beam and refines it without any explicit beam training. The approach gradually tracks the effects of mobility and the environment in the background, even when link throughput is not significantly affected. The beams are then periodically aligned with the mobile user. Therefore, it prevents links from falling into outages, as demonstrated through a prototype in Figure~\ref{fig:prototype}(c). \name's beam refinement is very fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. \textit{In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.}  


% The design philosophy of \name is different from other approaches. While recent proposals relies on assistance from device positioning system~\cite{zhou2018following,wei2017pose,va2015beam}, out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, or light sensors~\cite{haider2018listeer}, \name is deployed without any additional hardware or sensor support. In a similar line of research, BeamSpy~\cite{sur2016beamspy} and Beam-forcast~\cite{zhou2017beam} provides a model-driven approach to handle blockage and mobility, respectively; however, they lack a unified framework to integrate both vulnerabilities. Above all, the literature focusses on improving the average throughput of the system over a long timescale. On the other hand, \name's design philosophy is to improve system reliability at a short millisecond timescale. 


% An important observation here is that individual beams in a multi-beam are affected differently by these effects. Blockage significantly reduces the power of the beam oriented toward it, rotation of the user causes an almost equal drop in power across all beams, and translation causes an unequal power drop across beams. In case of blockage, \name reduces the power along the blocked beam, while in case of mobility, \name estimates the angle of movement.

% When \name detects blockage of a beam, it reduces the power along that beam. 



% \name achieves its goal by first setting up a multi-beam mmWave link and then proactively maintaining it. 
% To realize multi-beam tracking on a practical system, \name needs to address the following additional challenges.

% \noindent
% \textbf{Challenge 1) Multi-beam set up:} The first challenge for \name is to establish a multi-beam communication link. These beams travel through different path and add up at the receiver, could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput.
% and ensure that the signal along multiple beams adds up constructively at the receiver.



% \noindent
% \textbf{Solution:} \name takes advantage of recent advances in antenna design that allows high resolution in digital phase and amplitude control (6 bit and 4-bit resp. in our system). We showed that multi-beam patterns could be created by a weighted average of complex phasers of individual beams within multi-beam. The weights, however, if not appropriately set, may cause the signal along multi-paths to add up destructively at the receiver. We introduce a co-phasing factor that adjusts the relative phase of beams in multi-beam setup and device a method to tune that factor with low probing overhead.

% \noindent
% \textbf{Challenge 2) Multi-path separability:} \name is built on tracking per-beam amplitude in a multi-beam setup. Per-beam tracking is challenging since the received signal is a combination of all beams in the multi-beam due to analog beamforming. 

% \noindent
% \textbf{Solution:}  \name's key insight is to use the relative ToF information for each beam to learn its amplitude. However, with multiple beams often the multiple paths can have very close ToF, and cannot be resolved even with 15 cm resolution (2 GHz bandwidth at 60 GHz) or 75 cm resolution (400 MHz bandwidth at 28 GHz). To accurately resolve the beams, we build a super-resolution algorithm that leverages the relative ToF information (between beams) learned during the initial training phase, to produce accurate amplitude information per beam. 

% We then use the variation in per-beam amplitude over time to identify movement/blockage and modify the multi-beam pattern to maintain a reliable link.



% \noindent
% \textbf{Challenge 3) Multi-path parameter estimation:} 
% Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. 

% \noindent
% \textbf{Solution:}
% We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and related ToF (related to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.

% however, these parameters are typically estimated individually which pose  the mapping of AoA, AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. 

% Prior work \cite{palacios2018adaptive} relies on a custom training process to estimate absolute channel response per antenna and then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. 

% A key challenge is to associate the AoA with the AoD of corresponding reflectors.

% \name requires the knowledge of reflector location, orientation, and reflectively. Prior work suggest to get it offline manually \cite{wei2017facilitating} but \name need to get them in real-time.


% \name uses initial beam training to infer the strongest multi-paths in the environment, their angles of departure (AoD, beam from the transmitter), angles of arrival (AoA, beam at the receiver) and relative times-of-flight (relative ToF for each strong multi-path). \name uses the AoA, AoD, and relative ToF to learn reflector orientations in the environment by a smart ToF based association algorithm; the orientation of reflectors are necessary for proactive learning. 

% This knowledge of the multi-path environment augmented with recent advancements in mmWave antennas (achieving 6-bit phase and 7-bit amplitude control per antenna) to create a multi-beam link facilitates proactive learning as described below.
% enhanced by multi-path effects at both the transmitter and receiver.







% \begin{comment}


% Turns out 5G NR o
% super-resolution algorithm to recover Recall that during the initial beam training, we can learn about all the strong multi-path, we 
% can also use the initial 
% \item \textit{}
%     Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.


%     A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
    
% A natural question how does \name uses multi-beam to mitigate blockage and track user under mobility, 
% how does it maintain reliable connectivity using multi-beam. 



% To achieve reliable connectivity using multi-beam, \name builds an algorithm to track each of the individual beam 
% in the multiple beam from transmitter to the receiver. The individual track 



% % tell them how individual beam tracking in multi-beam solves both the 


% Challenge 1: individual beam tracking 

% Challenge 2: amplitude level tracking 
% % multi-beam tracking

% % amplitude level tracking 

% % ToF based seperation to achieve amplitude. 

% % rotation and translation 

% to the receiver but also help to track the user trajectory. \name refines the beam pattern over time to keep 
% it aligned with the mobile user, thus creating a stable WiFi-like link 
% %\textcolor{red}{[Should we mention that \name approximates the omni-pattern of sub-6GHz WiFi for directional mmWave link?]}. 
% The beam refinement\footnote{We use the IEEE 802.11ad terminology of beam training and beam refinement 
% which is discussed in Section \ref{sec:motivation}} with a multi-lobe pattern requires scanning of a constant 
% number of beams (0.1 ms latency) as compared to the beam training process that requires scanning 100's of beams 
% in the codebook at both transceiver (10 ms latency). \name's time complexity is of the order of the number of lobes, 
% which is typically directed towards 2-3 strong reflectors due to channel sparsity.

% Multi-lobe beam patterns has been explored in literature \textcolor{red}{[Cite Agile-link]} to reduce the 
% beam training delay, however, for the first time, \name exploits the unseen opportunity to use multi-lobe 
% patterns during the data transmission phase to enhance the link reliability. 

% The key challenges for \name are as follows:
% \begin{itemize}
%     \item \textit{The blockage mitigation has to be proactive.} \name creates custom multi-lobe patterns that are aligned with the strong reflectors providing multipath diversity. While some paths may suffer blockage, alternate unblocked paths are immediately available. A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
%     \item \textit{Beam alignment requires accurate tracking of mobile user with minimal overhead.} Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.
% \end{itemize}

% \end{comment}


% Instead of using a fix codebook based design, we first estimate the multipath directions and implement multipath aware beam patterns.
% Note the code book might contain thousands of beam patterns but there are only a 2-3 multipaths due to channel sparsity.
% In a nutshell, we propose a paradigm shift for millimeter wave communication to design multipath aware beam patterns. Finding the right beam out of thousands of possible beam patterns is time-consuming, however, creating a beam pattern based on direction inference is tractable since there are only a few multipath directions. Tracking the multipath components can lead to a robust and reliable connection.



% To reestablish the link quality, beam training is performed 

% Blockage and mobility~\cite{sur201560} are the most challenging and fundamental problems for mmWave system. The current solutions are not adequate: too naive and does not take advantage of unique mmWave properties such as high bandwidth, channel sparsity, and unique shape of beam patterns. 

% Due to the availability of higher bandwidth in the mmWave frequency range, the mmWave RAN can achieve data rates of the order of a few Gbps~\cite{CellularCap-Rap}, suitable for the QoS requirements for augmented reality (AR) and virtual reality (VR) applications. However, due to high path loss at mmWave frequencies, the coverage of mmWave RAN is limited. To improve the rate and coverage of mmWave networks, phased array antennas are used to create directional beams. Hundreds of antennas can be packed in a small area thanks to a low wavelength (a few millimeters) at these high frequencies. The directional antennas put a unique challenge for mmWave networks to find an optimal beam pattern at the access point (AP) and the user equipment (UE). IEEE 802.11ad standards describe a beam training algorithm that is used periodically to search for a suitable beam pattern. The beam pattern selected during the beamtraining phase (see Figure \ref{fig:twophases}) is used throughout the data transmission phase. 
% Mmwave links are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by more than 20 dB~\cite{georgeFading}. 




%  \textcolor{red}{Ish: I am throwing random ideas in next few paragraphs which need to be placed and rewritten properly.}

% Standards: IEEE 802.11ad \cite{ieee80211ad}, 802.15.3c~\cite{ieee802153c},  802.11ay~\cite{ieee80211ay}






% mmWave links are inherently directional to combat high path loss at higher frequencies. These directional links are highly susceptible to beam misalignment due to user mobility compared to a wide sector-level beam. Therefore, most commercial devices \textcolor{red}{[cite]} does not use fine beam patterns to avoid the signal degradation due to mobility. On the other hand, we take advantage of the fine beam patterns to track the user and refine the beam pattern to always align with the mobile user. 





% \begin{itemize}
%     \item \textit{Sparse channel:} The mmwave channel is sparse, i.e., only the LOS and a few NLOS paths characterize the channel. Furthermore, mmWave uses analog beams to focus the transmit energy in specific directions by choosing a particular combination of phase and attenuation at each transmit antenna \textcolor{red}{Figure: analog architecture}. 
    
%  \textit{   Note that the multi-stream communication may suffer from destructive interference due to the combination of multipath signal of opposite phase arriving at the receiver. 
%     In case two paths are interfering destructively, they won't appear in the CIR and so we won't consider those paths. They can be detected by their different AOD/TOF.}
%     \item \textit{Known patterns:} The directivity gain of the phased array antenna is a deterministic function of the codebook and antenna spacing and is known \textit{a-priori}. 
%     \item \textit{Advanced hardware:} Recent advances in antenna design allows high resolution in digital phase and amplitude control (6 bit and 4 bit resp. in our system). Furthermore, the phased array can generate close to ideal beam patterns by following various antenna calibration processes \textcolor{red}{[cite]}. This capability to generate regular beam patterns allow us to perform accurate RSSI based beam tracking.
%     \item \textit{CSI:} The CSI is used for many sensing application such as localization and tracking, and is readily available on commercial WiFi devices such as Quantenna \textcolor{red}{[cite]}. We expect the same trend for commercial mmWave system. 
%     \item \textit{Wideband:} We utilize the CSI and high bandwidth available at mmWave frequencies to separate multipaths via power-delay profile. prior work on blockage mitigation and beam alignment are based on narrow-band channel model~\cite{sur2016beamspy,zhou2017beam} which does not resolve multipaths.
% \end{itemize}



% Our main contributions are summarized as follows:
% \begin{itemize}
% \item \todo{Main contribution and results}
%     % \item We leverage the initial beam training to estimate the multipath parameters \{AOD, AOA, TOF\} and achieve high reliability through custom multi-lobe beam patterns. We also analyse reliability-throughput tradeoff for mmWave networks.
%     % \item We track the multipath and design a beam refinement algorithm to establish a stable link even under high user mobility scenario.
% \end{itemize}

% However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. 


% Thus, an unblocked Line of Sight (LOS) link is highly desirable for mmWave systems. When a LOS link is blocked, strong Non-Line of Sight (NLOS) links may also be helpful in achieving high reliability. However, NLOS links can also be blocked by mobile blockers. A mobile human blocker can block a link %between User Equipment (UE) and Base Station (BS) 
% for approximately 500 ms~\cite{georgeFading}. 


% At high frequencies, the attenuation due to obstacles is significant. For instance, 


==> Arxiv/1_intro_v12.tex <==
% !TEX root = main.tex
% Created by RS on June 25, using copy of intro_v10.tex. For camera ready shot
\vspace{-0.15in}
\section{Introduction}\label{sec:intro}

5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr, wang2020demystifying}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, 
defined as the fraction of time during which the link does not suffer an outage~\cite{ji2018ultra,jain2019impact}. 
%In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and is highly susceptible to blockage and user movement. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that blockage by humans always causes link outage, which
is detrimental to applications requiring high-reliability~\cite{ji2018ultra}.

A large fraction of existing work focuses on improving mmWave link establishment~\cite{ jeong2015random,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast}, throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive,Xarray2020} and coverage~\cite{zhou2019robot,wei2017facilitating}; while the link reliability requirement takes the backseat. The prevailing methods aim to reduce link outages by performing efficient \textit{beam-training}, i.e, the process where the mmWave base station and client tediously scan multiple beams to establish a directional link. Reducing beam-training time does not prevent outages as the process is usually reactive~\cite{zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} and kicks in only after a significant degradation in link quality. To improve reliability, some authors propose proactive approaches that constantly track the client using side-channel information from out-of-band LTE/WiFi~\cite{sur2017wifi,nitsche2015steering} or external sensors like GPS,  radar or lidar~\cite{haider2018listeer, wei2017pose,va2015beam, woodford2021spacebeam}. These solutions are not self-reliant, have limited accuracy, and possibly require sensitive information like user location~\cite{wei2017pose,va2015beam}; making the system dependant on external information and difficult to deploy with existing standards. In contrast, we aim to create the ideal mmWave link: one that can be created and maintained with high reliability (no link outage), supports high data-rates, and is easy to integrate into current standards.

% Our goal is to improve the continuity and reliability of mmWave links and their throughput without side-channel or external information.

% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
%\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.
%
%\textbf{\name's first design principle} is inspired by sub-6 GHz communication, 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/mmreliable_prototype_v2.pdf}
    \caption{\name utilizes beams with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beams}
    \label{fig:prototype}
    \vspace{-0.18in}
\end{figure}

Traditional mmWave beamforming prioritizes throughput by using a single RF chain and a phased array to create a narrow, directed beam for communication. This method is inherently unreliable because this beam is prone to blockage or misalignment. 


In this work, we introduce \name, a system that achieves both reliable and high-data-rate mmWave links while being protocol compliant. Inspired by sub-6 GHz communication, \name delivers on reliability and throughput by exploiting the multipath diversity in environmental reflections. \name creates custom beam patterns with multiple directional beams (\textit{multi-beam}) that are each aligned towards Line of Sight (LOS) and other paths as shown in  Fig.~\ref{fig:prototype}(b). Simultaneous blockage of multiple beams is unlikely, reducing the possibility of link outage and increasing its reliability. 

An obvious implication of splitting a single beam into a multi-beam is reduced power radiated per beam to conserve the Total Radiated Power (TRP). The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver i.e. trading off throughput for reliability. Turns out we can break this trade-off: we observe that the received signal is the sum of multiple copies of the transmitted signal, one from every beam in a multi-beam as shown in Fig.~\ref{fig:prototype}(b). If we can ensure constructive addition of these copies at the receiver (Section~\ref{sec:constructive_combining}), the received power and throughput can be increased to a value higher than that of a single beam while keeping TRP constant.

\highlightshep{To understand how multi-beam is superior, let us consider a familiar sub-6 GHz scenario where N transmit antennas are communicating with a single receive antenna. In this case, the transmitter pre-multiplies the signal from each antenna using a complex number such that all signal copies combine constructively at the receiver. This method maximizes SNR at the receiver, and is typically referred to as transmit diversity or Maximal Ratio Combining (MRC) in literature~\cite{tse2005fundamentals}. MRC optimally combines multiple environmental reflections, while directional beamforming ignores them. In Section~\ref{sec:creatingmultibeam}, we mathematically show that the optimal beamforming solution in practical sparse reflector scenarios reduces to a multi-beam. A multi-beam yields better SNR than a single-beam in the presence of environmental reflectors since the optimal beamforming solution in these scenarios is not a single-beam. Further, we show that if the beam directions, phase, and power for each constituent beam are chosen optimally, then a multi-beam will consistently achieve SNR higher than a single beam while maintaining TRP. Achieving optimal beam parameters would be hereafter referred to as \constructivemultibeam.}

The first contribution of this work is the development of an algorithm to establish a \constructivemultibeam link, with low-overhead and protocol compliance. To achieve \constructivemultibeam, one needs to estimate the optimal beam directions, beam-phase, and power per beam. Our key insight here is to decouple this problem into two: finding beam directions, and estimating the per beam power and phase.
\name first learns the directions of strong paths in the environment (i.e. paths viable for communication) during the mandatory beam-training phase. This could be done using exhaustive beam-scanning or any other improved algorithm~\cite{jeong2015random,barati2015directional,zhou2012efficient,barati2016initial,sur201560}. Then, with just one additional channel probe per viable beam, it learns the optimum power and phase to be applied to each beam in the multi-beam. Only two-to-three viable beams exist in typical environments due to the sparse nature of reflection clusters at mmWave~\cite{zhu2014demystifying, telecom2019analysis}; therefore, \name's algorithmic overhead remain fixed and independent of the number of elements in the antenna array.
%  Some authors~\cite{ACO,zhang2018multibeam,??} argue for a similar solution for mmWave phased arrays, but this requires channel estimation at each array element and reduces in practicality as array sizes increase~\cite{}.

Once the initial \constructivemultibeam is established; the critical challenge is in continuously maintaining it, as the wireless channel changes due to blockages and mobility. Link blockages could completely occlude one or more beams of a multi-beam. Mobility adversely affects the established links by causing misalignment between transmit and receive beams, degrading both throughput and reliability. In contrast to a single-beam system where only one beam is misaligned, in a multi-beam system, all the beams get misaligned simultaneously due to mobility. Hence Multi-beam presents unique challenges and opportunities to handle mobility and blockage in mmWave links. 

The second contribution of this work is a beam-maintenance algorithm, which proactively re-aligns each of the beam parameters (direction, phase and amplitude) in a multi-beam and continuously maintains its constructive nature. First, since the received signal is sum of signals from all beams, \name builds a novel super-resolution algorithm to estimate properties of each beam individually. Next, it uses the estimated per beam properties to infer the underlying cause of power loss i.e. blockage or mobility per beam, if any. Instead of waiting for beams to degrade, \name proactively optimizes each of the beam directions by jointly inferring the underlying cause, and achieves \constructivemultibeam. Since each measurements requires only two partial channel probes, the overhead remains low. This allows \name to achieve the elusive goal of creating and maintaining reliable high throughput mmWave links, free from sporadic outages.

We build a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array that supports channels of up to 400 MHz. We implement \name using 5G NR compliant reference signals. Using our NSF spectrum license, we perform experiments at 28 GHz in our university area by deploying \name in various indoor and outdoor scenarios. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 

%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 




==> Arxiv/1_intro_v7.tex <==
% !TEX root = main.tex

\section{Introduction}\label{sec:intro}


5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, defined as the fraction of time during which the link does not suffer an outage~\cite{driscoll2017enabling,ji2018ultra}. %In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that 
can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and therefore suffers from severe outage due to blockage and user's mobility. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that human blockages always bring down the link to an outage, which
is detrimental for high-reliability applications~\cite{ji2018ultra}.

% For example, blockage can reduce the signal strength by 20 dB, leading to an outage (no connectivity) for an extended period of 500 ms~\cite{maccartney2017rapid}, which is detrimental for high-reliability applications \cite{ji2018ultra}.
%When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam.
% Sub-6 GHz WiFi achieves high data-rate using spatial multiplexing which is function of existence of diverse multi-path in environment . However, 
% therefore even without multiplexing it can achieve multi-Gbps
% ~\footnote{Note that WiFi achieves high data-rate using spatial multiplexing which is function of existence of  diverse multi-path in environment and mmWave uses high bandwidth to achieve the same, but only requires existence  of a path between transmitter and receiver.}. To achieve 
% High bandwidth and directional beams allow mmWave to achieve high data rates required for video streaming applications.
% However, the directional link is vulnerable to blockages, device rotation, and user's mobility. A mobile blocker can reduce the signal strength by 20 dB, leading to outage which can be for an extended period of 500 ms~\cite{maccartney2017rapid}. When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam. In outdoor scenarios beam misalignment issue aggravates, 
% mmWave network if used for V2X has to support up to 500 km/h mobility while maintaining high throughput, high reliability, and ultra-low latency, which is challenging to achieve.
% Traditionally, mmWave network is optimized to provide high throughput of the order of a multi-Gbps~\cite{CellularCap-Rap}, thanks to high bandwidth and directional beams to combat higher pathloss at mmWave frequencies. 
%  The mmWave link can also degrade due to beam misalignment caused by device rotation and user's mobility. 
Ideally, we would like to create a reliable mmWave link (a link without outage) that achieves high data-rate, is self-reliant, and easy to deploy. However, conventional mmWave design~\cite{ieee80211ad} centers on improving the link throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive} and coverage~\cite{zhou2019robot,wei2017facilitating}, which inadvertently ends up relegating the reliability requirement. The mmWave base station and the user tediously scan multiple beams in their codebook to establish a directional link through \textit{beam training}. The beam training process is usually \textit{reactive}~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} which kicks in only after a significant degradation in link quality, leading to loss of connectivity and thereof reliability.
There are a few \textit{proactive} approaches that act before the link degrades by tracking the user. For this, these proactive approaches either require side-channel information from out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, which has limited accuracy and is limited to indoor environments, or external sensors ~\cite{haider2018listeer,zhou2018following,wei2017pose,va2015beam} which are not ubiquitous. All of these approaches make the system difficult to deploy and dependant on external information.
% \textcolor{blue}{Moreover, external sensors collect sensitive information such as user location, which pose a privacy concern. 
In contrast, our goal is to improve system reliability and overall throughput without side-channel or external information.% i.e., self-reliant and easy to deploy. 
% Above all, the existing literature focuses on improving the average throughput of the system over a longer timescale.
% In contrast, our goal is to improve system reliability at both shorter and longer timescales,
% without side-channel or external information i.e. a self-reliant and easy to deploy solution. 



% \textit{Long outage duration and high frequency of prolonged beam training reduce the reliability of mmWave link.}

% fast handover~\cite{sur2018towards} or joint transmission from multiple APs~\cite{zhang2018mmchoir}.

% Though most research focuses on reducing the beam training delay, the delay generally increases with the size of the phased array~\cite{abari2016millimeter,barati2016initial,hassanieh2018fast}. 
%Besides, the beam training process has to be triggered frequently to avoid the harmful consequences of blockage and the user's mobility.

% In this work, we ask, can we achieve high-reliability mmWave links?  Traditionally, mmWave work has focused on blockage mitigation and beam alignment procedures \cite{sur2016beamspy,hassanieh2018fast} intending to improve the link throughput, which inadvertently ends up relegating the reliability requirement, leading to prolonged outages. The mmWave AP and the user periodically scan multiple beams in their codebook to find the right directional beam, commonly known as \textit{beam training}. The beam training process has to be triggered more frequently to avoid the harmful consequences of blockage and the user's mobility and can last as long as 10 msec for a codebook of a large antenna array~\cite{ieee80211ad}. Furthermore, blockage/user mobility detection is usually reactive~\cite{feng2017dealing} and may kick in only after significant detrimental impact on link quality, leading to loss of reliability. Some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam to avoid signal degradation due to mobility, but at the cost of significantly lower throughput while still being susceptible to outage due to blockages. \textit{Long outage duration, high frequency of beam training, and long beam training delays reduce the reliability of mmWave link.}
% The beam training is conducted to recover from outage or initial beam training, . %for communication through a process commonly known as \textit{beam training}. Although beam training has been studied extensively \textcolor{red}{[cite]}, the beam training delay is of the order of the logarithm of number of beams in the codebook~\cite{dina}. The codebook size for a large phased array can be huge, and the training takes order of a few 10 ms, during which there is no communication.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/QIF_mmreliable.pdf}
    \caption{Shows the Conventional mmWave on the left and \name on the right. \name utilizes beam patterns with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beam pattern.\newtodo{gNB in corner. Use two beams.} }
    \label{fig:prototype}
    \vspace{-0.1in}
\end{figure}
% to take advantage of multi-path caused by strong reflectors in the environment to improve reliability. We get insights
% \textbf{\name's first design principle} is inspired from sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. To improve reliability, some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam as shown in Figure~\ref{fig:prototype}(a). However, a wide-beam suffers from significantly lower throughput and connectivity range while still being susceptible to outage due to blockages. In contrast, \name creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that are aligned towards LOS or strong reflected paths as shown in Figure~\ref{fig:prototype}(b). The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 



% In this paper, we present \name, which intends to create a reliable mmWave link, while maintaining high data rates. We get the insights from sub-6 GHz communication which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. 
% \name's first design principle is slightly counter-intuitive, where it creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that take advantage of multi-path caused by strong reflectors in the environment as shown in Figure~\ref{fig:prototype} (b). Beam splitting may reduce the range of connectivity, but provides reliability. 
% The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Notably, multi-beam provides an advantage in terms of range and throughput compared to a wide-beam since all the beams in a multi-beam pattern are aligned towards LOS or strong reflected paths. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

% Multi-lobe pattern has been used in MUTE and BounceNet ~\cite{jog2019many, ghasempour2018multi}.

% Theory work xxx needs channel by decoupling beam patterns which is challenging and time consuming [ACO, ]

In this paper, we introduce \name, the first system that achieves high-reliability and high-data-rate mmWave links while being self-reliant (on the mmWave link) and is easy to deploy. 
% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.

\textbf{\name's first design principle} is inspired by sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment through omni-directional patterns. The same is not valid for traditional mmWave, which uses a single directional beam along the Line of Sight (LOS) or toward a reflector. 
\name creates custom beam patterns with multiple directional beams (\textit{multi-beam} for brevity) that are each aligned towards LOS and strong reflected paths, while keeping the Total Radiated Power (TRP) same as a single beam (FCC compliant), as shown in Fig.~\ref{fig:prototype}(b). 
The insight here is that the probability of multiple beams simultaneously facing a blockage is low, reducing the possibility of link outage. 

% \todo{no!!, you are performing constrcutive combining which is helping it improve SNR!! talk about constructive combining and then give the example, your techniques should be summarized here...} 


An obvious implication of splitting the single beam to a multi-beam is the loss of EIRP (Equivalent Isotropic Radiated Power) per beam to meet the same TRP constraint. The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver. At first glance, it seems as if multi-beam trades throughput for reliability while the goal was to improve both. Our insight into breaking this trade-off is based on the observation that the received signal is the sum of multiple copies of the transmitted signal, each for every beam in a multi-beam. If we can ensure the signal adds up in the signal domain constructively, we can increase the signal strength and throughput. Let's see with an intuitive example, say a mmWave channel consisting of two paths and two-beam are aligned along those two-channel paths. For simplicity, assume the path loss is unity for each path, and the phase of each path is the same. The transmitter splits a total power of $a^2$ into two beams with power $a^2/2$ on each beam, i.e., amplitude $a/\sqrt{2}$ on each beam while the receiver receives it. Our constructive combining leads to the total amplitude of the received signal $ a/\sqrt{2} + a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR (signal-to-noise ratio) is proportional to $2a^2$. A single-beam link does not exploit the second path and would provide an SNR proportional to $a^2$, which is 3 dB lower compared to a multi-beam case. In summary, we can infer that the throughput gain is obtained by harnessing a multi-path environment without increasing the total transmit power. 

In the above simple example, we assumed a strong multi-path channel with similar gain as the direct path and aligned phase with the direct path at the receiver. However, real-world channels pose many challenges for multi-beam. They are complex with multi-paths that are weak and have phase value that doesn't align with the direct path. We develop novel analog beamforming techniques that optimize per-beam phase and power control in a multi-beam to enable constructive combining. We mathematically show that our multi-beam patterns with optimized phase and amplitude are optimal and maximizes the SNR for a given wireless channel. The second challenge for multi-beam is to estimate the phase, attenuation, and angle of each channel path required to generate phase-coherent multi-beam patterns. \name develops a beam probing mechanism to estimate the channel parameters. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. Finally, creating a multi-beam pattern in hardware poses an additional challenge due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed.


%  Furthermore, we prove that it would be always be better than ...  \name can therefore deliver a high reliability and high throughput link. 



% We present an intuitive example to explain the benefits of \name's constructive combining optimization. For simplicity, we consider the transmitter uses a 2-beam pattern aligned with two channel paths and the receiver is omni-directional. Assume the pathloss of each path is unity in which case \name allocates equal amplitude to each beam. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path, our constructive combining leads to the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. A careful reader would infer that the throughput gain is obtained by harnessing multi-path environment without increasing the total power. \name can therefore deliver reliable link while maintaining high throughput. 

% \textcolor{purple}{
% The intuitive example, however, does not explain multiple practical challenges in establishing a multi-beam link. (i) In practice, the reflected path channel suffers from higher attenuation which may affect the throughput gain. To deal with weaker paths, \name performs a joint optimization of phase and amplitude of each beam in a multi-beam to maximise SNR. (ii) The second challenge is to estimate the phase, attenuation and angle of each channel path which is required to generate phase-coherent multi-beam patterns. \name develops a beam probing mechanism to estimate the channel parameters. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. (iii) Finally, creating multi-beam pattern in hardware poses additional challenges due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed. }

% In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of optimal channel-dependent beam pattern. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.

% The critical insight is that the multi-beam model is equivalent to transmitter diversity for low-frequency communication~\cite{tse2005fundamentals}, where multiple antennae transmit together to add up the signals at the receiver constructively. Such a scheme can increase the signal power received by the factor of the number of transmitting antennae, while simultaneously meeting the TRP constraints. \name is the first practical system to realize the transmit diversity for the mmWave communication systems with a single phased array and without relying on multiple RF chain. 

% \textcolor{purple}{
% The diversity gain achieved by \name can be understood by a simple example.
% Let's say there are two paths, each with say each with equal pathloss of unity. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path. \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. 
% With our constructive amplitude combining the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. \name takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. In fact, we mathematically show that the phase-coherent multi-beam patterns are optimal under given multi-path channel when the number of beams are same as the number of channel paths. In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of ideal channel-dependent beam pattern. We propose a tractable approach to estimate the phase and amplitude per-beam with negligible overhead. Our approach requires only two probes for 2 beams and 4 probes for 3 beam case. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.}

% \todo{Mention that multi-beam requires attenuation control of more than 10 dB? but most commercially available arrays do not provide that control and so multi-beam was not feasible yet. We are the first to explore it.}

% An obvious implication of splitting the single lobe in to multiple beam is it would lead loss of signal radiated per beam of multiple beam on transmitter to meet EIRP (Equivalent Isotropic Radiated Power) constraint. 
% Therefore, the multi-beam concept may lead to the loss in signal strength received at the receiver, as the transmitted signal are individually reduced in power to meet EIRP. 
% The surprising observation is that in some scenarios, the signal received at the receiver increases by creating multi-beam compared to a single beam. 

% \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead.
% The above intuitive result is demonstrated in the Eq.3, where $\delta=1$ so $(1 + \delta^2) = 2$ i.e. 2 times the SNR. This is called diversity gain, or transmit beamforming gain, which is popularly taught in wireless classes as one of the first key principle, where the power is normalized as well. The paper explains the power normalization in the introduction, and when creating multiple beams, so

% To achieve full transmit diversity, i.e., improving signal to noise ratio optimally at the receiver, it requires the constructive combining of the signal from each beam (or transmitter).  \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. It takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.


% Furthermore, note that the reflected path can have up to 20 dB of signal degradation compared to direct path and still the throughput of \name would be better than single beam link. However, turns out for 28 GHz mmWave the difference in the path-loss of the signal from naturally occurring reflectors and the direct path signal is minimal~\cite{samimi2014characterization}.

% The key insight behind this increase in received signal power for multi-beam compared to the single beam is that multi-beam in mmWave is equivalent to transmitter diversity for low frequency communication\todo{~\cite{}}. For transmitter diversity the signal power is distributed among multiple antennas, whereas in mmWave it is distributed among multiple beams. If the received signal from these multi-beams (or transmitters) combine constructively at the receiver they increase the signal received by the factor of number of antenna, while even meeting the EIRP constraints.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figures/brp_timeline_fig2_crop.pdf}
%     \caption{Shows \name tracks the user mobility and proactively refines the multi-beam patterns. It shows the \name link performs well even without beam training overhead. In contrast, the reactive framework performs beam training to recover a dead link. }
%     \label{fig:prototype_2}
%     \vspace{-0.1in}
% \end{figure}


% % \name designs an innovative approach to create multi-beam patterns and distribute power along multiple directions.  
% \todo{make this paragraph challenges only, and say that you overcome in the paper}
% In order to achieve full transmit diversity, i.e. improving signal to noise ratio optimally at the receiver, it requires constructive combining of the signal from each beam (or transmitter). Said differently, the challenge with multi-beam communication is that the signal travels through different paths and adds up at the receiver, which could lead to destructive combining leading to the loss of the signal at the receiver. The loss in the signal can result in reduced throughput for multi-beam. To overcome this problem, \name builds a novel algorithm that creates phase per beam and adapts the phase per beam in real-time to make sure the signal combines constructively. Moreover, it takes advantage of recent advances\cite{IDT} in antenna design for 28 GHz and shows that efficient multi-beam patterns can be created with per-antenna analog phase and amplitude control. Furthermore, it uses the standard beam training process to learn the phase per beam for constructive combining, not creating any additional overhead for per beam phase estimation.
% While multi-beam helps improve link reliability for a static user under blockage, in a dynamic environment, it is still prone to link degradation due to user mobility.


% To achieve the multi-beam and proactive response with a goal of high throughput and high-reliability, \name needs to address the following challenges. The first challenge is that \name distributes the power across multiple beams, these beams travel through different path and add up at the receiver, would could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput. In order to overcome this problem, \name builds a novel algorithm which creates phase per beam, and adapts the phase per beam in real-time to make sure the signal combines constructively. \name takes advantage of recent advances in antenna design for 28 GHz, and shows that with per antenna analog phase and amplitude control (6 bit and 4-bit resp. in our system).
% While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 


\textbf{\name's second design principle} for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility. Mobility due to rotation (VR headset in motion, rotary industry parts) or translation (walking, moving vehicle) adversely affects the established links by causing misalignment between transmit and receive beams. \name's approach is to track the effects of mobility or blockage per-beam in the background by simply leveraging passive measurements of the mmWave received signal, making \name self-reliant. \name uses a tracking algorithm to periodically re-align each beam of the multi-beam and adjust their phase and amplitude, even when there is no significant link degradation. For example, in the blockage case, \name reduces the power along the blocked beam long before the link is degraded, thus increasing the power along the unblocked beam and maintaining the link. Similarly, in the case of user mobility, it continually re-aligns the beam directed towards the user. Therefore, \name prevents links from falling into outages.
% , as demonstrated through a prototype in Figure \ref{fig:prototype_2}. 




% To realize per beam tracking on a practical system even under mobility or blockage, \name needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to identify the blockage or user movement (self-reliant). Specifically, it measures the rate of degradation of the signal strength and creates thresholds for blockage and user movement and depending upon the observed degradation of the signal strength, it pro-actively calls it out as blockage or user movement. Furthermore, under user movement or mobility, the general motion is complex and hard to track, making beam re-alignment difficult. 

% In contrast, \name's key contribution is to decouple the complex user movement into rotation and translation movement and track them individually. An important observation is that all the beams within multi-beam undergo the same amount of angular movement for the rotation case, while for the translation case, the beams undergo different motion. We leverage this observation to design an angular rotation based beam tracking algorithm. A natural question is how do we measure the angular rotation per beam. In order to measure angular rotation per beam, we use the rate of change of amplitude per beam and phased-array antenna response, to determine the amount of rotation per beam. In summary, \name designs a novel amplitude-based tracking algorithm to track each beam individually. It only needs to measure 100 $\mu$sec of the received amplitude per beam to make the measurement. \textcolor{blue}{Also, note that \name only measures the angle to the UE for tracking and doesnot require exact user location, thus, preserving user privacy.}

%Second, \name needs to react to blockage or user movement per beam. The reaction to blockage is to reduce the power on the blocked beam. In contrast, to react for user mobility is challenging, it needs to  and the power and the phase for constructive combining, which requires it to identify the user movement. 

%First, to identify whether a particular beam is blocked or mis-aligned due to mobility, 

On a practical system, per beam tracking has to be performed even with user mobility and blockage. \name, therefore, needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to make this distinction. The challenge is that the received signal is a combination of all beams in the multi-beam due to a single receiver chain on the receiver (analog beamforming). A naive approach could be to use the received signal to measure the channel in time-domain and use the separation of different beams in time-of-flight to identify amplitude corresponding to each beam. However, the multiple beams can often have very close times-of-flight (ToF) and cannot be resolved even with the high-sampling rate of mmWave (2.5 ns resolution with 400 MHz). To accurately determine amplitude per beam, \name builds a super-resolution algorithm that leverages the relative time-of-flight information (between beams). \name's insight is that the relative time-of-flight remains constant across multiple packets between beams, and \name uses this insight to learn their amplitudes. Furthermore, the relative ToFs are easily acquired during the initial standard beam training phase, requiring no protocol changes to achieve the tracking algorithm. 

% Finally, an implicit assumption made while performing per-beam tracking is the ability to recover per-beam amplitude. 

\textbf{Evaluation:} We demonstrate \name on a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array, which can support channels of up to 400 MHz. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 
We deploy \name in various indoor and outdoor scenarios and evaluate its performance. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 


%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 

%The key insight to 

% first point is seperation between blockage vs mobility. 
%\name first leverages the multi-beam set up to identify any movement or blockage. Then, 

%While in case of mobility, \name estimates the change directly in each beam angle due to the mobility. Specifically, it leverages the multi-beams to jointly estimate the accurate tracking of the beam angle for each beam. \name's proactive beam alignment process is fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. 
%\textit{}  


 
 %\textcolor{blue}{ Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and relative ToF \textcolor{red}{[downplay relative ToF here?]}(relative to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.}
 
% \name's second design principle for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility, i.e., \name preemptively tracks the beam and refines it without any explicit beam training. The approach gradually tracks the effects of mobility and the environment in the background, even when link throughput is not significantly affected. The beams are then periodically aligned with the mobile user. Therefore, it prevents links from falling into outages, as demonstrated through a prototype in Figure~\ref{fig:prototype}(c). \name's beam refinement is very fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. \textit{In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.}  


% The design philosophy of \name is different from other approaches. While recent proposals relies on assistance from device positioning system~\cite{zhou2018following,wei2017pose,va2015beam}, out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, or light sensors~\cite{haider2018listeer}, \name is deployed without any additional hardware or sensor support. In a similar line of research, BeamSpy~\cite{sur2016beamspy} and Beam-forcast~\cite{zhou2017beam} provides a model-driven approach to handle blockage and mobility, respectively; however, they lack a unified framework to integrate both vulnerabilities. Above all, the literature focusses on improving the average throughput of the system over a long timescale. On the other hand, \name's design philosophy is to improve system reliability at a short millisecond timescale. 


% An important observation here is that individual beams in a multi-beam are affected differently by these effects. Blockage significantly reduces the power of the beam oriented toward it, rotation of the user causes an almost equal drop in power across all beams, and translation causes an unequal power drop across beams. In case of blockage, \name reduces the power along the blocked beam, while in case of mobility, \name estimates the angle of movement.

% When \name detects blockage of a beam, it reduces the power along that beam. 



% \name achieves its goal by first setting up a multi-beam mmWave link and then proactively maintaining it. 
% To realize multi-beam tracking on a practical system, \name needs to address the following additional challenges.

% \noindent
% \textbf{Challenge 1) Multi-beam set up:} The first challenge for \name is to establish a multi-beam communication link. These beams travel through different path and add up at the receiver, could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput.
% and ensure that the signal along multiple beams adds up constructively at the receiver.



% \noindent
% \textbf{Solution:} \name takes advantage of recent advances in antenna design that allows high resolution in digital phase and amplitude control (6 bit and 4-bit resp. in our system). We showed that multi-beam patterns could be created by a weighted average of complex phasers of individual beams within multi-beam. The weights, however, if not appropriately set, may cause the signal along multi-paths to add up destructively at the receiver. We introduce a co-phasing factor that adjusts the relative phase of beams in multi-beam setup and device a method to tune that factor with low probing overhead.

% \noindent
% \textbf{Challenge 2) Multi-path separability:} \name is built on tracking per-beam amplitude in a multi-beam setup. Per-beam tracking is challenging since the received signal is a combination of all beams in the multi-beam due to analog beamforming. 

% \noindent
% \textbf{Solution:}  \name's key insight is to use the relative ToF information for each beam to learn its amplitude. However, with multiple beams often the multiple paths can have very close ToF, and cannot be resolved even with 15 cm resolution (2 GHz bandwidth at 60 GHz) or 75 cm resolution (400 MHz bandwidth at 28 GHz). To accurately resolve the beams, we build a super-resolution algorithm that leverages the relative ToF information (between beams) learned during the initial training phase, to produce accurate amplitude information per beam. 

% We then use the variation in per-beam amplitude over time to identify movement/blockage and modify the multi-beam pattern to maintain a reliable link.



% \noindent
% \textbf{Challenge 3) Multi-path parameter estimation:} 
% Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. 

% \noindent
% \textbf{Solution:}
% We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and related ToF (related to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.

% however, these parameters are typically estimated individually which pose  the mapping of AoA, AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. 

% Prior work \cite{palacios2018adaptive} relies on a custom training process to estimate absolute channel response per antenna and then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. 

% A key challenge is to associate the AoA with the AoD of corresponding reflectors.

% \name requires the knowledge of reflector location, orientation, and reflectively. Prior work suggest to get it offline manually \cite{wei2017facilitating} but \name need to get them in real-time.


% \name uses initial beam training to infer the strongest multi-paths in the environment, their angles of departure (AoD, beam from the transmitter), angles of arrival (AoA, beam at the receiver) and relative times-of-flight (relative ToF for each strong multi-path). \name uses the AoA, AoD, and relative ToF to learn reflector orientations in the environment by a smart ToF based association algorithm; the orientation of reflectors are necessary for proactive learning. 

% This knowledge of the multi-path environment augmented with recent advancements in mmWave antennas (achieving 6-bit phase and 7-bit amplitude control per antenna) to create a multi-beam link facilitates proactive learning as described below.
% enhanced by multi-path effects at both the transmitter and receiver.







% \begin{comment}


% Turns out 5G NR o
% super-resolution algorithm to recover Recall that during the initial beam training, we can learn about all the strong multi-path, we 
% can also use the initial 
% \item \textit{}
%     Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.


%     A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
    
% A natural question how does \name uses multi-beam to mitigate blockage and track user under mobility, 
% how does it maintain reliable connectivity using multi-beam. 



% To achieve reliable connectivity using multi-beam, \name builds an algorithm to track each of the individual beam 
% in the multiple beam from transmitter to the receiver. The individual track 



% % tell them how individual beam tracking in multi-beam solves both the 


% Challenge 1: individual beam tracking 

% Challenge 2: amplitude level tracking 
% % multi-beam tracking

% % amplitude level tracking 

% % ToF based seperation to achieve amplitude. 

% % rotation and translation 

% to the receiver but also help to track the user trajectory. \name refines the beam pattern over time to keep 
% it aligned with the mobile user, thus creating a stable WiFi-like link 
% %\textcolor{red}{[Should we mention that \name approximates the omni-pattern of sub-6GHz WiFi for directional mmWave link?]}. 
% The beam refinement\footnote{We use the IEEE 802.11ad terminology of beam training and beam refinement 
% which is discussed in Section \ref{sec:motivation}} with a multi-lobe pattern requires scanning of a constant 
% number of beams (0.1 ms latency) as compared to the beam training process that requires scanning 100's of beams 
% in the codebook at both transceiver (10 ms latency). \name's time complexity is of the order of the number of lobes, 
% which is typically directed towards 2-3 strong reflectors due to channel sparsity.

% Multi-lobe beam patterns has been explored in literature \textcolor{red}{[Cite Agile-link]} to reduce the 
% beam training delay, however, for the first time, \name exploits the unseen opportunity to use multi-lobe 
% patterns during the data transmission phase to enhance the link reliability. 

% The key challenges for \name are as follows:
% \begin{itemize}
%     \item \textit{The blockage mitigation has to be proactive.} \name creates custom multi-lobe patterns that are aligned with the strong reflectors providing multipath diversity. While some paths may suffer blockage, alternate unblocked paths are immediately available. A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
%     \item \textit{Beam alignment requires accurate tracking of mobile user with minimal overhead.} Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.
% \end{itemize}

% \end{comment}


% Instead of using a fix codebook based design, we first estimate the multipath directions and implement multipath aware beam patterns.
% Note the code book might contain thousands of beam patterns but there are only a 2-3 multipaths due to channel sparsity.
% In a nutshell, we propose a paradigm shift for millimeter wave communication to design multipath aware beam patterns. Finding the right beam out of thousands of possible beam patterns is time-consuming, however, creating a beam pattern based on direction inference is tractable since there are only a few multipath directions. Tracking the multipath components can lead to a robust and reliable connection.



% To reestablish the link quality, beam training is performed 

% Blockage and mobility~\cite{sur201560} are the most challenging and fundamental problems for mmWave system. The current solutions are not adequate: too naive and does not take advantage of unique mmWave properties such as high bandwidth, channel sparsity, and unique shape of beam patterns. 

% Due to the availability of higher bandwidth in the mmWave frequency range, the mmWave RAN can achieve data rates of the order of a few Gbps~\cite{CellularCap-Rap}, suitable for the QoS requirements for augmented reality (AR) and virtual reality (VR) applications. However, due to high path loss at mmWave frequencies, the coverage of mmWave RAN is limited. To improve the rate and coverage of mmWave networks, phased array antennas are used to create directional beams. Hundreds of antennas can be packed in a small area thanks to a low wavelength (a few millimeters) at these high frequencies. The directional antennas put a unique challenge for mmWave networks to find an optimal beam pattern at the access point (AP) and the user equipment (UE). IEEE 802.11ad standards describe a beam training algorithm that is used periodically to search for a suitable beam pattern. The beam pattern selected during the beamtraining phase (see Figure \ref{fig:twophases}) is used throughout the data transmission phase. 
% Mmwave links are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by more than 20 dB~\cite{georgeFading}. 




%  \textcolor{red}{Ish: I am throwing random ideas in next few paragraphs which need to be placed and rewritten properly.}

% Standards: IEEE 802.11ad \cite{ieee80211ad}, 802.15.3c~\cite{ieee802153c},  802.11ay~\cite{ieee80211ay}






% mmWave links are inherently directional to combat high path loss at higher frequencies. These directional links are highly susceptible to beam misalignment due to user mobility compared to a wide sector-level beam. Therefore, most commercial devices \textcolor{red}{[cite]} does not use fine beam patterns to avoid the signal degradation due to mobility. On the other hand, we take advantage of the fine beam patterns to track the user and refine the beam pattern to always align with the mobile user. 





% \begin{itemize}
%     \item \textit{Sparse channel:} The mmwave channel is sparse, i.e., only the LOS and a few NLOS paths characterize the channel. Furthermore, mmWave uses analog beams to focus the transmit energy in specific directions by choosing a particular combination of phase and attenuation at each transmit antenna \textcolor{red}{Figure: analog architecture}. 
    
%  \textit{   Note that the multi-stream communication may suffer from destructive interference due to the combination of multipath signal of opposite phase arriving at the receiver. 
%     In case two paths are interfering destructively, they won't appear in the CIR and so we won't consider those paths. They can be detected by their different AOD/TOF.}
%     \item \textit{Known patterns:} The directivity gain of the phased array antenna is a deterministic function of the codebook and antenna spacing and is known \textit{a-priori}. 
%     \item \textit{Advanced hardware:} Recent advances in antenna design allows high resolution in digital phase and amplitude control (6 bit and 4 bit resp. in our system). Furthermore, the phased array can generate close to ideal beam patterns by following various antenna calibration processes \textcolor{red}{[cite]}. This capability to generate regular beam patterns allow us to perform accurate RSSI based beam tracking.
%     \item \textit{CSI:} The CSI is used for many sensing application such as localization and tracking, and is readily available on commercial WiFi devices such as Quantenna \textcolor{red}{[cite]}. We expect the same trend for commercial mmWave system. 
%     \item \textit{Wideband:} We utilize the CSI and high bandwidth available at mmWave frequencies to separate multipaths via power-delay profile. prior work on blockage mitigation and beam alignment are based on narrow-band channel model~\cite{sur2016beamspy,zhou2017beam} which does not resolve multipaths.
% \end{itemize}



% Our main contributions are summarized as follows:
% \begin{itemize}
% \item \todo{Main contribution and results}
%     % \item We leverage the initial beam training to estimate the multipath parameters \{AOD, AOA, TOF\} and achieve high reliability through custom multi-lobe beam patterns. We also analyse reliability-throughput tradeoff for mmWave networks.
%     % \item We track the multipath and design a beam refinement algorithm to establish a stable link even under high user mobility scenario.
% \end{itemize}

% However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. 


% Thus, an unblocked Line of Sight (LOS) link is highly desirable for mmWave systems. When a LOS link is blocked, strong Non-Line of Sight (NLOS) links may also be helpful in achieving high reliability. However, NLOS links can also be blocked by mobile blockers. A mobile human blocker can block a link %between User Equipment (UE) and Base Station (BS) 
% for approximately 500 ms~\cite{georgeFading}. 


% At high frequencies, the attenuation due to obstacles is significant. For instance, 


==> Arxiv/1_intro_v8.tex <==
% !TEX root = main.tex

\section{Introduction}\label{sec:intro}


5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, defined as the fraction of time during which the link does not suffer an outage~\cite{driscoll2017enabling,ji2018ultra}. %In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that 
can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and therefore suffers from severe outage due to blockage and user's mobility. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that human blockages always bring down the link to an outage, which
is detrimental for high-reliability applications~\cite{ji2018ultra}.

% For example, blockage can reduce the signal strength by 20 dB, leading to an outage (no connectivity) for an extended period of 500 ms~\cite{maccartney2017rapid}, which is detrimental for high-reliability applications \cite{ji2018ultra}.
%When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam.
% Sub-6 GHz WiFi achieves high data-rate using spatial multiplexing which is function of existence of diverse multi-path in environment . However, 
% therefore even without multiplexing it can achieve multi-Gbps
% ~\footnote{Note that WiFi achieves high data-rate using spatial multiplexing which is function of existence of  diverse multi-path in environment and mmWave uses high bandwidth to achieve the same, but only requires existence  of a path between transmitter and receiver.}. To achieve 
% High bandwidth and directional beams allow mmWave to achieve high data rates required for video streaming applications.
% However, the directional link is vulnerable to blockages, device rotation, and user's mobility. A mobile blocker can reduce the signal strength by 20 dB, leading to outage which can be for an extended period of 500 ms~\cite{maccartney2017rapid}. When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam. In outdoor scenarios beam misalignment issue aggravates, 
% mmWave network if used for V2X has to support up to 500 km/h mobility while maintaining high throughput, high reliability, and ultra-low latency, which is challenging to achieve.
% Traditionally, mmWave network is optimized to provide high throughput of the order of a multi-Gbps~\cite{CellularCap-Rap}, thanks to high bandwidth and directional beams to combat higher pathloss at mmWave frequencies. 
%  The mmWave link can also degrade due to beam misalignment caused by device rotation and user's mobility.

Ideally, we would like to create a reliable mmWave link (a link without outage) that achieves high data-rate, is self-reliant unlike non-stand-alone access, and easy to deploy. However, conventional mmWave design~\cite{ieee80211ad} centers on improving the link throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive} and coverage~\cite{zhou2019robot,wei2017facilitating}, which inadvertently ends up relegating the reliability requirement. The mmWave base station and the user tediously scan multiple beams in their codebook to establish a directional link through \textit{beam training}. The beam training process is usually \textit{reactive}~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} which kicks in only after a significant degradation in link quality, leading to loss of connectivity and thereof reliability.
There are a few \textit{proactive} approaches that act before the link degrades by tracking the user. For this, these proactive approaches either require side-channel information from out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, which has limited accuracy and is limited to indoor environments, or external sensors ~\cite{haider2018listeer,zhou2018following,wei2017pose,va2015beam} which are not ubiquitous and not self-reliant. All of these approaches make the system difficult to deploy and dependant on external information.
% \textcolor{blue}{Moreover, external sensors collect sensitive information such as user location, which pose a privacy concern. 
In contrast, our goal is to improve system reliability and overall throughput without side-channel or external information.% i.e., self-reliant and easy to deploy. 
% Above all, the existing literature focuses on improving the average throughput of the system over a longer timescale.
% In contrast, our goal is to improve system reliability at both shorter and longer timescales,
% without side-channel or external information i.e. a self-reliant and easy to deploy solution. 



% \textit{Long outage duration and high frequency of prolonged beam training reduce the reliability of mmWave link.}

% fast handover~\cite{sur2018towards} or joint transmission from multiple APs~\cite{zhang2018mmchoir}.

% Though most research focuses on reducing the beam training delay, the delay generally increases with the size of the phased array~\cite{abari2016millimeter,barati2016initial,hassanieh2018fast}. 
%Besides, the beam training process has to be triggered frequently to avoid the harmful consequences of blockage and the user's mobility.

% In this work, we ask, can we achieve high-reliability mmWave links?  Traditionally, mmWave work has focused on blockage mitigation and beam alignment procedures \cite{sur2016beamspy,hassanieh2018fast} intending to improve the link throughput, which inadvertently ends up relegating the reliability requirement, leading to prolonged outages. The mmWave AP and the user periodically scan multiple beams in their codebook to find the right directional beam, commonly known as \textit{beam training}. The beam training process has to be triggered more frequently to avoid the harmful consequences of blockage and the user's mobility and can last as long as 10 msec for a codebook of a large antenna array~\cite{ieee80211ad}. Furthermore, blockage/user mobility detection is usually reactive~\cite{feng2017dealing} and may kick in only after significant detrimental impact on link quality, leading to loss of reliability. Some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam to avoid signal degradation due to mobility, but at the cost of significantly lower throughput while still being susceptible to outage due to blockages. \textit{Long outage duration, high frequency of beam training, and long beam training delays reduce the reliability of mmWave link.}
% The beam training is conducted to recover from outage or initial beam training, . %for communication through a process commonly known as \textit{beam training}. Although beam training has been studied extensively \textcolor{red}{[cite]}, the beam training delay is of the order of the logarithm of number of beams in the codebook~\cite{dina}. The codebook size for a large phased array can be huge, and the training takes order of a few 10 ms, during which there is no communication.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.52\textwidth]{figures/mmReliable_prototype.pdf}
    \caption{Shows the Conventional mmWave on the left and \name on the right. \name utilizes beam patterns with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beam pattern.\newtodo{gNB in corner. Use two beams.} }
    \label{fig:prototype}
    \vspace{-0.1in}
\end{figure}
% to take advantage of multi-path caused by strong reflectors in the environment to improve reliability. We get insights
% \textbf{\name's first design principle} is inspired from sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. To improve reliability, some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam as shown in Figure~\ref{fig:prototype}(a). However, a wide-beam suffers from significantly lower throughput and connectivity range while still being susceptible to outage due to blockages. In contrast, \name creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that are aligned towards LOS or strong reflected paths as shown in Figure~\ref{fig:prototype}(b). The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 



% In this paper, we present \name, which intends to create a reliable mmWave link, while maintaining high data rates. We get the insights from sub-6 GHz communication which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. 
% \name's first design principle is slightly counter-intuitive, where it creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that take advantage of multi-path caused by strong reflectors in the environment as shown in Figure~\ref{fig:prototype} (b). Beam splitting may reduce the range of connectivity, but provides reliability. 
% The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Notably, multi-beam provides an advantage in terms of range and throughput compared to a wide-beam since all the beams in a multi-beam pattern are aligned towards LOS or strong reflected paths. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

% Multi-lobe pattern has been used in MUTE and BounceNet ~\cite{jog2019many, ghasempour2018multi}.

% Theory work xxx needs channel by decoupling beam patterns which is challenging and time consuming [ACO, ]

In this paper, we introduce \name, the first system that achieves both high-reliability and high-data-rate mmWave links while being self-reliant (on the mmWave link) and is easy to deploy. \name's key design principle is inspired by sub-6 GHz communication,  
% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
%\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.
%
%\textbf{\name's first design principle} is inspired by sub-6 GHz communication, 
which can deliver high reliability in part by exploiting the multi-path environment. However, the same is not valid for traditional mmWave, which uses a single directional beam along the Line of Sight (LOS) or toward a strong reflector (NLOS). 
\name key design principle is to create custom beam patterns with multiple directional beams (\textit{multi-beam} for brevity) that are each aligned towards LOS and strong reflected paths, while keeping the Total Radiated Power (TRP) same as a single beam (FCC compliant), as shown in Fig.~\ref{fig:prototype}(b). 
The insight here is that the probability of multiple beams simultaneously facing a blockage is low, reducing the possibility of link outage. 

% \todo{no!!, you are performing constrcutive combining which is helping it improve SNR!! talk about constructive combining and then give the example, your techniques should be summarized here...} 

A natural question is how does \name achieves high throughput with mutli-beam. An obvious implication of splitting the single beam to a multi-beam is loss in power per beam called as EIRP (Equivalent Isotropic Radiated Power) to meet the same total radiated power (TRP) constraint. The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver. At first glance, it seems as if multi-beam trades throughput for reliability while the goal was to improve both, but turns out we can break the trade-off. Our insight into breaking this trade-off is based on the observation that the received signal is the sum of multiple copies of the transmitted signal, for every beam in a multi-beam. If we can ensure the signal adds up in the signal domain constructively, we can increase the signal strength and throughput.

Let's see with an intuitive example, say a mmWave channel consisting of two paths; and two-beam are aligned along those two-channel paths as shown in Figure \ref{fig:prototype}(b). For simplicity, assume the path loss is unity for each path, and the phase of signal travelled for each path is the same. \name's transmitter for this channel, splits the total power of $a^2$ equally into two beams with power $a^2/2$ on each beam, i.e., amplitude $a/\sqrt{2}$ on each beam, which undergoes the channel and is received with omni-receiver. Since the phase align for both paths, the received signal adds in signal domain, i.e. total amplitude of the received signal $ a/\sqrt{2} + a/\sqrt{2} = \sqrt{2}a$. The received signal upon converting to SNR (signal-to-noise ratio) is proportional to $2a^2$. In contrast, a traditional mmWave single-beam link does not exploit the second path and would provide an SNR proportional to $a^2$, which is 3 dB lower compared to a multi-beam case. By using mutli-beam with constructive combining, we achieve both throughput and reliability gains, by harnessing a multi-path environment without increasing the total transmit power. 


 %We mathematically show that our multi-beam patterns with optimized phase and amplitude are optimal and maximizes the SNR for any given wireless channel.

In the above simple example, we assumed a strong multi-path channel with similar gain as the direct path and aligned phase with the direct path at the receiver (constructive combining). However, real-world channels are complex with multi-paths that are weak and have phase value that doesn't align with the direct path. First, we extend this analysis and mathematically prove that with proper power control per beam and phase shift per beam, one can achieve optimal constructive combining, that can maximize signal to noise ratio and thereby achieving both throughput and reliability gains. The second challenge for \name is to estimate the beam directions, optimal beam-phase and amplitude to be applied to achieve constructive combining. \name builds a novel algorithm which is 5G protocol complaint, and can extract all these parameters thereby developing a low-cost beam probing mechanism to estimate the beam parameters~\newtodo{}. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. Finally, creating a multi-beam pattern in hardware with the optimal beam directions with optimal phase and power control is challenging, as a beam super-position doesn't achieve the desired behaviour due to inter-product and quantization of the hardware, we build a novel algorithm to construct multi-beam with desired optimal phase and power control on 5G NR hardware. 
%  code-book addition cannot achieve  poses an additional challenge due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed.


% First, we develop novel analog beamforming techniques that optimize per-beam phase and power control in a multi-beam to enable constructive combining. 

% A natural question is how do we achieve constructive combing. Specifically, 



%  Furthermore, we prove that it would be always be better than ...  \name can therefore deliver a high reliability and high throughput link. 



% We present an intuitive example to explain the benefits of \name's constructive combining optimization. For simplicity, we consider the transmitter uses a 2-beam pattern aligned with two channel paths and the receiver is omni-directional. Assume the pathloss of each path is unity in which case \name allocates equal amplitude to each beam. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path, our constructive combining leads to the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. A careful reader would infer that the throughput gain is obtained by harnessing multi-path environment without increasing the total power. \name can therefore deliver reliable link while maintaining high throughput. 

% \textcolor{purple}{
% The intuitive example, however, does not explain multiple practical challenges in establishing a multi-beam link. (i) In practice, the reflected path channel suffers from higher attenuation which may affect the throughput gain. To deal with weaker paths, \name performs a joint optimization of phase and amplitude of each beam in a multi-beam to maximise SNR. (ii) The second challenge is to estimate the phase, attenuation and angle of each channel path which is required to generate phase-coherent multi-beam patterns. \name develops a beam probing mechanism to estimate the channel parameters. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. (iii) Finally, creating multi-beam pattern in hardware poses additional challenges due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed. }

% In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of optimal channel-dependent beam pattern. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.

% The critical insight is that the multi-beam model is equivalent to transmitter diversity for low-frequency communication~\cite{tse2005fundamentals}, where multiple antennae transmit together to add up the signals at the receiver constructively. Such a scheme can increase the signal power received by the factor of the number of transmitting antennae, while simultaneously meeting the TRP constraints. \name is the first practical system to realize the transmit diversity for the mmWave communication systems with a single phased array and without relying on multiple RF chain. 

% \textcolor{purple}{
% The diversity gain achieved by \name can be understood by a simple example.
% Let's say there are two paths, each with say each with equal pathloss of unity. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path. \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. 
% With our constructive amplitude combining the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. \name takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. In fact, we mathematically show that the phase-coherent multi-beam patterns are optimal under given multi-path channel when the number of beams are same as the number of channel paths. In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of ideal channel-dependent beam pattern. We propose a tractable approach to estimate the phase and amplitude per-beam with negligible overhead. Our approach requires only two probes for 2 beams and 4 probes for 3 beam case. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.}

% \todo{Mention that multi-beam requires attenuation control of more than 10 dB? but most commercially available arrays do not provide that control and so multi-beam was not feasible yet. We are the first to explore it.}

% An obvious implication of splitting the single lobe in to multiple beam is it would lead loss of signal radiated per beam of multiple beam on transmitter to meet EIRP (Equivalent Isotropic Radiated Power) constraint. 
% Therefore, the multi-beam concept may lead to the loss in signal strength received at the receiver, as the transmitted signal are individually reduced in power to meet EIRP. 
% The surprising observation is that in some scenarios, the signal received at the receiver increases by creating multi-beam compared to a single beam. 

% \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead.
% The above intuitive result is demonstrated in the Eq.3, where $\delta=1$ so $(1 + \delta^2) = 2$ i.e. 2 times the SNR. This is called diversity gain, or transmit beamforming gain, which is popularly taught in wireless classes as one of the first key principle, where the power is normalized as well. The paper explains the power normalization in the introduction, and when creating multiple beams, so

% To achieve full transmit diversity, i.e., improving signal to noise ratio optimally at the receiver, it requires the constructive combining of the signal from each beam (or transmitter).  \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. It takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.


% Furthermore, note that the reflected path can have up to 20 dB of signal degradation compared to direct path and still the throughput of \name would be better than single beam link. However, turns out for 28 GHz mmWave the difference in the path-loss of the signal from naturally occurring reflectors and the direct path signal is minimal~\cite{samimi2014characterization}.

% The key insight behind this increase in received signal power for multi-beam compared to the single beam is that multi-beam in mmWave is equivalent to transmitter diversity for low frequency communication\todo{~\cite{}}. For transmitter diversity the signal power is distributed among multiple antennas, whereas in mmWave it is distributed among multiple beams. If the received signal from these multi-beams (or transmitters) combine constructively at the receiver they increase the signal received by the factor of number of antenna, while even meeting the EIRP constraints.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figures/brp_timeline_fig2_crop.pdf}
%     \caption{Shows \name tracks the user mobility and proactively refines the multi-beam patterns. It shows the \name link performs well even without beam training overhead. In contrast, the reactive framework performs beam training to recover a dead link. }
%     \label{fig:prototype_2}
%     \vspace{-0.1in}
% \end{figure}


% % \name designs an innovative approach to create multi-beam patterns and distribute power along multiple directions.  
% \todo{make this paragraph challenges only, and say that you overcome in the paper}
% In order to achieve full transmit diversity, i.e. improving signal to noise ratio optimally at the receiver, it requires constructive combining of the signal from each beam (or transmitter). Said differently, the challenge with multi-beam communication is that the signal travels through different paths and adds up at the receiver, which could lead to destructive combining leading to the loss of the signal at the receiver. The loss in the signal can result in reduced throughput for multi-beam. To overcome this problem, \name builds a novel algorithm that creates phase per beam and adapts the phase per beam in real-time to make sure the signal combines constructively. Moreover, it takes advantage of recent advances\cite{IDT} in antenna design for 28 GHz and shows that efficient multi-beam patterns can be created with per-antenna analog phase and amplitude control. Furthermore, it uses the standard beam training process to learn the phase per beam for constructive combining, not creating any additional overhead for per beam phase estimation.
% While multi-beam helps improve link reliability for a static user under blockage, in a dynamic environment, it is still prone to link degradation due to user mobility.


% To achieve the multi-beam and proactive response with a goal of high throughput and high-reliability, \name needs to address the following challenges. The first challenge is that \name distributes the power across multiple beams, these beams travel through different path and add up at the receiver, would could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput. In order to overcome this problem, \name builds a novel algorithm which creates phase per beam, and adapts the phase per beam in real-time to make sure the signal combines constructively. \name takes advantage of recent advances in antenna design for 28 GHz, and shows that with per antenna analog phase and amplitude control (6 bit and 4-bit resp. in our system).
% While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

So far, we have explained how to perform beam training and establish a \name mutli-beam link.  Mobility adversely affects the established links by causing misalignment between transmit and receive beams. Moreover, the problem is complicated with mutli-beam as the \name needs to re-align all the multiple beams with power and phase control per beam depending upon blockage or mobility situations. Therefore, none of the prior work can be used, as it requires tracking multiple beams angle, phase and power tracking. \name builds a novel proactive approach to maintain and track power, phase and beam direction of each of the multiple beams. \name's approach is to track the effects of mobility or blockage per-beam in the background by simply leveraging passive measurements of the mmWave received signal, making \name self-reliant. \name uses a tracking algorithm to periodically re-align each beam of the multi-beam and adjust their phase and amplitude, even when there is no significant link degradation. For example, in the blockage case, \name reduces the power along the blocked beam long before the link is degraded, thus increasing the power along the unblocked beam and maintaining the link. Similarly, in the case of user mobility, it continually re-aligns the beam directed towards the user. Therefore, \name prevents links from falling into outages.
% , as demonstrated through a prototype in Figure \ref{fig:prototype_2}. 




% To realize per beam tracking on a practical system even under mobility or blockage, \name needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to identify the blockage or user movement (self-reliant). Specifically, it measures the rate of degradation of the signal strength and creates thresholds for blockage and user movement and depending upon the observed degradation of the signal strength, it pro-actively calls it out as blockage or user movement. Furthermore, under user movement or mobility, the general motion is complex and hard to track, making beam re-alignment difficult. 

% In contrast, \name's key contribution is to decouple the complex user movement into rotation and translation movement and track them individually. An important observation is that all the beams within multi-beam undergo the same amount of angular movement for the rotation case, while for the translation case, the beams undergo different motion. We leverage this observation to design an angular rotation based beam tracking algorithm. A natural question is how do we measure the angular rotation per beam. In order to measure angular rotation per beam, we use the rate of change of amplitude per beam and phased-array antenna response, to determine the amount of rotation per beam. In summary, \name designs a novel amplitude-based tracking algorithm to track each beam individually. It only needs to measure 100 $\mu$sec of the received amplitude per beam to make the measurement. \textcolor{blue}{Also, note that \name only measures the angle to the UE for tracking and doesnot require exact user location, thus, preserving user privacy.}

%Second, \name needs to react to blockage or user movement per beam. The reaction to blockage is to reduce the power on the blocked beam. In contrast, to react for user mobility is challenging, it needs to  and the power and the phase for constructive combining, which requires it to identify the user movement. 

%First, to identify whether a particular beam is blocked or mis-aligned due to mobility, 

On a practical system, per beam tracking has to be performed even with user mobility and blockage. \name, therefore, needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to make this distinction. The challenge is that the received signal is a combination of all beams in the multi-beam due to a single receiver chain on the receiver (analog beamforming). A naive approach could be to use the received signal to measure the channel in time-domain and use the separation of different beams in time-of-flight to identify amplitude corresponding to each beam. However, the multiple beams can often have very close times-of-flight (ToF) and cannot be resolved even with the high-sampling rate of mmWave (2.5 ns resolution with 400 MHz). To accurately determine amplitude per beam, \name builds a super-resolution algorithm that leverages the relative time-of-flight information (between beams). \name's insight is that the relative time-of-flight remains constant across multiple packets between beams, and \name uses this insight to learn their amplitudes. Furthermore, the relative ToFs are easily acquired during the initial standard beam training phase, requiring no protocol changes to achieve the tracking algorithm. 

% Finally, an implicit assumption made while performing per-beam tracking is the ability to recover per-beam amplitude. 

\textbf{Evaluation:} We demonstrate \name on a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array, which can support channels of up to 400 MHz. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 
We deploy \name in various indoor and outdoor scenarios and evaluate its performance. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 


%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 

%The key insight to 

% first point is seperation between blockage vs mobility. 
%\name first leverages the multi-beam set up to identify any movement or blockage. Then, 

%While in case of mobility, \name estimates the change directly in each beam angle due to the mobility. Specifically, it leverages the multi-beams to jointly estimate the accurate tracking of the beam angle for each beam. \name's proactive beam alignment process is fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. 
%\textit{}  


 
 %\textcolor{blue}{ Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and relative ToF \textcolor{red}{[downplay relative ToF here?]}(relative to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.}
 
% \name's second design principle for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility, i.e., \name preemptively tracks the beam and refines it without any explicit beam training. The approach gradually tracks the effects of mobility and the environment in the background, even when link throughput is not significantly affected. The beams are then periodically aligned with the mobile user. Therefore, it prevents links from falling into outages, as demonstrated through a prototype in Figure~\ref{fig:prototype}(c). \name's beam refinement is very fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. \textit{In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.}  


% The design philosophy of \name is different from other approaches. While recent proposals relies on assistance from device positioning system~\cite{zhou2018following,wei2017pose,va2015beam}, out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, or light sensors~\cite{haider2018listeer}, \name is deployed without any additional hardware or sensor support. In a similar line of research, BeamSpy~\cite{sur2016beamspy} and Beam-forcast~\cite{zhou2017beam} provides a model-driven approach to handle blockage and mobility, respectively; however, they lack a unified framework to integrate both vulnerabilities. Above all, the literature focusses on improving the average throughput of the system over a long timescale. On the other hand, \name's design philosophy is to improve system reliability at a short millisecond timescale. 


% An important observation here is that individual beams in a multi-beam are affected differently by these effects. Blockage significantly reduces the power of the beam oriented toward it, rotation of the user causes an almost equal drop in power across all beams, and translation causes an unequal power drop across beams. In case of blockage, \name reduces the power along the blocked beam, while in case of mobility, \name estimates the angle of movement.

% When \name detects blockage of a beam, it reduces the power along that beam. 



% \name achieves its goal by first setting up a multi-beam mmWave link and then proactively maintaining it. 
% To realize multi-beam tracking on a practical system, \name needs to address the following additional challenges.

% \noindent
% \textbf{Challenge 1) Multi-beam set up:} The first challenge for \name is to establish a multi-beam communication link. These beams travel through different path and add up at the receiver, could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput.
% and ensure that the signal along multiple beams adds up constructively at the receiver.



% \noindent
% \textbf{Solution:} \name takes advantage of recent advances in antenna design that allows high resolution in digital phase and amplitude control (6 bit and 4-bit resp. in our system). We showed that multi-beam patterns could be created by a weighted average of complex phasers of individual beams within multi-beam. The weights, however, if not appropriately set, may cause the signal along multi-paths to add up destructively at the receiver. We introduce a co-phasing factor that adjusts the relative phase of beams in multi-beam setup and device a method to tune that factor with low probing overhead.

% \noindent
% \textbf{Challenge 2) Multi-path separability:} \name is built on tracking per-beam amplitude in a multi-beam setup. Per-beam tracking is challenging since the received signal is a combination of all beams in the multi-beam due to analog beamforming. 

% \noindent
% \textbf{Solution:}  \name's key insight is to use the relative ToF information for each beam to learn its amplitude. However, with multiple beams often the multiple paths can have very close ToF, and cannot be resolved even with 15 cm resolution (2 GHz bandwidth at 60 GHz) or 75 cm resolution (400 MHz bandwidth at 28 GHz). To accurately resolve the beams, we build a super-resolution algorithm that leverages the relative ToF information (between beams) learned during the initial training phase, to produce accurate amplitude information per beam. 

% We then use the variation in per-beam amplitude over time to identify movement/blockage and modify the multi-beam pattern to maintain a reliable link.



% \noindent
% \textbf{Challenge 3) Multi-path parameter estimation:} 
% Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. 

% \noindent
% \textbf{Solution:}
% We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and related ToF (related to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.

% however, these parameters are typically estimated individually which pose  the mapping of AoA, AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. 

% Prior work \cite{palacios2018adaptive} relies on a custom training process to estimate absolute channel response per antenna and then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. 

% A key challenge is to associate the AoA with the AoD of corresponding reflectors.

% \name requires the knowledge of reflector location, orientation, and reflectively. Prior work suggest to get it offline manually \cite{wei2017facilitating} but \name need to get them in real-time.


% \name uses initial beam training to infer the strongest multi-paths in the environment, their angles of departure (AoD, beam from the transmitter), angles of arrival (AoA, beam at the receiver) and relative times-of-flight (relative ToF for each strong multi-path). \name uses the AoA, AoD, and relative ToF to learn reflector orientations in the environment by a smart ToF based association algorithm; the orientation of reflectors are necessary for proactive learning. 

% This knowledge of the multi-path environment augmented with recent advancements in mmWave antennas (achieving 6-bit phase and 7-bit amplitude control per antenna) to create a multi-beam link facilitates proactive learning as described below.
% enhanced by multi-path effects at both the transmitter and receiver.







% \begin{comment}


% Turns out 5G NR o
% super-resolution algorithm to recover Recall that during the initial beam training, we can learn about all the strong multi-path, we 
% can also use the initial 
% \item \textit{}
%     Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.


%     A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
    
% A natural question how does \name uses multi-beam to mitigate blockage and track user under mobility, 
% how does it maintain reliable connectivity using multi-beam. 



% To achieve reliable connectivity using multi-beam, \name builds an algorithm to track each of the individual beam 
% in the multiple beam from transmitter to the receiver. The individual track 



% % tell them how individual beam tracking in multi-beam solves both the 


% Challenge 1: individual beam tracking 

% Challenge 2: amplitude level tracking 
% % multi-beam tracking

% % amplitude level tracking 

% % ToF based seperation to achieve amplitude. 

% % rotation and translation 

% to the receiver but also help to track the user trajectory. \name refines the beam pattern over time to keep 
% it aligned with the mobile user, thus creating a stable WiFi-like link 
% %\textcolor{red}{[Should we mention that \name approximates the omni-pattern of sub-6GHz WiFi for directional mmWave link?]}. 
% The beam refinement\footnote{We use the IEEE 802.11ad terminology of beam training and beam refinement 
% which is discussed in Section \ref{sec:motivation}} with a multi-lobe pattern requires scanning of a constant 
% number of beams (0.1 ms latency) as compared to the beam training process that requires scanning 100's of beams 
% in the codebook at both transceiver (10 ms latency). \name's time complexity is of the order of the number of lobes, 
% which is typically directed towards 2-3 strong reflectors due to channel sparsity.

% Multi-lobe beam patterns has been explored in literature \textcolor{red}{[Cite Agile-link]} to reduce the 
% beam training delay, however, for the first time, \name exploits the unseen opportunity to use multi-lobe 
% patterns during the data transmission phase to enhance the link reliability. 

% The key challenges for \name are as follows:
% \begin{itemize}
%     \item \textit{The blockage mitigation has to be proactive.} \name creates custom multi-lobe patterns that are aligned with the strong reflectors providing multipath diversity. While some paths may suffer blockage, alternate unblocked paths are immediately available. A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
%     \item \textit{Beam alignment requires accurate tracking of mobile user with minimal overhead.} Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.
% \end{itemize}

% \end{comment}


% Instead of using a fix codebook based design, we first estimate the multipath directions and implement multipath aware beam patterns.
% Note the code book might contain thousands of beam patterns but there are only a 2-3 multipaths due to channel sparsity.
% In a nutshell, we propose a paradigm shift for millimeter wave communication to design multipath aware beam patterns. Finding the right beam out of thousands of possible beam patterns is time-consuming, however, creating a beam pattern based on direction inference is tractable since there are only a few multipath directions. Tracking the multipath components can lead to a robust and reliable connection.



% To reestablish the link quality, beam training is performed 

% Blockage and mobility~\cite{sur201560} are the most challenging and fundamental problems for mmWave system. The current solutions are not adequate: too naive and does not take advantage of unique mmWave properties such as high bandwidth, channel sparsity, and unique shape of beam patterns. 

% Due to the availability of higher bandwidth in the mmWave frequency range, the mmWave RAN can achieve data rates of the order of a few Gbps~\cite{CellularCap-Rap}, suitable for the QoS requirements for augmented reality (AR) and virtual reality (VR) applications. However, due to high path loss at mmWave frequencies, the coverage of mmWave RAN is limited. To improve the rate and coverage of mmWave networks, phased array antennas are used to create directional beams. Hundreds of antennas can be packed in a small area thanks to a low wavelength (a few millimeters) at these high frequencies. The directional antennas put a unique challenge for mmWave networks to find an optimal beam pattern at the access point (AP) and the user equipment (UE). IEEE 802.11ad standards describe a beam training algorithm that is used periodically to search for a suitable beam pattern. The beam pattern selected during the beamtraining phase (see Figure \ref{fig:twophases}) is used throughout the data transmission phase. 
% Mmwave links are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by more than 20 dB~\cite{georgeFading}. 




%  \textcolor{red}{Ish: I am throwing random ideas in next few paragraphs which need to be placed and rewritten properly.}

% Standards: IEEE 802.11ad \cite{ieee80211ad}, 802.15.3c~\cite{ieee802153c},  802.11ay~\cite{ieee80211ay}






% mmWave links are inherently directional to combat high path loss at higher frequencies. These directional links are highly susceptible to beam misalignment due to user mobility compared to a wide sector-level beam. Therefore, most commercial devices \textcolor{red}{[cite]} does not use fine beam patterns to avoid the signal degradation due to mobility. On the other hand, we take advantage of the fine beam patterns to track the user and refine the beam pattern to always align with the mobile user. 





% \begin{itemize}
%     \item \textit{Sparse channel:} The mmwave channel is sparse, i.e., only the LOS and a few NLOS paths characterize the channel. Furthermore, mmWave uses analog beams to focus the transmit energy in specific directions by choosing a particular combination of phase and attenuation at each transmit antenna \textcolor{red}{Figure: analog architecture}. 
    
%  \textit{   Note that the multi-stream communication may suffer from destructive interference due to the combination of multipath signal of opposite phase arriving at the receiver. 
%     In case two paths are interfering destructively, they won't appear in the CIR and so we won't consider those paths. They can be detected by their different AOD/TOF.}
%     \item \textit{Known patterns:} The directivity gain of the phased array antenna is a deterministic function of the codebook and antenna spacing and is known \textit{a-priori}. 
%     \item \textit{Advanced hardware:} Recent advances in antenna design allows high resolution in digital phase and amplitude control (6 bit and 4 bit resp. in our system). Furthermore, the phased array can generate close to ideal beam patterns by following various antenna calibration processes \textcolor{red}{[cite]}. This capability to generate regular beam patterns allow us to perform accurate RSSI based beam tracking.
%     \item \textit{CSI:} The CSI is used for many sensing application such as localization and tracking, and is readily available on commercial WiFi devices such as Quantenna \textcolor{red}{[cite]}. We expect the same trend for commercial mmWave system. 
%     \item \textit{Wideband:} We utilize the CSI and high bandwidth available at mmWave frequencies to separate multipaths via power-delay profile. prior work on blockage mitigation and beam alignment are based on narrow-band channel model~\cite{sur2016beamspy,zhou2017beam} which does not resolve multipaths.
% \end{itemize}



% Our main contributions are summarized as follows:
% \begin{itemize}
% \item \todo{Main contribution and results}
%     % \item We leverage the initial beam training to estimate the multipath parameters \{AOD, AOA, TOF\} and achieve high reliability through custom multi-lobe beam patterns. We also analyse reliability-throughput tradeoff for mmWave networks.
%     % \item We track the multipath and design a beam refinement algorithm to establish a stable link even under high user mobility scenario.
% \end{itemize}

% However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. 


% Thus, an unblocked Line of Sight (LOS) link is highly desirable for mmWave systems. When a LOS link is blocked, strong Non-Line of Sight (NLOS) links may also be helpful in achieving high reliability. However, NLOS links can also be blocked by mobile blockers. A mobile human blocker can block a link %between User Equipment (UE) and Base Station (BS) 
% for approximately 500 ms~\cite{georgeFading}. 


% At high frequencies, the attenuation due to obstacles is significant. For instance, 


==> Arxiv/1_intro_v9.tex <==
% !TEX root = main.tex

\section{Introduction}\label{sec:intro}


5G New Radio (NR) is expected to support cutting edge applications such as V2X, factory automation, autonomous driving, and remote surgery~\cite{5gnr}. A key requirement for such applications beyond the high data rate is exceptionally high reliability, 
defined as the fraction of time during which the link does not suffer an outage~\cite{driscoll2017enabling,ji2018ultra}. %In fact, mission-critical applications such as telesurgery and autonomous driving require ultra-high reliability with less than one in a million outage events~\cite{ji2018ultra}.
% \textcolor{red}{Ish: Mention a URLLC application that they require link to be available all the time with 100 \% reliability. V2X link failure for even a fraction of second may lead to a fatal accident.} 
As such, 5G NR utilizes millimeter-wave (mmWave, FR2) frequencies due to abundant bandwidth (400MHz-2GHz) that 
can provide the high-data-rate compared to traditional sub-6 GHz FR1 (20-100MHz bandwidth) bands 
~\cite{Rappaport2013Millimeter}. However, unlike its sub-6 GHz counterparts, mmWave uses directional beams to reduce the impact of higher path loss at mmWave frequencies and therefore suffers from severe outage due to blockage and user's mobility. For instance, a measurement study of 28 GHz network deployment in 
Chicago~\cite{narayanan2019first} shows that human blockages always bring down the link to an outage, which
is detrimental for high-reliability applications~\cite{ji2018ultra}.

% For example, blockage can reduce the signal strength by 20 dB, leading to an outage (no connectivity) for an extended period of 500 ms~\cite{maccartney2017rapid}, which is detrimental for high-reliability applications \cite{ji2018ultra}.
%When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam.
% Sub-6 GHz WiFi achieves high data-rate using spatial multiplexing which is function of existence of diverse multi-path in environment . However, 
% therefore even without multiplexing it can achieve multi-Gbps
% ~\footnote{Note that WiFi achieves high data-rate using spatial multiplexing which is function of existence of  diverse multi-path in environment and mmWave uses high bandwidth to achieve the same, but only requires existence  of a path between transmitter and receiver.}. To achieve 
% High bandwidth and directional beams allow mmWave to achieve high data rates required for video streaming applications.
% However, the directional link is vulnerable to blockages, device rotation, and user's mobility. A mobile blocker can reduce the signal strength by 20 dB, leading to outage which can be for an extended period of 500 ms~\cite{maccartney2017rapid}. When the user is mobile, even an unblocked and properly aligned beam will suffer from signal degradation due to the angular deviation from the direction of the beam. In outdoor scenarios beam misalignment issue aggravates, 
% mmWave network if used for V2X has to support up to 500 km/h mobility while maintaining high throughput, high reliability, and ultra-low latency, which is challenging to achieve.
% Traditionally, mmWave network is optimized to provide high throughput of the order of a multi-Gbps~\cite{CellularCap-Rap}, thanks to high bandwidth and directional beams to combat higher pathloss at mmWave frequencies. 
%  The mmWave link can also degrade due to beam misalignment caused by device rotation and user's mobility.

Ideally, we would like to create a reliable mmWave link (a link without outage) that achieves high data-rate, and easy to deploy with upcoming 5G infrastructure. However, conventional mmWave design~\cite{ieee80211ad} centers on improving the link throughput~\cite{sur2016beamspy, zhou2017beam,palacios2018adaptive} and coverage~\cite{zhou2019robot,wei2017facilitating}, which inadvertently ends up relegating the reliability requirement. The mmWave base station and the user tediously scan multiple beams to establish a directional link through \textit{beam training}. The beam training process is usually \textit{reactive}~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast} which kicks in only after a significant degradation in link quality, leading to loss of connectivity and thereof reliability.
There are a few \textit{proactive} approaches that act before the link degrades by tracking the user. These proactive approaches either require side-channel information from out-of-band LTE/WiFi~\cite{sur2017wifi,nitsche2015steering} or rely on external sensors. These solutions apart from not being ubiquitous and self-reliant, have limited accuracy 
% and are limited to indoor environments
~\cite{haider2018listeer,zhou2018following,wei2017pose,va2015beam}. All these approaches make the system difficult to deploy and dependant on external information or non-stand-alone access.
% \textcolor{blue}{Moreover, external sensors collect sensitive information such as user location, which pose a privacy concern. 
In contrast, our goal is to improve the inherent mmWave system reliability and overall throughput without side-channel or external information.% i.e., self-reliant and easy to deploy. 
% Above all, the existing literature focuses on improving the average throughput of the system over a longer timescale.
% In contrast, our goal is to improve system reliability at both shorter and longer timescales,
% without side-channel or external information i.e. a self-reliant and easy to deploy solution. 



% \textit{Long outage duration and high frequency of prolonged beam training reduce the reliability of mmWave link.}

% fast handover~\cite{sur2018towards} or joint transmission from multiple APs~\cite{zhang2018mmchoir}.

% Though most research focuses on reducing the beam training delay, the delay generally increases with the size of the phased array~\cite{abari2016millimeter,barati2016initial,hassanieh2018fast}. 
%Besides, the beam training process has to be triggered frequently to avoid the harmful consequences of blockage and the user's mobility.

% In this work, we ask, can we achieve high-reliability mmWave links?  Traditionally, mmWave work has focused on blockage mitigation and beam alignment procedures \cite{sur2016beamspy,hassanieh2018fast} intending to improve the link throughput, which inadvertently ends up relegating the reliability requirement, leading to prolonged outages. The mmWave AP and the user periodically scan multiple beams in their codebook to find the right directional beam, commonly known as \textit{beam training}. The beam training process has to be triggered more frequently to avoid the harmful consequences of blockage and the user's mobility and can last as long as 10 msec for a codebook of a large antenna array~\cite{ieee80211ad}. Furthermore, blockage/user mobility detection is usually reactive~\cite{feng2017dealing} and may kick in only after significant detrimental impact on link quality, leading to loss of reliability. Some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam to avoid signal degradation due to mobility, but at the cost of significantly lower throughput while still being susceptible to outage due to blockages. \textit{Long outage duration, high frequency of beam training, and long beam training delays reduce the reliability of mmWave link.}
% The beam training is conducted to recover from outage or initial beam training, . %for communication through a process commonly known as \textit{beam training}. Although beam training has been studied extensively \textcolor{red}{[cite]}, the beam training delay is of the order of the logarithm of number of beams in the codebook~\cite{dina}. The codebook size for a large phased array can be huge, and the training takes order of a few 10 ms, during which there is no communication.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.43\textwidth]{figures/mmreliable_prototype_v2.pdf}
    \caption{Shows the Conventional mmWave on the left and \name on the right. \name utilizes beam patterns with multiple lobes (\textit{Multi Beam}) to provide high reliability compared to a single-lobe beam pattern.\newtodo{gNB in corner. Use two beams. DB: I don't like the figure, I like mmReliable_prototype.pdf } }
    \label{fig:prototype}
    \vspace{-0.1in}
\end{figure}
% to take advantage of multi-path caused by strong reflectors in the environment to improve reliability. We get insights
% \textbf{\name's first design principle} is inspired from sub-6 GHz communication, which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. To improve reliability, some commercial mmWave devices, e.g., Talon AD7200~\cite{talonad7200}, Airfide 5G~\cite{airfide}, use a wide sector-level beam as shown in Figure~\ref{fig:prototype}(a). However, a wide-beam suffers from significantly lower throughput and connectivity range while still being susceptible to outage due to blockages. In contrast, \name creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that are aligned towards LOS or strong reflected paths as shown in Figure~\ref{fig:prototype}(b). The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 



% In this paper, we present \name, which intends to create a reliable mmWave link, while maintaining high data rates. We get the insights from sub-6 GHz communication which can deliver high reliability in part by exploiting the multi-path rich environment. The same is not true for traditional mmWave, which uses highly directional beams directed either towards a Line of Sight (LOS) or a reflected path. 
% \name's first design principle is slightly counter-intuitive, where it creates custom beam patterns with multiple main lobes (We call it \textit{multi-beam} for brevity) that take advantage of multi-path caused by strong reflectors in the environment as shown in Figure~\ref{fig:prototype} (b). Beam splitting may reduce the range of connectivity, but provides reliability. 
% The insight is that the probability of all the beams within multi-beam simultaneously facing a blockage is low, reducing the chances of the link outage. Notably, multi-beam provides an advantage in terms of range and throughput compared to a wide-beam since all the beams in a multi-beam pattern are aligned towards LOS or strong reflected paths. Note that the number of beams in multi-beam need not be large since the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

% Multi-lobe pattern has been used in MUTE and BounceNet ~\cite{jog2019many, ghasempour2018multi}.

% Theory work xxx needs channel by decoupling beam patterns which is challenging and time consuming [ACO, ]

In this paper, we introduce \name, a system which achieves both high-reliability and high-data-rate mmWave links, while being 5G NR compliant. \name's key design principle is inspired by sub-6 GHz communication,  
% \textcolor{blue}{Importantly, \name achieves high performance without collecting user location data and so preserves user's privacy.} 
%\name relies on two novel design principles to achieve the goal of high reliability: %In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.
%
%\textbf{\name's first design principle} is inspired by sub-6 GHz communication, 
which delivers high reliability and throughput, by exploiting multipath diversity from environmental reflections\cite{}. 
However, the same is not valid for traditional mmWave, which uses a single directional beam along the Line of Sight (LOS) or toward a strong reflector (NLOS). 
\name's key design principle is to create custom beam patterns with multiple directional beams (\textit{multi-beam} for brevity) that are each aligned towards LOS and strong reflected paths, while keeping the Total Radiated Power (TRP) same as a single beam (FCC compliant), as shown in Fig.~\ref{fig:prototype}(b). 
The insight here is that the probability of multiple beams simultaneously facing a blockage is low, reducing the possibility of link outage. 

% \todo{no!!, you are performing constrcutive combining which is helping it improve SNR!! talk about constructive combining and then give the example, your techniques should be summarized here...} 

A natural question is how does \name achieve high throughput with mutli-beam. An obvious implication of splitting the single beam to a multi-beam is loss in power per beam, called EIRP (Equivalent Isotropic Radiated Power) to meet the total radiated power (TRP) constraint. The reduction in per-beam power could reduce the received signal strength and lead to throughput loss at the receiver. At first glance, it seems as if multi-beam trades throughput for reliability while the goal was to improve both, but turns out we can break the trade-off. Our insight into breaking this trade-off is based on the observation that the received signal is the sum of multiple copies of the transmitted signal, for every beam in a multi-beam. If we can ensure the signal adds up in the signal domain constructively, we can increase the signal strength at the receiver.

Let's see with an intuitive example, say a mmWave channel consisting of two paths; and two-beam are aligned along those two-channel paths as shown in Figure \ref{fig:prototype}(b). For simplicity, assume the path loss is unity for each path, and the phase of signal travelled for each path is the same. \name's transmitter for this channel, splits the total power of $a^2$ equally into two beams with power $a^2/2$ on each beam, i.e., amplitude $a/\sqrt{2}$ on each beam, which undergoes the channel and is received with omni-receiver. Since the phase align for both paths, the received signal adds in signal domain, i.e. total amplitude of the received signal $ a/\sqrt{2} + a/\sqrt{2} = \sqrt{2}a$. The received signal upon converting to SNR (signal-to-noise ratio) is proportional to $2a^2$. In contrast, a traditional mmWave single-beam link does not exploit the second path and would provide an SNR proportional to $a^2$, which is 3 dB lower compared to a multi-beam case. By using mutli-beam with constructive combining, we establish a high throughput and high reliability links, by harnessing a multi-path environment without increasing the total transmit power. 


 %We mathematically show that our multi-beam patterns with optimized phase and amplitude are optimal and maximizes the SNR for any given wireless channel.

In the above simple example, we assumed a strong multi-path channel with similar gain as the direct path and aligned phase with the direct path at the receiver (constructive combining). However, real-world channels are complex with multi-paths that are weak and have phase value that doesn't align with the direct path. First, we extend this analysis and mathematically prove that with appropriate amplitude and phase per beam, one can achieve optimal constructive combining that maximizes the signal-to-noise ratio. The second challenge for \name is to estimate the beam directions, optimal beam-phase, and amplitude to be applied to achieve constructive combining. \name builds a novel algorithm to extract all these parameters by exploring the intricacies of the 5G protocol, thereby developing a low-cost beam probing mechanism to estimate the beam parameters. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. 
After estimating beam directions, the last step in multi-beam design is to create orthogonal beamforming vectors along with these directions. This is an important step to minimize cross-talk between beams and is essential in obtaining the desired constructive combining gains mentioned earlier. 
Finally, we implement the discussed multi-beam design steps on our phased array testbed and verify the robustness of our solution to quantization errors and other hardware non-idealities.

% \newtodo{ Achieving multi-beam in hardware is challenging, as a beam super-position doesn't achieve the desired behaviour due to inter-product and quantization of the hardware, we build a novel algorithm to construct multi-beam with desired optimal phase and power control on 5G NR hardware.} 
%  code-book addition cannot achieve  poses an additional challenge due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed.


% First, we develop novel analog beamforming techniques that optimize per-beam phase and power control in a multi-beam to enable constructive combining. 

% A natural question is how do we achieve constructive combing. Specifically, 



%  Furthermore, we prove that it would be always be better than ...  \name can therefore deliver a high reliability and high throughput link. 



% We present an intuitive example to explain the benefits of \name's constructive combining optimization. For simplicity, we consider the transmitter uses a 2-beam pattern aligned with two channel paths and the receiver is omni-directional. Assume the pathloss of each path is unity in which case \name allocates equal amplitude to each beam. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path, our constructive combining leads to the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. A careful reader would infer that the throughput gain is obtained by harnessing multi-path environment without increasing the total power. \name can therefore deliver reliable link while maintaining high throughput. 

% \textcolor{purple}{
% The intuitive example, however, does not explain multiple practical challenges in establishing a multi-beam link. (i) In practice, the reflected path channel suffers from higher attenuation which may affect the throughput gain. To deal with weaker paths, \name performs a joint optimization of phase and amplitude of each beam in a multi-beam to maximise SNR. (ii) The second challenge is to estimate the phase, attenuation and angle of each channel path which is required to generate phase-coherent multi-beam patterns. \name develops a beam probing mechanism to estimate the channel parameters. It exploits the mmWave channel sparsity~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first} to keep the probing overhead low. (iii) Finally, creating multi-beam pattern in hardware poses additional challenges due to hardware imperfections and limited resolution of phased arrays. \name takes advantage of recent advances~\cite{IDT, samsung_array, raychaudhuri2020challenge} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create efficient multi-beam patterns in our testbed. }

% In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of optimal channel-dependent beam pattern. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.

% The critical insight is that the multi-beam model is equivalent to transmitter diversity for low-frequency communication~\cite{tse2005fundamentals}, where multiple antennae transmit together to add up the signals at the receiver constructively. Such a scheme can increase the signal power received by the factor of the number of transmitting antennae, while simultaneously meeting the TRP constraints. \name is the first practical system to realize the transmit diversity for the mmWave communication systems with a single phased array and without relying on multiple RF chain. 

% \textcolor{purple}{
% The diversity gain achieved by \name can be understood by a simple example.
% Let's say there are two paths, each with say each with equal pathloss of unity. Say, we have a total power of $a^2$ to transmit, if we use only one path we would get SNR proportional to $a^2$. If we split the power, that is half power $a^2/2$ on each path i.e., the amplitude of $a/\sqrt{2}$ on each path. \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. 
% With our constructive amplitude combining the total amplitude of the received signal $2 a/\sqrt{2} = \sqrt{2}a$, which upon converting to SNR is proportional to $2a^2$, providing 3 dB gain compared to single-beam case. \name takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. In fact, we mathematically show that the phase-coherent multi-beam patterns are optimal under given multi-path channel when the number of beams are same as the number of channel paths. In practice, the mmWave channel is sparse and bounded by 2 or 3 strong paths~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first}. We evaluated through measurements that a 3 beam pattern achieves 99\% of the gain of ideal channel-dependent beam pattern. We propose a tractable approach to estimate the phase and amplitude per-beam with negligible overhead. Our approach requires only two probes for 2 beams and 4 probes for 3 beam case. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.}

% \todo{Mention that multi-beam requires attenuation control of more than 10 dB? but most commercially available arrays do not provide that control and so multi-beam was not feasible yet. We are the first to explore it.}

% An obvious implication of splitting the single lobe in to multiple beam is it would lead loss of signal radiated per beam of multiple beam on transmitter to meet EIRP (Equivalent Isotropic Radiated Power) constraint. 
% Therefore, the multi-beam concept may lead to the loss in signal strength received at the receiver, as the transmitted signal are individually reduced in power to meet EIRP. 
% The surprising observation is that in some scenarios, the signal received at the receiver increases by creating multi-beam compared to a single beam. 

% \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead.
% The above intuitive result is demonstrated in the Eq.3, where $\delta=1$ so $(1 + \delta^2) = 2$ i.e. 2 times the SNR. This is called diversity gain, or transmit beamforming gain, which is popularly taught in wireless classes as one of the first key principle, where the power is normalized as well. The paper explains the power normalization in the introduction, and when creating multiple beams, so

% To achieve full transmit diversity, i.e., improving signal to noise ratio optimally at the receiver, it requires the constructive combining of the signal from each beam (or transmitter).  \name builds a novel algorithm that controls per beam phase and amplitude and adapts in real-time to make sure the signal combines constructively. It takes advantage of recent advances~\cite{IDT} in antenna design for 28 GHz and shows that the per-antenna analog phase and amplitude control can create
% efficient multi-beam patterns. \name requires only the standard beam training process to learn the phase per beam for constructive combining and does not create any additional overhead. While multi-beam helps improve link reliability for a static user in blockage events, it is still prone to link degradation in a dynamic environment due to user mobility.


% Furthermore, note that the reflected path can have up to 20 dB of signal degradation compared to direct path and still the throughput of \name would be better than single beam link. However, turns out for 28 GHz mmWave the difference in the path-loss of the signal from naturally occurring reflectors and the direct path signal is minimal~\cite{samimi2014characterization}.

% The key insight behind this increase in received signal power for multi-beam compared to the single beam is that multi-beam in mmWave is equivalent to transmitter diversity for low frequency communication\todo{~\cite{}}. For transmitter diversity the signal power is distributed among multiple antennas, whereas in mmWave it is distributed among multiple beams. If the received signal from these multi-beams (or transmitters) combine constructively at the receiver they increase the signal received by the factor of number of antenna, while even meeting the EIRP constraints.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figures/brp_timeline_fig2_crop.pdf}
%     \caption{Shows \name tracks the user mobility and proactively refines the multi-beam patterns. It shows the \name link performs well even without beam training overhead. In contrast, the reactive framework performs beam training to recover a dead link. }
%     \label{fig:prototype_2}
%     \vspace{-0.1in}
% \end{figure}


% % \name designs an innovative approach to create multi-beam patterns and distribute power along multiple directions.  
% \todo{make this paragraph challenges only, and say that you overcome in the paper}
% In order to achieve full transmit diversity, i.e. improving signal to noise ratio optimally at the receiver, it requires constructive combining of the signal from each beam (or transmitter). Said differently, the challenge with multi-beam communication is that the signal travels through different paths and adds up at the receiver, which could lead to destructive combining leading to the loss of the signal at the receiver. The loss in the signal can result in reduced throughput for multi-beam. To overcome this problem, \name builds a novel algorithm that creates phase per beam and adapts the phase per beam in real-time to make sure the signal combines constructively. Moreover, it takes advantage of recent advances\cite{IDT} in antenna design for 28 GHz and shows that efficient multi-beam patterns can be created with per-antenna analog phase and amplitude control. Furthermore, it uses the standard beam training process to learn the phase per beam for constructive combining, not creating any additional overhead for per beam phase estimation.
% While multi-beam helps improve link reliability for a static user under blockage, in a dynamic environment, it is still prone to link degradation due to user mobility.


% To achieve the multi-beam and proactive response with a goal of high throughput and high-reliability, \name needs to address the following challenges. The first challenge is that \name distributes the power across multiple beams, these beams travel through different path and add up at the receiver, would could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput. In order to overcome this problem, \name builds a novel algorithm which creates phase per beam, and adapts the phase per beam in real-time to make sure the signal combines constructively. \name takes advantage of recent advances in antenna design for 28 GHz, and shows that with per antenna analog phase and amplitude control (6 bit and 4-bit resp. in our system).
% While multi-beam helps improve link reliability for a static user, in a dynamic environment, it is still prone to link degradation due to user mobility. 

So far, we have explained how to perform beam training and establish a multi-beam link for a static user. 
Mobility adversely affects the established links by causing misalignment between transmit and receive beams, degrading both throughput and reliability.
Multi-beam presents a unique challenge to handle mobility in mmWave links. 
In contrast to a single-beam system where only one beam gets misaligned,  in a multi-beam system, all the beams get misaligned simultaneously due to user mobility. 
Our key insight is that we can infer the user mobility dynamics by estimating how the wireless channel changes across all the beams.
Thus, our solution handles mobile multi-beam links by estimating each beam's channel response independently, which allows us to generate a proactive response to mobility dynamics.
However, it is not trivial to tap into these gains in practice, given that the channel responses from multiple beams may get conflated due to narrow bandwidth. 
Hence, \name designs a super-resolution algorithm based on sinc interpolation to extract the per beam channel response from the observed combined channel response.
After isolating the per beam channel, \name can associate the key parameters required to handle mobility, like the direction of user and path loss, to track the beams adaptively and prevent any further misalignments.
This allows \name to achieve an elusive goal with mmWave links, which is to provide continuously high throughput and reliability, free from sporadic outages.

% Therefore the challenge is to estimate the user mobility dynamics affecting each beam's wireless channel.

% all the beams in multi beam pattern will get misaligned, and by observing the signal strength changes across multiple beams, we can tap into these correlations to enable a proactive response to the misalignments.
% However, this key step requires 
% per beam power from CIR, needs superreoslution
% In order to tap into these gains from multiple beams, we need to formulate novel tracking methods since the tracking problem is complicated with mutli-beams. 
% This is because \name needs to re-align all the multiple beams with power and phase control per beam depending upon blockage or mobility situations. Therefore, none of the prior work can be used, as it requires tracking multiple beams angle, phase and power tracking. \name builds a novel proactive approach to maintain and track power, phase and beam direction of each of the multiple beams. \name's approach is to track the effects of mobility or blockage per-beam in the background by simply leveraging passive measurements of the mmWave received signal, making \name self-reliant. \name uses a tracking algorithm to periodically re-align each beam of the multi-beam and adjust their phase and amplitude, even when there is no significant link degradation. For example, in the blockage case, \name reduces the power along the blocked beam long before the link is degraded, thus increasing the power along the unblocked beam and maintaining the link. Similarly, in the case of user mobility, it continually re-aligns the beam directed towards the user. Therefore, \name prevents links from falling into outages.
% , as demonstrated through a prototype in Figure \ref{fig:prototype_2}. 




% To realize per beam tracking on a practical system even under mobility or blockage, \name needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to identify the blockage or user movement (self-reliant). Specifically, it measures the rate of degradation of the signal strength and creates thresholds for blockage and user movement and depending upon the observed degradation of the signal strength, it pro-actively calls it out as blockage or user movement. Furthermore, under user movement or mobility, the general motion is complex and hard to track, making beam re-alignment difficult. 

% In contrast, \name's key contribution is to decouple the complex user movement into rotation and translation movement and track them individually. An important observation is that all the beams within multi-beam undergo the same amount of angular movement for the rotation case, while for the translation case, the beams undergo different motion. We leverage this observation to design an angular rotation based beam tracking algorithm. A natural question is how do we measure the angular rotation per beam. In order to measure angular rotation per beam, we use the rate of change of amplitude per beam and phased-array antenna response, to determine the amount of rotation per beam. In summary, \name designs a novel amplitude-based tracking algorithm to track each beam individually. It only needs to measure 100 $\mu$sec of the received amplitude per beam to make the measurement. \textcolor{blue}{Also, note that \name only measures the angle to the UE for tracking and doesnot require exact user location, thus, preserving user privacy.}

%Second, \name needs to react to blockage or user movement per beam. The reaction to blockage is to reduce the power on the blocked beam. In contrast, to react for user mobility is challenging, it needs to  and the power and the phase for constructive combining, which requires it to identify the user movement. 

%First, to identify whether a particular beam is blocked or mis-aligned due to mobility, 

% On a practical system, per beam tracking has to be performed even with user mobility and blockage. \name, therefore, needs to identify whether a particular perturbation in the received signal is due to blockage or user movement. \name leverages received amplitude per beam to make this distinction. The challenge is that the received signal is a combination of all beams in the multi-beam due to a single receiver chain on the receiver (analog beamforming). A naive approach could be to use the received signal to measure the channel in time-domain and use the separation of different beams in time-of-flight to identify amplitude corresponding to each beam. However, the multiple beams can often have very close times-of-flight (ToF) and cannot be resolved even with the high-sampling rate of mmWave (2.5 ns resolution with 400 MHz). To accurately determine amplitude per beam, \name builds a super-resolution algorithm that leverages the relative time-of-flight information (between beams). \name's insight is that the relative time-of-flight remains constant across multiple packets between beams, and \name uses this insight to learn their amplitudes. Furthermore, the relative ToFs are easily acquired during the initial standard beam training phase, requiring no protocol changes to achieve the tracking algorithm. 

% Finally, an implicit assumption made while performing per-beam tracking is the ability to recover per-beam amplitude. 

\textbf{Evaluation:} We build a first-of-its-kind software-defined 5G NR testbed on 28 GHz mmWave bands with 64 element phased array, which can support channels of up to 400 MHz. 
% We prototyped \name on an Xilinx FPGA KCU105~\cite{kcu}) testbed connected with FMCDAC2 which has high-speed ADCs and DACs, that can support upto 1 Gsps. We used these ADC's and DAC's to support 5G NR digital baseband with 400 MHz. The output of DAC's and ADC is up-converted to 28 GHz (with multi-stage IF) and connected to custom built 8x8 (64 antenna element)~\cite{IDT}, the largest antenna array built with a full system at 28 GHz. 
We obtained NSF license to perform experiments at 28 GHz in our university area. We deploy \name in various indoor and outdoor scenarios. Our evaluation shows that in scenarios where user movement and blockage co-occur, \name has a reliability close to 100\% while maintaining an average throughput of 1.5 bits/sec/Hz as compared to the single-beam reactive baseline which has a reliability of 65\% and on-average throughput of 1 bits/sec/Hz. The throughput-reliability product is improved by 2.3$\times$ compared to best reactive baseline. 


%In summary, the novelty of this paper comes from three significant contributions. First, we showed the opportunity to use multi-lobe beam patterns to provide reliablity and high-data both simultaneously. Second, we design an algorithm to proactively track the blockage or mobility per beam and thus periodically re-align the beam without any training overhead. We develop novel super-resolution to enable accurate and co-phasing algorithm to facilitate tracking. Finally, we built an end-to-end testbed for 5G NR at 28 GHz and demonstrated a reliable mmWave link in a dynamic environment through extensive experiments. 

%The key insight to 

% first point is seperation between blockage vs mobility. 
%\name first leverages the multi-beam set up to identify any movement or blockage. Then, 

%While in case of mobility, \name estimates the change directly in each beam angle due to the mobility. Specifically, it leverages the multi-beams to jointly estimate the accurate tracking of the beam angle for each beam. \name's proactive beam alignment process is fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. 
%\textit{}  


 
 %\textcolor{blue}{ Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and relative ToF \textcolor{red}{[downplay relative ToF here?]}(relative to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.}
 
% \name's second design principle for reliability is to be \textit{proactive} instead of reactive to blockage and user mobility, i.e., \name preemptively tracks the beam and refines it without any explicit beam training. The approach gradually tracks the effects of mobility and the environment in the background, even when link throughput is not significantly affected. The beams are then periodically aligned with the mobile user. Therefore, it prevents links from falling into outages, as demonstrated through a prototype in Figure~\ref{fig:prototype}(c). \name's beam refinement is very fast as it requires scanning only a constant number of beam patterns independent of the antenna array and codebook size. \textit{In a nutshell, we propose a new mmWave system which utilizes multi-path aware multi-beam patterns that are realigned proactively; therefore facilitating reliable and stable links.}  


% The design philosophy of \name is different from other approaches. While recent proposals relies on assistance from device positioning system~\cite{zhou2018following,wei2017pose,va2015beam}, out-of-band WiFi~\cite{sur2017wifi,nitsche2015steering}, or light sensors~\cite{haider2018listeer}, \name is deployed without any additional hardware or sensor support. In a similar line of research, BeamSpy~\cite{sur2016beamspy} and Beam-forcast~\cite{zhou2017beam} provides a model-driven approach to handle blockage and mobility, respectively; however, they lack a unified framework to integrate both vulnerabilities. Above all, the literature focusses on improving the average throughput of the system over a long timescale. On the other hand, \name's design philosophy is to improve system reliability at a short millisecond timescale. 


% An important observation here is that individual beams in a multi-beam are affected differently by these effects. Blockage significantly reduces the power of the beam oriented toward it, rotation of the user causes an almost equal drop in power across all beams, and translation causes an unequal power drop across beams. In case of blockage, \name reduces the power along the blocked beam, while in case of mobility, \name estimates the angle of movement.

% When \name detects blockage of a beam, it reduces the power along that beam. 



% \name achieves its goal by first setting up a multi-beam mmWave link and then proactively maintaining it. 
% To realize multi-beam tracking on a practical system, \name needs to address the following additional challenges.

% \noindent
% \textbf{Challenge 1) Multi-beam set up:} The first challenge for \name is to establish a multi-beam communication link. These beams travel through different path and add up at the receiver, could lead to destructive combing leading to the loss of the signal at the receiver. The loss in signal can result in reduced throughput.
% and ensure that the signal along multiple beams adds up constructively at the receiver.



% \noindent
% \textbf{Solution:} \name takes advantage of recent advances in antenna design that allows high resolution in digital phase and amplitude control (6 bit and 4-bit resp. in our system). We showed that multi-beam patterns could be created by a weighted average of complex phasers of individual beams within multi-beam. The weights, however, if not appropriately set, may cause the signal along multi-paths to add up destructively at the receiver. We introduce a co-phasing factor that adjusts the relative phase of beams in multi-beam setup and device a method to tune that factor with low probing overhead.

% \noindent
% \textbf{Challenge 2) Multi-path separability:} \name is built on tracking per-beam amplitude in a multi-beam setup. Per-beam tracking is challenging since the received signal is a combination of all beams in the multi-beam due to analog beamforming. 

% \noindent
% \textbf{Solution:}  \name's key insight is to use the relative ToF information for each beam to learn its amplitude. However, with multiple beams often the multiple paths can have very close ToF, and cannot be resolved even with 15 cm resolution (2 GHz bandwidth at 60 GHz) or 75 cm resolution (400 MHz bandwidth at 28 GHz). To accurately resolve the beams, we build a super-resolution algorithm that leverages the relative ToF information (between beams) learned during the initial training phase, to produce accurate amplitude information per beam. 

% We then use the variation in per-beam amplitude over time to identify movement/blockage and modify the multi-beam pattern to maintain a reliable link.



% \noindent
% \textbf{Challenge 3) Multi-path parameter estimation:} 
% Individual beam in multi-beam can be identified by their AoA, AoD, and ToF parameters. Joint estimation of AoA and AoD requires a high-overhead customized training~\cite{palacios2018adaptive}, which makes it infeasible for high-reliability applications. 

% \noindent
% \textbf{Solution:}
% We leverage from our observation that each multipath has a unique ToF. The LOS path is identified as the path with the lowest ToF, and related ToF (related to the LOS path) is used to identify other paths. \name utilizes the initial beam training to first  estimate AoA and AoD, and then associate them using relative ToF without any additional training overhead.

% however, these parameters are typically estimated individually which pose  the mapping of AoA, AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. 

% Prior work \cite{palacios2018adaptive} relies on a custom training process to estimate absolute channel response per antenna and then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. 

% A key challenge is to associate the AoA with the AoD of corresponding reflectors.

% \name requires the knowledge of reflector location, orientation, and reflectively. Prior work suggest to get it offline manually \cite{wei2017facilitating} but \name need to get them in real-time.


% \name uses initial beam training to infer the strongest multi-paths in the environment, their angles of departure (AoD, beam from the transmitter), angles of arrival (AoA, beam at the receiver) and relative times-of-flight (relative ToF for each strong multi-path). \name uses the AoA, AoD, and relative ToF to learn reflector orientations in the environment by a smart ToF based association algorithm; the orientation of reflectors are necessary for proactive learning. 

% This knowledge of the multi-path environment augmented with recent advancements in mmWave antennas (achieving 6-bit phase and 7-bit amplitude control per antenna) to create a multi-beam link facilitates proactive learning as described below.
% enhanced by multi-path effects at both the transmitter and receiver.







% \begin{comment}


% Turns out 5G NR o
% super-resolution algorithm to recover Recall that during the initial beam training, we can learn about all the strong multi-path, we 
% can also use the initial 
% \item \textit{}
%     Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.


%     A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
    
% A natural question how does \name uses multi-beam to mitigate blockage and track user under mobility, 
% how does it maintain reliable connectivity using multi-beam. 



% To achieve reliable connectivity using multi-beam, \name builds an algorithm to track each of the individual beam 
% in the multiple beam from transmitter to the receiver. The individual track 



% % tell them how individual beam tracking in multi-beam solves both the 


% Challenge 1: individual beam tracking 

% Challenge 2: amplitude level tracking 
% % multi-beam tracking

% % amplitude level tracking 

% % ToF based seperation to achieve amplitude. 

% % rotation and translation 

% to the receiver but also help to track the user trajectory. \name refines the beam pattern over time to keep 
% it aligned with the mobile user, thus creating a stable WiFi-like link 
% %\textcolor{red}{[Should we mention that \name approximates the omni-pattern of sub-6GHz WiFi for directional mmWave link?]}. 
% The beam refinement\footnote{We use the IEEE 802.11ad terminology of beam training and beam refinement 
% which is discussed in Section \ref{sec:motivation}} with a multi-lobe pattern requires scanning of a constant 
% number of beams (0.1 ms latency) as compared to the beam training process that requires scanning 100's of beams 
% in the codebook at both transceiver (10 ms latency). \name's time complexity is of the order of the number of lobes, 
% which is typically directed towards 2-3 strong reflectors due to channel sparsity.

% Multi-lobe beam patterns has been explored in literature \textcolor{red}{[Cite Agile-link]} to reduce the 
% beam training delay, however, for the first time, \name exploits the unseen opportunity to use multi-lobe 
% patterns during the data transmission phase to enhance the link reliability. 

% The key challenges for \name are as follows:
% \begin{itemize}
%     \item \textit{The blockage mitigation has to be proactive.} \name creates custom multi-lobe patterns that are aligned with the strong reflectors providing multipath diversity. While some paths may suffer blockage, alternate unblocked paths are immediately available. A key innovation of \name is its ability to detect per-beam blockage rather than relying on the overall drop in received signal strength.
%     \item \textit{Beam alignment requires accurate tracking of mobile user with minimal overhead.} Tracking algorithms designed for sub-6 GHz requires multiple antennas and stable TOF while mmWave system typically has a single phased array antenna and the TOF estimated from the signal phase is oversensitive to millimeter change in user location. Therefore, prior work on mmWave beam tracking relies on probing a large set of beam patterns. The tracking overhead increases linearly with the size of the phased array and quadratically when the process is repeated at both transceivers. \name leverages the shape of the directional beam pattern generated by the phased array and uses the per-beam strength to track the user accurately. It requires probing only four beams irrespective of the number of antennas in the phased array. 
%     \item \textit{Beam alignment requires a distinction between translation and rotation of mobile user.} When the user device rotates on its axis, e.g., rotation of VR headset, the beam at the AP is unaffected while the directional beam at the user is misaligned. It is contrary to the user translation, which causes beam misalignment at both transceivers.  \name observes the distinct change in the multipath profile of the received signal to distinguish between translation and rotation and triggers beam refinement at the user for the rotation case and both transceivers for translation case.
% \end{itemize}

% \end{comment}


% Instead of using a fix codebook based design, we first estimate the multipath directions and implement multipath aware beam patterns.
% Note the code book might contain thousands of beam patterns but there are only a 2-3 multipaths due to channel sparsity.
% In a nutshell, we propose a paradigm shift for millimeter wave communication to design multipath aware beam patterns. Finding the right beam out of thousands of possible beam patterns is time-consuming, however, creating a beam pattern based on direction inference is tractable since there are only a few multipath directions. Tracking the multipath components can lead to a robust and reliable connection.



% To reestablish the link quality, beam training is performed 

% Blockage and mobility~\cite{sur201560} are the most challenging and fundamental problems for mmWave system. The current solutions are not adequate: too naive and does not take advantage of unique mmWave properties such as high bandwidth, channel sparsity, and unique shape of beam patterns. 

% Due to the availability of higher bandwidth in the mmWave frequency range, the mmWave RAN can achieve data rates of the order of a few Gbps~\cite{CellularCap-Rap}, suitable for the QoS requirements for augmented reality (AR) and virtual reality (VR) applications. However, due to high path loss at mmWave frequencies, the coverage of mmWave RAN is limited. To improve the rate and coverage of mmWave networks, phased array antennas are used to create directional beams. Hundreds of antennas can be packed in a small area thanks to a low wavelength (a few millimeters) at these high frequencies. The directional antennas put a unique challenge for mmWave networks to find an optimal beam pattern at the access point (AP) and the user equipment (UE). IEEE 802.11ad standards describe a beam training algorithm that is used periodically to search for a suitable beam pattern. The beam pattern selected during the beamtraining phase (see Figure \ref{fig:twophases}) is used throughout the data transmission phase. 
% Mmwave links are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by more than 20 dB~\cite{georgeFading}. 




%  \textcolor{red}{Ish: I am throwing random ideas in next few paragraphs which need to be placed and rewritten properly.}

% Standards: IEEE 802.11ad \cite{ieee80211ad}, 802.15.3c~\cite{ieee802153c},  802.11ay~\cite{ieee80211ay}






% mmWave links are inherently directional to combat high path loss at higher frequencies. These directional links are highly susceptible to beam misalignment due to user mobility compared to a wide sector-level beam. Therefore, most commercial devices \textcolor{red}{[cite]} does not use fine beam patterns to avoid the signal degradation due to mobility. On the other hand, we take advantage of the fine beam patterns to track the user and refine the beam pattern to always align with the mobile user. 





% \begin{itemize}
%     \item \textit{Sparse channel:} The mmwave channel is sparse, i.e., only the LOS and a few NLOS paths characterize the channel. Furthermore, mmWave uses analog beams to focus the transmit energy in specific directions by choosing a particular combination of phase and attenuation at each transmit antenna \textcolor{red}{Figure: analog architecture}. 
    
%  \textit{   Note that the multi-stream communication may suffer from destructive interference due to the combination of multipath signal of opposite phase arriving at the receiver. 
%     In case two paths are interfering destructively, they won't appear in the CIR and so we won't consider those paths. They can be detected by their different AOD/TOF.}
%     \item \textit{Known patterns:} The directivity gain of the phased array antenna is a deterministic function of the codebook and antenna spacing and is known \textit{a-priori}. 
%     \item \textit{Advanced hardware:} Recent advances in antenna design allows high resolution in digital phase and amplitude control (6 bit and 4 bit resp. in our system). Furthermore, the phased array can generate close to ideal beam patterns by following various antenna calibration processes \textcolor{red}{[cite]}. This capability to generate regular beam patterns allow us to perform accurate RSSI based beam tracking.
%     \item \textit{CSI:} The CSI is used for many sensing application such as localization and tracking, and is readily available on commercial WiFi devices such as Quantenna \textcolor{red}{[cite]}. We expect the same trend for commercial mmWave system. 
%     \item \textit{Wideband:} We utilize the CSI and high bandwidth available at mmWave frequencies to separate multipaths via power-delay profile. prior work on blockage mitigation and beam alignment are based on narrow-band channel model~\cite{sur2016beamspy,zhou2017beam} which does not resolve multipaths.
% \end{itemize}



% Our main contributions are summarized as follows:
% \begin{itemize}
% \item \todo{Main contribution and results}
%     % \item We leverage the initial beam training to estimate the multipath parameters \{AOD, AOA, TOF\} and achieve high reliability through custom multi-lobe beam patterns. We also analyse reliability-throughput tradeoff for mmWave networks.
%     % \item We track the multipath and design a beam refinement algorithm to establish a stable link even under high user mobility scenario.
% \end{itemize}

% However, mmWave communication systems are quite vulnerable to blockages due to higher penetration losses and reduced diffraction. Even the human body can reduce the signal strength by 20 dB~\cite{georgeFading}. 


% Thus, an unblocked Line of Sight (LOS) link is highly desirable for mmWave systems. When a LOS link is blocked, strong Non-Line of Sight (NLOS) links may also be helpful in achieving high reliability. However, NLOS links can also be blocked by mobile blockers. A mobile human blocker can block a link %between User Equipment (UE) and Base Station (BS) 
% for approximately 500 ms~\cite{georgeFading}. 


% At high frequencies, the attenuation due to obstacles is significant. For instance, 


==> Arxiv/2_motivation_v2.tex <==
\section{Background and Motivation}\label{sec:motivation}
5G NR provides a protocol to handle system-level challenges to establish a directional beam necessitated by mmWave propagation behavior. Directional beams are fickle natured; they provide high throughput at the cost of being narrow shaped and thus prone to blockages. Therefore, the 5G NR protocol has been designed in a way to be resilient to these challenges by paying particular attention to beam management for mitigation against blockages. 

\name intends to improve upon this fickle nature of narrow directional beams by providing resilience in the form of having multiple beams that typically aren't blocked simultaneously. Further, \name's design, by being 5G NR compliant, leverages important features of the protocol, at the same time improving the resilience by the increased multi-beam reliability. One can naively argue that by just having a wider beam, we can get increased resilience to blockage while being 5G NR compliant. So, why do we need multi-beam? The key point here is that the naive solution makes a tradeoff between increased reliability and decreased throughput. However, \name design gives more variables to tweak around, viz. each individual beam's phases and amplitudes, which enable \name to increase reliability while not degrading throughput.

% brought by directional beams at mmWave. 

% We provide a background on 5G NR beam management and how traditional single-beam based mmWave system is implemented in practice. We then detail how we can leverage the 5G NR waveform to establish a reliable multi-beam link. We show that \name is standard complaint and requires no additional overhead to 




% This section will provide a brief background on mmWave 5G NR waveform and how \name leverages the waveform structure to establish a reliable and high throughput link. 
% % We'll also explain why traditional single-beam systems suffer from low reliability.
% We define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
% \begin{equation}
%     \text{Reliability} = 1-\text{Prob}(\text{Outage})
% \end{equation}
% where the probability of outage can be practically computed as the fraction of duration when the SNR (signal to noise ratio) is below a certain threshold. As we can see, the directional nature of mmWave links make them suspectable blockage and user mobility, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}, bringing the link down to an outage. The high overhead in reviving a dead link with vanilla 5G NR (FR2: 24.25 GHz to 52.6 GHz) can further exacerbate the impact of an outage. 



% We first provide a primer on 5G NR and then show how traditional mmWave system suffers from low throughput and low-reliability in dynamic scenarios. We provide a motivation for multi-beam system for 5G NR which can handle environment vulnerabilities to establish a high throughput and reliable link. 

% \subsection{Reliability of mmWave links}



% Before we present the multi-beam for mmWave communication, we would elaborate and explain the basics of mmWave communication briefly. Recall that the highly directional nature of a conventional mmWave link makes it susceptible to degradation due to movement and blockages. A blockage occurs due to higher penetration losses and reduced diffraction around entities like walls and people, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}. Mobility due to rotation (VR headset in motion, rotary industry parts) or translation (walking, moving vehicle) adversely affects the established links by causing misalignment between transmit and receive beams. These effects cause significant throughput loss leading to frequent communication outages. mmWave systems detect such outages and trigger the beam-training phase to recover an alternate link, which adds up to the amount of time spent not communicating (66 $\mu$s per beam-direction which scales to 67.6 ms for 1024 sized codebook for 5G NR~\cite{5gnr,giordani2018tutorial}).

% The outage leads to a drop in reliability. Therefore, we formally define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam-training, and therefore unavailable for communication. 
% \begin{equation}
%     \text{reliability} = 1-\text{Pr}(\text{outage})
% \end{equation}
% In this section, we go over the multi-beam aspect of \name and how it improves throughput and reliability for a stationary user while blockers move around and block the link. In the next section, we build on this concept and detail \name's ability to handle user mobility using proactive tracking to allow high throughput and high reliability.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
%     \caption{Multi-beam communication enhances the throughput and reliability of a mmWave link.}
%     \label{fig:motivation}
% \end{figure}


% \textcolor{blue}{Before we build the theoretical model for multi-beam communication, we present some insights and observations to contrast common myths about multi-beam.\\
% \textbf{Myth1:} Multi-beam might have low EIRP compared to single-beam by 3 dB\\
% \textbf{Observation:} In many cases the EIRP reduces only by 2.5 dB as shown in Figure xxx. Multibeam does not consume more power. We show results for the same TRP (total rediated power). Multi-beam requires uneven power distribution across each antennas. Modern phased arrays at 28 GHz provides high attenuation control phased arrays (e.g. 27 dB in our phased arrays).\\
% \textbf{Myth2:} Multi-beam might reduce throughput in normal operation without blockage\\
% \textbf{Observation:} Even in the absence of blockage, multi-beam achieves comparable throughput to single-beam because of our constructive combining algorithm. In fact, for a narrowband system, multi-beam achieves higher gain compared to single-beam and comparable for a  wideband system as shown in Figure xxx[show constructive combining over a wideband vs over a narrowband channel].\\
% \textbf{Myth3:} Multi-beam requires strong reflectors.\\
% \textbf{Observation:} 28 GHz does not suffer from severe reflection loss compared to 60 GHz (show figure). Even in the absense of strong reflectors, multi-beam system falls back to single-beam system because of our power-control algorithm.}
% \todo{DONE: Add overview section on 5G NR and how we fit there}



% \todo{R4: <Done with 5G NR primer> The writing style needs to be significantly improved. The design overview (Sec 5 and Fig. 8) should come way earlier in the paper. It is difficult to follow different pieces of the design without having a big picture and overview early on.
% }

% \todo{R5: DONE: A short paragraph to give readers some background on 5G NR mmWave would be better. 
% How much overhead does it save in mmWave beam training using their beam tracking technique compared to vanilla 5G NR?
% }
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/5GNR_structure.pdf}
    \caption{5G NR downlink waveform uses SSB for beam training and CSI-RS for proactive beam refinement.}
    \label{fig:5GNRdownlink}
    \vspace{-.3cm}
\end{figure}





% \subsection{Why 5G mmWave suffers from low throughput and reliability?}
% The traditional mmWave system establishes a single directional link with the UE (user equipment) to combat high path loss at mmWave frequencies. Though this approach is simple and works in practice, it is not optimal for establishing a high throughput high-reliability link for two main reasons. First, a single-beam acts as a single point of failure with link blockage. A blockage occurs due to higher penetration losses and reduced diffraction around entities like walls and people, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}. Thus, a single-beam link can bring down a link to an outage, limiting the reliability of such a system.
% Second, a single directional beam does not exploit the channel-dependent beamforming~\cite{ratnam2019continuous, palacios2018adaptive, alkhateeb2014channel, jeong2015random}, which are shown to maximize link throughput. 

% % a single directional beam contains undesired side-lobes due to the limited size of the phased array, which may cause strong reflections to interfere with the direct-path signal resulting in low throughput. Even when multi-paths interfere constructively at the receiver, a single-beam does not amplify such reflection to improve throughput. \todo{I don't like the second reason here, you should limit that it is not optimal, here you can talk about transmit beamforming may be... It says the problem is you don't create right single beams, it should say the channel is not used optimally, don't make limited size as an issue, if that is an issue how did you overcome that in creating multi-beam??}


% Another important reason for low reliability is how the traditional system reacts to user mobility. Mobility due to rotation (VR headset in motion, rotary industry parts) or translation (walking, moving vehicle) adversely affects the established links by causing misalignment between transmit and receive beams. These effects cause significant throughput loss leading to frequent communication outages. Traditional in-band solutions use a pre-computed back-up beam hoping that they are still available and not blocked. An alternate solution is to gradually widen the beam with user mobility~\cite{giordani2016comparative} which trade-offs throughput for reliability while still prone to outages. Past work that tracks a mobile user~\cite{zhou2017beam} ignores the misalignment due to device rotation.

% \todo{may be get rid of this para now?, as we want to focus on phase and power control -- I am not sure about this... }
\subsection{Primer on mmWave 5G NR beam management}

\newtodo{Let me provide a more detailed primer on how the mm-wave link works in context of 5G and how it revives the beam.}

5G NR periodically performs the beam training using Synchronization Signal Block (SSB) to recover the directional link, as shown in Figure \ref{fig:5GNRdownlink}. Multiple SSBs form an SS-Burst, which takes 5 ms of channel air time to probe up to 64 beam directions. The user equipment (UE) will measure the received SSB and report measurement~\citep[TS 38.215]{5GNRRelease16} to gNB (5G NR base station) so gNB will know the best beam. SS-Bursts are transmitted periodically with a transmission period that varies from $5$ms to $160$ms (default periodicity is 20 ms)~\citep[TS 38.311]{5GNRRelease16}. A link in outage has to wait until the next beam training is performed. Moreover, in scenarios with frequent blockages and high user mobility, the beam scan periodicity is high, which eats up precious communication time. For instance, the default 20 ms periodicity of a 5 ms beam training phase causes 25\% probing overhead~\cite{giordani2018tutorial}. A vast literature focuses on reducing the beam training duration~\cite{ zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast}, but the high periodicity of SSB in mobile scenarios would still keep the overhead high.
~\todo{careful with the statements you make here....}


% 5G NR in FR2 (24.25 GHz to 52.6 GHz) provides a protocol for beam management in the directed mmWave regime. For simplicity, we consider a downlink waveform with a sub-carrier spacing of 120kHz. The waveform uses Synchronization Signal Block (SSB) and Channel Status Information Reference Signal (CSI-RS) for beam management, as shown in Figure \ref{fig:5GNRdownlink}. SSB plays a vital role in the initial access procedure. Multiple SSBs form an SS-Burst, which takes 5 ms of channel air time and can probe up to 64 beam directions. The user equipment (UE) will measure the received SSB and report measurement~\citep[TS 38.215]{5GNRRelease16} to gNB so gNB will know the best beam. SS-Bursts are transmitted periodically with a transmission period that varies from $5$ms to $160$ms (default periodicity is 20 ms)~\citep[TS 38.311]{5GNRRelease16}. 




% The high overhead in reviving a dead link can further exacerbate the impact of an outage. 5G NR periodically performs the beam training to recover the directional link. A link in outage has to wait until the next beam training is performed. Moreover, in scenarios with frequent blockages and high user mobility, the beam scan periodicity remains high, which eats up precious communication time. For instance, the default 20 ms periodicity of a 5 ms beam training period causes 25\% probing overhead. A vast literature focuses on reducing the beam training duration, but the high periodicity in mobile scenarios would still keep the overhead high. ~\todo{careful with the statements you make here....}


% \todo{move this up it's an odd location to define it...}


\subsection{Motivation for \name}
\newtodo{this is still referring to pro-active stuff... please reverse the focus... }

We leverage the 5G NR waveform structure to enable reliable and high throughput links with low overhead. Instead of focusing on initial beam training, \name focuses on establishing and maintaining a multi-beam link during the data communication through multi-beam constructive combining and user tracking. It leverages the Channel Status Information Reference Signal (CSI-RS) in 5G NR, which provides the knowledge of propagation channel~\citep[TS 38.215]{5GNRRelease16} and can be used for beam refinement. CSI-RS can be transmitted periodically or aperiodically, and if periodically sent, its period varies from 4 slots to 640 slots, which is 0.5 ms to 80 ms. One CSI-RS only occupies one symbol (8.93$\mu$s) in the slot and only a few frequency subcarriers~\citep[TS 38.211]{5GNRRelease16}. So the overhead caused by CSI-RS is much less compared to SSB. We propose a tractable approach to periodically update the per-beam angle, phase, and amplitude with negligible overhead. Our approach requires only three probes for the 2-beam case and five probes for the 3-beam case, which requires less than 2 ms for three refinement phases. Therefore, \name reduces the periodicity of SSB-based training with low overhead CSI-RS-based beam maintenance. In this way, \name achieves high reliability with low overhead while being compatible with 5G NR standards. \newtodo{We use DMRS for fine graind tracking.}

% \noindent
% \textbf{Overview:} A multi-beam system is a better choice of analog beamforming than a single beam system even when there are no blockages or user mobility. We show in Section \ref{subsec:multi-beam-reliability} that multi-beams belong to the class of channel-dependent beam patterns, which exploits multipath diversity to improve the signal strength at the receiver and are resilient to blockages.  Section \ref{sec:creatingmultibeam} provides a design of multi-beam system and Section~\ref{sec:design} discusses \name's proactive response to blockages and user mobility. 

% For instance, it amplifies the paths that constructively interfere at the receiver and rotates the beam's phase which would otherwise cause a destructive interference. Creating optimal beam pattern is generally intractable due to high overhead in obtaining per-antenna CSI in an analog phased array, which is required to generate channel-dependent patterns~\cite{palacios2018adaptive}. 
% In Section \ref{subsec:multi-beam-reliability}, we show that multi-beams are close to optimal and can be obtained with low overhead (Section \ref{sec:creatingmultibeam}). With user tracking, \name can achieve high reliability even with a low periodicity of SSB as detailed in Section~\ref{sec:design}.   

% In addition to improving throughput in normal operating conditions (without blockage or mobility), multi-beams are more resilient to occasional blockages since the probability that all the paths to the receiver blocked simultaneously remains low. With user mobility, we propose using CSI-RS for multi-beam tracking and refinement, which incurs much less overhead than SSB. With user tracking, \name can achieve high reliability even with a low periodicity of SSB as detailed in Section~\ref{sec:design}.   

% After the connection is established, CSI-RS provides the knowledge of propagation channel~\citep[TS 38.215]{5GNRRelease16} and can be used for beam refinement. It can be transmitted periodically or aperiodically, and if periodically sent, its period varies from 4 slots to 640 slots, which is 0.5 ms to 80 ms. One CSI-RS only occupies one symbol (8.93$\mu$s) in the slot and only a few frequency subcarriers~\citep[TS 38.211]{5GNRRelease16}. So the overhead caused by CSI-RS is much less compared to SSB. The specific design of codebook for beam training is left to the vendors. 



% \textcolor{purple}{We propose a tractable approach to periodically update the per-beam angle, phase and amplitude with negligible overhead. Our approach requires only three probes for 2 beams and five probes for 3 beam case which can be efficiently done in less than 2 ms. }

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
    \caption{Multi-beam communication enhances the throughput and reliability of a mmWave link through constructive combining optimization.}
    \label{fig:motivation}
\end{figure}



\subsection{How multi-beam helps with throughput and reliability?}
We next elaborate on the intuitive example presented in Section \ref{sec:intro} and show how multi-beam with optimal constructive combining and power-control can improve mmWave link reliability under frequent blockages while maintaining a high throughput link. We first focus on a scenario without blockage and later study the links under blockage.

\subsubsection{Multi-beam with constructive combining provides high throughput:} Here, we provide a mmWave signal propagation model and derive an expression for the multi-beam mmWave link capacity. We show that a multi-beam link leverages a multipath channel to improve link capacity compared to the channel-agnostic single-beam link. We consider a two-path channel with complex channel attenuation $h$ and $h\delta e^{j\sigma}$ along the direct and reflected path respectively as shown in Figure \ref{fig:motivation}. Note that $\delta$ is the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. The gNB creates a two-beam pattern and align each beam towards each channel paths. 

Our key insight is that we can optimize the relative phase and amplitude of the two beams to maximize the receiver's signal strength without increasing the total transmit power. Our constructive combining and power control algorithm provides a transmit antenna gain proportional $1$ and $\delta e^{-j\sigma}$ along the two paths. 
The UE receives the signal $y$ through an omni-directional beam pattern as: 
\begin{equation}
    y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{-j\sigma}}{\sqrt{1+\delta^2}}h \delta e^{j\sigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
\end{equation}
where $x$ is the signal transmitted by the gNB through a single RF-chain and $n$ is the receiver noise. A normalization factor of $1/\sqrt{1+\delta^2}$ ensures that we do not increase the total transmit power (Section~\ref{subsec:creating_mb}). The capacity of such phase-coherent two-beam link can be written as
\begin{equation}\label{eq:multibeam}
    C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_T}{P_N}\right)\; \textbf{(multi-beam)}
\end{equation}
 where $P_N$ is the receiver noise power and $P_T=\mathbb{E}[x]^2$ is average transmit power.

On the other hand, a single beam link directs the power towards the direct path while the reflected path signal is severely attenuated. It provides a capacity of: 
\begin{equation}
   C_{sb} = \log_2(1+|h|^2P_T/P_N) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
\end{equation}




We surprisingly note that the multi-beam capacity is higher than that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. In general, we show that we can further improve the link capacity by considering more than two beams as proven in Theorem \ref{th:mb_capacity}.
% We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 

\begin{theorem}\label{th:mb_capacity}
Multi-beam patterns maximises the SNR at the receiver when the number of beams in multi-beam is the same as the number of channel paths providing a capacity gain of
\begin{equation}
    C_{mb} = \log_2(1+\frac{\sum_{p=0}^{P-1}||\gamma_p||^2P_T}{P_N})
\end{equation}
where $\gamma_p$ is the complex channel attenuation along path $p$.
\end{theorem}
\begin{proof}
We provide the proof in Appendix \ref{appendix:A}
\end{proof}


\newtodo{Put intuition that the gains are coming because of constructive combining by harnessing a multi-path channel.}
\newtodo{A statement on reflectors are strong at 28 GHz, typically only 3-6 dB attenuation of strong multipath~\cite{zhu2014demystifying, telecom2019analysis}.}

Creating these optimal multi-beam patterns is challenging for two reasons. (i) The gNB needs to accurately estimate the direction, phase, and attenuation of each channel path and (ii) create a multi-beam pattern that provides the required per-beam antenna gain for constructive combining while satisfying the total radiated power constraint. We solve these design challenges in Section \ref{sec:creatingmultibeam}.

\subsubsection{Multi-beam link provides high reliability:}
We next introduce blockage to our model. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. \newtodo{provide explanation for correlated blockage}.
\newtodo{We define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
where the probability of outage can be practically computed as the fraction of duration when the SNR (signal to noise ratio) is below a certain threshold. As we can see, the directional nature of mmWave links make them suspectable blockage and user mobility, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}, bringing the link down to an outage. The high overhead in reviving a dead link with vanilla 5G NR (FR2: 24.25 GHz to 52.6 GHz) can further exacerbate the impact of an outage. }


% as shown in Figure~\ref{fig:toyrel}. Our mathematical result shows 
% that the multi-beam achieves close to 100\% reliability for typical blockage probabilities ($<20\%$). 

% The design of optimal multi-beam link is challenging for two reasons. (i) The gNB need to accurately estimate the direction, phase, and attenuation of each channel paths and (ii) create a multi-beam pattern that provides the requires antenna gain for constructive combining while satisfying the total radiated power constraint. We discuss these design aspect of \name in Section \ref{sec:creatingmultibeam}.

% From (\ref{eq:multibeam}), we see that the throughput gain of a multi-beam system is dependent on the factor $\delta^2$, which is the relative attenuation of the reflected path with respect to the direct path. We performed a study of attenuation caused by common reflecting surfaces and verified that 28 GHz attenuation is less severe compared to a 60 GHz link \cite{telecom2019analysis}. Shown in Table \ref{tab:reftype}, a metal reflector causes only 3 dB attenuation (including path loss and reflection loss) while other surfaces may create up to 16 dB attenuation. Measurement study for outdoor links \cite{zhu2014demystifying} also shows that reflected paths from buildings and vehicles are strong with only 5-7 dB attenuation.
% Note that in certain scenarios when the reflections are weak, multi-beams does not compromise on throughput in normal condition (without blockage) while significantly improving the throughput when one of the paths is blocked (Figure\ref{fig:toyexample}(b)) as we discuss in the following subsection. 
% \begin{table}[!t]
%     \centering
%     \begin{tabular}{ccccc}\toprule
%       \textbf{Objects} & Metal & Monitor & Wood&Wall\\ \midrule% \specialrule{1pt}{1pt}{1pt}
%         Attenuation (dB) & -3 & -12 & -15 & -16\\
%         \bottomrule
%     \end{tabular}
%     \vspace{.5cm}
%     \caption{Signal attenuation by common materials (path loss plus reflection loss) with respect to the direct path signal.}
%     \label{tab:reftype}
%     \vspace{-1cm}
% \end{table}





==> Arxiv/2_motivation_v3.tex <==
\section{Background and Motivation}\label{sec:motivation}

% summary:

% New ideas
% Summary: Single beam unreliable, beam management is important, protocols have provisions, people have even done multibeam - but not well
% Beam Management Techniques in Context: Lot of work on beam training. Some work ack use of multi-beam for comm, but focus only on training and set-up
% - Setup can't be repeated for multi beam again and again - talk about SSB overhead
% Motivation for mmReliable - Need to not just create, but maintain 

It is well known that conventional beamforming with highly-directional beams is unreliable due to its sensitivity to blockage and mobility effect~\cite{zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast}. This creates the need for beam-management schemes for link maintenance. Beam-management can be divided into two broad functions: first involves the search an setup of a beam, known as beam-training. This is typically a slow process, due to the large search space involved in looking for and setting up the optimal beam. The second function is beam-maintenance, and involves the upkeep of the beam despite environmental factors such as blockages, mobility and fading. The efficacy of the beam-maintenance function is critical to enabling reliable mmWave links with low overhead. Protocols such as 5G-NR contain exclusive signaling and control provisions for such beam-management. 


%There is a huge body of work that addresses the beam-training process~\cite{zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast}. These works aim to ascertain the strongest beamforming directions between two devices with the least overhead.
\subsection{Prior Work on Multi-beam and Need for \name}

Multi-beamforming to a single client is an exciting direction in enabling new mmWave capabilities. 
%Our work does not propose a beam-training method, but rather a robust beam-maintenance scheme for multi-beam communication links. 
Multi-beams have been shown to aid with the beam-training process\cite{hassanieh2018fast, aykin2019multi,aykin2019smartlink,feng2017dealing}. In \cite{hassanieh2018fast}, the authors employ multi-beams for fast beam-training, and use it to set up single-beam links for communication. The effectiveness of multi-beams in improving link reliability only under blockages is described in \cite{aykin2019multi} where an efficient beam-training method is developed. However, this work does not address the maintenance of these links under blockage and mobility. 
 While beam-maintenance for single-beam links have been studied by some authors \cite{aykin2020mamba,marzi2016compressive} \cite{anonpaper}, there is no work that addresses multi-beam links. Due to this gap, multi-beams have not been adopted widely despite their benefits. \name develops a maintenance scheme specific to multi-beam which even works with a single RF chain, making reliable high-throughput links practical for the first time. \name estimates per-beam angle, amplitude and phase in real-time with low overhead to maintain \constructivemultibeam. Finally, \name is 5G-NR compatible and can be deployed over any beam-training scheme.
\vspace{-3mm}
\subsection{\name and 5G-NR}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/5GNR_structure.pdf}
    \caption{5G NR downlink waveform uses SSB for beam training and CSI-RS for proactive beam refinement.}
    \label{fig:5GNRdownlink}
    % \vspace{-3cm}
\end{figure}
In the context of 5G-NR, the beam-training process relies on the Synchronization Signal Block (SSB), as shown in Fig. \ref{fig:5GNRdownlink}. Multiple SSBs form an SS-Burst, which takes 5 ms of channel air time to probe up to 64 beam directions. The user equipment (UE) will measure the received SSB and report the measurement~\citep[TS 38.215]{5GNRRelease16} to gNB (5G NR base station). SS-Bursts are transmitted periodically, with the transmissions being more frequent when recurring beam-training is necessitated by frequent blockages or high user mobility~\citep[TS 38.311]{5GNRRelease16}. In such scenarios, the default 20 ms periodicity of a 5 ms beam training phase can cause up to 25\% probing overhead~\cite{giordani2018tutorial}; making sole dependence on SSB for beam-maintenance intractable.

\name leverages the Channel State Information Reference Signal (CSI-RS), which can provide propagation channel estimates~\citep[TS 38.215]{5GNRRelease16} and is intended for beam refinement. CSI-RS can be sent arbitrarily with a spacing ranging from 0.5 ms to 80 ms. A CSI-RS occupies only one symbol (8.93$\mu$s) in the slot and only a few frequency subcarriers~\citep[TS 38.211]{5GNRRelease16}, contributing much less overhead than a SSB. Our approach periodically updates the per-beam angle, phase, and amplitude with negligible overhead, requiring only three channel estimates for a 2-beam multi-beam and five estimates for a 3-beam multi-beam. The entire process is completed within 0.6 ms for the latter, making multi-beam maintenance possible with low overhead. Alternatively other reference signals such as Demodulation Reference Signal (DMRS) may also be used for beam-maintenance.





% \newtodo{Let me provide a more detailed primer on how the mm-wave link works in context of 5G and how it revives the beam.}

% Summary:
% 1. SSB, SS-Burst - used for beam search
% 2. What happens if the beam is misaligned?  - maybe we can do search again?
% 3. Such overhead, much wow. Literature talks about reducing them, but still high

% New Flow:
% pt1. SSB and Beam Training. Many solutions, but this is not enough, high overhead
% pt2. This paper provides a method for maintaining reliable mmwave links
% pt3. It leverages CSI-RS instead of the high overhead SSB. Talk about specifics.

% Ideas at play in motivation
% a. Single beam is single point of failure and hence unreliable
% b. multi-beam is a good way to prevent this - but 
% c. Beam training is high overhead and cannot be repeated - with 5G-NR example
% d. Beam tracking is lower overhead and maintains link - with 5G-NR example, mmreliable stats of CSIRS
% e. We are doing tracking and not beam-search. Tracking is the important thing, any beam search can be used with us
% f. Setting up/motivating challenge of multi-beam with constructive combining.




% These works aim to reduce the beam-training time by utilizing techniques ranging from random sampling to hierarchical search. 

% Conventional beamforming involves the creation of a highly-directional beam to offset mmWave propagation losses. The beam's directional nature makes it sensitive to blockage and misalignment due to movement, creating the need for beam-management schemes for link maintenance. Protocols such as 5G-NR contain exclusive signaling and control provisions for such beam-management. However, using these provisions for conventional beamforming does not address the fundamental problem: \textit{single directional links when used by themselves, create a single point of failure and go into outage for a finite time due to blockages.} In light of this, mmWave deployments often use broad-beams with reduced directional gain to trade-off throughput for wider coverage and reliability\newtodo{CITE?}. Naturally, a solution that simultaneously optimizes both parameters is the elusive goal of mmWave beamforming. Motivated by this, \name uses coherent multi-beamforming and beam-management provisions in 5G-NR to achieve this goal.


% \subsection{How multi-beam helps with throughput and reliability?}
% We next elaborate on the intuitive example presented in Section \ref{sec:intro} and show how multi-beam with optimal constructive combining and power-control can improve mmWave link reliability under frequent blockages while maintaining a high throughput link. We first focus on a scenario without blockage and later study the links under blockage.

% \subsubsection{Multi-beam with constructive combining provides high throughput:} Here, we provide a mmWave signal propagation model and derive an expression for the multi-beam mmWave link capacity. We show that a multi-beam link leverages a multipath channel to improve link capacity compared to the channel-agnostic single-beam link. We consider a two-path channel with complex channel attenuation $h$ and $h\delta e^{j\sigma}$ along the direct and reflected path respectively as shown in Fig. \ref{fig:motivation}. Note that $\delta$ is the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. The gNB creates a two-beam pattern and align each beam towards each channel paths. 

% Our key insight is that we can optimize the relative phase and amplitude of the two beams to maximize the receiver's signal strength without increasing the total transmit power. Our constructive combining and power control algorithm provides a transmit antenna gain proportional $1$ and $\delta e^{-j\sigma}$ along the two paths. 
% The UE receives the signal $y$ through an omni-directional beam pattern as: 
% \begin{equation}
%     y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{-j\sigma}}{\sqrt{1+\delta^2}}h \delta e^{j\sigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
% \end{equation}
% where $x$ is the signal transmitted by the gNB through a single RF-chain and $n$ is the receiver noise. A normalization factor of $1/\sqrt{1+\delta^2}$ ensures that we do not increase the total transmit power (Section~\ref{subsec:creating_mb}). The capacity of such phase-coherent two-beam link can be written as
% \begin{equation}\label{eq:multibeam}
%     C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_T}{P_N}\right)\; \textbf{(multi-beam)}
% \end{equation}
%  where $P_N$ is the receiver noise power and $P_T=\mathbb{E}[x]^2$ is average transmit power.

% On the other hand, a single beam link directs the power towards the direct path while the reflected path signal is severely attenuated. It provides a capacity of: 
% \begin{equation}
%   C_{sb} = \log_2(1+|h|^2P_T/P_N) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
% \end{equation}




% We surprisingly note that the multi-beam capacity is higher than that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. In general, we show that we can further improve the link capacity by considering more than two beams as proven in Theorem \ref{th:mb_capacity}.
% % We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 

% \begin{theorem}\label{th:mb_capacity}
% Multi-beam patterns maximises the SNR at the receiver when the number of beams in multi-beam is the same as the number of channel paths providing a capacity gain of
% \begin{equation}
%     C_{mb} = \log_2\left(1+\frac{\sum_{p=0}^{P-1}||\gamma_p||^2P_T}{P_N}\right)
% \end{equation}
% where $\gamma_p$ is the complex channel attenuation along path $p$.
% \end{theorem}
% \begin{proof}
% We provide the proof in Appendix \ref{appendix:A}
% \end{proof}


% \newtodo{Put intuition that the gains are coming because of constructive combining by harnessing a multi-path channel.}

% Since \name's \constructivemultibeam approach depends on existance of two or more paths channel models, a valid question here is what physical phenomenon can give rise to such underlying channels. There have been a lot of channel measurement papers for both 28 GHz and 60 GHz mmWave links which have shown that in a typical deployment, there are strong reflectors like metals, concrete walls, tinted glasses etc, which reflect the signals by only attenuating the reflections by about 5-6 dB \cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}.
% % \newtodo{A statement on reflectors are strong at 28 GHz, typically only 3-6 dB attenuation of strong multipath~\cite{zhu2014demystifying, telecom2019analysis}.}

% Creating these optimal multi-beam patterns is challenging for two reasons. (i) The gNB needs to accurately estimate the direction, phase, and attenuation of each channel path and (ii) create a multi-beam pattern that provides the required per-beam antenna gain for constructive combining while satisfying the total radiated power constraint. We solve these design challenges in Section \ref{sec:creatingmultibeam}.

% \subsubsection{Multi-beam link provides high reliability:}
% We next introduce blockage to our model. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. \newtodo{provide explanation for correlated blockage}.
% \newtodo{We define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
% \begin{equation}
%     \text{Reliability} = 1-\text{Prob}(\text{Outage})
% \end{equation}
% where the probability of outage can be practically computed as the fraction of duration when the SNR (signal to noise ratio) is below a certain threshold. As we can see, the directional nature of mmWave links make them suspectable blockage and user mobility, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}, bringing the link down to an outage. The high overhead in reviving a dead link with vanilla 5G NR (FR2: 24.25 GHz to 52.6 GHz) can further exacerbate the impact of an outage. }


% as shown in Figure~\ref{fig:toyrel}. Our mathematical result shows 
% that the multi-beam achieves close to 100\% reliability for typical blockage probabilities ($<20\%$). 

% The design of optimal multi-beam link is challenging for two reasons. (i) The gNB need to accurately estimate the direction, phase, and attenuation of each channel paths and (ii) create a multi-beam pattern that provides the requires antenna gain for constructive combining while satisfying the total radiated power constraint. We discuss these design aspect of \name in Section \ref{sec:creatingmultibeam}.

% From (\ref{eq:multibeam}), we see that the throughput gain of a multi-beam system is dependent on the factor $\delta^2$, which is the relative attenuation of the reflected path with respect to the direct path. We performed a study of attenuation caused by common reflecting surfaces and verified that 28 GHz attenuation is less severe compared to a 60 GHz link \cite{telecom2019analysis}. Shown in Table \ref{tab:reftype}, a metal reflector causes only 3 dB attenuation (including path loss and reflection loss) while other surfaces may create up to 16 dB attenuation. Measurement study for outdoor links \cite{zhu2014demystifying} also shows that reflected paths from buildings and vehicles are strong with only 5-7 dB attenuation.
% Note that in certain scenarios when the reflections are weak, multi-beams does not compromise on throughput in normal condition (without blockage) while significantly improving the throughput when one of the paths is blocked (Figure\ref{fig:toyexample}(b)) as we discuss in the following subsection. 
% \begin{table}[!t]
%     \centering
%     \begin{tabular}{ccccc}\toprule
%       \textbf{Objects} & Metal & Monitor & Wood&Wall\\ \midrule% \specialrule{1pt}{1pt}{1pt}
%         Attenuation (dB) & -3 & -12 & -15 & -16\\
%         \bottomrule
%     \end{tabular}
%     \vspace{.5cm}
%     \caption{Signal attenuation by common materials (path loss plus reflection loss) with respect to the direct path signal.}
%     \label{tab:reftype}
%     \vspace{-1cm}
% \end{table}





==> Arxiv/2_motivation_v4.tex <==
\section{Background and Motivation}\label{sec:motivation}

% summary:

% New ideas
% Summary: Single beam unreliable, beam management is important, protocols have provisions, people have even done multibeam - but not well
% Beam Management Techniques in Context: Lot of work on beam training. Some work ack use of multi-beam for comm, but focus only on training and set-up
% - Setup can't be repeated for multi beam again and again - talk about SSB overhead
% Motivation for mmReliable - Need to not just create, but maintain 

In this section, we would present primer on beam-training protocols, and how it could become tedious to maintain single beam and potenial of multi-beam.

\textbf{Basics of Beam Management}
It is well known that conventional beamforming with highly-directional beams is unreliable due to its sensitivity to blockage and mobility effect. This creates the need for beam-management schemes for link maintenance. Beam-management can be divided into two broad functions: first involves the search an setup of a beam, known as beam-training. This is typically a slow process, due to the large search space involved in looking for and setting up the optimal beam. The second function is beam-maintenance, and involves the upkeep of the beam despite environmental factors such as blockages, mobility and fading. The efficacy of the beam-maintenance function is critical to enabling reliable mmWave links with low overhead. Protocols such as 5G-NR contain exclusive signaling and control provisions for such beam-management.

In the context of 5G-NR, the beam-training process relies on the Synchronization Signal Block (SSB), as shown in Fig. \ref{fig:5GNRdownlink}. Multiple SSBs form an SS-Burst, which takes 5 ms of channel air time to probe up to 64 beam directions. The user equipment (UE) will measure the received SSB and report the measurement~\citep[TS 38.215]{5GNRRelease16} to gNB (5G NR base station). SS-Bursts are transmitted periodically, with the transmissions being more frequent when recurring beam-training is necessitated by frequent blockages or high user mobility~\citep[TS 38.311]{5GNRRelease16}. In such scenarios, the default 20 ms periodicity of a 5 ms beam training phase can cause up to 25\% probing overhead~\cite{giordani2018tutorial}; making sole dependence on SSB for beam-maintenance intractable. 

 To overcome this, there is a huge body of work that addresses the beam-training process~\cite{zhu2014demystifying, jeong2015random,barati2015directional,zhou2012efficient,zhou2012efficient,barati2016initial, sur201560, abari2016millimeter,hassanieh2018fast}. These works aim to ascertain the strongest beamforming directions between two devices with the least overhead. However, till-date they suffer from reliability and lack of able to continously maintain the link. 
 

\subsection{Prior Work on Multi-beam and Need for \name}
Multi-beamforming is an exciting direction in enabling new mmWave capabilities. 
%Our work does not propose a beam-training method, but rather a robust beam-maintenance scheme for multi-beam communication links. 
Multi-beams have been shown to aid with the beam-training process to make them faster\newtodo{more multibeam citations}. In \newtodo{\cite{hassanieh2018fast}}, the authors employ multi-beams for fast beam-training, and use it to set up single-beam links for communication. The effectiveness of multi-beams in improving link reliability only under blockages is described in \newtodo{add more citation }\cite{aykin2019multi} where an efficient beam-training method is developed. However, this work does not address the maintenance of these links under blockage and mobility. 

While beam-maintenance for single-beam links have been studied by some authors\newtodo{\cite{}}, there is no work that addresses multi-beam links. Due to this gap, multi-beams have not been adopted widely despite their benefits. \name develops a maintenance scheme specific to multi-beam, making reliable high-throughput links practical for the first time. \name estimates per-beam angle, amplitude and phase in real-time with low overhead to maintain \constructivemultibeam. Finally, \name is 5G-NR compatible and can be deployed over any beam-training scheme.


\name leverages the Channel State Information Reference Signal (CSI-RS), which can provide propagation channel estimates~\citep[TS 38.215]{5GNRRelease16} and is intended for beam refinement. CSI-RS can be sent arbitrarily with a spacing ranging from 0.5 ms to 80 ms. A CSI-RS occupies only one symbol (8.93$\mu$s) in the slot and only a few frequency subcarriers~\citep[TS 38.211]{5GNRRelease16}. Therefore, the overhead caused by CSI-RS is much less in comparison to SSB. Our approach periodically updates the per-beam angle, phase, and amplitude with negligible overhead, requiring only three channel estimates for a 2-beam multi-beam and five estimates for a 3-beam multi-beam. The entire process is completed within 0.6 ms for the latter, making multi-beam maintenance possible with low overhead.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/5GNR_structure.pdf}
    \caption{5G NR downlink waveform uses SSB for beam training and CSI-RS for proactive beam refinement.}
    \label{fig:5GNRdownlink}
    \vspace{-.3cm}
\end{figure}




% \newtodo{Let me provide a more detailed primer on how the mm-wave link works in context of 5G and how it revives the beam.}

% Summary:
% 1. SSB, SS-Burst - used for beam search
% 2. What happens if the beam is misaligned?  - maybe we can do search again?
% 3. Such overhead, much wow. Literature talks about reducing them, but still high

% New Flow:
% pt1. SSB and Beam Training. Many solutions, but this is not enough, high overhead
% pt2. This paper provides a method for maintaining reliable mmwave links
% pt3. It leverages CSI-RS instead of the high overhead SSB. Talk about specifics.

% Ideas at play in motivation
% a. Single beam is single point of failure and hence unreliable
% b. multi-beam is a good way to prevent this - but 
% c. Beam training is high overhead and cannot be repeated - with 5G-NR example
% d. Beam tracking is lower overhead and maintains link - with 5G-NR example, mmreliable stats of CSIRS
% e. We are doing tracking and not beam-search. Tracking is the important thing, any beam search can be used with us
% f. Setting up/motivating challenge of multi-beam with constructive combining.




% These works aim to reduce the beam-training time by utilizing techniques ranging from random sampling to hierarchical search. 

% Conventional beamforming involves the creation of a highly-directional beam to offset mmWave propagation losses. The beam's directional nature makes it sensitive to blockage and misalignment due to movement, creating the need for beam-management schemes for link maintenance. Protocols such as 5G-NR contain exclusive signaling and control provisions for such beam-management. However, using these provisions for conventional beamforming does not address the fundamental problem: \textit{single directional links when used by themselves, create a single point of failure and go into outage for a finite time due to blockages.} In light of this, mmWave deployments often use broad-beams with reduced directional gain to trade-off throughput for wider coverage and reliability\newtodo{CITE?}. Naturally, a solution that simultaneously optimizes both parameters is the elusive goal of mmWave beamforming. Motivated by this, \name uses coherent multi-beamforming and beam-management provisions in 5G-NR to achieve this goal.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
    \caption{Multi-beam communication enhances the throughput and reliability of a mmWave link through constructive combining optimization.}
    \label{fig:motivation}
\end{figure}


\subsection{How multi-beam helps with throughput and reliability?}
We next elaborate on the intuitive example presented in Section \ref{sec:intro} and show how multi-beam with optimal constructive combining and power-control can improve mmWave link reliability under frequent blockages while maintaining a high throughput link. We first focus on a scenario without blockage and later study the links under blockage.

\subsubsection{Multi-beam with constructive combining provides high throughput:} Here, we provide a mmWave signal propagation model and derive an expression for the multi-beam mmWave link capacity. We show that a multi-beam link leverages a multipath channel to improve link capacity compared to the channel-agnostic single-beam link. We consider a two-path channel with complex channel attenuation $h$ and $h\delta e^{j\sigma}$ along the direct and reflected path respectively as shown in Fig. \ref{fig:motivation}. Note that $\delta$ is the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. The gNB creates a two-beam pattern and align each beam towards each channel paths. 

Our key insight is that we can optimize the relative phase and amplitude of the two beams to maximize the receiver's signal strength without increasing the total transmit power. Our constructive combining and power control algorithm provides a transmit antenna gain proportional $1$ and $\delta e^{-j\sigma}$ along the two paths. 
The UE receives the signal $y$ through an omni-directional beam pattern as: 
\begin{equation}
    y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{-j\sigma}}{\sqrt{1+\delta^2}}h \delta e^{j\sigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
\end{equation}
where $x$ is the signal transmitted by the gNB through a single RF-chain and $n$ is the receiver noise. A normalization factor of $1/\sqrt{1+\delta^2}$ ensures that we do not increase the total transmit power (Section~\ref{subsec:creating_mb}). The capacity of such phase-coherent two-beam link can be written as
\begin{equation}\label{eq:multibeam}
    C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_T}{P_N}\right)\; \textbf{(multi-beam)}
\end{equation}
 where $P_N$ is the receiver noise power and $P_T=\mathbb{E}[x]^2$ is average transmit power.

On the other hand, a single beam link directs the power towards the direct path while the reflected path signal is severely attenuated. It provides a capacity of: 
\begin{equation}
   C_{sb} = \log_2(1+|h|^2P_T/P_N) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
\end{equation}




We surprisingly note that the multi-beam capacity is higher than that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. In general, we show that we can further improve the link capacity by considering more than two beams as proven in Theorem \ref{th:mb_capacity}.
% We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 

\begin{theorem}\label{th:mb_capacity}
Multi-beam patterns maximises the SNR at the receiver when the number of beams in multi-beam is the same as the number of channel paths providing a capacity gain of
\begin{equation}
    C_{mb} = \log_2\left(1+\frac{\sum_{p=0}^{P-1}||\gamma_p||^2P_T}{P_N}\right)
\end{equation}
where $\gamma_p$ is the complex channel attenuation along path $p$.
\end{theorem}
\begin{proof}
We provide the proof in Appendix \ref{appendix:A}
\end{proof}


\newtodo{Put intuition that the gains are coming because of constructive combining by harnessing a multi-path channel.}

Since \name's \constructivemultibeam approach depends on existance of two or more paths channel models, a valid question here is what physical phenomenon can give rise to such underlying channels. There have been a lot of channel measurement papers for both 28 GHz and 60 GHz mmWave links which have shown that in a typical deployment, there are strong reflectors like metals, concrete walls, tinted glasses etc, which reflect the signals by only attenuating the reflections by about 5-6 dB \cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}.
% \newtodo{A statement on reflectors are strong at 28 GHz, typically only 3-6 dB attenuation of strong multipath~\cite{zhu2014demystifying, telecom2019analysis}.}

Creating these optimal multi-beam patterns is challenging for two reasons. (i) The gNB needs to accurately estimate the direction, phase, and attenuation of each channel path and (ii) create a multi-beam pattern that provides the required per-beam antenna gain for constructive combining while satisfying the total radiated power constraint. We solve these design challenges in Section \ref{sec:creatingmultibeam}.

\subsubsection{Multi-beam link provides high reliability:}
We next introduce blockage to our model. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. \newtodo{provide explanation for correlated blockage}.
\newtodo{We define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
where the probability of outage can be practically computed as the fraction of duration when the SNR (signal to noise ratio) is below a certain threshold. As we can see, the directional nature of mmWave links make them suspectable blockage and user mobility, penalizing Signal to Noise Ratio (SNR) by 20 to 30 dB~\cite{maccartney2017rapid}, bringing the link down to an outage. The high overhead in reviving a dead link with vanilla 5G NR (FR2: 24.25 GHz to 52.6 GHz) can further exacerbate the impact of an outage. }


% as shown in Figure~\ref{fig:toyrel}. Our mathematical result shows 
% that the multi-beam achieves close to 100\% reliability for typical blockage probabilities ($<20\%$). 

% The design of optimal multi-beam link is challenging for two reasons. (i) The gNB need to accurately estimate the direction, phase, and attenuation of each channel paths and (ii) create a multi-beam pattern that provides the requires antenna gain for constructive combining while satisfying the total radiated power constraint. We discuss these design aspect of \name in Section \ref{sec:creatingmultibeam}.

% From (\ref{eq:multibeam}), we see that the throughput gain of a multi-beam system is dependent on the factor $\delta^2$, which is the relative attenuation of the reflected path with respect to the direct path. We performed a study of attenuation caused by common reflecting surfaces and verified that 28 GHz attenuation is less severe compared to a 60 GHz link \cite{telecom2019analysis}. Shown in Table \ref{tab:reftype}, a metal reflector causes only 3 dB attenuation (including path loss and reflection loss) while other surfaces may create up to 16 dB attenuation. Measurement study for outdoor links \cite{zhu2014demystifying} also shows that reflected paths from buildings and vehicles are strong with only 5-7 dB attenuation.
% Note that in certain scenarios when the reflections are weak, multi-beams does not compromise on throughput in normal condition (without blockage) while significantly improving the throughput when one of the paths is blocked (Figure\ref{fig:toyexample}(b)) as we discuss in the following subsection. 
% \begin{table}[!t]
%     \centering
%     \begin{tabular}{ccccc}\toprule
%       \textbf{Objects} & Metal & Monitor & Wood&Wall\\ \midrule% \specialrule{1pt}{1pt}{1pt}
%         Attenuation (dB) & -3 & -12 & -15 & -16\\
%         \bottomrule
%     \end{tabular}
%     \vspace{.5cm}
%     \caption{Signal attenuation by common materials (path loss plus reflection loss) with respect to the direct path signal.}
%     \label{tab:reftype}
%     \vspace{-1cm}
% \end{table}





==> Arxiv/3_design_multibeam.tex <==
\section{Design of Multi-beam system}\label{sec:creatingmultibeam}
% The multi-beam patterns have high antenna gain in single or multiple main lobes that orient towards the reflectors or the LOS path.  We show that an effective way of generating multi-beam patterns is to take the weighted sum of beamforming weights of individual beams in the multi-beam. 
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/mmReliableOverview1_v2.pdf}
    \caption{Shows an overview of building blocks of \name that leverages SSB and CSI-RS resources in 5G NR to establish a multi-beam link.}
    \label{fig:overview1_v2}
\end{figure}

In this section, we present \name's algorithm for creating a reliable and high-throughput multi-beam link. Multi-beam patterns are channel-dependent and require an estimate of angle, phase, and attenuation of each channel path. We propose a two step procedure to estimate these parameters as shown in Fig. \ref{fig:overview1_v2}. First, We leverage the standard beam training procedure in 5G NR to estimate the angle of each multipath \cite{ghasempour2018multi, jog2019many}. We then design a customized procedure to estimate the per-path phase and attenuation with low overhead using CSI-RS. Finally, we explain our novel analog beamforming to establish a multi-beam link using these parameters.




% There are three parameters we phase, amplitude and then form a mult

% We present \name, a novel mmWave system that creates multi-beam patterns to improve link reliability while maintaining high throughput. 


%  We present the overall working of \name with the help of a flow-chart in Figure~\ref{fig:design_overview}. At a high level, \name has two major phases: the \textbf{Beam Training Phase} (BTP) and the \textbf{Data Transmission Phase} (DTP). During the BTP, \name leverages the standard exhaustive beam search to estimate some initial parameters such as AoA, AoD, and ToF of each channel path, which is required to establish a multi-beam link. The DTP establishes and periodically refines a multi-beam link through constructive combining optimization. It achieves constructive combining of multi-path signal through two novel contributions: 
% (i) It provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining.
% (ii) It develops a novel analog beamforming method to create phase-coherent multi-beams. 
% The DTP ends when the beam is no longer recoverable by tracking alone (due to accumulated errors in tracking over time) and signals the next BTP. The cycle of BTP and DTP repeats periodically. \newtodo{Does it need to be periodic? or can it be triggered only when needed?}
 
%  It then proceeds to set up the initial multi-beam link with the constructive combining optimization and signals the start of the DTP. The DTP relies on techniques developed in Section~\ref{sec:design} to perform proactive beam refinement. We elaborate on these two phases below:}


% \name achieves high throughput and high reliability by exploiting multi-path diversity using custom designed multi-beam patterns. It achieves constructive combining of multi-path signal through two novel contributions: (i) it develops novel analog beamforming method to create multi-beams and (ii) it provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining. We delineate the process of constructive combining as follows:




% In this phase, we estimate initial parameters of each path in the environment from the transmitter to the receiver. This is done at the initial user location by leveraging the standard beam training protocol. The primary purpose of beam training is to find all the right beams by scanning all a large set of beams in the codebook and observing the highest SNR beam pattern. We leverage the beam training process to also estimate the AoA and AoD profile of all the LOS and reflected paths. 

% A key challenge, however, is to associate the AoA with the AoD of corresponding reflectors. The mapping of AoA and AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. Prior work \cite{palacios2018adaptive} relies on a custom beam training process to estimate absolute channel response per antenna independent of the beam pattern; then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. Other works assume an Omni-directional user pattern to avoid the issue \cite{aykin2020mamba}.

% We leverage the ToF to solve the association problem. Each reflected path has a unique ToF. Note that due to the directional beam pattern, some paths are strengthened while other paths weaken. When the beam is aligned with some reflector, the strongest signal comes from reflected path corresponding to that reflector. We use the CIR corresponding to the beam directed along the AoA/AoD and estimate the ToF. The ToF is the delay corresponding to the highest power in CIR. The LOS path is identified as the path with the lowest ToF. This way \name estimates the AoA, AoD, ToF of each reflected path and associate them with each other. 

% \name leverages the process not only to select the highest SNR beam but plots the highest SNR of each beam with the beam direction and finds all the local maxima and estimates their corresponding directions. These directions are reported as the AoA/AoD of all the reflected paths. After the initial training, \name creates a multi-lobe beam pattern with power adjusted to match EIRP constraints along the direction of strong paths, therefore establishing the multi-beam link. The constructive combining optimisation completes this phase.
% \textcolor{purple}{
% \subsubsection{Data Transmission Phase}
% While beam refinement is performed very frequently with minimal overhead to establish a reliable connection, the large overhead beam training process can be delayed but cannot be avoided. \name uses the techniques developed in Section~\ref{sec:design} to delay the complex beam training process as much as possible. It updates the channel parameters (AoA, AoD, ToF) every time the beam training is repeated. The data transmission phase consists of multiple cycle beam refinements. Each beam refinement cycle involves observing multiple OFDM packets in the background and uses our super-resolution and constructive combining algorithm to achieve high throughput and high reliability. }

% The parameters AoA/AoD/ToF are updated whenever the beam training is repeated. During the period in between two BTP, the AoA and AoD can change significantly due to user rotation and translation. However, the relative ToF remains stable. The ToF does not change with device rotation. With translation, the change in ToF is minor. This enables \name to use the novel super-resolution algorithm (Section~\ref{sec:establish-multi-beam}) that takes the combined multi-beam received signal at the receiver to deconstruct the per-beam amplitude/power for each packet's CIR received. 

% Armed with knowledge of the per-beam amplitude, \name monitors them for changes over time, performing a hierarchical classification between blockage events and mobility events. Within mobility events, \name uses the angular deviations to approximate the motion as rotation and translation and performs proactive beam refinement.




 \subsection{Obtaining parameters for multi-beam constructive combining}\label{sec:constructive_combining}
% We propose a novel constructive combining optimization algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ per beam required for constructive combining. For the 2-beam case, our algorithm requires only two probes to estimate these parameters and in-general $2(K-1)$ probes for $K$ beams. For simplicity, we explain the 2-beam case here. To start with, gNB and the UE create a 2-beam pattern directed towards the AoD and AoA estimates, respectively (Assuming downlink case). The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam as follows:

\newtodo{explain the channel model before you present constructive combining algorithm, I don't know the variable reference in the first sentence.}

In this sub-section, we present our constructive combining algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ for the two-beam case. The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam. It then estimates the channel $\pbf_1$ and $\pbf_2$  for each probes as:
\begin{equation}\label{eq:two_probe_cc}
    \begin{split}
        \pbf_1 &= e^{j0}\hbf_1 + e^{j0} \hbf_2 = \hbf_1  + \hbf_2\\
        \pbf_2 &= e^{j0}\hbf_1  + e^{j\pi} \hbf_2 = \hbf_1  - \hbf_2
    \end{split}
\end{equation}
% \begin{equation}\label{eq:two_probe_cc}
%     \begin{split}
%         H_1(f_i) &= h_1(f_i) + e^{j0} h_2(f_i) = h_1(f_i) + h_2(f_i)\\
%         H_2(f_i) &= h_1(f_i) + e^{j\pi} h_2(f_i) = h_1(f_i) - h_2(f_i)
%     \end{split}
% \end{equation}
where $\hbf_1 $ and $\hbf_2$ is the complex per-path CSI (channel state information) observed by each of two beams across all frequency subcarriers. Using the set of two equations in (\ref{eq:two_probe_cc}), we estimate the complex per-path channel as $\hbf_1  = (\pbf_1+\pbf_2)/2$ and $\hbf_2 = (\pbf_1-\pbf_2)/2$. We then formulate an optimization problem that maximizes the average received signal strength over all frequencies to jointly estimate $\{\hat{\delta},\hat{\sigma}\}$ as:
% The relative phase $\sigma$ is approximately constant across frequency subcarriers because of high frequency of mmWave compared to bandwidth (Shown in Appendix \ref{appendix:A}). So we take an average over all of the frequency subcarriers to get a robust estimate. 
% Note that we inherently cannot estimate $\hat{\sigma}$ that works well for all the subcarriers simultaneously. 
% Our constructive combining approach maximizes the average received signal strength over all frequencies as:
\begin{equation}\label{eq:snroverall}
   \{\hat{\delta}, \hat{\sigma}\} = \argmax_{\delta,\sigma}\;\; \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
\end{equation}
% \begin{equation}\label{eq:snroverall}
%   \{\hat{\delta}, \hat{\sigma}\} = \arg\max_{\delta,\sigma}\sum_{f_i} \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
% \end{equation}

We solve the above optimization to a closed form expression as:
\begin{equation}
    \hat{\delta}e^{j \hat{\sigma}} = -{\hbf_2^H\hbf_1}/{\hbf_2^H\hbf_2},
\end{equation}
which simply reduces to $\hat{\delta}e^{j \hat{\sigma}} = -h_1/h_2 $ for a narrowband channel (e.g. in IEEE 802.11ad 60 GHz standard \cite{ieee80211ad}).
% We then use the estimates $\hat{\delta}$ and $\hat{\sigma}$ to create phase-coherent multi-beam patterns as detailed in the following subsection.
% where $\hbf_2$ and $\hbf_1$ are vectors of per-path CSI for all frequencies.
% \begin{equation}
%     \hat{\delta}e^{i \hat{\sigma}} = \frac{\sum_i h_2(f_i)^*h_1(f_i)}{\sum_i h_2(f_i)^*h_2(f_i)}
% \end{equation}

% Since, we are only interested in the relative channel, we represent $ \delta e^{j\sigma} =\frac{h_2(f_i)}{h_1(f_i)}$. We obtain the estimate of relative phase and amplitude in closed form as follow:
% \begin{equation}\label{eq:phase_estimate}
%     \hat{\delta}e^{i \hat{\sigma}} = \sum_i\frac{H_1(f_i)-H_2(f_i)}{H_1(f_i) + H_1(f_i)}. 
% \end{equation}


% We start by setting a multi-beam link with amplitude $\delta$ measured during initial beam training (Section \ref{sec:buildingblock}) and  a random phase-per-beam $\sigma$. 
% We consider a wideband system (such as 5G NR) and observe the effective channel response at each frequency subcarrier $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 

% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j,0)$ and $ H_{\text{eff}}(f_j,180)$ by setting two distinct values of $\sigma$ ($0^o$ and $180^o$) and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. 
% \begin{equation}
%     \begin{split}
%         H_{\text{eff}(f_j, 0)}
%     \end{split}
% \end{equation}

% From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. 



\todo{R3: The solution requires full channel state information, which may not be practical.
ToDo: Explain Full CSI is available in both 5G NR and 802.11ad
}
Our algorithm estimates these parameters using only two consecutive CSI-RS probes in NR for the two-beam case. In general, it requires $2(K-1)$ probes for $K$ beams independent of the number of antenna elements in the phased array.  
Note that \name requires the full CSI at the receiver for every probe to perform constructive combining. For the 5G NR system, the CSI is readily available from the CSI-RS signal. Even for 802.11ad commercial routers, there is firmware available to extract the CSI~\cite{qualcomm2017wil6210, wang2020demystifying, palacios2018adaptive}. Finally, the optimal phase, amplitude, and angle will change over time as the user moves. We propose to periodically estimate these parameters along with our novel tracking algorithm that we'll discuss in Section~\ref{sec:design}. 

%   \begin{figure} [!t]
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_factor_with_AOD.pdf}\label{fig:onormal_factor_with_AOD}}
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_SNR_with_AOD.pdf}\label{fig:onormal_SNR_with_AOD}}
%     \vspace{-4mm}
%     \caption{(a) Orthonormality factor is close to zero when beams are separated by more than $12^o$). (b) The resulting SNR gain approaches 3 dB when beams are orthonormal and stays within $\pm$ 0.7 dB, sometimes even higher than 3 dB.}
%     \label{fig:orthonormality}
%  \end{figure}


\subsection{Creating multi-beam patterns with normalized total radiated power}\label{subsec:creating_mb}

We device a simple method to create multi-beam pattern by combining the beamforming weights of respective single beam patterns. The beamforming weights for a single beam pointing at an angle $\phi_1$ is given by
\begin{equation}
    \textbf{w}_{\phi_1} = \frac{1}{\sqrt{N}}[1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_1)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_1)} ]^T
\end{equation}
where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of antennas. The total radiated power (TRP) is normalized to unity (i.e., $||\textbf{w}_{\phi_1}||^2=1$). We design beamforming weights $\textbf{w}$ for multi-beam with two lobes as follow:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{\text{NF}}}(\textbf{w}_{\phi_1}+\hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_2}),
 \end{equation}
where the normalizing factor (NF) is chosen to restrict the TRP to unity as follow
\begin{equation}\label{eq:nf}
\begin{split}
        \text{NF} &= ||\textbf{w}_{\phi_1} + \hat{\delta} e^{-j\hat{\sigma}}  \textbf{w}_{\phi_2}||^2\\ 
        &= ||\textbf{w}_{\phi_1}||^2 + \hat{\delta}^2 ||\textbf{w}_{\phi_2}||^2 + 
        \hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2} + 
        \hat{\delta} e^{j\hat{\sigma}}\textbf{w}_{\phi_2}^H\textbf{w}_{\phi_1}\\
        &=1+\hat{\delta}^2 +\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})
        %&\approx 1+\hat{\delta}^2
\end{split}
\end{equation}
We observe that the NF becomes $1+\hat{\delta}^2$ when the two single beams are orthonormal (i.e., $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}=0$ ). Intuitively, a single beam pattern contains unwanted side-lobes which may interact with the other beam in multi-beam to cause interference. We provide an analog beamforming optimization to remove this interference and create perfect orthonormal beams. Our solution is inspired from the class of null-constraint based beamforming techniques \cite{akdagli2001null,karaboga2002null} which create a single directional beam oriented at a desired direction while at the same time also put a null in the direction of interference. We obtain $\wbf_{{\phi_1},\text{null}}$ from $\wbf_{\phi_1}$ through the following optimization:
\begin{equation}
\begin{split}
     \wbf_{{\phi_1},\text{null}} = &\argmin_{\wbf} ||\wbf-\wbf_{\phi_1}||^2\\
     & \text{such that } \wbf^H\wbf_{\phi_2} = 0 \text{ and } ||\wbf||^2=1
\end{split}
\end{equation}
It is a standard convex optimization problem for which a closed-form solution exists \cite{boyd2004convex,cvx}. We finally create multi-beam pattern using the following beamforming vector:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{1+\delta^2}}(\wbf_{{\phi_1},\text{null}}+\hat{\delta} e^{-j\hat{\sigma}}\wbf_{\phi_1}),
 \end{equation}
\newtodo{Talk about quantization a bit. We quantized the beamforming vector according to our phased array resolution in our testbed implementation.}


% We empirically found that $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}$ in (\ref{eq:nf}) is order of magnitude less than the $1+\hat{\delta}^2$ when the beams are far by more than half-power beamwidth which is $12^o$ in our system. 
% We define orthonormality factor as the ratio $\frac{\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})}{1+\hat{\delta}^2}$ and show that it indeed is close to zero for a beam separation of half-power beamwidth which is $12^o$ in our system as shown in Figure \ref{fig:onormal_factor_with_AOD}. We get the SNR gain of $3$ dB when the two beams are orthonormal (assuming two paths suffer equal channel attenuation), varying in the range of $2.3$ dB to $3.7$ dB when the beams are not orthonormal as shown in Figure~\ref{fig:onormal_SNR_with_AOD}. 
% Intuitively, when the two beams are extremely close, the channel across two beams becomes correlated due to the wide beam aperture, and it becomes equivalent to the single-beam case when they merge. Thus, the results of (\ref{eq:multibeam}) hold in general. We emphasize that we used the NF from (\ref{eq:nf}) for normalization (and not the approximate value) to satisfy the TRP constraint in our testbed implementation strictly. 

% The resulting SNR varies around 3dB (assuming two paths suffers equal channel attenuation) with a maximum variation of $\pm 0.7 dB$ shown in Figure~\ref{fig:onormal_SNR_with_AOD}. Intuitively, when the two beams are very close, the channel across two beams becomes correlated due to the wide beam aperture.  
 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/plot2D_multibeam_SNR_with_perbeam_phase_and_power.pdf}
    \caption{Sensitivity analysis (simulation):  SNR gain (dB) of 2-beam w.r.t. single-beam for varying 2nd beam's phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ in multi-beam. We show for -3 dB weaker multi-path channel, the multi-beam's highest SNR gain is 1.76 dB which is not very sensitive even for high phase error of $\pm75^o$. However, if the phase error is highest ($180^o$), the SNR drops significantly. }
    \label{fig:sensitivity}
\end{figure}
% \todo{R1: A practical issue with the proposed approach is that creating very precise and directional multi-beam patterns without significant side lobes requires better antennas (more elements and higher resolution phase shifters) than antennas targeting a single lobe; the more constraints you put on the beam pattern, the harder it gets to also obtain a high gain given the hardware constraints. It would be interesting to discuss this tradeoff.}

% \todo{R5: The 6-bit phase resolution used in their phased array gives high-quality beams. How does it work in lower bit phase resolution? For example, the 60 GHz gNBs only have 2-bit resolution.}

% \todo{ R4: Also, in practice, phase shifters provide discrete phase control with limited resolution. Yet, this work uses arbitrarily phase control for constructive combining. }

% \textcolor{purple}{
% We demonstrate a high-throughput and reliable mmWave link with our state-of-the-art 64 element phased arrays which provides 6 bit of phase control and 27 dB of gain control per antenna element. The high resolution phase and gain control helps in creating phase-coherent multi-beams. Such an advanced arrays are getting deployed by vendors for 28 GHz base station. For instance, Verizon in collaboration with Samsung is deploying 64 element array (8 such arrays for MIMO)\cite{samsung_array} and IBM developed 128 element dual-polarized arrays to be used for COSMOS testbed\cite{raychaudhuri2020challenge}. That said, some phased arrays (e.g. 60 GHz routers based on IEEE 802.11ad) \cite{talonad7200} have low-resolution phase shifters which limits the ability to create multi-beam. Despite low resolution, such system would also benefit from our novel tracking algorithm to establish a reliable link. }





\noindent
\textbf{Sensitivity analysis:} We show that although accurate estimation of phase and amplitude provides the highest SNR, it is not very sensitive to estimation errors in these parameters. To quantify the sensitivity, we simulate a two-path channel and set the relative phase and attenuation to $-40^o$ and $-3$ dB, respectively. We vary the relative phase and amplitude of the 2nd beam in a 2-beam pattern (w.r.t. the first beam) and show the 2D plot of SNR gain in Fig. \ref{fig:sensitivity}. The highest SNR gain is 1.76 dB for perfect estimation, which reduces gradually with an increasing mismatch between the beam and channel parameters. We show that multi-beam SNR exceeds the single-beam SNR as long as the estimated phase is within $\pm 75^o$ and for reasonably high amplitude errors of -20 dB. Thus, the sensitivity to phase and amplitude estimation is low.

% The SNR gain of multi-beam w.r.t. single-beam relies on accurate estimation of the per-beam phase and amplitude. We show that the SNR gain has low sensitivity to the estimation error in phase and amplitude. We 
% The SNR gain is a maximum of 1.76 dB when the 2nd beam phase and amplitude match with the channel phase and attenuation. The SNR gain drops 
% . Moreover, the multi-beam outperforms the single-beam system even with a high amplitude estimation error of -20 dB.
\noindent
\textbf{Reliability-first principle:} 
At this point, one may wonder that when the multi-path is weak, the multi-beam pattern allocates less power along the reflected-path beam to maximize throughput, which may harm the reliability when the reflected path signal has power below an outage threshold. We solve this challenge by redistributing per-beam amplitudes to satisfy a minimum power constraint \newtodo{put number what threshold we used} along the reflected beam for a fixed total radiated power. Such optimization will ensure high reliability but at a sub-optimal throughput gain. Our insight follows from sensitivity analysis in Fig. ~\ref{fig:sensitivity}, which shows that even when we do sub-optimal power allocation per beam, e.g., distributing equal power to two beams, the throughput-gain reduces from 1.76 dB to 1.64 dB, which is still better compared to the single-beam case. \textit{Moreover, when the LOS path is not available for a long duration (e.g., persistent static blockage), having two beams at two reflectors with comparable attenuation is significantly better than a single beam at one reflector from both throughput and reliability points of view. }


% Recall that multi-beam pattern is obtained as weighted combination of the constituent single-beam patterns. We showed that the weights of the second beam is $\delta e^{-j\sigma}$ relative to the first beam achieves the optimal throughput performance. 


% We estimate the attenuation $\delta$ and AOD, AOA during the initial beam training phase as detailed in the overview section.\\ We next describe our process of obtaining $\sigma$ for constructive combining.

%  In the previous section, we provided the optimal choice of weights $c_1$ and $c_2$, but we didn't explain how to estimate them. In particular, the Tx needs to estimate the phase shift $\sigma$ which controls the relative phase between two beams, i.e., $\sigma = \angle c_2-\angle c_1$ = $\angle c_2$ (assume $\angle c_1=0$).
 
 
%  We define the cophasing factor $\sigma$ as the relative phase between those two beams i.e., $\sigma=\angle c_2-\angle c_1$, where $c_1$ and $c_2$ are defined in (\ref{eq:beampattern}). For simplicity, we consider $\angle c_1=0$ and $\angle c_2=\sigma$. 
 
 
%  For a wideband system (such as 5G NR), we write the effective channel $H_{\text{eff}}$ at subcarrier frequency $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
 
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 

% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j)$ by setting two distinct values of $\sigma$ and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm. is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically estimate it along with our novel tracking algorithm as discussed in the following Section. 

\

% \textcolor{blue}{
% \textbf{Complexity of multi-beam system:} There are two ways to implement multi-beam on hardware. First codebook based system need to store all possible multi-beams with different attenuation and phase-per-beam. Such codebook based system require extremely high storage (xxx size codebook for just 2 beam patterns) and also suffer from table-lookup latency. We propose an alternative solution that requires a small codebook of the same size of single-beam patterns. We use a small FPGA-board (Artix-7) generate multi-beam antenna weights by combining two single-beam weights. The FPGA only need to perform $2N$ complex multiplications/additions for $N$ antennas which we do with with a latency of xxx ns.}

% We highlight three significance of our fast constructive combining algorithm.
% \begin{enumerate}
%     \item Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically tune the fast co-phasing algorithm during \textcolor{red}{beam refinement phases} along with our novel tracking algorithm. 
%     \item The co-phasing needs to be tuned at only one of the transceivers (typically the access point) while the other transceiver keeps a fixed co-phasing factor all the time.
%     \item The time complexity of our co-phasing algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array.
% \end{enumerate}



 
 
 
%  \begin{equation}\label{eq:beampattern}
%     \textbf{w} = \sum_{k=1}^K c_k\textbf{w}_{\phi_k},
%  \end{equation}
%  where $\textbf{w}_{\phi_k} = [1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_k)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_k)} ]^T$ is the beamforming weight of a single-beam pattern directed along $\phi_k$ (for $k=1,\ldots,K$ beams); where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of transmit or receive antennas. 
 
%  The complex weights $c_k$ are chosen to control the power along each beam in multi-beam and satisfy the power constraint.
 
%  We show the effectiveness of our multi-beam patterns in  Figure~\ref{fig:multilobebeampattern}. We also measure beampatterns through our mmWave phased array (Section~\ref{sec:implementation}) in an anechoic chamber closely resembles the ones generated in theory using (\ref{eq:beampattern}).
 
%  Figure~\ref{fig:multilobebeampattern} that multi-beam patterns 
 
%  \noindent
%  \textbf{Cophasing Optimization:}
%  We highlight an issue with multi-beam communication that the signal along multiple paths may arrive with opposite phases causing destructive interference at the receiver. Fortunately, it is possible to avoid this happening by deliberately tuning the relative phase (co-phase) among multiple beams in the multi-beam pattern. 
 
%  Without loss of generality, we assume a communication link is established with two beams. 

==> Arxiv/3_design_multibeam_v2.tex <==


\section{Design of Multi-beam system}\label{sec:creatingmultibeam}
% The multi-beam patterns have high antenna gain in single or multiple main lobes that orient towards the reflectors or the LOS path.  We show that an effective way of generating multi-beam patterns is to take the weighted sum of beamforming weights of individual beams in the multi-beam. 

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/mmReliableOverview1_v2.pdf}
    \caption{Shows an overview of building blocks of \name that leverages SSB and CSI-RS in 5G NR to establish a multi-beam link.}
    \label{fig:overview1_v2}
    \vspace{-10pt}
\end{figure}
In this section, we present \name's algorithm for creating a reliable and high-throughput multi-beam link. First, we establish a mathematical framework to model the throughput and reliability gains in a multi-beam system. Then, we show that multi-beam patterns are channel-dependent and require an estimate of angle, phase, and attenuation of each channel path. We propose a two step procedure to estimate these parameters as shown in Fig. \ref{fig:overview1_v2}. We leverage any standard beam training procedure in 5G NR to estimate the angle of each multipath \cite{ghasempour2018multi, jog2019many}. We then design a customized procedure to estimate the per-path phase and attenuation with low overhead using CSI-RS. Finally, we explain our novel analog beamforming to establish a multi-beam link using these parameters.

\subsection{Multi-beam: Throughput and Reliability Models}
We next elaborate on the intuitive example presented in Section \ref{sec:intro} and show how multi-beam with optimal constructive combining and power-control can improve mmWave link reliability under frequent blockages while maintaining a high throughput link. We first focus on a scenario without blockage and later study the links under blockage.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
    \caption{Multi-beam communication enhances the throughput \& reliability of mmWave link through constructive combining.}
    \label{fig:motivation}
\end{figure}

\subsubsection{Multi-beam with constructive combining provides high throughput:} Here, we provide a mmWave signal propagation model and derive an expression for the multi-beam mmWave link capacity. We show that a multi-beam link leverages a multipath channel to improve link capacity compared to the channel-agnostic single-beam link. We consider a two-path channel with complex channel attenuation $h$ and $h\delta e^{j\sigma}$ along the direct and reflected path respectively as shown in Fig. \ref{fig:motivation}. Note that $\delta$ is the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. The gNB creates a two-beam pattern and align each beam towards each channel paths. 

Our key insight is that we can optimize the relative phase and amplitude of the two beams to maximize the receiver's signal strength without increasing the total transmit power. Our constructive combining and power control algorithm provides a transmit antenna gain proportional $1$ and $\delta e^{-j\sigma}$ along the two paths. 
The UE receives the signal $y$ through an omni-directional beam pattern as: 
\begin{equation}
    y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{-j\sigma}}{\sqrt{1+\delta^2}}h \delta e^{j\sigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
\end{equation}
where $x$ is the signal transmitted by the gNB through a single RF-chain and $n$ is the receiver noise. A normalization factor of $1/\sqrt{1+\delta^2}$ ensures that we do not increase the total transmit power (Section~\ref{subsec:creating_mb}). The capacity of such phase-coherent two-beam link can be written as
\begin{equation}\label{eq:multibeam}
    C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_T}{P_N}\right)\; \textbf{(multi-beam)}
\end{equation}
 where $P_N$ is the receiver noise power and $P_T=\mathbb{E}[x]^2$ is average transmit power.

On the other hand, a single beam link directs the power towards the direct path while the reflected path signal is severely attenuated. It provides a capacity of: 
\begin{equation}
   C_{sb} = \log_2(1+|h|^2P_T/P_N) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
\end{equation}




We surprisingly note that the multi-beam capacity is higher than that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. In general, we show that we can further improve the link capacity by considering more than two beams as proven in Theorem \ref{th:mb_capacity}.
% We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 

\begin{theorem}\label{th:mb_capacity}
Multi-beam patterns maximises the SNR at the receiver when the number of beams in multi-beam is the same as the number of channel paths providing a capacity gain of
\begin{equation}
    C_{mb} = \log_2\left(1+\frac{\sum_{p=0}^{P-1}||\gamma_p||^2P_T}{P_N}\right)
\end{equation}
where $\gamma_p$ is the complex channel attenuation along path $p$.
\end{theorem}
\begin{proof}
We provide the proof in Appendix \ref{appendix:A}
\end{proof}
Intuitively, we are constructively utilizing the reflections in a multi-path channel to increase the signal power and throughput.

Since \name's \constructivemultibeam approach depends on existance of two or more paths channel models, a valid question here is what physical phenomenon can give rise to such underlying channels. There have been a lot of channel measurement papers for both 28 GHz and 60 GHz mmWave links which have shown that in a typical deployment, there are strong reflectors like metals, concrete walls, tinted glasses etc, which reflect the signals by only attenuating the reflections by about 5-6 dB \cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}.
% \newtodo{A statement on reflectors are strong at 28 GHz, typically only 3-6 dB attenuation of strong multipath~\cite{zhu2014demystifying, telecom2019analysis}.}

Creating these optimal multi-beam patterns is challenging for two reasons. (i) The gNB needs to accurately estimate the direction, phase, and attenuation of each channel path and (ii) create a multi-beam pattern that provides the required per-beam antenna gain for constructive combining while satisfying the total radiated power constraint. We solve these design challenges in later subsections.

\subsubsection{Multi-beam link provides high reliability:}
We next introduce blockage to our model. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. 
We formally define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
In practice, the probability of outage is computed as the fraction of duration where the SNR is below a minimum threshold. The directional nature of single-beam mmWave links make them suspectable to blockage \& user mobility, reducing SNR by 20 to 30 dB~\cite{maccartney2017rapid} and causing outages.


\review{R2: Another strong assumption is that the probability of blocking each lobe of a multi-beam pattern is independent. However, that’s not the case in the real-world as the lobes are often highly correlated.}
\newtodo{The reviewer is concerned about correlated blockages. We have omitted them from Section 3.4 for simplicity, but have evaluated our system considering this correlation. We will put a note in Section 3.4.}



% There are three parameters we phase, amplitude and then form a mult

% We present \name, a novel mmWave system that creates multi-beam patterns to improve link reliability while maintaining high throughput. 


%  We present the overall working of \name with the help of a flow-chart in Figure~\ref{fig:design_overview}. At a high level, \name has two major phases: the \textbf{Beam Training Phase} (BTP) and the \textbf{Data Transmission Phase} (DTP). During the BTP, \name leverages the standard exhaustive beam search to estimate some initial parameters such as AoA, AoD, and ToF of each channel path, which is required to establish a multi-beam link. The DTP establishes and periodically refines a multi-beam link through constructive combining optimization. It achieves constructive combining of multi-path signal through two novel contributions: 
% (i) It provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining.
% (ii) It develops a novel analog beamforming method to create phase-coherent multi-beams. 
% The DTP ends when the beam is no longer recoverable by tracking alone (due to accumulated errors in tracking over time) and signals the next BTP. The cycle of BTP and DTP repeats periodically. \newtodo{Does it need to be periodic? or can it be triggered only when needed?}
 
%  It then proceeds to set up the initial multi-beam link with the constructive combining optimization and signals the start of the DTP. The DTP relies on techniques developed in Section~\ref{sec:design} to perform proactive beam refinement. We elaborate on these two phases below:}


% \name achieves high throughput and high reliability by exploiting multi-path diversity using custom designed multi-beam patterns. It achieves constructive combining of multi-path signal through two novel contributions: (i) it develops novel analog beamforming method to create multi-beams and (ii) it provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining. We delineate the process of constructive combining as follows:




% In this phase, we estimate initial parameters of each path in the environment from the transmitter to the receiver. This is done at the initial user location by leveraging the standard beam training protocol. The primary purpose of beam training is to find all the right beams by scanning all a large set of beams in the codebook and observing the highest SNR beam pattern. We leverage the beam training process to also estimate the AoA and AoD profile of all the LOS and reflected paths. 

% A key challenge, however, is to associate the AoA with the AoD of corresponding reflectors. The mapping of AoA and AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. Prior work \cite{palacios2018adaptive} relies on a custom beam training process to estimate absolute channel response per antenna independent of the beam pattern; then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. Other works assume an Omni-directional user pattern to avoid the issue \cite{aykin2020mamba}.

% We leverage the ToF to solve the association problem. Each reflected path has a unique ToF. Note that due to the directional beam pattern, some paths are strengthened while other paths weaken. When the beam is aligned with some reflector, the strongest signal comes from reflected path corresponding to that reflector. We use the CIR corresponding to the beam directed along the AoA/AoD and estimate the ToF. The ToF is the delay corresponding to the highest power in CIR. The LOS path is identified as the path with the lowest ToF. This way \name estimates the AoA, AoD, ToF of each reflected path and associate them with each other. 

% \name leverages the process not only to select the highest SNR beam but plots the highest SNR of each beam with the beam direction and finds all the local maxima and estimates their corresponding directions. These directions are reported as the AoA/AoD of all the reflected paths. After the initial training, \name creates a multi-lobe beam pattern with power adjusted to match EIRP constraints along the direction of strong paths, therefore establishing the multi-beam link. The constructive combining optimisation completes this phase.
% \textcolor{purple}{
% \subsubsection{Data Transmission Phase}
% While beam refinement is performed very frequently with minimal overhead to establish a reliable connection, the large overhead beam training process can be delayed but cannot be avoided. \name uses the techniques developed in Section~\ref{sec:design} to delay the complex beam training process as much as possible. It updates the channel parameters (AoA, AoD, ToF) every time the beam training is repeated. The data transmission phase consists of multiple cycle beam refinements. Each beam refinement cycle involves observing multiple OFDM packets in the background and uses our super-resolution and constructive combining algorithm to achieve high throughput and high reliability. }

% The parameters AoA/AoD/ToF are updated whenever the beam training is repeated. During the period in between two BTP, the AoA and AoD can change significantly due to user rotation and translation. However, the relative ToF remains stable. The ToF does not change with device rotation. With translation, the change in ToF is minor. This enables \name to use the novel super-resolution algorithm (Section~\ref{sec:establish-multi-beam}) that takes the combined multi-beam received signal at the receiver to deconstruct the per-beam amplitude/power for each packet's CIR received. 

% Armed with knowledge of the per-beam amplitude, \name monitors them for changes over time, performing a hierarchical classification between blockage events and mobility events. Within mobility events, \name uses the angular deviations to approximate the motion as rotation and translation and performs proactive beam refinement.




 \subsection{Obtaining parameters for multi-beam constructive combining}\label{sec:constructive_combining}
% We propose a novel constructive combining optimization algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ per beam required for constructive combining. For the 2-beam case, our algorithm requires only two probes to estimate these parameters and in-general $2(K-1)$ probes for $K$ beams. For simplicity, we explain the 2-beam case here. To start with, gNB and the UE create a 2-beam pattern directed towards the AoD and AoA estimates, respectively (Assuming downlink case). The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam as follows:
Just as in prior sub-sections, we use $\delta$ as the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. In this sub-section, we present our constructive combining algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ for the two-beam case. The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam. It then estimates the channel $\pbf_1$ and $\pbf_2$  for each probes as:
\begin{equation}\label{eq:two_probe_cc}
    \begin{split}
        \pbf_1 &= e^{j0}\hbf_1 + e^{j0} \hbf_2 = \hbf_1  + \hbf_2\\
        \pbf_2 &= e^{j0}\hbf_1  + e^{j\pi} \hbf_2 = \hbf_1  - \hbf_2
    \end{split}
\end{equation}
% \begin{equation}\label{eq:two_probe_cc}
%     \begin{split}
%         H_1(f_i) &= h_1(f_i) + e^{j0} h_2(f_i) = h_1(f_i) + h_2(f_i)\\
%         H_2(f_i) &= h_1(f_i) + e^{j\pi} h_2(f_i) = h_1(f_i) - h_2(f_i)
%     \end{split}
% \end{equation}
where $\hbf_1 $ and $\hbf_2$ is the complex per-path CSI (channel state information) observed by each of two beams across all frequency subcarriers. Using the set of two equations in (\ref{eq:two_probe_cc}), we estimate the complex per-path channel as $\hbf_1  = (\pbf_1+\pbf_2)/2$ and $\hbf_2 = (\pbf_1-\pbf_2)/2$. We then formulate an optimization problem that maximizes the average received signal strength over all frequencies to jointly estimate $\{\hat{\delta},\hat{\sigma}\}$ as:
% The relative phase $\sigma$ is approximately constant across frequency subcarriers because of high frequency of mmWave compared to bandwidth (Shown in Appendix \ref{appendix:A}). So we take an average over all of the frequency subcarriers to get a robust estimate. 
% Note that we inherently cannot estimate $\hat{\sigma}$ that works well for all the subcarriers simultaneously. 
% Our constructive combining approach maximizes the average received signal strength over all frequencies as:
\begin{equation}\label{eq:snroverall}
   \{\hat{\delta}, \hat{\sigma}\} = \argmax_{\delta,\sigma}\;\; \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
\end{equation}
% \begin{equation}\label{eq:snroverall}
%   \{\hat{\delta}, \hat{\sigma}\} = \arg\max_{\delta,\sigma}\sum_{f_i} \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
% \end{equation}

We solve the above eqn to a closed form expression as:
\begin{equation}
    \hat{\delta}e^{j \hat{\sigma}} = -{\hbf_2^H\hbf_1}/{\hbf_2^H\hbf_2},
\end{equation}
which simply reduces to $\hat{\delta}e^{j \hat{\sigma}} = -h_1/h_2 $ for a narrowband channel (e.g. in IEEE 802.11ad 60 GHz standard \cite{ieee80211ad}).
% We then use the estimates $\hat{\delta}$ and $\hat{\sigma}$ to create phase-coherent multi-beam patterns as detailed in the following subsection.
% where $\hbf_2$ and $\hbf_1$ are vectors of per-path CSI for all frequencies.
% \begin{equation}
%     \hat{\delta}e^{i \hat{\sigma}} = \frac{\sum_i h_2(f_i)^*h_1(f_i)}{\sum_i h_2(f_i)^*h_2(f_i)}
% \end{equation}
% Since, we are only interested in the relative channel, we represent $ \delta e^{j\sigma} =\frac{h_2(f_i)}{h_1(f_i)}$. We obtain the estimate of relative phase and amplitude in closed form as follow:
% \begin{equation}\label{eq:phase_estimate}
%     \hat{\delta}e^{i \hat{\sigma}} = \sum_i\frac{H_1(f_i)-H_2(f_i)}{H_1(f_i) + H_1(f_i)}. 
% \end{equation}
% We start by setting a multi-beam link with amplitude $\delta$ measured during initial beam training (Section \ref{sec:buildingblock}) and  a random phase-per-beam $\sigma$. 
% We consider a wideband system (such as 5G NR) and observe the effective channel response at each frequency subcarrier $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 
% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j,0)$ and $ H_{\text{eff}}(f_j,180)$ by setting two distinct values of $\sigma$ ($0^o$ and $180^o$) and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. 
% \begin{equation}
%     \begin{split}
%         H_{\text{eff}(f_j, 0)}
%     \end{split}
% \end{equation}
% From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. 
\todo{R3: The solution requires full channel state information, which may not be practical.
ToDo: Explain Full CSI is available in both 5G NR and 802.11ad
}
Our algorithm estimates these parameters using only two consecutive CSI-RS probes in NR for the two-beam case. In general, it requires $2(K-1)$ probes for $K$ beams independent of the number of antenna elements in the phased array.  
Note that \name requires the full CSI at the receiver for every probe to perform constructive combining. For the 5G NR system, the CSI is readily available from the CSI-RS signal. Even for 802.11ad commercial routers, there is firmware available to extract the CSI~\cite{qualcomm2017wil6210, wang2020demystifying, palacios2018adaptive}. Finally, the optimal phase, amplitude, \& angle will change over time as the user moves. We propose to periodically estimate these parameters along with our novel tracking algorithm that we'll discuss in Section~\ref{sec:design}. 

\review{In Section 3.2, the authors describe a two-probe based approach to estimate the two-beam channels. However, Equation (6) seems to suggest one should apply different phases to different directions h1 and h2: the first probe applies the same phase to both directions whereas the second probe applies different phases to the two directions. Then this requires our knowledge of h1 and h2. Isn't it a chicken-and-egg problem? Unless we know h1 and h2, how can we apply different phases to different directions?
}
\newtodo{The reviewer addressed a misunderstanding on mmReliable algorithm in Eq (6). We will clarify this misunderstanding by improving the writing of Section 3.2.
}
%   \begin{figure} [!t]
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_factor_with_AOD.pdf}\label{fig:onormal_factor_with_AOD}}
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_SNR_with_AOD.pdf}\label{fig:onormal_SNR_with_AOD}}
%     \vspace{-4mm}
%     \caption{(a) Orthonormality factor is close to zero when beams are separated by more than $12^o$). (b) The resulting SNR gain approaches 3 dB when beams are orthonormal and stays within $\pm$ 0.7 dB, sometimes even higher than 3 dB.}
%     \label{fig:orthonormality}
%  \end{figure}


\subsection{Creating multi-beam patterns with normalized total radiated power}\label{subsec:creating_mb}

We device a simple method to create multi-beam pattern by combining the beamforming weights of respective single beam patterns. The beamforming weights for a single beam pointing at an angle $\phi_1$ is given by
\begin{equation}
    \textbf{w}_{\phi_1} = \frac{1}{\sqrt{N}}[1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_1)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_1)} ]^T
\end{equation}
where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of antennas. The total radiated power (TRP) is normalized to unity (i.e., $||\textbf{w}_{\phi_1}||^2=1$). We design beamforming weights $\textbf{w}$ for multi-beam with two lobes as follow:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{\text{NF}}}(\textbf{w}_{\phi_1}+\hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_2}),
 \end{equation}
where the normalizing factor (NF) is chosen to restrict the TRP to unity as follow
\begin{equation*}\label{eq:nf}
\begin{split}
        \text{NF} &= ||\textbf{w}_{\phi_1} + \hat{\delta} e^{-j\hat{\sigma}}  \textbf{w}_{\phi_2}||^2\\ 
        &= ||\textbf{w}_{\phi_1}||^2 + \hat{\delta}^2 ||\textbf{w}_{\phi_2}||^2 + 
        \hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2} + 
        \hat{\delta} e^{j\hat{\sigma}}\textbf{w}_{\phi_2}^H\textbf{w}_{\phi_1}\\
        &=1+\hat{\delta}^2 +\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})
        %&\approx 1+\hat{\delta}^2
\end{split}
\end{equation*}
We observe that the NF becomes $1+\hat{\delta}^2$ when the two single beams are orthonormal (i.e., $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}=0$ ). Intuitively, a single beam pattern contains unwanted side-lobes which may interact with the other beam in multi-beam to cause interference. We provide an analog beamforming optimization to remove this interference and create perfect orthonormal beams. Our solution is inspired from the class of null-constraint based beamforming techniques \cite{akdagli2001null,karaboga2002null} which create a single directional beam oriented at a desired direction while at the same time also put a null in the direction of interference. We obtain $\wbf_{{\phi_1},\text{null}}$ from $\wbf_{\phi_1}$ through the following optimization:
\begin{equation}
\begin{split}
     \wbf_{{\phi_1},\text{null}} = &\argmin_{\wbf} ||\wbf-\wbf_{\phi_1}||^2\\
     & \text{such that } \wbf^H\wbf_{\phi_2} = 0 \text{ and } ||\wbf||^2=1
\end{split}
\end{equation}
It is a standard convex optimization problem for which a closed-form solution exists \cite{boyd2004convex,cvx}. We finally create multi-beam pattern using the following beamforming vector:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{1+\delta^2}}(\wbf_{{\phi_1},\text{null}}+\hat{\delta} e^{-j\hat{\sigma}}\wbf_{\phi_2}),
 \end{equation}
We then appropriately quantize the beamforming vector phases \& amplitudes to be compatible with our testbed. We show the sensitivity of beamforming to phase and amplitude errors in Appendix~\ref{appendix:S}.


% We empirically found that $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}$ in (\ref{eq:nf}) is order of magnitude less than the $1+\hat{\delta}^2$ when the beams are far by more than half-power beamwidth which is $12^o$ in our system. 
% We define orthonormality factor as the ratio $\frac{\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})}{1+\hat{\delta}^2}$ and show that it indeed is close to zero for a beam separation of half-power beamwidth which is $12^o$ in our system as shown in Figure \ref{fig:onormal_factor_with_AOD}. We get the SNR gain of $3$ dB when the two beams are orthonormal (assuming two paths suffer equal channel attenuation), varying in the range of $2.3$ dB to $3.7$ dB when the beams are not orthonormal as shown in Figure~\ref{fig:onormal_SNR_with_AOD}. 
% Intuitively, when the two beams are extremely close, the channel across two beams becomes correlated due to the wide beam aperture, and it becomes equivalent to the single-beam case when they merge. Thus, the results of (\ref{eq:multibeam}) hold in general. We emphasize that we used the NF from (\ref{eq:nf}) for normalization (and not the approximate value) to satisfy the TRP constraint in our testbed implementation strictly. 

% The resulting SNR varies around 3dB (assuming two paths suffers equal channel attenuation) with a maximum variation of $\pm 0.7 dB$ shown in Figure~\ref{fig:onormal_SNR_with_AOD}. Intuitively, when the two beams are very close, the channel across two beams becomes correlated due to the wide beam aperture.  
 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/plot2D_multibeam_SNR_with_perbeam_phase_and_power.pdf}
%     \caption{Sensitivity analysis (simulation):  SNR gain (dB) of 2-beam w.r.t. single-beam for varying 2nd beam's phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ in multi-beam. We show for -3 dB weaker multi-path channel, the multi-beam's highest SNR gain is 1.76 dB which is not very sensitive even for high phase error of $\pm75^o$. However, if the phase error is highest ($180^o$), the SNR drops significantly. }
%     \label{fig:sensitivity}
% \end{figure}

% \todo{R1: A practical issue with the proposed approach is that creating very precise and directional multi-beam patterns without significant side lobes requires better antennas (more elements and higher resolution phase shifters) than antennas targeting a single lobe; the more constraints you put on the beam pattern, the harder it gets to also obtain a high gain given the hardware constraints. It would be interesting to discuss this tradeoff.}

% \todo{R5: The 6-bit phase resolution used in their phased array gives high-quality beams. How does it work in lower bit phase resolution? For example, the 60 GHz gNBs only have 2-bit resolution.}

% \todo{ R4: Also, in practice, phase shifters provide discrete phase control with limited resolution. Yet, this work uses arbitrarily phase control for constructive combining. }

% \textcolor{purple}{
% We demonstrate a high-throughput and reliable mmWave link with our state-of-the-art 64 element phased arrays which provides 6 bit of phase control and 27 dB of gain control per antenna element. The high resolution phase and gain control helps in creating phase-coherent multi-beams. Such an advanced arrays are getting deployed by vendors for 28 GHz base station. For instance, Verizon in collaboration with Samsung is deploying 64 element array (8 such arrays for MIMO)\cite{samsung_array} and IBM developed 128 element dual-polarized arrays to be used for COSMOS testbed\cite{raychaudhuri2020challenge}. That said, some phased arrays (e.g. 60 GHz routers based on IEEE 802.11ad) \cite{talonad7200} have low-resolution phase shifters which limits the ability to create multi-beam. Despite low resolution, such system would also benefit from our novel tracking algorithm to establish a reliable link. }





% \noindent
% \textbf{Sensitivity analysis:} We show that although accurate estimation of phase and amplitude provides the highest SNR, it is not very sensitive to estimation errors in these parameters. To quantify the sensitivity, we simulate a two-path channel and set the relative phase and attenuation to $-40^o$ and $-3$ dB, respectively. We vary the relative phase and amplitude of the 2nd beam in a 2-beam pattern (w.r.t. the first beam) and show the 2D plot of SNR gain in Fig. \ref{fig:sensitivity}. The highest SNR gain is 1.76 dB for perfect estimation, which reduces gradually with an increasing mismatch between the beam and channel parameters. We show that multi-beam SNR exceeds the single-beam SNR as long as the estimated phase is within $\pm 75^o$ and for reasonably high amplitude errors of -20 dB. Thus, the sensitivity to phase and amplitude estimation is low.

% The SNR gain of multi-beam w.r.t. single-beam relies on accurate estimation of the per-beam phase and amplitude. We show that the SNR gain has low sensitivity to the estimation error in phase and amplitude. We 
% The SNR gain is a maximum of 1.76 dB when the 2nd beam phase and amplitude match with the channel phase and attenuation. The SNR gain drops 
% . Moreover, the multi-beam outperforms the single-beam system even with a high amplitude estimation error of -20 dB.


% new
% \noindent
% \textbf{Reliability-first principle:} 
% At this point, one may wonder that when the multi-path is weak, the multi-beam pattern allocates less power along the reflected-path beam to maximize throughput, which may harm the reliability when the reflected path signal has power below an outage threshold. We solve this challenge by redistributing per-beam amplitudes to satisfy a minimum power constraint \newtodo{put number what threshold we used} along the reflected beam for a fixed total radiated power. Such optimization will ensure high reliability but at a sub-optimal throughput gain. Our insight follows from sensitivity analysis in Fig. ~\ref{fig:sensitivity}, which shows that even when we do sub-optimal power allocation per beam, e.g., distributing equal power to two beams, the throughput-gain reduces from 1.76 dB to 1.64 dB, which is still better compared to the single-beam case. \textit{Moreover, when the LOS path is not available for a long duration (e.g., persistent static blockage), having two beams at two reflectors with comparable attenuation is significantly better than a single beam at one reflector from both throughput and reliability points of view. }


% Recall that multi-beam pattern is obtained as weighted combination of the constituent single-beam patterns. We showed that the weights of the second beam is $\delta e^{-j\sigma}$ relative to the first beam achieves the optimal throughput performance. 


% We estimate the attenuation $\delta$ and AOD, AOA during the initial beam training phase as detailed in the overview section.\\ We next describe our process of obtaining $\sigma$ for constructive combining.

%  In the previous section, we provided the optimal choice of weights $c_1$ and $c_2$, but we didn't explain how to estimate them. In particular, the Tx needs to estimate the phase shift $\sigma$ which controls the relative phase between two beams, i.e., $\sigma = \angle c_2-\angle c_1$ = $\angle c_2$ (assume $\angle c_1=0$).
 
 
%  We define the cophasing factor $\sigma$ as the relative phase between those two beams i.e., $\sigma=\angle c_2-\angle c_1$, where $c_1$ and $c_2$ are defined in (\ref{eq:beampattern}). For simplicity, we consider $\angle c_1=0$ and $\angle c_2=\sigma$. 
 
 
%  For a wideband system (such as 5G NR), we write the effective channel $H_{\text{eff}}$ at subcarrier frequency $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
 
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 

% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j)$ by setting two distinct values of $\sigma$ and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm. is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically estimate it along with our novel tracking algorithm as discussed in the following Section. 

% \textcolor{blue}{
% \textbf{Complexity of multi-beam system:} There are two ways to implement multi-beam on hardware. First codebook based system need to store all possible multi-beams with different attenuation and phase-per-beam. Such codebook based system require extremely high storage (xxx size codebook for just 2 beam patterns) and also suffer from table-lookup latency. We propose an alternative solution that requires a small codebook of the same size of single-beam patterns. We use a small FPGA-board (Artix-7) generate multi-beam antenna weights by combining two single-beam weights. The FPGA only need to perform $2N$ complex multiplications/additions for $N$ antennas which we do with with a latency of xxx ns.}

% We highlight three significance of our fast constructive combining algorithm.
% \begin{enumerate}
%     \item Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically tune the fast co-phasing algorithm during \textcolor{red}{beam refinement phases} along with our novel tracking algorithm. 
%     \item The co-phasing needs to be tuned at only one of the transceivers (typically the access point) while the other transceiver keeps a fixed co-phasing factor all the time.
%     \item The time complexity of our co-phasing algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array.
% \end{enumerate}



 
 
 
%  \begin{equation}\label{eq:beampattern}
%     \textbf{w} = \sum_{k=1}^K c_k\textbf{w}_{\phi_k},
%  \end{equation}
%  where $\textbf{w}_{\phi_k} = [1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_k)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_k)} ]^T$ is the beamforming weight of a single-beam pattern directed along $\phi_k$ (for $k=1,\ldots,K$ beams); where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of transmit or receive antennas. 
 
%  The complex weights $c_k$ are chosen to control the power along each beam in multi-beam and satisfy the power constraint.
 
%  We show the effectiveness of our multi-beam patterns in  Figure~\ref{fig:multilobebeampattern}. We also measure beampatterns through our mmWave phased array (Section~\ref{sec:implementation}) in an anechoic chamber closely resembles the ones generated in theory using (\ref{eq:beampattern}).
 
%  Figure~\ref{fig:multilobebeampattern} that multi-beam patterns 
 
%  \noindent
%  \textbf{Cophasing Optimization:}
%  We highlight an issue with multi-beam communication that the signal along multiple paths may arrive with opposite phases causing destructive interference at the receiver. Fortunately, it is possible to avoid this happening by deliberately tuning the relative phase (co-phase) among multiple beams in the multi-beam pattern. 
 
%  Without loss of generality, we assume a communication link is established with two beams. 

==> Arxiv/3_design_multibeam_v3.tex <==


\section{Design of Multi-beam system}\label{sec:creatingmultibeam}
% The multi-beam patterns have high antenna gain in single or multiple main lobes that orient towards the reflectors or the LOS path.  We show that an effective way of generating multi-beam patterns is to take the weighted sum of beamforming weights of individual beams in the multi-beam. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/mmReliableOverview1_v2.pdf}
%     \caption{Shows an overview of building blocks of \name that leverages SSB and CSI-RS in 5G NR to establish a multi-beam link.}
%     \label{fig:overview1_v2}
%     \vspace{-10pt}
% \end{figure}
In this section, we present \name's algorithm for creating a reliable and high-throughput multi-beam link. First, we establish a mathematical framework to model the throughput and reliability gains in a multi-beam system. Then, we show that multi-beam patterns are channel-dependent and require an estimate of angle, phase, and attenuation of each channel path. We propose a two step procedure to estimate these parameters as shown in Fig.~\ref{fig:5GNR_mmReliable_ovreview}. We leverage any standard beam training procedure in 5G NR to estimate the angle of each multipath~\cite{ghasempour2018multi, jog2019many}. We design a customized procedure to estimate the per-path phase and attenuation with low overhead using reference signals. Finally, we explain our novel analog beamforming to establish a multi-beam link using these parameters.


\subsection{Multi-beam link provides high reliability}
We show how multi-beam links are reliable even under the impact of blockage events because it avoids a single point of failure. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. In practice, even with correlated blockages, the occurrence of complete outage of multi-beam (all beams blocked in multi-beam) is less probable than that of single beam. Therefore, multi-beam links are probabilistically better reliable than single beam links.


We formally define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
In practice, the probability of outage is computed as the fraction of duration where the SNR is below a minimum threshold. The directional nature of single-beam mmWave links make them susceptible to blockage \& user mobility, reducing SNR by 20 to 30 dB~\cite{maccartney2017rapid} and causing outages.


\review{R2: Another strong assumption is that the probability of blocking each lobe of a multi-beam pattern is independent. However, that’s not the case in the real-world as the lobes are often highly correlated.}
\newtodo{The reviewer is concerned about correlated blockages. We have omitted them from Section 3.4 for simplicity, but have evaluated our system considering this correlation. We will put a note in Section 3.4.}

\highlightshep{
\subsection{Multi-beam Throughput Model}

We next elaborate on the claims made in Section~\ref{sec:intro} and show that multi-beam with optimal constructive combining and power-control can provide higher throughput than a single-beam link.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
    \caption{Multi-beam communication enhances the throughput \& reliability of mmWave link through constructive combining.}
    \label{fig:motivation}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/single_and_multi_beam_fixed.pdf}
%     % \caption{For a single-path channel in (a), the optimal analog beamforming is to use a single beam pattern with all the energy direct along that channel path. }
%     \caption{(a) For single-path channel, (b) the optimal analog beamforming technique is to use a single beam pattern with all the energy directed along that channel path. (c) For two-path channel, (d) a phase coherent multi-beam pattern with two lobes provides higher SNR compared to the single beam system by utilizing transmit diversity.}
%     \label{fig:single_and_multi_beam}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/single_path_system_v2-crop.pdf}
    % \caption{For a single-path channel in (a), the optimal analog beamforming is to use a single beam pattern with all the energy direct along that channel path. }
    \caption{(a) For single-path channel, (b) the optimal analog beamforming technique is to use a single beam pattern with all the energy directed along that channel path.}
    \label{fig:single_path_system_v2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/multi_path_system_v2-crop.pdf}
    % \caption{For a single-path channel in (a), the optimal analog beamforming is to use a single beam pattern with all the energy direct along that channel path. }
    \caption{(a) For two-path channel, (b) a phase coherent multi-beam pattern with two lobes provides higher SNR compared to the single beam system by utilizing transmit diversity.}
    \label{fig:multi_path_system_v2}
\end{figure}


We introduce a model for a multi-antenna base station transmitting to the user device using a mmWave link and derive optimal the optimal beamforming solution that maximizes the received SNR for a given wireless channel. First, we show that single-beam is optimal only when the wireless channel consists of a single path from the transmitter to the receiver. A single-beam system is sub-optimal for a multi-path channel, which is generally the case even for mmWave links. We then show that a multi-beam with two beam pattern is optimal for a two-path channel and maximizes the received SNR. We conclude with a note on generalizing our formulation to a channel with arbitrary multi-path.

\subsubsection{Primer: Optimal channel-dependent beamforming}
Consider the base-station (gNB phased array) consisting of $N$ antennas connected to a single RF chain. The transmit phased array applies beam weights $\wbf$ ($N\times 1$) to transmit signal $s$ which is received by a single antenna receiver.  The received signal $y$ is expressed as 
\begin{equation}
    y = \hbf^T \wbf s + n,
\end{equation}
where $\hbf$ is  $N\times 1$ channel from $N$ transmit antennas to one receive antenna and $n$ is white Gaussian noise at the receiver. The capacity or maximum throughput of a wireless link is evaluated in term of SNR (the ratio of signal power to noise power): 
\begin{equation}\label{eq:snr}
    \text{SNR} = {||\hbf^T \wbf ||^2 P_s}/{P_n},
\end{equation}
 where $P_s$ is the average transmit power (without transmit array gain) and $P_n$ is the noise power\footnote{We can mathematically derive the expression for SNR using $E[yy^H] = E[(\hbf^H \wbf s + n)(\hbf^H \wbf s + n)^H]] = \|\hbf^H \wbf\|^2 E[ss^H] + E[nn^H]$ and we denote $P_s = E[ss^T]$ and $P_n =E[nn^T]$}. Our goal is to estimate beamforming weights $\wbf$, that maximizes the SNR. Using Cauchy-Schwartz inequality, it follows that $||\hbf^T \wbf ||$ is maximized when $\hbf$ and $\wbf$ vectors point in the same direction. Finally, the beam weights $\wbf$ needs to be unitary to keep the power constant, i.e., $\|\wbf\|=1 $. This way, we get the optimal beam weights ${\wbf}^{\text{opt}}$ as:
\begin{equation}\label{eq:wmrc}
    {\wbf}^{\text{opt}} = {\hbf^*}/{||\hbf||},
\end{equation}
where $\hbf^*$ is conjugate of $\hbf$. The optimal beamforming provides the highest SNR of $\frac{||\hbf||^2P_s}{P_n}$. Note that the optimal beamforming weight is dependent on the channel $\hbf$. Wireless channel consists of multiple paths (direct or reflected paths), where each path is characterized by its angle of departure and attenuation. Therefore, beamforming is affected by the nature of multi-path channel as we discuss in the following subsections.  

% \todo{It is hard to obtain channels on a per-antenna basis for large arrays with many elements. Therefore, mmWave system tediously scan multiple beams in space to estimate the channel vector~\cite{palacios2018adaptive}.}{RS: the utility of these sentences is unclear}

\subsubsection{Primer: Single-beam is optimal for a single-path channel}
We first take a simple case when the channel is consists of only one path from the gNB to the UE as shown in Figure \ref{fig:single_path_system_v2}(a). The channel magnitude of the direct path is represented by a complex number $h$ and path angle is $\phi_1$. When the channel consists of only one path, the $N\times 1$ channel vector $\hbf^{\text{single}}$ is expressed as:
\begin{equation}\label{eq:1pathchannel}
    \hbf^{\text{single}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} 
\end{equation}
where $n$ is the antenna index, $d$ is the antenna spacing, and $\lambda$ is the wavelength ($d=\frac{\lambda}{2}$ in our phased array).
The optimal beam pattern for this single-path channel in (\ref{eq:1pathchannel}) is actually a single-beam pattern shown in Figure \ref{fig:single_path_system_v2}(b).
The expression for single-beam beamformer $\wbf_{\phi_1}$ to create a directional pattern along angle $\phi_1$ is:
\begin{equation}\label{eq:wphi1}
\begin{split}
     \wbf_{\phi_1}=\frac{ \hbf^{\text{single}^*}}{\| \hbf^{\text{single}}\|} =\frac{1}{\sqrt{N}}[1, e^{j2\pi \frac{d}{\lambda}\sin(\phi_1)},\ldots,  e^{j2\pi(N-1) \frac{d}{\lambda}\sin(\phi_1)}]^T
\end{split}
\end{equation}
In this case, we note that the single-beam is optimal (i.e., $\wbf_{\phi_1}= {\wbf}^{\text{opt}}$). However, in practice, the wireless channel could consist of multiple paths from the gNB to the UE, and the single-beam ceases to be optimal in these scenarios.

\subsubsection{Multi-beam is optimal for multi-path channel}
\label{sec:mbeam_th_der}
For simplicity, we consider a two path channel as shown in Figure \ref{fig:multi_path_system_v2}(a) with path magnitude $h$ and $h \delta e^{j\sigma}$ respectively and angles of departure $\phi_1$ and $\phi_2$ respectively. Here, $\delta \in \R$ is relative attenuation and $\sigma \in [0,2\pi]$ is relative phase of second channel path w.r.t. the first channel path. Two-path channel vector $\hbf^{\text{multi}}$ at antenna $n$ is:
\begin{equation}\label{eq:hmultieq}
    \hbf^{\text{multi}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} + h \delta e^{j\sigma} e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_2)}
\end{equation}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/multi_two_path_system.pdf}
%     \caption{When there are multiple reflectors in the environment as in (a), the single-beam system in (b) is no longer optimal because it does not utilize the multi-path nature of the underlying channel and thus suffers from low SNR. A phase coherent multi-beam pattern with two lobes in (b) or three lobes in (c) provides better SNR compared to the single beam system through transmit diversity. The optimal (or oracle) solution for three path channel is a multi-beam pattern with three lobes.} 
%     \label{fig:multi_two_path_system}
% \end{figure}
In this case, if we apply the same single-beamforming weights from the LoS channel (\ref{eq:wphi1}), it provides sub-optimal gain since the power along $\phi_2$ is severely attenuated and not coherently adding up at the receiver.
% it amplifies the first path and significantly attenuates the signal along the second path. 
For this single-beam case, we get an approximate SNR:

%  highlight the intuition that if you use the same beamforming vector $w$ from the LoS channel, then the power going towards angle $\alpha_2$ is not coherently adding up at the receiver.

\begin{equation}
    \text{SNR}^{\text{single}} = {|h|^2P_s}/{P_n}.
\end{equation}

In contrast, multi-beamforming weights are obtained by optimizing the SNR for the given channel. From (\ref{eq:wmrc}), we obtain multi-beam weight as $\textbf{w}^{\text{multi}} = {\hbf^{\text{multi}^*}}/{\|\hbf^{\text{multi}}\|}$ which is visualized in Fig. \ref{fig:multi_path_system_v2}(b). The SNR of multi-beam is obtained as $\|h^{\text{multi}}\|^2 P_s/P_n$ from (\ref{eq:snr}) which we simplify and approximate to the following expression:
\begin{equation}
    \text{SNR}^{\text{multi}} = {(1+\delta^2)|h|^2P_s}/{P_n}.
\end{equation}
The multi-beam SNR is higher than that of a single-beam system by a factor of $1+\delta^2$. The multi-beam is the optimal beamforming solution for multi-path channels and works by spliting the transmit signal constructively along both the paths in a manner that they maximally combine at the receiver. We discuss in Appendix~\ref{appendix:A} how this result can be generalized to show that a k-multi-beam is the optimal solution for a k-path channel.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.24\textwidth]{figures/reflector_relative_power_cdf.pdf}
%     \caption{Relative attenuation of reflected paths compared to the direct path at multiple locations in indoor environment.}
%     \label{fig:reflector_relative_power_cdf}
% \end{figure}
\begin{figure*} [!t]
    \subfigure{{\includegraphics[width=0.30\columnwidth]{figures/expt_setup_mmreliable.pdf}\label{fig:expt_setup_mmreliable}}}
    \subfigure{{\includegraphics[width=0.56\columnwidth]{figures/reflector_relative_power_cdf.pdf}\label{fig:reflector_relative_power_cdf}}}
    \subfigure{{\includegraphics[width=0.56\columnwidth]{figures/mobility_vis_example_noblock-crop-crop.pdf}\label{fig:reflector_movt_example_noblock}}}
    \subfigure{{\includegraphics[width=0.59\columnwidth]{figures/mobility_vis_example_block-crop-crop.pdf}\label{fig:reflector_movt_example_block}}}
    \vspace{-4mm}
    \caption{(a) Experiment test scenario (b) CDF of the relative attenuation of the strongest reflected path compared to the direct path at over various locations. (c) A heatmap of strong paths in the environment while the UE moves w.r.t gNB, strong reflectors appear at different points in time. (d) The experiment in (c) in a scenario where the direct path is blocked by a static object between 6 and 12 seconds.}
    % \vspace{-2mm}
    \label{fig:todo_put_nicely}
\end{figure*}
 

 
 
We note that \name's \constructivemultibeam approach depends on existence of two or more paths in the environment. This is a valid assumption based on measurement studies in both 28 GHz and 60 GHz mmWave~\cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}. These studies indicate that in a typical deployment, reflectors like metals, concrete walls, and tinted glass strongly reflect signals while attenuating them by about 5-6 dB ($\delta\approx0.5$). We also performed a measurement study of reflector strengths at 50 different indoor locations. As shown in Figure \ref{fig:reflector_relative_power_cdf}, common indoor reflectors cause 1-10 dB attenuation with a median attenuation of 6.1 dB relative to the direct path signal strength. This analysis shows that strong reflectors do exist and can be utilized to establish a multi-beam link.

\subsection{Creating multi-beam patterns with normalized total radiated power}\label{subsec:creating_mb}

In this section, we devise a method to create a multi-beam pattern by combining beamforming weights of respective single-beam patterns. While we consider a two-lobe beam in this section, the technique extends to any general multi-beam. We assume that the two strongest paths in the channel are known from the default beam-training method. Once these paths are known, we need to create a multi-lobe beam pattern that constructively adds up at the receiver. From Eq.~\ref{eq:wmrc} and Eq.~\ref{eq:hmultieq}, it follows that the multi-beam weights are in fact a linear sum of the constituent single-beam weights corresponding to $\phi_1,\phi_2$. If the relative attenuation $\delta$ and the relative phase $\sigma$ between the constituent beams are known, we can create the optimal multi-beam by simple addition.

Concretely, the beamforming weights $\textbf{w}$ for a two-lobe multi-beam is:
\begin{equation}\label{eq:beampattern}
    \textbf{w}(\phi_1,\phi_2,\delta,\sigma) = \frac{(\textbf{w}_{\phi_1}+{\delta} e^{-j{\sigma}}\textbf{w}_{\phi_2})}{\|(\textbf{w}_{\phi_1}+{\delta} e^{-j{\sigma}}\textbf{w}_{\phi_2})\|},
 \end{equation}
% where the normalizing factor (NF) is chosen to restrict the TRP to unity as follow
% \begin{equation*}\label{eq:nf}
% \begin{split}
%         \text{NF} &= ||\textbf{w}_{\phi_1} + \hat{\delta} e^{-j\hat{\sigma}}  \textbf{w}_{\phi_2}||^2\\ 
%         &= ||\textbf{w}_{\phi_1}||^2 + \hat{\delta}^2 ||\textbf{w}_{\phi_2}||^2 + 
%         \hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2} + 
%         \hat{\delta} e^{j\hat{\sigma}}\textbf{w}_{\phi_2}^H\textbf{w}_{\phi_1}\\
%         &=1+\hat{\delta}^2 +\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})
%         %&\approx 1+\hat{\delta}^2
% \end{split}
% \end{equation*}

The denominator ensures that the TRP is conserved by enforcing $\|\textbf{w}\|=1$ . We then appropriately quantize the beamforming vector phases \& amplitudes to be compatible with our phased array. In~\cite{aykin2019multi}, a sub-optimal multi-beam is created by splitting the array into sub-arrays, each responsible for a particular component beam. In contrast, \name utilizes amplitude control to create the optimal channel dependent multi-beam.


% We show the sensitivity of beamforming to phase and amplitude errors in \todo{Appendix~\ref{appendix:S}}.


 \subsection{Obtaining parameters for multi-beam constructive combining}\label{sec:constructive_combining}
% We propose a novel constructive combining optimization algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ per beam required for constructive combining. For the 2-beam case, our algorithm requires only two probes to estimate these parameters and in-general $2(K-1)$ probes for $K$ beams. For simplicity, we explain the 2-beam case here. To start with, gNB and the UE create a 2-beam pattern directed towards the AoD and AoA estimates, respectively (Assuming downlink case). The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam as follows:
Just as in prior sub-sections, we use $\delta$ as the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. In this sub-section, we present our constructive combining algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ for the two-beam case. From the beam-training phase, we already know the directions $\phi_1,\phi_2$ of the two paths. Let the wireless channel along each of these paths be $h_1$ and $h_2$ respectively. The gNB uses two RS to probe two 2-beam patterns: first it sets the beam $w(\phi_1,\phi_2,1,0)$, and then $w(\phi_1,\phi_2,1,\pi)$. It then estimates the channel $\pbf_1$ and $\pbf_2$  for each probe as:
\begin{equation}\label{eq:two_probe_cc}
    \begin{split}
        \pbf_1 &= e^{j0}\hbf_1 + e^{j0} \hbf_2 = \hbf_1  + \hbf_2\\
        \pbf_2 &= e^{j0}\hbf_1  + e^{j\pi} \hbf_2 = \hbf_1  - \hbf_2
    \end{split}
\end{equation}
% \begin{equation}\label{eq:two_probe_cc}
%     \begin{split}
%         H_1(f_i) &= h_1(f_i) + e^{j0} h_2(f_i) = h_1(f_i) + h_2(f_i)\\
%         H_2(f_i) &= h_1(f_i) + e^{j\pi} h_2(f_i) = h_1(f_i) - h_2(f_i)
%     \end{split}
% \end{equation}
where $\hbf_1 $ and $\hbf_2$ is the complex per-path CSI (Channel State Information) observed by each of two beams across all frequency subcarriers. Using the set of two equations in (\ref{eq:two_probe_cc}), we estimate the complex per-path channel as $\hbf_1  = (\pbf_1+\pbf_2)/2$ and $\hbf_2 = (\pbf_1-\pbf_2)/2$. We then formulate an optimization problem that maximizes the average received signal strength over all frequencies to jointly estimate $\{\hat{\delta},\hat{\sigma}\}$ as:
% The relative phase $\sigma$ is approximately constant across frequency subcarriers because of high frequency of mmWave compared to bandwidth (Shown in Appendix \ref{appendix:A}). So we take an average over all of the frequency subcarriers to get a robust estimate. 
% Note that we inherently cannot estimate $\hat{\sigma}$ that works well for all the subcarriers simultaneously. 
% Our constructive combining approach maximizes the average received signal strength over all frequencies as:
\begin{equation}\label{eq:snroverall}
   \{\hat{\delta}, \hat{\sigma}\} = \argmax_{\delta,\sigma}\;\; \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
\end{equation}
% \begin{equation}\label{eq:snroverall}
%   \{\hat{\delta}, \hat{\sigma}\} = \arg\max_{\delta,\sigma}\sum_{f_i} \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
% \end{equation}

We solve the above to obtain a closed form solution:
\begin{equation}
    \hat{\delta}e^{j \hat{\sigma}} = -{\hbf_2^H\hbf_1}/{\hbf_2^H\hbf_2},
\end{equation}
which simply reduces to $\hat{\delta}e^{j \hat{\sigma}} = -h_1/h_2 $ for a narrowband channel (e.g. in IEEE 802.11ad 60 GHz standard \cite{ieee80211ad}).

\todo{R3: The solution requires full channel state information, which may not be practical.
ToDo: Explain Full CSI is available in both 5G NR and 802.11ad}

Our algorithm estimates these parameters using only two consecutive RS probes for the two-beam case. In general, it requires $2(K-1)$ probes for $K$ beams independent of the number of antenna elements in the phased array.  
Note that \name requires the full CSI at the receiver for every probe to perform constructive combining. For the 5G NR system, the CSI is readily available from the RS. Even for 802.11ad commercial routers, the CSI can be extracted in the firmware~\cite{qualcomm2017wil6210, wang2020demystifying, palacios2018adaptive}. Finally, the optimal phase, amplitude, \& angle will change over time as the user moves. We periodically estimate these parameters while implementing our tracking algorithm discussed in Section~\ref{sec:design}. 

\review{In Section 3.2, the authors describe a two-probe based approach to estimate the two-beam channels. However, Equation (6) seems to suggest one should apply different phases to different directions h1 and h2: the first probe applies the same phase to both directions whereas the second probe applies different phases to the two directions. Then this requires our knowledge of h1 and h2. Isn't it a chicken-and-egg problem? Unless we know h1 and h2, how can we apply different phases to different directions?
}
\newtodo{The reviewer addressed a misunderstanding on mmReliable algorithm in Eq (6). We will clarify this misunderstanding by improving the writing of Section 3.2.
}

}% highlightshep

==> Arxiv/3_design_multibeam_v3_backup.tex <==
% Created by RS on 26 June 2021. backup of v3
\section{Design of Multi-beam system}\label{sec:creatingmultibeam}
% The multi-beam patterns have high antenna gain in single or multiple main lobes that orient towards the reflectors or the LOS path.  We show that an effective way of generating multi-beam patterns is to take the weighted sum of beamforming weights of individual beams in the multi-beam. 

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/mmReliableOverview1_v2.pdf}
    \caption{Shows an overview of building blocks of \name that leverages SSB and CSI-RS in 5G NR to establish a multi-beam link.}
    \label{fig:overview1_v2}
    \vspace{-10pt}
\end{figure}
In this section, we present \name's algorithm for creating a reliable and high-throughput multi-beam link. First, we establish a mathematical framework to model the throughput and reliability gains in a multi-beam system. Then, we show that multi-beam patterns are channel-dependent and require an estimate of angle, phase, and attenuation of each channel path. We propose a two step procedure to estimate these parameters as shown in Fig. \ref{fig:overview1_v2}. We leverage any standard beam training procedure in 5G NR to estimate the angle of each multipath \cite{ghasempour2018multi, jog2019many}. We then design a customized procedure to estimate the per-path phase and attenuation with low overhead using CSI-RS. Finally, we explain our novel analog beamforming to establish a multi-beam link using these parameters.


\subsection{Multi-beam link provides high reliability}
We show how multi-beam links are reliable even under the impact of blockage events. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid}. 
We formally define link reliability as the fraction of time when the link is available for communication. This fraction is vis-a-vis the total time the link is not in outage (due to natural effects) or in beam training, and therefore unavailable for communication. 
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
In practice, the probability of outage is computed as the fraction of duration where the SNR is below a minimum threshold. The directional nature of single-beam mmWave links make them susceptible to blockage \& user mobility, reducing SNR by 20 to 30 dB~\cite{maccartney2017rapid} and causing outages.


\review{R2: Another strong assumption is that the probability of blocking each lobe of a multi-beam pattern is independent. However, that’s not the case in the real-world as the lobes are often highly correlated.}
\newtodo{The reviewer is concerned about correlated blockages. We have omitted them from Section 3.4 for simplicity, but have evaluated our system considering this correlation. We will put a note in Section 3.4.}
\subsection{Multi-beam Throughput Model}


We next elaborate on the intuitive example presented in Section \ref{sec:intro} and show how multi-beam with optimal constructive combining and power-control can help maintaining a high throughput link. 
% We first focus on a scenario without blockage and later study the links under blockage.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/toyexampleV2.pdf}
    \caption{Multi-beam communication enhances the throughput \& reliability of mmWave link through constructive combining.}
    \label{fig:motivation}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/single_and_multi_beam_fixed.pdf}
    % \caption{For a single-path channel in (a), the optimal analog beamforming is to use a single beam pattern with all the energy direct along that channel path. }
    \caption{(a) For single-path channel, (b) the optimal analog beamforming technique is to use a single beam pattern with all the energy directed along that channel path. (c) For two-path channel, (d) a phase coherent multi-beam pattern with two lobes provides higher SNR compared to the single beam system by utilizing transmit diversity.}
    \label{fig:single_and_multi_beam}
\end{figure}
We introduce a model for a multi-antenna base station transmitting to the user device using a mmWave link and prove optimal beamforming decision that maximizes the received signal-to-noise (SNR) for a given wireless channel. We would show that single beam-based beamforming is optimal only when the wireless channel consists of a single path from the transmitter to the receiver. A single beam system becomes sub-optimal for a multi-path channel, which is generally the case even for mmWave links. We then show that a multi-beam with two beam pattern is optimal for a two-path channel and maximizes the received SNR. We finally conclude that our formulation generalizes to an arbitrary multi-path channel providing a high throughput link. 

\subsubsection{Primer: Optimal channel-dependent beamforming}
Consider the base-station (gNB phased array) consists of $N$ antennas connected to a single RF chain. The transmit phased array applies beam weights $\wbf$ ($N\times 1$) to transmit signal $s$ which is received by a single antenna receiver.  The received signal $y$ is expressed as 
\begin{equation}
    y = \hbf^T \wbf s + n,
\end{equation}
where $\hbf$ is  $N\times 1$ channel from $N$ transmit antennas to one receive antenna and $n$ is white Gaussian noise at the receiver. The capacity or maximum throughput of a wireless link is evaluated in term of SNR (signal-to-noise ratio). SNR is defined as the ratio of signal power by noise power and is obtained as: 
\begin{equation}\label{eq:snr}
    \text{SNR} = {||\hbf^T \wbf ||^2 P_s}/{P_n},
\end{equation}
 where $P_s$ is the average transmit power (without transmit antenna gain) and $P_n$ is the noise power\footnote{We can mathematically derive the expression for SNR using $E[yy^H] = E[(\hbf^H \wbf s + n)(\hbf^H \wbf s + n)^H]] = \|\hbf^H \wbf\|^2 E[ss^H] + E[nn^H]$ and we denote $P_s = E[ss^T]$ and $P_n =E[nn^T]$}. The goal is to estimate beamforming weights $\wbf$, which maximizes the SNR. Using Cauchy-Schwartz inequality, w deduce that the expression $||\hbf^T \wbf ||$ is maximized when $\hbf$ and $\wbf$ vectors point in the same direction. Finally, the beam weights $\wbf$ needs to be unitary to keep the power constant, i.e., $\|\wbf\|=1 $. This way, we get the optimal beam weights ${\wbf}^{\text{opt}}$ as:
\begin{equation}\label{eq:wmrc}
    {\wbf}^{\text{opt}} = {\hbf^*}/{||\hbf||},
\end{equation}
where $\hbf^*$ is conjugate of $\hbf$. The optimal beamforming provides the highest SNR of $\frac{||\hbf||^2P_s}{P_n}$. Note that the optimal beamforming weight is dependent on the channel $\hbf[n]$ for every antenna $n\in[1,N]$. It is hard to obtain per-antenna channel from an analog phased array because the signal at each antenna gets adds up at the phased array. Therefore, mmWave system tediously scan multiple beams in space to estimate the channel vector~\cite{palacios2018adaptive}.
% Existing channel estimation schemes involve tedious beam probing procedures which suffers from a high overhead and low accuracy in low SNR scenarios~\cite{palacios2018adaptive}.

% i.e.,  ${\wbf^*} \propto {\hbf}$.

\subsubsection{Primer: Single-beam is optimal for single-path channel}
We first take a simple case when the channel is consists of only one path from the gNB to the UE as shown in Figure \ref{fig:single_and_multi_beam}(a). The channel magnitude of the direct path signal is represented by a complex number $h$ and path angle is $\phi_1$. When the channel consists of only one path, the $N\times 1$ channel vector $\hbf^{\text{single}}$ is expressed as:
\begin{equation}\label{eq:1pathchannel}
    \hbf^{\text{single}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} 
\end{equation}
where $n$ is the antenna index, $d$ is the antenna spacing, and $\lambda$ is the wavelength ($d=\frac{\lambda}{2}$ in our phased array).
The optimal beam pattern for this single-path channel in (\ref{eq:1pathchannel}) is actually a single-beam pattern considered widely in literature (Figure \ref{fig:single_and_multi_beam}(b)) \cite{jain2020mmobile}. 
% The single beam system utilizes a phased array of $N$ antennas to create a directional pattern along angle $\phi_1$. 
The expression for single-beam beamformer $\wbf_{\phi_1}$ to create a directional pattern along angle $\phi_1$ is:
\begin{equation}\label{eq:wphi1}
\begin{split}
     \wbf_{\phi_1}=\frac{ \hbf^{\text{single}^*}}{\| \hbf^{\text{single}}\|} =\frac{1}{\sqrt{N}}[1, e^{j2\pi \frac{d}{\lambda}\sin(\phi_1)},\ldots,  e^{j2\pi(N-1) \frac{d}{\lambda}\sin(\phi_1)}]^T
\end{split}
\end{equation}
We note that a single beam pattern is optimal for a single-path channel (i.e., $\wbf_{\phi_1}= {\wbf}^{\text{opt}}$). But, in practice, the wireless channel consists of multiple components reflected off the wall, shelves, glass, and other high-reflecting materials. For a multi-path channel, the single-beam system is not an optimal solution, and in such a case, the multi-beam provides a higher gain than the single beam.


\subsubsection{Single beam is not optimal for multi-path channel}
For simplicity, we consider a two path channel as shown in Figure \ref{fig:single_and_multi_beam}(c) with path magnitude $h$ and $h \delta e^{j\sigma}$ respectively and angles of departure $\phi_1$ and $\phi_2$ respectively. Here, $\delta \in \R$ is relative attenuation and $\sigma \in [0,2\pi]$ is relative phase of second channel path w.r.t. the first channel path. Two-path channel vector $\hbf^{\text{multi}}$ at antenna $n$ is:
\begin{equation}
    \hbf^{\text{multi}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} + h \delta e^{j\sigma} e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_2)}
\end{equation}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/multi_two_path_system.pdf}
%     \caption{When there are multiple reflectors in the environment as in (a), the single-beam system in (b) is no longer optimal because it does not utilize the multi-path nature of the underlying channel and thus suffers from low SNR. A phase coherent multi-beam pattern with two lobes in (b) or three lobes in (c) provides better SNR compared to the single beam system through transmit diversity. The optimal (or oracle) solution for three path channel is a multi-beam pattern with three lobes.} 
%     \label{fig:multi_two_path_system}
% \end{figure}
In this case, if we apply a single-beam pattern from (\ref{eq:wphi1}), it provides sub-optimal gain since it amplifies the first path and significantly attenuates the signal along the second path. Thus, by ignoring the second path, we get an approximate SNR of the single beam as
\begin{equation}
    \text{SNR}^{\text{single}} = {|h|^2P_s}/{P_n}.
\end{equation}


In contrast, multi-beamforming weights are obtained by optimizing the SNR for the given channel. From (\ref{eq:wmrc}), we obtain multi-beam weight as $\textbf{w}^{\text{multi}} = {\hbf^{\text{multi}^*}}/{\|\hbf^{\text{multi}}\|}$. 
% creates a beam pattern with two lobes and optimizes the angle, phase, and amplitude of the two lobes to match with the channel such that the SNR is maximized. We developed a novel way of generating multi-beam pattern and showed that they are optimal (i.e., they maximizes the SNR). The multi-beam beamformer with two lobes is
% \begin{equation}\label{eq:beampattern}
%     \textbf{w}^{\text{multi}} = {\hbf^{\text{multi}^*}}/{\|\hbf^{\text{multi}}\|}.
%  \end{equation}
% Note that $\|\textbf{w}^{\text{multi}}\| = 1$ ensures that the total radiated power is a constant. 
% For better intuition on multi-beam gain, we approximate the denominator of (\ref{eq:beampattern}) to $\sqrt{1+\delta^2}$, which is reasonable when the two angles $\phi_1$ and $\phi_2$ are separated by more than beamwidth ($12^\circ$ for $N=8$).  
Thus, the approximate SNR of multi-beam can be obtained from (\ref{eq:snr}) as :
\begin{equation}
    \text{SNR}^{\text{multi}} = {(1+\delta^2)|h|^2P_s}/{P_n}.
\end{equation}
% We see that the SNR of multi-beam is higher than that of the single beam by the factor of $1+\delta^2$. The SNR gain comes from careful utilization of the multi-path channel.


% \subsubsection{Multi-beam with constructive combining provides high throughput:} Here, we provide a mmWave signal propagation model and derive an expression for the multi-beam mmWave link capacity. We show that a multi-beam link leverages a multipath channel to improve link capacity compared to the channel-agnostic single-beam link. We consider a two-path channel with complex channel attenuation $h$ and $h\delta e^{j\sigma}$ along the direct and reflected path respectively as shown in Fig. \ref{fig:motivation}. Note that $\delta$ is the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. The gNB creates a two-beam pattern and align each beam towards each channel paths. 

% Our key insight is that we can optimize the relative phase and amplitude of the two beams to maximize the receiver's signal strength without increasing the total transmit power. Our constructive combining and power control algorithm provides a transmit antenna gain proportional $1$ and $\delta e^{-j\sigma}$ along the two paths. 
% The UE receives the signal $y$ through an omni-directional beam pattern as: 
% \begin{equation}
%     y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{-j\sigma}}{\sqrt{1+\delta^2}}h \delta e^{j\sigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
% \end{equation}
% where $x$ is the signal transmitted by the gNB through a single RF-chain and $n$ is the receiver noise. A normalization factor of $1/\sqrt{1+\delta^2}$ ensures that we do not increase the total transmit power (Section~\ref{subsec:creating_mb}). The capacity of such phase-coherent two-beam link can be written as
% \begin{equation}\label{eq:multibeam}
%     C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_s}{P_n}\right)\; \textbf{(multi-beam)}
% \end{equation}
%  where $P_n$ is the receiver noise power and $P_s=\mathbb{E}[x]^2$ is average transmit power.

% On the other hand, a single beam link directs the power towards the direct path while the reflected path signal is severely attenuated. It provides a capacity of: 
% \begin{equation}
%   C_{sb} = \log_2(1+|h|^2P_s/P_n) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
% \end{equation}




We surprisingly note that the multi-beam SNR is higher than that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. In general, we show that we can further improve the link capacity by considering more than two beams as proven in Appendix \ref{appendix:A}.
% We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 

% \begin{theorem}\label{th:mb_capacity}
% Multi-beam patterns maximises the SNR at the receiver when the number of beams in multi-beam is the same as the number of channel paths providing a capacity gain of
% \begin{equation}
%     C_{mb} = \log_2\left(1+\frac{\sum_{p=0}^{P-1}||\gamma_p||^2P_s}{P_n}\right)
% \end{equation}
% where $\gamma_p$ is the complex channel attenuation along path $p$.
% \end{theorem}
% \begin{proof}
% We provide the proof in Appendix \ref{appendix:A}
% \end{proof}
% Intuitively, we are constructively utilizing the reflections in a multi-path channel to increase the signal power and throughput.

Since \name's \constructivemultibeam approach depends on existance of two or more paths channel models, a valid question here is what physical phenomenon can give rise to such underlying channels. There have been a lot of channel measurement papers for both 28 GHz and 60 GHz mmWave links which have shown that in a typical deployment, there are strong reflectors like metals, concrete walls, tinted glasses etc, which reflect the signals by only attenuating the reflections by about 5-6 dB \cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}.
% \newtodo{A statement on reflectors are strong at 28 GHz, typically only 3-6 dB attenuation of strong multipath~\cite{zhu2014demystifying, telecom2019analysis}.}

% Creating these optimal multi-beam patterns is challenging for two reasons. (i) The gNB needs to accurately estimate the direction, phase, and attenuation of each channel path and (ii) create a multi-beam pattern that provides the required per-beam antenna gain for constructive combining while satisfying the total radiated power constraint. We solve these design challenges in later subsections.





% There are three parameters we phase, amplitude and then form a mult

% We present \name, a novel mmWave system that creates multi-beam patterns to improve link reliability while maintaining high throughput. 


%  We present the overall working of \name with the help of a flow-chart in Figure~\ref{fig:design_overview}. At a high level, \name has two major phases: the \textbf{Beam Training Phase} (BTP) and the \textbf{Data Transmission Phase} (DTP). During the BTP, \name leverages the standard exhaustive beam search to estimate some initial parameters such as AoA, AoD, and ToF of each channel path, which is required to establish a multi-beam link. The DTP establishes and periodically refines a multi-beam link through constructive combining optimization. It achieves constructive combining of multi-path signal through two novel contributions: 
% (i) It provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining.
% (ii) It develops a novel analog beamforming method to create phase-coherent multi-beams. 
% The DTP ends when the beam is no longer recoverable by tracking alone (due to accumulated errors in tracking over time) and signals the next BTP. The cycle of BTP and DTP repeats periodically. \newtodo{Does it need to be periodic? or can it be triggered only when needed?}
 
%  It then proceeds to set up the initial multi-beam link with the constructive combining optimization and signals the start of the DTP. The DTP relies on techniques developed in Section~\ref{sec:design} to perform proactive beam refinement. We elaborate on these two phases below:}


% \name achieves high throughput and high reliability by exploiting multi-path diversity using custom designed multi-beam patterns. It achieves constructive combining of multi-path signal through two novel contributions: (i) it develops novel analog beamforming method to create multi-beams and (ii) it provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining. We delineate the process of constructive combining as follows:




% In this phase, we estimate initial parameters of each path in the environment from the transmitter to the receiver. This is done at the initial user location by leveraging the standard beam training protocol. The primary purpose of beam training is to find all the right beams by scanning all a large set of beams in the codebook and observing the highest SNR beam pattern. We leverage the beam training process to also estimate the AoA and AoD profile of all the LOS and reflected paths. 

% A key challenge, however, is to associate the AoA with the AoD of corresponding reflectors. The mapping of AoA and AoD is non-trivial because the orientation of transceiver and reflecting surfaces is generally unknown. Prior work \cite{palacios2018adaptive} relies on a custom beam training process to estimate absolute channel response per antenna independent of the beam pattern; then apply the traditional MUSIC algorithm to estimate AoA and AoD jointly. Other works assume an Omni-directional user pattern to avoid the issue \cite{aykin2020mamba}.

% We leverage the ToF to solve the association problem. Each reflected path has a unique ToF. Note that due to the directional beam pattern, some paths are strengthened while other paths weaken. When the beam is aligned with some reflector, the strongest signal comes from reflected path corresponding to that reflector. We use the CIR corresponding to the beam directed along the AoA/AoD and estimate the ToF. The ToF is the delay corresponding to the highest power in CIR. The LOS path is identified as the path with the lowest ToF. This way \name estimates the AoA, AoD, ToF of each reflected path and associate them with each other. 

% \name leverages the process not only to select the highest SNR beam but plots the highest SNR of each beam with the beam direction and finds all the local maxima and estimates their corresponding directions. These directions are reported as the AoA/AoD of all the reflected paths. After the initial training, \name creates a multi-lobe beam pattern with power adjusted to match EIRP constraints along the direction of strong paths, therefore establishing the multi-beam link. The constructive combining optimisation completes this phase.
% \textcolor{purple}{
% \subsubsection{Data Transmission Phase}
% While beam refinement is performed very frequently with minimal overhead to establish a reliable connection, the large overhead beam training process can be delayed but cannot be avoided. \name uses the techniques developed in Section~\ref{sec:design} to delay the complex beam training process as much as possible. It updates the channel parameters (AoA, AoD, ToF) every time the beam training is repeated. The data transmission phase consists of multiple cycle beam refinements. Each beam refinement cycle involves observing multiple OFDM packets in the background and uses our super-resolution and constructive combining algorithm to achieve high throughput and high reliability. }

% The parameters AoA/AoD/ToF are updated whenever the beam training is repeated. During the period in between two BTP, the AoA and AoD can change significantly due to user rotation and translation. However, the relative ToF remains stable. The ToF does not change with device rotation. With translation, the change in ToF is minor. This enables \name to use the novel super-resolution algorithm (Section~\ref{sec:establish-multi-beam}) that takes the combined multi-beam received signal at the receiver to deconstruct the per-beam amplitude/power for each packet's CIR received. 

% Armed with knowledge of the per-beam amplitude, \name monitors them for changes over time, performing a hierarchical classification between blockage events and mobility events. Within mobility events, \name uses the angular deviations to approximate the motion as rotation and translation and performs proactive beam refinement.

\subsection{Creating multi-beam patterns with normalized total radiated power}\label{subsec:creating_mb}
Here we describe how we create multi-beam pattern for a general multi-path channel.
For a given multi-path channel, we first identify two strongest channel taps and create a two-beam pattern that's aligned along the two paths. We device a simple method to create multi-beam pattern by combining the beamforming weights of respective single beam patterns.
% The beamforming weights for a single beam pointing at an angle $\phi_1$ is given by
% \begin{equation}
%     \textbf{w}_{\phi_1} = \frac{1}{\sqrt{N}}[1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_1)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_1)} ]^T
% \end{equation}
% where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of antennas. The total radiated power (TRP) is normalized to unity (i.e., $||\textbf{w}_{\phi_1}||^2=1$). 
We design beamforming weights $\textbf{w}$ for multi-beam with two lobes as follow:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{\text{NF}}}(\textbf{w}_{\phi_1}+\hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_2}),
 \end{equation}
where the normalizing factor (NF) is chosen to restrict the TRP to unity as follow
\begin{equation*}\label{eq:nf}
\begin{split}
        \text{NF} &= ||\textbf{w}_{\phi_1} + \hat{\delta} e^{-j\hat{\sigma}}  \textbf{w}_{\phi_2}||^2\\ 
        &= ||\textbf{w}_{\phi_1}||^2 + \hat{\delta}^2 ||\textbf{w}_{\phi_2}||^2 + 
        \hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2} + 
        \hat{\delta} e^{j\hat{\sigma}}\textbf{w}_{\phi_2}^H\textbf{w}_{\phi_1}\\
        &=1+\hat{\delta}^2 +\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})
        %&\approx 1+\hat{\delta}^2
\end{split}
\end{equation*}
We observe that the NF becomes $1+\hat{\delta}^2$ when the two single beams are orthonormal (i.e., $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}=0$ ). Intuitively, a single beam pattern contains unwanted side-lobes which may interact with the other beam in multi-beam to cause interference. We provide an analog beamforming optimization to remove this interference and create perfect orthonormal beams. Our solution is inspired from the class of null-constraint based beamforming techniques \cite{akdagli2001null,karaboga2002null} which create a single directional beam oriented at a desired direction while at the same time also put a null in the direction of interference. We obtain $\wbf_{{\phi_1},\text{null}}$ from $\wbf_{\phi_1}$ through the following optimization: \textcolor{red}{Ish: This optimization is not needed to create optimal beam pattern. This optimization in fact harm multi-beam when the two paths are close.}
\begin{equation}
\begin{split}
     \wbf_{{\phi_1},\text{null}} = &\argmin_{\wbf} ||\wbf-\wbf_{\phi_1}||^2\\
     & \text{such that } \wbf^H\wbf_{\phi_2} = 0 \text{ and } ||\wbf||^2=1
\end{split}
\end{equation}
It is a standard convex optimization problem for which a closed-form solution exists \cite{boyd2004convex,cvx}. We finally create multi-beam pattern using the following beamforming vector:
\begin{equation}\label{eq:beampattern}
    \textbf{w} = \frac{1}{\sqrt{1+\delta^2}}(\wbf_{{\phi_1},\text{null}}+\hat{\delta} e^{-j\hat{\sigma}}\wbf_{\phi_2}),
 \end{equation}
We then appropriately quantize the beamforming vector phases \& amplitudes to be compatible with our testbed. We show the sensitivity of beamforming to phase and amplitude errors in Appendix~\ref{appendix:S}.


 \subsection{Obtaining parameters for multi-beam constructive combining}\label{sec:constructive_combining}
% We propose a novel constructive combining optimization algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ per beam required for constructive combining. For the 2-beam case, our algorithm requires only two probes to estimate these parameters and in-general $2(K-1)$ probes for $K$ beams. For simplicity, we explain the 2-beam case here. To start with, gNB and the UE create a 2-beam pattern directed towards the AoD and AoA estimates, respectively (Assuming downlink case). The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam as follows:
Just as in prior sub-sections, we use $\delta$ as the relative attenuation ($\delta<1$) and $\sigma$ is the relative phase shift $0<\sigma\le 2\pi$ of the reflected path w.r.t. the direct path. In this sub-section, we present our constructive combining algorithm to estimate the relative phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ for the two-beam case. The gNB uses two CSI-RS to probe two 2-beam patterns, each with opposite phases of individual beams in the 2-beam. It then estimates the channel $\pbf_1$ and $\pbf_2$  for each probes as:
\begin{equation}\label{eq:two_probe_cc}
    \begin{split}
        \pbf_1 &= e^{j0}\hbf_1 + e^{j0} \hbf_2 = \hbf_1  + \hbf_2\\
        \pbf_2 &= e^{j0}\hbf_1  + e^{j\pi} \hbf_2 = \hbf_1  - \hbf_2
    \end{split}
\end{equation}
% \begin{equation}\label{eq:two_probe_cc}
%     \begin{split}
%         H_1(f_i) &= h_1(f_i) + e^{j0} h_2(f_i) = h_1(f_i) + h_2(f_i)\\
%         H_2(f_i) &= h_1(f_i) + e^{j\pi} h_2(f_i) = h_1(f_i) - h_2(f_i)
%     \end{split}
% \end{equation}
where $\hbf_1 $ and $\hbf_2$ is the complex per-path CSI (channel state information) observed by each of two beams across all frequency subcarriers. Using the set of two equations in (\ref{eq:two_probe_cc}), we estimate the complex per-path channel as $\hbf_1  = (\pbf_1+\pbf_2)/2$ and $\hbf_2 = (\pbf_1-\pbf_2)/2$. We then formulate an optimization problem that maximizes the average received signal strength over all frequencies to jointly estimate $\{\hat{\delta},\hat{\sigma}\}$ as:
% The relative phase $\sigma$ is approximately constant across frequency subcarriers because of high frequency of mmWave compared to bandwidth (Shown in Appendix \ref{appendix:A}). So we take an average over all of the frequency subcarriers to get a robust estimate. 
% Note that we inherently cannot estimate $\hat{\sigma}$ that works well for all the subcarriers simultaneously. 
% Our constructive combining approach maximizes the average received signal strength over all frequencies as:
\begin{equation}\label{eq:snroverall}
   \{\hat{\delta}, \hat{\sigma}\} = \argmax_{\delta,\sigma}\;\; \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
\end{equation}
% \begin{equation}\label{eq:snroverall}
%   \{\hat{\delta}, \hat{\sigma}\} = \arg\max_{\delta,\sigma}\sum_{f_i} \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
% \end{equation}

We solve the above eqn to a closed form expression as:
\begin{equation}
    \hat{\delta}e^{j \hat{\sigma}} = -{\hbf_2^H\hbf_1}/{\hbf_2^H\hbf_2},
\end{equation}
which simply reduces to $\hat{\delta}e^{j \hat{\sigma}} = -h_1/h_2 $ for a narrowband channel (e.g. in IEEE 802.11ad 60 GHz standard \cite{ieee80211ad}).
% We then use the estimates $\hat{\delta}$ and $\hat{\sigma}$ to create phase-coherent multi-beam patterns as detailed in the following subsection.
% where $\hbf_2$ and $\hbf_1$ are vectors of per-path CSI for all frequencies.
% \begin{equation}
%     \hat{\delta}e^{i \hat{\sigma}} = \frac{\sum_i h_2(f_i)^*h_1(f_i)}{\sum_i h_2(f_i)^*h_2(f_i)}
% \end{equation}
% Since, we are only interested in the relative channel, we represent $ \delta e^{j\sigma} =\frac{h_2(f_i)}{h_1(f_i)}$. We obtain the estimate of relative phase and amplitude in closed form as follow:
% \begin{equation}\label{eq:phase_estimate}
%     \hat{\delta}e^{i \hat{\sigma}} = \sum_i\frac{H_1(f_i)-H_2(f_i)}{H_1(f_i) + H_1(f_i)}. 
% \end{equation}
% We start by setting a multi-beam link with amplitude $\delta$ measured during initial beam training (Section \ref{sec:buildingblock}) and  a random phase-per-beam $\sigma$. 
% We consider a wideband system (such as 5G NR) and observe the effective channel response at each frequency subcarrier $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 
% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j,0)$ and $ H_{\text{eff}}(f_j,180)$ by setting two distinct values of $\sigma$ ($0^o$ and $180^o$) and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. 
% \begin{equation}
%     \begin{split}
%         H_{\text{eff}(f_j, 0)}
%     \end{split}
% \end{equation}
% From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. 
\todo{R3: The solution requires full channel state information, which may not be practical.
ToDo: Explain Full CSI is available in both 5G NR and 802.11ad
}
Our algorithm estimates these parameters using only two consecutive CSI-RS probes in NR for the two-beam case. In general, it requires $2(K-1)$ probes for $K$ beams independent of the number of antenna elements in the phased array.  
Note that \name requires the full CSI at the receiver for every probe to perform constructive combining. For the 5G NR system, the CSI is readily available from the CSI-RS signal. Even for 802.11ad commercial routers, there is firmware available to extract the CSI~\cite{qualcomm2017wil6210, wang2020demystifying, palacios2018adaptive}. Finally, the optimal phase, amplitude, \& angle will change over time as the user moves. We propose to periodically estimate these parameters along with our novel tracking algorithm that we'll discuss in Section~\ref{sec:design}. 

\review{In Section 3.2, the authors describe a two-probe based approach to estimate the two-beam channels. However, Equation (6) seems to suggest one should apply different phases to different directions h1 and h2: the first probe applies the same phase to both directions whereas the second probe applies different phases to the two directions. Then this requires our knowledge of h1 and h2. Isn't it a chicken-and-egg problem? Unless we know h1 and h2, how can we apply different phases to different directions?
}
\newtodo{The reviewer addressed a misunderstanding on mmReliable algorithm in Eq (6). We will clarify this misunderstanding by improving the writing of Section 3.2.
}
%   \begin{figure} [!t]
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_factor_with_AOD.pdf}\label{fig:onormal_factor_with_AOD}}
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/onormal_SNR_with_AOD.pdf}\label{fig:onormal_SNR_with_AOD}}
%     \vspace{-4mm}
%     \caption{(a) Orthonormality factor is close to zero when beams are separated by more than $12^o$). (b) The resulting SNR gain approaches 3 dB when beams are orthonormal and stays within $\pm$ 0.7 dB, sometimes even higher than 3 dB.}
%     \label{fig:orthonormality}
%  \end{figure}





% We empirically found that $\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2}$ in (\ref{eq:nf}) is order of magnitude less than the $1+\hat{\delta}^2$ when the beams are far by more than half-power beamwidth which is $12^o$ in our system. 
% We define orthonormality factor as the ratio $\frac{\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})}{1+\hat{\delta}^2}$ and show that it indeed is close to zero for a beam separation of half-power beamwidth which is $12^o$ in our system as shown in Figure \ref{fig:onormal_factor_with_AOD}. We get the SNR gain of $3$ dB when the two beams are orthonormal (assuming two paths suffer equal channel attenuation), varying in the range of $2.3$ dB to $3.7$ dB when the beams are not orthonormal as shown in Figure~\ref{fig:onormal_SNR_with_AOD}. 
% Intuitively, when the two beams are extremely close, the channel across two beams becomes correlated due to the wide beam aperture, and it becomes equivalent to the single-beam case when they merge. Thus, the results of (\ref{eq:multibeam}) hold in general. We emphasize that we used the NF from (\ref{eq:nf}) for normalization (and not the approximate value) to satisfy the TRP constraint in our testbed implementation strictly. 

% The resulting SNR varies around 3dB (assuming two paths suffers equal channel attenuation) with a maximum variation of $\pm 0.7 dB$ shown in Figure~\ref{fig:onormal_SNR_with_AOD}. Intuitively, when the two beams are very close, the channel across two beams becomes correlated due to the wide beam aperture.  
 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/plot2D_multibeam_SNR_with_perbeam_phase_and_power.pdf}
%     \caption{Sensitivity analysis (simulation):  SNR gain (dB) of 2-beam w.r.t. single-beam for varying 2nd beam's phase $\hat{\sigma}$ and amplitude $\hat{\delta}$ in multi-beam. We show for -3 dB weaker multi-path channel, the multi-beam's highest SNR gain is 1.76 dB which is not very sensitive even for high phase error of $\pm75^o$. However, if the phase error is highest ($180^o$), the SNR drops significantly. }
%     \label{fig:sensitivity}
% \end{figure}

% \todo{R1: A practical issue with the proposed approach is that creating very precise and directional multi-beam patterns without significant side lobes requires better antennas (more elements and higher resolution phase shifters) than antennas targeting a single lobe; the more constraints you put on the beam pattern, the harder it gets to also obtain a high gain given the hardware constraints. It would be interesting to discuss this tradeoff.}

% \todo{R5: The 6-bit phase resolution used in their phased array gives high-quality beams. How does it work in lower bit phase resolution? For example, the 60 GHz gNBs only have 2-bit resolution.}

% \todo{ R4: Also, in practice, phase shifters provide discrete phase control with limited resolution. Yet, this work uses arbitrarily phase control for constructive combining. }

% \textcolor{purple}{
% We demonstrate a high-throughput and reliable mmWave link with our state-of-the-art 64 element phased arrays which provides 6 bit of phase control and 27 dB of gain control per antenna element. The high resolution phase and gain control helps in creating phase-coherent multi-beams. Such an advanced arrays are getting deployed by vendors for 28 GHz base station. For instance, Verizon in collaboration with Samsung is deploying 64 element array (8 such arrays for MIMO)\cite{samsung_array} and IBM developed 128 element dual-polarized arrays to be used for COSMOS testbed\cite{raychaudhuri2020challenge}. That said, some phased arrays (e.g. 60 GHz routers based on IEEE 802.11ad) \cite{talonad7200} have low-resolution phase shifters which limits the ability to create multi-beam. Despite low resolution, such system would also benefit from our novel tracking algorithm to establish a reliable link. }





% \noindent
% \textbf{Sensitivity analysis:} We show that although accurate estimation of phase and amplitude provides the highest SNR, it is not very sensitive to estimation errors in these parameters. To quantify the sensitivity, we simulate a two-path channel and set the relative phase and attenuation to $-40^o$ and $-3$ dB, respectively. We vary the relative phase and amplitude of the 2nd beam in a 2-beam pattern (w.r.t. the first beam) and show the 2D plot of SNR gain in Fig. \ref{fig:sensitivity}. The highest SNR gain is 1.76 dB for perfect estimation, which reduces gradually with an increasing mismatch between the beam and channel parameters. We show that multi-beam SNR exceeds the single-beam SNR as long as the estimated phase is within $\pm 75^o$ and for reasonably high amplitude errors of -20 dB. Thus, the sensitivity to phase and amplitude estimation is low.

% The SNR gain of multi-beam w.r.t. single-beam relies on accurate estimation of the per-beam phase and amplitude. We show that the SNR gain has low sensitivity to the estimation error in phase and amplitude. We 
% The SNR gain is a maximum of 1.76 dB when the 2nd beam phase and amplitude match with the channel phase and attenuation. The SNR gain drops 
% . Moreover, the multi-beam outperforms the single-beam system even with a high amplitude estimation error of -20 dB.


% new
% \noindent
% \textbf{Reliability-first principle:} 
% At this point, one may wonder that when the multi-path is weak, the multi-beam pattern allocates less power along the reflected-path beam to maximize throughput, which may harm the reliability when the reflected path signal has power below an outage threshold. We solve this challenge by redistributing per-beam amplitudes to satisfy a minimum power constraint \newtodo{put number what threshold we used} along the reflected beam for a fixed total radiated power. Such optimization will ensure high reliability but at a sub-optimal throughput gain. Our insight follows from sensitivity analysis in Fig. ~\ref{fig:sensitivity}, which shows that even when we do sub-optimal power allocation per beam, e.g., distributing equal power to two beams, the throughput-gain reduces from 1.76 dB to 1.64 dB, which is still better compared to the single-beam case. \textit{Moreover, when the LOS path is not available for a long duration (e.g., persistent static blockage), having two beams at two reflectors with comparable attenuation is significantly better than a single beam at one reflector from both throughput and reliability points of view. }


% Recall that multi-beam pattern is obtained as weighted combination of the constituent single-beam patterns. We showed that the weights of the second beam is $\delta e^{-j\sigma}$ relative to the first beam achieves the optimal throughput performance. 


% We estimate the attenuation $\delta$ and AOD, AOA during the initial beam training phase as detailed in the overview section.\\ We next describe our process of obtaining $\sigma$ for constructive combining.

%  In the previous section, we provided the optimal choice of weights $c_1$ and $c_2$, but we didn't explain how to estimate them. In particular, the Tx needs to estimate the phase shift $\sigma$ which controls the relative phase between two beams, i.e., $\sigma = \angle c_2-\angle c_1$ = $\angle c_2$ (assume $\angle c_1=0$).
 
 
%  We define the cophasing factor $\sigma$ as the relative phase between those two beams i.e., $\sigma=\angle c_2-\angle c_1$, where $c_1$ and $c_2$ are defined in (\ref{eq:beampattern}). For simplicity, we consider $\angle c_1=0$ and $\angle c_2=\sigma$. 
 
 
%  For a wideband system (such as 5G NR), we write the effective channel $H_{\text{eff}}$ at subcarrier frequency $f_j$ as
%  \begin{equation}\label{eq:Heff}
%      H_{\text{eff}}(f_j,\sigma) = H_1(f_j) +  \delta e^{j\sigma} H_2(f_j),
%  \end{equation}
%  where $H_1(f_j)$ and $H_2(f_j)$ represents channel state information (CSI) for direct path and reflected path respectively at subcarrier frequency $f_j$.
 
% Note that we inherently cannot estimate $\sigma$ that works well for all the subcarriers simultaneously. We formulate an optimization to estimate $\sigma$ such that we maximize the average received signal strength over all frequencies:
% \begin{equation}\label{eq:snroverall}
%     \hat{\sigma} = \arg\max_{\sigma}\sum_{f_j} \norm{ H_1(f_j) + \delta e^{j\sigma} H_2(f_j)}^2.
% \end{equation}
% A naive approach to get estimate $\hat{\sigma}$ is to exhaustively scan all possible $\sigma\in [0,2\pi]$ that optimizes (\ref{eq:snroverall}), however, at the cost of long training delays. 

% Our insight is that we can tune it using only two probes as follows. We measure $ H_{\text{eff}}(f_j)$ by setting two distinct values of $\sigma$ and solve a set of two linear equations in (\ref{eq:Heff}) to estimate $H_1(f_j)$ and $H_2(f_j)$ for each subcarriers $f_j$. From these estimates, we can recover the signal strength for all possible values of phase shift $\sigma$ and extract the optimal $\sigma$ that maximizes the overall signal strength (See Figure~\ref{fig:cophasing}). The time complexity of our constructive combining algorithm. is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array. Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically estimate it along with our novel tracking algorithm as discussed in the following Section. 

% \textcolor{blue}{
% \textbf{Complexity of multi-beam system:} There are two ways to implement multi-beam on hardware. First codebook based system need to store all possible multi-beams with different attenuation and phase-per-beam. Such codebook based system require extremely high storage (xxx size codebook for just 2 beam patterns) and also suffer from table-lookup latency. We propose an alternative solution that requires a small codebook of the same size of single-beam patterns. We use a small FPGA-board (Artix-7) generate multi-beam antenna weights by combining two single-beam weights. The FPGA only need to perform $2N$ complex multiplications/additions for $N$ antennas which we do with with a latency of xxx ns.}

% We highlight three significance of our fast constructive combining algorithm.
% \begin{enumerate}
%     \item Note that the optimal $\sigma$ will change over time as the user moves. We propose to periodically tune the fast co-phasing algorithm during \textcolor{red}{beam refinement phases} along with our novel tracking algorithm. 
%     \item The co-phasing needs to be tuned at only one of the transceivers (typically the access point) while the other transceiver keeps a fixed co-phasing factor all the time.
%     \item The time complexity of our co-phasing algorithm is proportional to the number of beams in multi-beam (typically 2 or 3) independent of the size of the phased array.
% \end{enumerate}



 
 
 
%  \begin{equation}\label{eq:beampattern}
%     \textbf{w} = \sum_{k=1}^K c_k\textbf{w}_{\phi_k},
%  \end{equation}
%  where $\textbf{w}_{\phi_k} = [1 \  e^{j2\pi\frac{ d}{\lambda}\sin(\phi_k)} \  \ldots \ e^{j2\pi(N-1)\frac{d}{\lambda}\sin(\phi_k)} ]^T$ is the beamforming weight of a single-beam pattern directed along $\phi_k$ (for $k=1,\ldots,K$ beams); where $d$ is antenna spacing, $\lambda$ is the carrier wavelength, $N$ is number of transmit or receive antennas. 
 
%  The complex weights $c_k$ are chosen to control the power along each beam in multi-beam and satisfy the power constraint.
 
%  We show the effectiveness of our multi-beam patterns in  Figure~\ref{fig:multilobebeampattern}. We also measure beampatterns through our mmWave phased array (Section~\ref{sec:implementation}) in an anechoic chamber closely resembles the ones generated in theory using (\ref{eq:beampattern}).
 
%  Figure~\ref{fig:multilobebeampattern} that multi-beam patterns 
 
%  \noindent
%  \textbf{Cophasing Optimization:}
%  We highlight an issue with multi-beam communication that the signal along multiple paths may arrive with opposite phases causing destructive interference at the receiver. Fortunately, it is possible to avoid this happening by deliberately tuning the relative phase (co-phase) among multiple beams in the multi-beam pattern. 
 
%  Without loss of generality, we assume a communication link is established with two beams. 

==> Arxiv/3_design_multibeam_v4.tex <==
% Ish: I don't know who created this version but I am modifying it

\section{Design of Multi-beam system}\label{sec:creatingmultibeam}
% The multi-beam patterns have high antenna gain in single or multiple main lobes that orient towards the reflectors or the LOS path.  We show that an effective way of generating multi-beam patterns is to take the weighted sum of beamforming weights of individual beams in the multi-beam. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/mmReliableOverview1_v2.pdf}
%     \caption{Shows an overview of building blocks of \name that leverages SSB and CSI-RS in 5G NR to establish a multi-beam link.}
%     \label{fig:overview1_v2}
%     \vspace{-10pt}
% \end{figure}
In this section, we present \name's algorithm for creating a reliable and high-throughput multi-beam link. First, we establish a mathematical framework to model the reliability and throughput gains in a multi-beam system. Then, we show that multi-beam patterns are channel-dependent and require an estimate of angle, phase, and attenuation of each channel path. We propose a two step procedure to estimate these parameters as shown in Fig.~\ref{fig:5GNR_mmReliable_ovreview}. We leverage any standard beam training procedure in 5G NR to estimate the angle of each multipath~\cite{ghasempour2018multi,jog2019many}. We then design a procedure to estimate the per-path phase and attenuation with low overhead using reference signals. Finally, we explain our novel analog beamforming to establish a multi-beam link using these parameters. 


\subsection{Multi-beam links are more reliable}
To compare various techniques on equal footing, we formally define link reliability as the fraction of time when the link is available for communication within a large observation interval. Link outage (due to natural effects), or procedures like beam-training reduce the reliability as they temporarily render the link unavailable for communication. Therefore, we can express reliability as:
\begin{equation}
    \text{Reliability} = 1-\text{Prob}(\text{Outage})
\end{equation}
We empirically compute the probability of outage as the fraction of duration where the SNR is below a minimum threshold. The directional nature of single-beam mmWave links make them susceptible to link outages since blockage \& user mobility effects can reduce SNR by up to 30 dB~\cite{maccartney2017rapid}. Multi-beams prevent these outages by avoiding a single point of failure.

Multi-beam links are reliable even under the impact of blockage events. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which represents the fraction of time the link is in outage with respect to the observation interval. For simplicity, we assume the beams in our multi-beam are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike its single-beam counterparts~\cite{sur2016beamspy,maccartney2017rapid}. \textcolor{orange}{In practice, blockages may be correlated and scenarios could arise where two or more paths are blocked simultaneously. While no solution can prevent link outage if all paths are blocked (e.g. user inadvertently blocks all antennas with their body), multi-beam links can be sustained as long as there is at least one unblocked path to the receiver. Simultaneous blockage of multiple paths is always less probable than blockage of a single path, therefore, multi-beam links are \textit{always} more reliable than single-beam links.}

% \textcolor{orange}{In practice, blockages may be correlated, e.g., scenarios such as two or more paths blocked simultaneously or blockage of one path followed by the blockage of other paths. Multi-beam is reliable even in such scenarios as long as there exists at least one unblocked path to the receiver. Note that similar to single-beam based schemes~\cite{sur2016beamspy}, multi-beam cannot prevent simultaneous blockage of all paths (e.g. user holding their phone, bocking the antennas). In general, multi-beam links are probabilistically better reliable than single beam links.} 
%  Note that multi-beam prevents occasional blockage of one or more constituent beams, but it cannot avoid
% In practice, even with correlated blockages, the occurrence of complete outage of multi-beam (all beams blocked in multi-beam) is less probable than that of single beam. Therefore, multi-beam links are probabilistically better reliable than single beam links. 

% But, unlike single-beam approach, multi-beam provides higher SNR due to constructive combining even when the paths are attenuated due to blockage.


\begin{figure*}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/channel_single_multipath.pdf}
    \includegraphics[width=0.46\textwidth]{figures/reliability_snr.pdf}
    % \caption{For a single-path channel in (a), the optimal analog beamforming is to use a single beam pattern with all the energy direct along that channel path. }
    \caption{Multi-beam communication enhances the throughput \& reliability of mmWave link through constructive combining. (a) System with a single-path channel, (b) With multi-path (2-path) channel. (c) The optimal beamforming technique for single-path channel is single beam with all the energy directed along that channel path. (d) Phase coherent multi-beam with two lobes provides higher SNR and higher reliability compared to single beam.}
    \label{fig:reliability_snr}
\end{figure*}
\noindent
\subsection{Multi-beam Throughput Model}
We next elaborate on Section~\ref{sec:intro} and show that multi-beam with optimal constructive combining and power-control can provide higher throughput than a single-beam link.
We introduce a model for a multi-antenna base station transmitting to the user device using a mmWave link and derive the optimal beamforming solution that maximizes the received SNR for a given wireless channel. We make two important observations. First, we show that single-beam is optimal only when the wireless channel consists of a single path from the transmitter to the receiver. A single-beam system is sub-optimal for a multi-path channel, which is generally the case even for mmWave links. We then show that a multi-beam with two beams is optimal for a two-path channel and maximizes the received SNR. We conclude with a note on generalizing our formulation to arbitrary number of beams in multi-beam.

\noindent
\textbf{Primer on optimal beamforming:}
We derive an expression for optimal beamforming weights at a multi-antenna base-station (gNB phased array) communicating with a single antenna receiver using mmWave (Multi-antenna receiver discussed in Section~\ref{sec:multibeamUE}). The gNB beamforms using a uniform linear phased array with $N$ antenna elements. Beamforming is implemented by applying a $N\times 1$ beam weights vector $\wbf$ at each antenna using a combination of phase shifters and attenuators (~Fig. \ref{fig:reliability_snr}(a)). Our goal is to determine the optimal $\wbf$ that maximises the receive SNR. 

Let $s$ be the transmit signal from the gNB, the received signal $y$ is expressed as:
\begin{equation}
    y = \hbf^T \wbf s + \eta,
\end{equation}
where $\hbf$ is  $N\times 1$ channel from $N$ transmit antennas to one receive antenna and $\eta$ is white Gaussian noise at the receiver. The capacity or maximum throughput of a wireless link is evaluated in term of SNR (the ratio of signal power to noise power) as: 
\begin{equation}\label{eq:snr}
    \text{SNR} = {||\hbf^T \wbf ||^2 P_s}/{P_\eta},
\end{equation}
 where $P_s$ is the average transmit power (without transmit array gain) and $P_\eta$ is the noise power\footnote{We can mathematically derive the expression for SNR using $E[yy^H] = E[(\hbf^H \wbf s + n)(\hbf^H \wbf s + n)^H]] = \|\hbf^H \wbf\|^2 E[ss^H] + E[nn^H]$ and we denote $P_s = E[ss^H]$ and $P_\eta =E[nn^H]$}. Our goal is to estimate beamforming weights $\wbf$, that maximizes the SNR. Using Cauchy-Schwartz inequality, it follows that $||\hbf^T \wbf ||$ is maximized when $\hbf^{*}$ (complex conjugate of $\hbf$) and $\wbf$ align in vector space. Therefore, \textit{the optimal weight vector is channel-dependent}. Additionally, the weights need to be unitary to keep the power constant, i.e., $\|\wbf\|=1$. This way, we get the optimal weights ${\wbf}^{\text{opt}}$ as:
\begin{equation}\label{eq:wmrc}
    {\wbf}^{\text{opt}} = {\hbf^*}/{||\hbf||},
\end{equation}
The optimal beamforming provides the highest SNR of $\frac{||\hbf||^2P_s}{P_\eta}$. The practical wireless channel consists of multiple paths (direct or reflected paths), where each path is characterized by its angle of departure and attenuation. Since the optimal beamforming vector depends on the channel $\hbf$, it is affected by the nature of these paths.  

\noindent
\textbf{Single-beam is optimal for a single-path channel:}
A natural question is why the conventional mmWave create a single directional link? It turns out that single beam is optimal when the wireless channel consists of only one path from transmitter to receiver. To verify it, we represent the single-path channel vector by $\hbf^{\text{single}}$ and derive the optimal beamforming weights for such channel. Note that a single-path channel can be entirely characterized by two parameters: the direction of departure $\phi_1$ and complex attenuation $h$ as follows:
\begin{equation}\label{eq:1pathchannel}
    \hbf^{\text{single}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} 
\end{equation}
where $n$ is the antenna index, $d$ is the antenna spacing, and $\lambda$ is the wavelength ($d=\frac{\lambda}{2}$ in our phased array). We now calculate the optimal beamforming weights (\ref{eq:wmrc}) for single path channel (\ref{eq:1pathchannel}) and show the natural solution is in fact a single beam. We obtain single-beam weights $\wbf_{\phi_1}$ as:  
% The optimal beam pattern for this single-path channel in (\ref{eq:1pathchannel}) is actually a single-beam pattern shown in Fig. \ref{fig:reliability_snr}(c).
% The expression for single-beam beamformer $\wbf_{\phi_1}$ to create a directional pattern along angle $\phi_1$ is:
\begin{equation}\label{eq:wphi1}
\begin{split}
     \wbf_{\phi_1}=\frac{ \hbf^{\text{single}^*}}{\| \hbf^{\text{single}}\|} =\frac{1}{\sqrt{N}}[1, e^{j2\pi \frac{d}{\lambda}\sin(\phi_1)},\ldots,  e^{j2\pi(N-1) \frac{d}{\lambda}\sin(\phi_1)}]^T
\end{split}
\end{equation}
Note that $\wbf_{\phi_1}$ is optimal (i.e., $\wbf_{\phi_1}= {\wbf}^{\text{opt}}$) and is widely used in conventional single-beam system~\cite{sur2016beamspy}. However, such single-beam pattern become sub-optimal for typical mmWave channel which consist of multiple paths from the gNB to the UE.
% In practice, the wireless channel could consist of multiple paths from the gNB to the UE, and the single-beam ceases to be optimal in these scenarios.

\noindent
\textbf{Multi-beam is optimal for multi-path channel:}
\label{sec:mbeam_th_der}
We now show how single-beam is sub-optimal and multi-beam is a natural solution for a multi-path channel. For simplicity, we consider the multi-path channel consists of two major paths as shown in Fig. \ref{fig:reliability_snr}(b). We use the same notation $h$ for the complex attenuation of the first path and represent the second path attenuation relative to that of the first path. In particular, the second path has a relative attenuation of $\delta \in \R$ and a phase shift of $\sigma \in [0,2\pi]$ relative to the first path, thus providing the attenuation of $h \delta e^{j\sigma}$. We can write the expression of two-path channel $\hbf^{\text{multi}}$ as:
% For simplicity, we consider a two path channel as shown in Fig. \ref{fig:reliability_snr}(b) with path magnitude $h$ and $h \delta e^{j\sigma}$ respectively and angles of departures $\phi_1$ and $\phi_2$ respectively. Here, $\delta \in \R$ is relative attenuation and $\sigma \in [0,2\pi]$ is relative phase of second channel path w.r.t. the first channel path. Two-path channel vector $\hbf^{\text{multi}}$ at antenna $n$ is:
\begin{equation}\label{eq:hmultieq}
    \hbf^{\text{multi}}[n] = h e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_1)} + h \delta e^{j\sigma} e^{-j2\pi \frac{d}{\lambda} (n-1) \sin(\phi_2)}
\end{equation}
where $\phi_1$ and $\phi_2$ are the respective directions of departure of the two paths respectively. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/multi_two_path_system.pdf}
%     \caption{When there are multiple reflectors in the environment as in (a), the single-beam system in (b) is no longer optimal because it does not utilize the multi-path nature of the underlying channel and thus suffers from low SNR. A phase coherent multi-beam pattern with two lobes in (b) or three lobes in (c) provides better SNR compared to the single beam system through transmit diversity. The optimal (or oracle) solution for three path channel is a multi-beam pattern with three lobes.} 
%     \label{fig:multi_two_path_system}
% \end{figure}
In this case, if we apply the same single-beam weights (\ref{eq:wphi1}), it provides sub-optimal gain since the power along $\phi_2$ is severely attenuated and not coherently adding up at the receiver (Fig. \ref{fig:reliability_snr}(c)).
% it amplifies the first path and significantly attenuates the signal along the second path. 
For this single-beam case, we get an approximate SNR:
%  highlight the intuition that if you use the same beamforming vector $w$ from the LoS channel, then the power going towards angle $\alpha_2$ is not coherently adding up at the receiver.
\begin{equation}
    \text{SNR}^{\text{single}} = {|h|^2P_s}/{P_\eta}.
\end{equation}

In contrast, multi-beamforming weights are obtained by optimizing the SNR for the given channel. From (\ref{eq:wmrc}), we obtain multi-beam weight as $\textbf{w}^{\text{multi}} = {\hbf^{\text{multi}^*}}/{\|\hbf^{\text{multi}}\|}$ which is visualized in Fig. \ref{fig:reliability_snr}(d). The SNR of multi-beam is obtained as $\text{SNR}^{\text{multi}}=\|h^{\text{multi}}\|^2 P_s/P_\eta$ from (\ref{eq:snr}) which we simplify and approximate to the following expression:
\begin{equation}
    \text{SNR}^{\text{multi}} \approx {(1+\delta^2)|h|^2P_s}/{P_\eta}.
\end{equation}
The multi-beam SNR is higher than that of a single-beam system by a factor of $1+\delta^2$. The multi-beam is the optimal beamforming solution for multi-path channels and works by spliting the transmit signal constructively along both the paths in a manner that they maximally combine at the receiver. We discuss in Appendix~\ref{appendix:A} how this result can be generalized to show that a k-multi-beam is the optimal solution for a k-path channel.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.24\textwidth]{figures/reflector_relative_power_cdf.pdf}
%     \caption{Relative attenuation of reflected paths compared to the direct path at multiple locations in indoor environment.}
%     \label{fig:reflector_relative_power_cdf}
% \end{figure}

% \begin{figure*} [!t]
%     \subfigure{{\includegraphics[width=0.30\columnwidth]{figures/expt_setup_mmreliable.pdf}\label{fig:expt_setup_mmreliable}}}
%     \subfigure{{\includegraphics[width=0.56\columnwidth]{figures/cdf_all_data_refl_atten.pdf}\label{fig:reflector_relative_power_cdf}}}
%     \subfigure{{\includegraphics[width=0.56\columnwidth]{figures/mobility_vis_example_noblock-crop-crop.pdf}\label{fig:reflector_movt_example_noblock}}}
%     \subfigure{{\includegraphics[width=0.59\columnwidth]{figures/mobility_vis_example_block-crop-crop.pdf}\label{fig:reflector_movt_example_block}}}
%     \vspace{-4mm}
%     \caption{(a) Experiment test scenario (b) CDF of the relative attenuation of the strongest reflected path compared to the direct path at over various locations. (c) A heatmap of strong paths in the environment while the UE moves w.r.t gNB, strong reflectors appear at different points in time. (d) The experiment in (c) in a scenario where the direct path is blocked by a static object between 6 and 12 seconds.}
%     % \vspace{-2mm}
%     \label{fig:reflector_characterize}
% \end{figure*}

\begin{figure} [!t]
    \subfigure{{\includegraphics[width=0.48\columnwidth]{figures/cdf_all_data_refl_atten.pdf}\label{fig:reflector_relative_power_cdf}}}
    \subfigure{{\includegraphics[width=0.48\columnwidth]{figures/mobility_vis_example_noblock-crop-crop.pdf}\label{fig:reflector_movt_example_noblock}}}
    % \vspace{-2mm}
    \caption{(a) CDF of the relative attenuation of the strongest reflected path compared to the direct path at over various locations. (b) A heatmap of strong paths in the environment while the UE moves w.r.t gNB, strong reflectors appear at different points in time.}
    % \vspace{-2mm}
    \label{fig:reflector_characterize}
\end{figure}
 
\noindent
\textbf{How strong are multi-path for mmWave?} At this point, one may ask if mmWave channel does really consist of multiple paths? There are numerous measurement studies for both 28 GHz and 60 Ghz mmWave channel which indicate the presence of strong multipath channel~\cite{Rappaport2013Millimeter,zhu2014demystifying, telecom2019analysis,nitsche2014ieee,xu2002spatial}. These studies show that in a typical deployment, reflectors like metals, concrete walls, and tinted glass strongly reflect signals while attenuating them by about 5-6 dB ($\delta\approx0.5$). We also performed a measurement study of reflector strengths at 50 different indoor locations. As shown in Figure \ref{fig:reflector_relative_power_cdf}, common indoor reflectors cause 1-10 dB attenuation with a median attenuation of 7.2 dB indoors and 5 dB outdoors relative to the direct path signal strength. Figure \ref{fig:reflector_movt_example_noblock} shows an example of signal strengths in lab environment. It shows that reflectors as strong as the direct path do exist and can be utilized to establish a multi-beam link. 

\subsection{Creating multi-beam patterns with normalized total radiated power}\label{subsec:creating_mb}

In this section, we devise a method to create a multi-beam pattern by combining beamforming weights of respective single-beam patterns. While we consider a two-lobe beam in this section, the technique extends to any general multi-beam. We assume that the two strongest paths in the channel are known from the default beam-training method. Once these paths are known, we need to create a multi-lobe beam pattern that constructively adds up at the receiver. From Eq.~\ref{eq:wmrc} and Eq.~\ref{eq:hmultieq}, it follows that the multi-beam weights are in fact a linear sum of the constituent single-beam weights corresponding to $\phi_1,\phi_2$. If the relative attenuation $\delta$ and the relative phase $\sigma$ between the constituent beams are known, we can create the optimal multi-beam by simple addition.

Concretely, the beamforming weights $\textbf{w}$ for a two-lobe multi-beam is:
\begin{equation}\label{eq:beampattern}
    \textbf{w}(\phi_1,\phi_2,\delta,\sigma) = \frac{(\textbf{w}_{\phi_1}+{\delta} e^{-j{\sigma}}\textbf{w}_{\phi_2})}{\|(\textbf{w}_{\phi_1}+{\delta} e^{-j{\sigma}}\textbf{w}_{\phi_2})\|},
 \end{equation}
% where the normalizing factor (NF) is chosen to restrict the TRP to unity as follow
% \begin{equation*}\label{eq:nf}
% \begin{split}
%         \text{NF} &= ||\textbf{w}_{\phi_1} + \hat{\delta} e^{-j\hat{\sigma}}  \textbf{w}_{\phi_2}||^2\\ 
%         &= ||\textbf{w}_{\phi_1}||^2 + \hat{\delta}^2 ||\textbf{w}_{\phi_2}||^2 + 
%         \hat{\delta} e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2} + 
%         \hat{\delta} e^{j\hat{\sigma}}\textbf{w}_{\phi_2}^H\textbf{w}_{\phi_1}\\
%         &=1+\hat{\delta}^2 +\hat{\delta} \text{ Real}(e^{-j\hat{\sigma}}\textbf{w}_{\phi_1}^H \textbf{w}_{\phi_2})
%         %&\approx 1+\hat{\delta}^2
% \end{split}
% \end{equation*}

The denominator ensures that the TRP is conserved by enforcing $\|\textbf{w}\|=1$ . We then appropriately quantize the beamforming vector phases \& amplitudes to be compatible with our phased array. In~\cite{aykin2019multi}, a sub-optimal multi-beam is created by splitting the array into sub-arrays, each responsible for a particular component beam. In contrast, \name utilizes amplitude control to create the optimal channel dependent multi-beam.


% We show the sensitivity of beamforming to phase and amplitude errors in \todo{Appendix~\ref{appendix:S}}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/derivation_multibeam.pdf}
    \caption{Channel probing procedure to obtain parameters ($\delta, \sigma$) for multi-beam constructive combining that's robust to CFO/SFO impairments.}
    \label{fig:derivation_multibeam}
\end{figure}
\subsection{Obtaining parameters for multi-beam constructive combining}
\label{sec:constructive_combining}
In this subsection, we present our algorithm that reliably estimates the parameters required to establish a \constructivemultibeam. First, we show how our solution works for a two-beam multi-beam in a narrow-band channel, and then extend it to the general case of $K$-multi-beam and wideband channels. In the two-beam case, we need to estimate $\delta$ (relative attenuation, $\delta \in \R$) and $\sigma$ (relative phase shift, $0<\sigma\le 2\pi$) of the reflected path w.r.t. the direct path. From the beam-training phase, we already know the directions $\phi_1,\phi_2$ of the two paths. We denote the narrow-band complex wireless channel along each individual path as $\hbf_1$ and $\hbf_2$ respectively.

If the gNB measures both $\hbf_1$ and $\hbf_2$, then it can estimate the relative amplitude and phase shift using their ratio. A simple way to do this would be to measure each individual beam's channel one after another by setting one beam at a time, as suggested in~\cite{aykin2019multi}. However, due to hardware offsets such as Carrier Frequency Offset (CFO) and Sampling Frequency Offset (SFO), these estimates would be unreliable\todo{~\cite{}}. CFO and SFO lead to time varying channel phase and introduces large errors in the estimation of $\sigma$, and makes \constructivemultibeam difficult. Only one aspect of the wireless channel remains fixed despite these offsets: its magnitude. Therefore, we develop an estimation method using channel magnitude alone.

First, we observe that only the relative channel between the two beams is of interest to us, which means that we can treat $\hbf_1$ as a reference and assume $\hbf_1$ is real, i.e., $\hbf_1\in \mathbb{R}^+$ without loss of generality.
Then, we observe that the magnitudes $\pbf_1=|\hbf_1|^2$ and $\pbf_2=|\hbf_2|^2$ are already available from the initial beam-training phase. Now, the estimation can be done with just two extra channel probes. The gNB uses two RS to probe two 2-beam patterns: first it sets the beam $w(\phi_1,\phi_2,1,0)$, and then $w(\phi_1,\phi_2,1,\frac{\pi}{2})$. For each of the two probes, it estimates the channel magnitudes $\pbf_3$ and $\pbf_4$ as:
\begin{equation}\label{eq:two_probe_cc}
    \begin{split}
        \pbf_3 &= |\hbf_1 + e^{j0} \hbf_2|^2 = |\hbf_1  + \hbf_2|^2 = |\hbf_1|^2+|\hbf_2|^2+2\hbf_1\operatorname{Re}(\hbf_2)\\
        \pbf_4 &= |\hbf_1  + e^{j\frac{\pi}{2}} \hbf_2|^2 = |\hbf_1  + j\hbf_2|^2 = |\hbf_1|^2+|\hbf_2|^2-2\hbf_1\operatorname{Im}(\hbf_2)
    \end{split}
\end{equation}
% \begin{equation}\label{eq:two_probe_cc}
%     \begin{split}
%         H_1(f_i) &= h_1(f_i) + e^{j0} h_2(f_i) = h_1(f_i) + h_2(f_i)\\
%         H_2(f_i) &= h_1(f_i) + e^{j\pi} h_2(f_i) = h_1(f_i) - h_2(f_i)
%     \end{split}
% \end{equation}
where $j=\sqrt{-1}$ and $\hbf_1\in \mathbb{R}^+$ as discussed before. Using (\ref{eq:two_probe_cc}), we estimate $\hbf_1$ and $\hbf_2$ individually, and express their ratio using the following matrix linear equation:
% \begin{equation}\label{eq:two_probe_result}
%     \begin{split}
%     \frac{h_2}{h_1} &= \frac{\begin{bmatrix}
%      1 & j
%     \end{bmatrix}}{2\sqrt{p_1}}\begin{bmatrix}
%     -1 & -1 & 1 & 0\\ 
%      1 &  1 & 0 & -1
%     \end{bmatrix}\begin{bmatrix}
%     p_1\\ 
%     p_2\\ 
%     p_3\\ 
%     p_4
%     \end{bmatrix}
%     \end{split}
% \end{equation}

\begin{equation}\label{eq:two_probe_result}
    \begin{split}
    \frac{\hbf_2}{\hbf_1} &= \hat{\delta} e^{j\hat{\sigma}} =\frac{1}{2\sqrt{\pbf_1}}\begin{bmatrix}
    -1 & -1 & 1 & 0\\ 
     j &  j & 0 & -j
    \end{bmatrix}\begin{bmatrix}
    \pbf_1\\ 
    \pbf_2\\ 
    \pbf_3\\ 
    \pbf_4
    \end{bmatrix}
    \end{split}
\end{equation}
Where $\{\hat{\delta},\hat{\sigma}\}$ are the estimates of the relative amplitude and phase respectively between the two multi-beam paths. Thus, our algorithm estimates the required parameters using only two consecutive RS probes for the two-beam case. The algorithm can be generalized to any $K$ multi-beam by performing additional probes and augmenting the matrix in (\ref{eq:two_probe_result}) to yield $K-1$ relative channels w.r.t $\hbf_1$. In~\cite{palacios2018adaptive}, the authors develop a similar technique, albeit for measuring per-element channel in a phased array. The channel probing overhead in~\cite{palacios2018adaptive} is proportional to the number of antennas $N$ ($\approx5N$). In contrast, our solution to measure the per-beam channel requires $3(K-1)+1$ probes for $K$ beams (including the $K$ estimates from beam-training phase) and is independent of the number of antenna elements in the phased array; making it tractable for large arrays.

\textbf{Handling wideband channels}: Typically, the Channel State Information (CSI) is measured across multiple frequency subcarriers over a wide bandwith. For the 5G NR system, the CSI is readily available from the RS. Even for 802.11ad commercial routers, the CSI can be extracted in the firmware~\cite{qualcomm2017wil6210, wang2020demystifying, palacios2018adaptive}. The prior analysis can easily be extended to multiple subcarriers by simply treating each subcarrier's channel independently. We denote $\hbf_1(f)$ and $\hbf_2(f)$ as the wideband CSI across frequency index $f$. We first estimate $\hbf_1(f), \hbf_2(f)$ using Eq.(\ref{eq:two_probe_result}). Then, we formulate an optimization problem that maximizes the average received signal strength over all frequencies to jointly estimate $\{\hat{\delta},\hat{\sigma}\}$ as:
% The relative phase $\sigma$ is approximately constant across frequency subcarriers because of high frequency of mmWave compared to bandwidth (Shown in Appendix \ref{appendix:A}). So we take an average over all of the frequency subcarriers to get a robust estimate. 
% Note that we inherently cannot estimate $\hat{\sigma}$ that works well for all the subcarriers simultaneously. 
% Our constructive combining approach maximizes the average received signal strength over all frequencies as:
\begin{equation}\label{eq:snroverall}
   \{\hat{\delta}, \hat{\sigma}\} = \argmax_{\delta,\sigma}\;\; \norm{ \hbf_1(f)  + \delta e^{-j\sigma} \hbf_2(f)}^2.
\end{equation}
% \begin{equation}\label{eq:snroverall}
%   \{\hat{\delta}, \hat{\sigma}\} = \arg\max_{\delta,\sigma}\sum_{f_i} \norm{ \hbf_1  + \delta e^{-j\sigma} \hbf_2}^2.
% \end{equation}

We solve the above to obtain a closed form solution ($\langle\cdot,\cdot\rangle$ is the inner product over the frequency dimension):
\begin{equation}
    \hat{\delta}e^{j \hat{\sigma}} = -\langle\hbf_1(f),\hbf_2(f)\rangle/\,\norm{\hbf_2(f)}^2
\end{equation}
which reduces, as expected, to $\hat{\delta}e^{j \hat{\sigma}} = -\hbf_1/\hbf_2 $ for a narrowband channel (e.g. in IEEE 802.11ad 60 GHz standard \cite{ieee80211ad}). The optimal phase, amplitude, \& angle will change over time as the user moves. We periodically estimate these parameters using our tracking algorithm discussed in the next section. 

% \todo{R3: The solution requires full channel state information, which may not be practical.
% ToDo: Explain Full CSI is available in both 5G NR and 802.11ad}

  
 

\review{In Section 3.2, the authors describe a two-probe based approach to estimate the two-beam channels. However, Equation (6) seems to suggest one should apply different phases to different directions h1 and h2: the first probe applies the same phase to both directions whereas the second probe applies different phases to the two directions. Then this requires our knowledge of h1 and h2. Isn't it a chicken-and-egg problem? Unless we know h1 and h2, how can we apply different phases to different directions?
}
\newtodo{The reviewer addressed a misunderstanding on mmReliable algorithm in Eq (6). We will clarify this misunderstanding by improving the writing of Section 3.2.
}

% highlightshep

==> Arxiv/3_multibeam_reliability.tex <==
\section{How Multi-beam helps with throughput and reliability?} \label{subsec:multi-beam-reliability}

We provide a simple mathematical model to analyze the throughput and reliability performance of the multi-beam link and contrast it with that of a single-beam link. We first discuss a scenario without any blockage and later analyse the impact of blockages on link reliability and throughput. 

\subsection{Multi-beam vs Single-beam}
% We utilize a geometric channel model which models the channel individually for each path between Tx and Rx~\cite{alkhateeb2014channel,sayeed2007maximizing}. 

% \newtodo{provide context before describing single beam...}
Here, we evaluate the throughput and reliability of single-beam and multi-beam systems, assuming complete knowledge of the wireless channel.
We consider a single-RF chain architecture with an analog phased array. The phased array generates a directional beam pattern (single-beam), which is directed towards the receiver, as shown in Figure~\ref{fig:motivation}(a). We assume the single-beam pattern provides an EIRP of $P_t$. The transmitter transmits a signal $x$ using a single RF chain. The signal experiences a channel attenuation of $h$ along the direct LOS path. For mathematical simplicity, we ignore other paths assuming the high directionality of a single-beam. The received signal would be $hx$ added with the receiver noise. For now, we consider an omnidirectional receiver with the antenna gain of unity and later extend to the directional receiver case. This single-beam link can provide a maximum throughput of \cite{tse2005fundamentals}
% A single beam link essentially observes a single path channel $h$ due to high directionality (Figure~\ref{fig:motivation}(a)) which results in a maximum throughput \cite{tse2005fundamentals} of
\begin{equation}
   C_{sb} = \log_2(1+|h|^2P_t/N_r) \text{ bits/s/Hz } \quad\textbf{(single-beam)} 
\end{equation}
 where $N_r$ is the receiver noise power. 
% $P_t=\mathbb{E}[x]^2$ is average transmit power

Next, we consider a multi-beam link and assume there are two paths (direct path and reflected path) that reach the receiver, as shown in Figure~\ref{fig:motivation}(b). We assume that initial beam training has been performed and the two-beams in the multi-beam pattern are perfectly aligned along the two paths. The reflected path suffers large attenuation due to higher path-loss and reflection loss; however, it provides an alternate independent path to the receiver. We model the reflected channel as $h\delta e^{j\varsigma}$, where  $\delta$ ($\delta<1$) is the attenuation factor and $\varsigma$ is a path-dependent phase shift. 


% and without loss of generality assume, there are only two lobes at both Tx and Rx that are aligned perfectly with each other. In this case, there is an additional reflected path with channel $h_r$, which suffers higher attenuation compared to the direct path channel $h$ due to higher path-loss and reflection loss; however, it provides an alternate independent path to the receiver. 

To understand how multi-beam can be helpful for throughput, we first need to know how multi-beam patterns are created. We show that two-lobe beam patterns can be generated as a weighted sum of two equivalent single-lobe patterns, which are oriented towards the direct and reflected path, respectively. 
% Our key insight is to treat multi-beam links similar to a MIMO system with two transmit and one receive antenna, which can deliver high throughput due to transmit diversity~\cite{tse2005fundamentals}. We ask if we can utilize such insight to improve the throughput of a multi-beam link using only an analog phased array without using more than one complex Radio-chains (as in a MIMO system).
The weights, however, if not set properly, may lead to the two signals adding up in the opposite phase and reduce the throughput.
% Our choice of multi-beam weights is inspired 
\begin{figure} [!t]
%   \subfigure[]{\includegraphics[width=0.32\textwidth]{figures/reflectortype.pdf}
%   \label{fig:reftype}}
       \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/multibeamToyRel.pdf}
       \label{fig:toyrel}}
    \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/multibeamToyThput.pdf}
    \label{fig:toythput}}
    \vspace{-4mm}
    \caption{(a) Reliability achieved with blockage probability for \name with 2-beam or 3-beam pattern (b) Throughput gain for \name with a 2-beam pattern w.r.t. single beam for different reflecting surfaces, while all beam patterns meeting the TRP constraint. }
    % \vspace{-2mm}
    \label{fig:toyexample}
 \end{figure}



%%-----------------------
\todo{R1: The multi-beam capacity analysis in 3.1 is incorrect, specifically Eqn. 3. The authors do not consider the antenna gain, which is important since the gain of lobes of multi-beam patterns is lower than that of single beam patterns! You cannot simply assume that the same energy is now radiated via two lobes. Intuitively, radiating energy in more directions spreads it and delivers less to each single direction. 
}

% Our choice of multi-beam weights is inspired by the concept of transmit beamforming in a MIMO system \cite{tse2005fundamentals}. 
Our key insight is to optimize the weights such that the two signal combines constructively at the receiver.
We choose the weights such that the two-beams in multi-beam provides a transmit antenna gain proportional to $1$ and $\delta e^{-j\varsigma}$. We normalize the weights to constrain the multi-beam power the same as that of a single-beam. We will derive a formal expression of normalization factor in Section~\ref{sec:creatingmultibeam}, which turns out to be $\frac{1}{\sqrt{1+\delta^2}}$ when the beams in multi-beam are \textit{orthogonal}. 
The choice of weights ensures that the received signal combine constructively at the receiver and maximize the SNR. Similar to the single-beam case, we assume the receiver is omnidirectional, and the receive antenna gain is unity. The received signal in multi-beam case is
\begin{equation}
    y=\big(\frac{1}{\sqrt{1+\delta^2}} h+ \frac{\delta e^{j\varsigma}}{\sqrt{1+\delta^2}}h \delta e^{-j\varsigma}\big)x + n = (h\sqrt{1+\delta^2})x + n
\end{equation}
 which results in the following throughput \cite{tse2005fundamentals}

\begin{equation}\label{eq:multibeam}
    C_{mb}=\log_2\left(1+(1+\delta^2)|h|^2\frac{P_t}{N_r}\right)\; \textbf{(multi-beam)}
\end{equation}


We surprisingly note that the multi-beam throughput is higher compared to that of a single-beam system by a factor of $1+\delta^2$ (which is $2\times$ or 3 dB gain when $\delta=1$). On a quick glance, the results may seem counter-intuitive since we split power across beams in multi-beam, which results in low EIRP. Despite lower individual EIRP per-beam, multi-beam achieves higher throughput for the same TRP because of the constructive combining of two signals. Intuitively, a multi-beam link enjoys a diversity gain similar to a MIMO system with multiple transmit antennas and one receive antenna. MIMO pre-codes the transmit signal across multiple antennas such that they combine constructively at the receiver. In a multi-beam case, the individual beams are analogous to multiple antennas in a MIMO transmitter. If the phased array can \textit{pre-code} individual beams in a multi-beam, we can get them to combine constructively at the receiver. 
We discuss our novel analog beamforming method to create such \textit{pre-coded} multi-beam patterns and optimizing them for constructive combining in Section \ref{sec:creatingmultibeam}.
% However, the throughput gain comes with the additional complexity of estimating channel parameters $\delta$ and $\varsigma$ for each path from a combined channel response. We learn $\delta$ by leveraging initial beam training process (Section \ref{sec:buildingblock}) and design novel constructive combining optimization to tune phase-per-beam $\varsigma$ in real time (Section \ref{sec:creatingmultibeam}).


We now show that multi-beam patterns belongs to the class of channel-dependent beam patterns that are optimal for a given multi-path channel, maximizing the SNR at the receiver. 
\begin{theorem}
Multi-beam patterns are equivalent to optimal channel-dependent patterns when the number of beams in multi-beam is the same as the number of channel paths.
\end{theorem}
\begin{proof}
We provide the proof in Appendix \ref{appendix:A}
\end{proof}



From (\ref{eq:multibeam}), we see that the throughput gain of a multi-beam system is dependent on the factor $\delta^2$, which is the relative attenuation of the reflected path with respect to the direct path. We performed a study of attenuation caused by common reflecting surfaces and verified that 28 GHz attenuation is less severe compared to a 60 GHz link \cite{telecom2019analysis}. Shown in Table \ref{tab:reftype}, a metal reflector causes only 3 dB attenuation (including path loss and reflection loss) while other surfaces may create up to 16 dB attenuation. Measurement study for outdoor links \cite{zhu2014demystifying} also shows that reflected paths from buildings and vehicles are strong with only 5-7 dB attenuation.
Note that in certain scenarios when the reflections are weak, multi-beams does not compromise on throughput in normal condition (without blockage) while significantly improving the throughput when one of the paths is blocked (Figure\ref{fig:toyexample}(b)) as we discuss in the following subsection. 

% \todo{R3: DONE: The system may not work efficiently when a user only has an extremely strong LOS path.
% ToDo: Explain that in such cases the power control will ensure that our multi-beam falls back to single beam.
% }

% \textcolor{purple}{
% We argue that \name would work as long as there is at least one path available and by design it switches back to the traditional singal-beam system and radiate all the energy in that path. Thus, multi-beam is always better compared to single beam and falls back to single beam when the channel consists of only a single strong path.}



% Later in section \ref{sec:creatingmultibeam}, we show a novel method to estimate multi-beam parameters $\delta$ and $\varsigma$ from channel measurements and create orthogonal multi-beam patterns.
% The analysis suggests that a multi-beam link provides higher throughput compared to a single-beam link. The throughput, however, is affected by the attenuation of the reflected path.  We next study the attenuation caused by various reflectors in the environment.


 
%  \noindent
% \textbf{Effect of Reflective Surfaces:}
% We perform a simple test to find out attenuation by common indoor objects at 28 GHz. The attenuation can be due to higher path loss of the reflected path and reflection loss due to material properties.  We establish a communication link with Tx and Rx placed 6m apart and introduce various reflectors at 30$^o$ from the LOS link. The attenuation results are shown in Figure~\ref{fig:reftype}. As expected, metal reflectors provide the strongest signal, with only 3 dB of attenuation. Other natural reflectors such as monitor screen or wooden wall suffer from higher reflection loss of 12 dB and 16 dB, respectively. 
\begin{table}[!t]
    \centering
    \begin{tabular}{ccccc}\toprule
       \textbf{Objects} & Metal & Monitor & Wood&Wall\\ \midrule% \specialrule{1pt}{1pt}{1pt}
        Attenuation (dB) & -3 & -12 & -15 & -16\\
        \bottomrule
    \end{tabular}
    \vspace{.5cm}
    \caption{Signal attenuation by common materials (path loss plus reflection loss) with respect to the direct path signal.}
    \label{tab:reftype}
    \vspace{-1cm}
\end{table}
% \begin{figure} [!t]
%     \subfigure[]{\includegraphics[width=0.49\columnwidth]{figures/multibeamToyRel.pdf}\label{fig:toyrel}}
%     \subfigure[]{\includegraphics[width=0.49\columnwidth]{figures/multibeamToyThput.pdf}\label{fig:toythput}}
%     \vspace{-4mm}
%     \caption{Reliability and Throughput Gain comparison of multi-beam with single-beam.}
%     % \vspace{-2mm}
%     \label{fig:toyexample}
%  \end{figure}
 
 
 \noindent
\subsection{Impact of Blockage on Link Reliability}
We next introduce blockage to our model. Consider a blockage probability $\beta \;(0\le\beta\le1)$, which intuitively represents the fraction of time over a period when the link suffered an outage. For simplicity, we assume the beams in our multi-beam set up are blocked independently. Thus, the probability that $k$ beams simultaneously experience an outage is $\beta^k$. By definition, the reliability would be $1-\beta$ for the single-beam case and $1-\beta^k, k\ge2$ for the multi-beam case. Multi-beam provides higher reliability because it prevents the link to suffer an outage due to blockage, unlike single-beam counterparts \cite{sur2016beamspy,maccartney2017rapid} as shown in Figure~\ref{fig:toyrel}. Our mathematical result shows that the multi-beam achieves close to 100\% reliability for typical blockage probabilities ($<20\%$). 

We next calculate the average throughput gain in the case of blockages. For \textbf{single beam} case, the link is sustained only for $1-\beta$ fraction of time so that the average throughput would be 
\begin{equation}
    C_{sb}^{\text{avg}}=(1-\beta)*\log_2(1+|h|^2P_t/N_r).
\end{equation}
In contrast, for the case of \textbf{multi-beam with 2-lobes}, the average throughput would be obtained by considering whether both beams or only one of the two beams are available:
\begin{equation}
\begin{split}
        &C_{mb}^{\text{avg}} = (1-\beta)^2\log_2\left(1+(1+\delta^2)|h|^2\frac{P_t}{N_r}\right)\\ &+\beta(1-\beta)\log_2(1+|h|^2\frac{P_t}{N_r})+\beta(1-\beta)\log_2(1+\delta^2|h|^2\frac{P_t}{N_r})
\end{split}
\end{equation}
We plot the throughput gain of multi-beam against that of the single beam in Figure \ref{fig:toythput}. It shows that multi-beam can achieve up to 1.2$\times$ higher throughput for 20\% blockage instances. So far the analysis assumes an omnidirectional pattern at the user. Our analysis also holds true when the user has a directional pattern. In that case, we propose to use a multi-beam pattern at the user. Interestingly, the user does not need to perform any optimization as only the gNB's phase optimization suffices for constructive combining. 

\todo{R2: DONE: There are some strong assumptions. For example, the fact that the  the probability of blocking each beam is independent. However, in real life this is not the case. Blockages of each path can be highly correlated.}

We note that the simplistic example presented above assumes the blockages are independent. In practice, single or multiple blockers might block multiple links at the same time. \name adapts to blockages by tracking its impact on each beam and controlling the power radiated along each blocked or unblocked link. We discuss our blockage detection and power adaptation in Section \ref{sec:design}.
 A simultaneous blockage of all the paths is also not rare for mmWave (e.g., self-blockage by user's hand or body), and it equally affects both the single-beam and multi-beam systems. In such scenarios, the mmWave system may initiate efficient handovers~\cite{wei2017pose, palacios2019leap} which is out-of-scope of this work. 

% The results indicated that the average throughput with multi-beam are higher than that obtained for the single-beam case. The plots in Figure~\ref{fig:toythput} indicates that multi-beam can theoretically provide $1.8\times$ higher avg. throughput for metallic reflector (3 dB loss) which only reduces to $1.1\times$ for wooden surfaces (16 dB loss). The results indicates that a static link can achieve high throughput and high reliability through multi-beam communication. However, to avail these gains for a practical system, the transmit phased array should establish a multi-beam pattern that ensures constructive combining at the receiver.





==> Arxiv/4_design_proactive.tex <==
% !TEX root = main.tex

\section{\name Proactive Response}\label{sec:design}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/mmReliableOverview.pdf}
    \caption{Overview of \name's proactive response to blockage and mobility. It observes the per-beam amplitude from periodic DMRS channel estimates and classifies whether the user has gone into blockage or mobility. It also classifies mobility into translation or rotation motion and acts differently in each case. Finally, the cycle is concluded by constructive combining optimization and refining of multi-beam patterns at both the gNB and the UE. The cycle is repeated until the link is no longer recoverable by proactive response alone.}
    \label{fig:design_overview2} 
\end{figure}
We present the overall working of \name with the help of a flow-chart in Figure~\ref{fig:design_overview2}. At a high level, \name has two major phases: the \textbf{Beam Training Phase} (BTP) and the \textbf{Data Transmission Phase} (DTP). During the BTP, \name leverages standard beam scan and constructive combining optimization to establish an initial multi-beam link as we discussed in Section \ref{sec:design}. During the DTP, \name proactively maintains the multi-beam link under the impending blockage and mobility events while the communication link is active. It continuously monitors the channel estimates provided by DMRS (demodulation reference signal) in 5G NR to identify blockage or mobility on a per-beam basis. It tracks the user mobility in the background and refines the multi-beam periodically. The DTP ends when the beam is no longer recoverable by tracking alone (due to accumulated errors in tracking over time) and signals the next BTP.


% So far we discussed how \name establishes a multi-beam link. We now describe how we proactively maintain it under the impeding blockage and mobility events.  

% We present the overall working of \name with the help of a flow-chart in Figure~\ref{fig:design_overview2}. At a high level, \name has two major phases: the \textbf{Beam Training Phase} (BTP) and the \textbf{Data Transmission Phase} (DTP). During the BTP, \name leverages the standard exhaustive beam search to estimate some initial parameters such as AoA, AoD, and ToF of each channel path, which is required to establish a multi-beam link. The DTP establishes and periodically refines a multi-beam link through constructive combining optimization. It achieves constructive combining of multi-path signal through two novel contributions: 
% (i) It provides an efficient algorithm and procedure to estimate per-path channel parameters ($\delta$ and $\sigma$) required for constructive combining.
% (ii) It develops a novel analog beamforming method to create phase-coherent multi-beams. 

% The DTP ends when the beam is no longer recoverable by tracking alone (due to accumulated errors in tracking over time) and signals the next BTP. The cycle of BTP and DTP repeats periodically. \newtodo{Does it need to be periodic? or can it be triggered only when needed?}


% In this section, we detail how \name proactively identifies impending blockage and mobility events and responds to them while the communication link is active. An overview is shown in Figure~\ref{fig:design_overview2}. By continuously monitoring the per-beam amplitude (in multi-beam) for changes over time, \name first declares an event as a blockage or mobility. In the case of mobility, it further classifies the user motion into translation or rotation. It recovers the per-beam amplitude at high resolution from the Channel Impulse Response (CIR), obtained from DMRS (Demodulation Reference Signal) channel estimates in 5G NR. We can use this information to refine the beam differently in response to each event.

% Under blockage, \name proactively reduces the power on the beam that is blocked and shifts that power to the other beams. Under mobility, \name performs user tracking by measuring the rotation per beam. In order to measure rotation per beam, \name builds a novel algorithm which uses the change in amplitude over time, reported per beam in the multi-beam pattern to estimate the \textit{angular deviation} suffered by each beam. The estimate of angular deviation is used to refine the beam pattern and realign it with the mobile user. 
% In this section, we provide how \name operates during the transmission phase by establishing and refining the multi-beam link. 

 \subsection{Proactive Blockage Mitigation}
% Now that we have solved for the individual beam tracking, we can estimate the per-path amplitude $\alpha_k$ 
%In previous section, we have seen that \name relies on accurate power measurements of each individual beams to track the user and mitigate the effect of blockage. A simple solution to get per-beam power measurement corresponding to the ToF of individual path. However, the resolution in ToF is low (2.5 ns resolution for 400MHz bandwidth). The CIR is ideally represented as a series of shifted delta functions (shifted by ToF), however, in practice the measured CIR is sinc interpolated version. The side lobe of sinc interpolation of individual peaks may overlap with each other. This overlap may be treated as interference for the power measurement of individual beams. Thus, it may happen that when one path suffers significant blockage, it may not be detected because of the interference of the sinc interpolation of a nearby stronger peak corresponding to unblocked path. 
% \name utilizes per-beam power over time to detect if any of the paths underwent blockage or user motion. In order to detect blockage, \name analyzes the rate of change of amplitude per beam. If the rate of change is more than $10$ dB in a duration of 10 number of symbols, \name declares blockage. We have empirically tested the algorithm and achieve $98$ \% accuracy. The response of \name is proactive because of the nature of multi-beam link which ensures that the communication link is maintained while one path undergoes blockage. As soon as blockage is detected on a particular beam, \name would repurpose the power to other unblocked beams.
% Said differently, the transceiver reduces the number of lobes whenever blockage is detected along some paths. It is less likely that all the paths are blocked simultaneously, nonetheless, in case of complete outage, the radio can initiate beam training to search for other reflected paths or perform efficient handover~\cite{wei2017pose}. To avoid frequent beam training, our beam refinement stage keeps track of all the unblocked paths to keep the beams aligned towards the other transceiver, as explained in the following sub-section. 
Mobile blockers interact with the multi-beam system by suddenly occluding one or more active beams. \name analyzes the rate of change of amplitude per beam to detect such events. Empirical evaluation shows that typical blockage events cause per-beam amplitude to degrade by 10 dB in just 10 OFDM symbols. Once a blockage event is detected, \name responds by re-purposing the power on the blocked beam to other unblocked ones. Since there are always multiple beams active, there is no significant impact on link reliability, even if one is blocked.
Said differently, the transceiver reduces the number of beams whenever blockage is detected along some paths. It is rare that all paths are blocked simultaneously; nonetheless, in case of a complete outage, the radio can initiate a new phase of beam training to search for other alternate paths or perform an efficient handover~\cite{wei2017pose}. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/mmReliableOverview1.pdf}
    \caption{Design Overview: The beam training phase estimates the parameters (AoA, AoD, ToF) required for multi-beam. The data transmission phase establishes and refines the multi-beam providing a proactive response to blockages and user's mobility. }
    % Design Overview: Beam training phase begins with trying different beams and estimates the relative locations of reflectors in the environment, establishing the link. During the data transmission phase, CIR is monitored for every packet transmitted to detect the occurrence of blockage or mobility to trigger blockage mitigation or mobility management.
    \label{fig:design_overview} 
\end{figure}




 \begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/trans_rot_crop.pdf}
    %FPGAblockDiag_crop
    \caption{Two cases of user motion: Rotation or Translation for a single beam. Rotation causes misalignment only at the user, while the translation causes misalignment at both the gNB and user.}
    \label{fig:motion}
\end{figure}

\subsection{Proactive User-Mobility Management }

Notes:
what is the problem,
Tracking the user motion per-beam. Prior work assume omni-user. Doesn't work because SNR could be low.

why is it hard, 
User also uses directional beam leading to complex motion with translation and rotation. 

Why different response to translation and rotation?
Translation causes both gNB and UE beam change and rotation causes only gNB beam change

(i) distinguish motion and classify into two
(ii) Estmate the angle of movement in each case.

what is a simple solution and why it won't work, 


what is your amazing solution...


If per-beam amplitude changes appreciably, but not quickly, then \name classifies them as caused due to underlying user motion. User motion is difficult to deal with since it is difficult to predict how the user moves without relying on external sensors.

% \vspace{3pt}
\subsubsection{Classification of user motion (translation vs rotation):}
Our insight here is to decouple complex user motion into one of translation or rotation motion for the small duration of tracking. Since \name's tracking works for every OFDM channel estimate, which is as fast as one in every 33$\mu$s for a 5G NR system. Therefore, practical user motion can be piece-wise decomposed into translation and rotation, significantly simplifying system design. 

First, we proactively detect user mobility and classify it into translation and rotation by leveraging per-beam power estimates. For instance, rotation causes the individual beams in a multi-beam to deviate (from the optimal direction) by the same angle at the user. In contrast, if the user undergoes translation, the individual beams on the receiver undergo different angular deviations for each beam. Said differently, the amplitude change for each beam would be different over time as the angular deviation is different for each beam.

% Our first key insight is to decouple complex user motion into one of translation or rotation motion for a small duration. Since \name's tracking works for every OFDM symbol estimate which is as fast as one in every 33$\mu$s for a 5G NR system; any practical user motion can be piece wise classified into translation and rotation. This significantly simplifies the system design. 

% The consequence of user translation and rotation differs in the amount of angular deviation caused by them. For instance, the rotation of the user device around its axis would mis-align the beam just at the user, and the gNB beam does not suffer from any misalignment. On the other hand, the translation of the user would cause beam misalignment at both the gNB and the user, as shown in Figure~\ref{fig:motion}. Therefore, \name designs different models for translation and rotation to estimate the angular deviation caused by beam misalignment's in both cases. 

% The second insight is to proactively detect user mobility and classify it into translation and rotation case. \name leverages the multi-beam setup and per-beam power estimates for this classification. For instance, rotation causes the individual beams in multi-beam to rotate by the same angle at the user. In contrast, if the user undergoes translation, then, the individual beam on the receiver undergoes different angular deviation for each beam (See Figure~\ref{fig:translation}). Said differently, the amplitude change for each beam would be different over time as the angular deviation is different for each beam. We use the above observation to classify the user motion into rotation and translation. 


% Our first key insight is to decouple the user mobility into translation and rotation for the 
% sake of simplifying the understanding and how \name detects those and proactively reacts to those. 
% Say for example, if user/receiver only rotates around it's axis, the \name individual beams rotate 
% by the same amount of rotation for all the multiple beams as shown in Figure~\ref{fig:motion}. 
% If the rotation is similar which means that per beam amplitude change would be quite similar over time. 
% In contrast, if the user undergoes translation, then, \name individual beam on the receiver undergoes 
% different rotation change for each beam. Said differently, the amplitude change for each beam would be 
% different over time as the angular deviation is different for each beam. We use the above observation to 
% classify the user motion into rotation and translation. 

% Even after classification to the two different kind of user motion, a natural question is how do we proactively align
% the different beams of the multi-beam to the user direction. In order to learn track the user, we need to learn 
% angular deviation per beam under both the motions. We for the first time build a model to take the change in 
% amplitude and compute the angular deviation. Furthermore, this model differs under the assumption of rotation 
% or translation. Therefore, we would build independently models for user rotation and user translation to take the change in amplitude over time to predict the angular deviation. 

% Traditionally, with a single main-lobe pattern, the blockage of the main path will cause significant degradation of link quality. In such cases, the pre-selected beam patterns may not be suitable to serve the user due to beam misalignments at high user mobility. Through multi-lobe patterns, we adopt an approach to detect per-lobe blockage by analyzing the drop in signal strength below a threshold.


% \subsubsection{Proactive User Mobility Mitigation}
% \subsection{Finding Angular deviation under Rotation and Translation}
% IEEE802.11ad defines a beam refinement protocol where the gNB scans a set of beam patterns in the codebook. The beam refinement process is not as tedious as the beam training process. 

% \begin{figure}
%     \centering
%     \includegraphics{figures/rot.png}
%     \caption{Caption}
%     \label{fig:rot}
% \end{figure}

%  \begin{figure}
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/rot}\label{fig:rot}}
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{figures/trans}\label{fig:trans}}
%     \caption{Two cases of user motion: (a) Rotation and (b) Translation}
%     \label{fig:motion}
%  \end{figure}

\vspace{3pt}
\noindent

\subsubsection{Tracking user translation: }
In contrast to the rotation case, translation causes misalignment at both the gNB and the user. Interestingly, we notice that the angular deviation, $\varphi_k(t)$, is the same at both the gNB and the user (See  Figure \ref{fig:motion}(b)). The received power $P_k(t)$ for translation case can be written as
\begin{equation}
     P_k(t) = G_T(\phi_k+\varphi_k(t))+G_R(\theta_k+\varphi_k(t))+P_T-P_h \; (\text{in dB}).
\end{equation}

Since the transmit and receive beam patterns are known, the relative power decay can be obtained as:
\begin{equation}\label{eq:translation_tracking}
    \begin{array}{l}
     P_k(t_0) -P_k(0)= G_T\left(\phi_k+\varphi(t_0)\right) - G_T\left(\phi_k\right) + \\  
     \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;
     G_R\left(\theta_k+\varphi(t_0)\right) - G_R\left(\theta_k\right) \; (\text{in dB})
    \end{array}
\end{equation}

Similar to the case in rotation, we have two possible solutions of $\varphi_k(t)$, which can be resolved similarly to the rotation case.  

%This is a one-time overhead to estimate the direction of translation and scales with the number of beams oriented toward strong paths (usually 2 or 3 ~\cite{anderson2004building,rappaport2012broadband,rappaport201238,sur201560,narayanan2019first,alkhateeb2014channel,sayeed2007maximizing}) and not with the number of antennas.
\todo{R5: In Eq(14), how does the RX know the TX's beam pattern G\_T for it to calculate the received power? It seems to imply coordination between TX and RX to do 2K beam-scans together but how it's done is not detailed. If explicit feedback is involved, the extra overhead needs to be accounted. Also, the RX's transmitting beam needs to be adjusted as well. 
ToDo Discuss the feedback overhead.}
We note from Eq (\ref{eq:translation_tracking}) that the receiver needs to know the transmit beam pattern for beam tracking. Fortunately, the beam patterns can be shared with low overhead through the 5G NR control channel. The overhead is low because a multi-beam pattern is generated through a weighted combination of single beam patterns, which are stored in the codebook. The transceiver can share their codebook once, and then they only need to share the codebook index and relative weights of multi-beam pattern in real-time.

\textbf{Estimating initial multi-beam parameters:}
The beam training phase's primary purpose is to scan multiple beams and observe the highest SNR beam pattern. \name leverages this exhaustive scanning process not only to select the highest SNR beam but plots the SNR of each beam with the beam direction and finds all the local maxima and estimates their corresponding directions. The AoA and AoD can be obtained during the transmit scan and received beam scan, respectively. A key challenge, however, is to associate the AoA with the AoD of corresponding reflectors. The mapping of AoA and AoD is non-trivial because of the unknown orientation of transceivers and reflecting surfaces.
We leverage the ToF to solve the association problem. Each reflected path has a unique ToF. When the beam is aligned with some reflector, the strongest signal comes from the reflected path corresponding to that reflector. We take the corresponding path-dependent CIR and estimate the ToF by looking at the highest power index for each path. We performed an $8\times$ upsampling and cosine interpolation of CIR to get the ToF estimates with high precision. We identify the LOS path as the path with the lowest ToF. This way, \name estimates the AoA, AoD, and ToF of each path and associate them with each other. After the initial training, \name creates a multi-lobe beam pattern with constructive combining to establish the directional beam.

 
\subsubsection{Tracking user rotation: }
% % We observe that the UE rotation affects the beam pattern at the UE, but the pattern remains the same at the gNB side, as shown in Figure \ref{fig:motion}. Therefore, the goal is to estimate the rotation of the user and correct for it. 
% Consider a multi-beam pattern with $K$ beams at the user (receiver) as well as at the gNB (transmitter). The beams are initially aligned towards LOS or strong reflectors at the beginning of the user motion. As the user moves, \name uses the CIR to report per-beam power $P_k(t)$ for each OFDM packet received over time $t$, where $k=1,\ldots,K$ is the beam index in multi-beam pattern. $P_k(t)$ can be modeled as:
% % We model the received power $P_k$, corresponding to the $k$th beam ($k=1,\ldots,K$) as
% \begin{equation} \label{eq:pkdb}
%     P_k(0) = G_R(\theta_k) + G_T(\phi_k) + P_T - P_h\quad \text{(in dB)},
% \end{equation}
% where $G_R(\theta_k)$ and $G_T(\phi_k)$ are the received and transmit antenna gains along the AoA $\theta_k$ and AoD\footnote{Note that AoA and AoD have been estimated during initial beam training as detailed in Section~\ref{sec:buildingblock}.} $\phi_k$  respectively, $P_T$ is the transmit power, and $P_h$ is the loss due to wireless channel. The channel loss $P_h$ can be due to path loss or reflection loss, which needs to be eliminated from \eqref{eq:pkdb} to track the user's motion. Fortunately, the channel can be assumed to be static for a small duration of user rotation. Also, recall that all the beams in the user's multi-beam pattern undergo the same angle of rotation, say $\varphi(t)$ over time $t$. Thus, the received power varies over time as follows:
% % We observe that the rotation of UE affects the main lobe as well as side lobes by the same angular deviation, say $\varphi$. The variation in received signal strength at the UE over timefor the $k$th path is written as:
% \begin{equation}
%     P_k(t) = G_T(\phi_k)+G_R(\theta_k+\varphi(t))+ P_T - P_h\; (\text{in dB}).
% \end{equation}
% % where $G_T(\phi_k)$ is the antenna gain along AoD $\phi_k$, $G_R(\theta_k+\varphi(t))$ is antenna gain along direction sum of AoA $\theta_k$ and user rotation angle $\varphi(t)$ at time $t$.
Consider a multi-beam pattern with $K$ beams at the user (receiver) as well as at the gNB (transmitter). The beams are initially aligned towards LOS or strong reflectors at the beginning of the user motion. As the user rotates, the beam at the user gets misaligned due to rotation, but since the user does not translate, the beams at the gNB will remain aligned with the user (Figure\ref{fig:motion}(a)). We, therefore, estimate the angle of rotation and proactively refine the beams at the user.

 \name uses the CIR to report per-beam power $P_k(t)$ for each OFDM packet received over time $t$, where $k=1,\ldots,K$ is the individual beam index in multi-beam pattern. $P_k(t)$ can be modeled as (A detailed model is presented in Appendix~\ref{appendix:B}):
\begin{equation}
    P_k(t) = G_T(\phi_k)+G_R(\theta_k+\varphi(t))+ P_T - P_h\; (\text{in dB}),
\end{equation}
where $G_T(\phi_k)$ and $G_R(\theta_k)$ are the received and transmit antenna gains along the Angle of Departure (AoD) $\phi_k$ and Angle of Arrival (AoA)
% \footnote{Note that AoD and AoA have been estimated during initial beam training as detailed in Section~\ref{sec:buildingblock}.}  
$\theta_k+\varphi(t)$ respectively. Recall that all the individual beams in the user's multi-beam pattern deviate by the same angle when the user rotates, and is captured by $\varphi(t)$ ($\varphi(0) = 0$) in the AoA. $P_T$ is the transmit power, and $P_h$ is the loss due to wireless channel. The channel loss $P_h$ can be due to path loss or reflection loss, and can be assumed to be static for a small duration of user rotation. 
 To eliminate the unknown channel loss, we calculate the relative decay in power, from $t=0$ to $t=t_0$ as
\begin{equation}
     P_k(t_0) -P_k(0)= G_R\left(\theta_k+\varphi(t_0)\right) - G_R\left(\theta_k\right) \; (\text{in dB}).
\end{equation}
We see that the relative power decay depends only on the user's antenna pattern $G_R(.)$. Intuitively, the beam pattern is usually symmetric, and two possible values $\varphi(t_0)$ and $-\varphi(t_0)$ could have caused the observed change in $G_R$. To deal with the ambiguity of the direction of rotation, \name tries one of the two possibilities using CSI-RS probing in the hope that it improves the SNR. If it doesn't improve SNR, possibly the other angle is correct, and thus, \name refines the beam to that angle.
The refinement adds an overhead of only one additional probe in addition to $2(K-1)$ probes required for constructive combining for the K-beam case. \name periodically estimates the value of the per-beam angle, phase, and amplitude and updates the beam pattern at the UE to realign towards the gNB. 

% We will show later in Equation \eqref{eq:pk} that $G_R(\theta)$ is a quadratic function of $\theta$.

% Note that $P_k(t) -P_k(0)$ is a deterministic function of receive antenna gain and can be utilized to estimate $\varphi(t)$ by inverting the beampattern. We will show later in \eqref{eq:pk} that $G_R(\cdot),G_T(\cdot)$ are quadratic functions. 
% This property of $G_R(\cdot)$ plays an important role in user tracking, by making the problem mathematically tractable. This also limits the solution set to enable a proactive solution search.

% We note that the beam pattern is generally not invertible, but there are only two possible solution $\varphi$ and $-\varphi$ due to the symmetry of beam patterns, as $G_k(\cdot)$ is a quadratic function \eqref{eq:pk}.  So, we try both possibilities through beam refinement phase as mentioned in \ref{sec:motivation} and choose the value of $\varphi$, which gives better signal strength. Thus, the time complexity of beam refinement is only two beam patterns. We estimate the value of $\varphi$ and update the beam pattern at the UE to always align towards the gNB. 



% We will show next how can we further reduce this time complexity.

% \subsection{User Tracking}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/trans_crop.pdf}
%     %FPGAblockDiag_crop
%     \caption{Tracking the user through triangulation.}
%     \label{fig:translation}
% \end{figure}

% % \vspace{3pt}

% \noindent\textbf{User tracking: }
% So far, we have shown that beam refinement could be done to track each beam. However, not all the reflected paths provide a robust signal for accurate tracking in practice and can be very noisy. For robust tracking, we observe that there are only two parameters to be estimated to resolve for the user location, namely the x and y coordinate of user location. Thus, only two strong paths are enough to resolve the user location. 

% We estimate the angle deviation of the user by using only two beams and triangulate the user location, as shown in Figure~\ref{fig:translation}.  The angular deviation corresponding to a reflected path can be measured as a deviation from a \textit{virtual gNB} (image of the gNB via a reflector) location.  Thus, motion tracking requires the knowledge of the exact location of the virtual gNBs. The location of the virtual gNBs depends on the reflector location and orientation. Fortunately, the reflector parameters do not change during the transmission phase. We will discuss in Section~\ref{sec:buildingblock} how \name estimates those reflector parameters during the initial training phase. Note that user tracking works even when the LOS path is blocked as long as there are two unblocked reflected paths.
% The beam refinement phase, in this case, requires scanning of only four beam patterns, two for each path. Thus, the maximum time complexity of \name is just four beams (30.8 $\mu$sec).

% We consider the virtual gNB in Figure~\ref{fig:translation} as the image of \textit{actual} gNB via the reflector. 






% In the similar way as the rotation case, we take the derivative of the received signal strength to predict $\varphi$. 

% \begin{equation}
%     \frac{dP_k(t)}{dt} = \frac{dG_T(\phi_k+\varphi(t))}{d\varphi}\frac{d\varphi(t)}{dt} + \frac{dG_R(\theta_k+\varphi(t))}{d\varphi}\frac{d\varphi(t)}{dt}
% \end{equation}

% \vspace{3pt}
% \noindent\textbf{Complex motion: }
 
%   Recall that \name can distinguish translation and rotation by observing per-beam power. However, the user may undergo simultaneous translation and rotation motion. Fortunately, we can still classify the complex motion into one of the translations or rotation case (which has a higher probability). The error due to this misclassification is at most 1 dB, which is insignificant. Further note that the probability of complex motion is quite low in practice. 

 
 
 
 
 
 
 
 
 
 
 
% During the short period of time between two beam training stages, we assume the user can have either rotation or translation but the probability of both rotation and translation simultaneously is very low and such analysis is out of scope of this paper (or say future work). How do the gNB know whether it is a case of translation or rotation? To resolve this issue, we leverage the beam refinement protocol mentioned in IEEE 802.11ad. 
% We estimate the angle $\varphi_r$ by first assuming rotation and then estimate $\varphi_t$ by assuming translation. Finally, we try the two choice of beams and choose one of them which gives better signal strength.

% We observe that rotation always causes the same angle movement of all multipath; however, the translation mostly causes different angle movement. Thus, we can distinguish between translation and rotation case separately and apply separate algorithms to estimate the angle.


\subsection{Superresolution: Improving Per-Beam Tracking} \label{sec:establish-multi-beam}
Due to the bandlimited nature of practical systems, we do not have an infinite resolution to tease apart individual beams in a multi-beam at the receiver. Therefore, we present a sinc interpolation approach to recover per-beam amplitude from combined multi-beam channel response and show its importance for user tracking. When receiving a multi-beam transmission, it can be shown that the signal at the receiver consists of a superposition of a delayed and attenuated version of each individual transmit beam. If we consider the delay and attenuation experienced by beam-index $k$ as $\delta_k$ and $\alpha_k$ respectively, then the effective multi-beam channel can be expressed as:

\begin{equation}
\begin{split}
        h_{\text{eff}}& = \sum_k \alpha_k\delta(t-\tau_k),
        \label{eqn:heff}
\end{split}
\end{equation}

Where $\alpha_k$ is a function of the transmitter and receiver beam pattern, while $\delta_k$ relates to the Time of Flight (ToF) of each multi-beam channel path. Recall that our goal is to estimate the individual $\alpha_k$ for each beam ($k=1,\ldots, K$). 


\begin{figure} [!t]
    \subfigure[]{\includegraphics[width=0.49\columnwidth]{figures/superresMSE.pdf}\label{fig:suptimeseries}}
    \subfigure[]{\includegraphics[width=0.49\columnwidth]{figures/sincInterp.pdf}\label{fig:supmse}}
    \vspace{-4mm}
    \caption{Efficiency of superresolution algorithm: (a) Simulation: Superresolution provides low MSE of per-beam power estimate even when the relative ToF is less than system resolution of 2.5 ns. (b) Hardware measurement: shows two sincs can be recovered from measured combined CIR. }
    % \vspace{-2mm}
    \label{fig:superresexample}
 \end{figure}

For a frequency-selective wideband system the received signal is sampled at sampling rate and sinc interpolated due to limited bandwidth as follows:
\begin{equation}
\begin{split}
    h_{\text{eff}}[n] &= \sum_k \alpha_k \text{sinc}\left(B(nT_s-\tau_k)\right)\\
\end{split}
\end{equation}
where $B$ is the bandwidth of the waveform, $T_s$ is the sampling rate of the receiver, and $\alpha_k$ is total signal attenuation along path $k$.  

We can re-write the above formulation as an optimization problem where our objective is to find $\alpha_k$ such that it fits the channel best. Let say the collected CIR is represented by column vector $\mathbf{h}$.
We solve the following optimization to extract $\alpha = [ \alpha_1 \alpha_2  \ldots \alpha_K]^T$, which amplitude
per beam.
\begin{equation}\label{eq:optim}
    \alpha_{est} = \arg\min_\alpha \|\mathbf{h}-\textbf{S}\alpha\|^2+\lambda\|\alpha\|^2  
\end{equation}
where the matrix $\textbf{S}$ consists of all the ToF. We are essentially solving a super-resolution problem by fitting a sinc model over the entire CIR response. The optimization is a convex
formulation, with L2 norm regularization. We use standard techniques~\cite{cvx} to solve this problem in $100\mu$s. Here, we make a key observation that, after training, the absolute ToF may have changed, but the relative ToF changes slowly. Our key idea is that we shift the $\mathbf{h}$ first so that the strongest path is shifted to zero delays and since we know relative to the first path, the delay of the second and third path. We can populate the $\textbf{S}$ matrix with only a few columns, thereby achieving accurate and reliable solutions to $\alpha_k$. We account for the small variations in relative-ToF by trying a few values around the initial value that best fits our model. In summary, we have built an accurate super-resolution algorithm by leveraging the initial relative-ToF information between the multi-beams. 


% The cardinality of the solution space and super-resolution is large and results quite often incorrect solution. 

% Here, we make a key observation that, after training the absolute ToF may have changed, but the relative ToF remains the same after the initial beam training. \todo{giva a scnerio and put numbers how much ToF and relative-ToF changes with mobility.} We can use this observation to narrow the possible number of ToF to solve for just the $K$ paths. 
% Our key idea is that we shift the $\mathbf{h}$ first so that the strongest path 0 delay, and since we know relative to first path the delay of the second and third path. We can actually populate the $\textbf{S}$ matrix with only few columns, and thereby achieving accurate and reliable solutions to $\alpha_k$. 
% \textcolor{blue}{We account for the small variations in relative-ToF by solving (\ref{eq:optim}) for multiple iterations with different values of relative-ToF in our model in a brute-force manner. It converges within xxx iterations in our evaluation.}
% We assume the ToF estimated after beam training phase does not change significantly for a short duration of tracking. 
% In summary, we have build accurate super-resolution algorithm by leveraging the initial relative-ToF information between the multi-beams. 


\noindent
\textbf{Efficiency of super-resolution algorithm:} 
In Figure \ref{fig:superresexample}(a), we show that our super-resolution algorithm can indeed achieve high resolution in estimating per-beam amplitude even when the relative ToF is lower than what corresponds to the resolution (2.5 ns for 400 MHz bandwidth). We also measure the channel impulse response through our testbed (6m link with a reflector placed at 30$^o$) in Figure \ref{fig:superresexample}(b) and show that our super-resolution can efficiently extract the two sinc which are superimposed in the received CIR.



==> Arxiv/5_implementation.tex <==
% !TEX root = main.tex
\vspace{-0.1in}
\section{Implementation}\label{sec:implementation}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/test_setup2.pdf}
%     \caption{We custom design a testbed at 28 GHz with 64 element phased array and an FPGA board for baseband processing.}
%     \label{fig:testbed2}
% \end{figure}
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/test_setup.pdf}
%     \caption{Outdoor and Indoor test scenarios. The far right figure shows our phased array mounted on a gantry system which provides precise translation and rotation motion ground truth information.\newtodo{Only two figure + set up} }
%     \label{fig:test_setup}
% \end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/test_setup_v3.pdf}
    \caption{Shows our experimental setup and Outdoor and Indoor test scenarios. Our phased array is mounted on a gantry system which provides precise translation and rotation motion ground truth information.}
    \label{fig:test_setup}
\end{figure*}

We build a custom mmWave testbed at 28 GHz to evaluate the performance of \name. Our testbed consists of three major components (i) an 8$\times$8 phased array integrated with an RF mixer, (ii) off-the-shelf IF mixer \cite{qorvo} and (iii) FPGA baseband processing with 1Gbps ADCs/DACs \cite{kcu,fmcdaq2}, as shown in Fig. \ref{fig:test_setup}(a). For outdoor experiments, we used USRP X310 with 100 MHz bandwidth. We connect a single phased array with our baseband platform (single-RF chain) to establish analog beam patterns.
We generate OFDM waveforms with 400 MHz effective bandwidth for our evaluation. A host PC handles pre/post data processing and waveform generation. A MATLAB controlled Arduino SPI platform is used to interface with the phased array and enables fast switching of beam patterns. 
We used a Cinetics Axis-360~\cite{axis360} gantry system to measure the precise ground truth of user motion.
% \newtodo{We use a SINGLE RF chain.}


\noindent
\textbf{Beam Pattern Quantization:}
Phase-coherent multi-beam patterns can be generated using minimum 2-bit phase shifters and 1-bit amplitude control (turning antenna on or off) \cite{orfanidis2002electromagnetic, loch2017zero, palacios2018adaptive} which is available in commercial 802.11ad devices~\cite{qualcomm2017wil6210, talonad7200} as well as 28 GHz 5G NR~\cite{samsung_array, raychaudhuri2020challenge}. Having higher resolution in phase and amplitude control helps both the single-beam and multi-beam to reduce side-lobe noise~\cite{}. We demonstrate a high-throughput and reliable mmWave link with our state-of-the-art 64 elements phased arrays built in-house~\cite{jain2020mmobile}. It provides 6 bit of phase control and 27 dB of gain control per antenna element similar to commercial arrays deployed by Samsung \cite{samsung_array} and IBM~\cite{raychaudhuri2020challenge,sadhu2018128} at 28 GHz\footnote{Verizon, Ericsson, \& other commercial vendors deploy high-resolution 28 GHz phased arrays developed by Samsung, IBM \& others \cite{verizon_IBM,verizon_Samsung}}. 



% We build a custom mmWave testbed at 28 GHz to evaluate the performance of \name as shown in Figure~\ref{fig:testbed2}. The testbed~\cite{jain2020mmobile} consists of three main components: (i) Baseband processing module: Gsps digital and analog front-end unit (Analog Devices FMCDAQ2~\cite{fmcdaq2}) connected to a bespoke Baseband processing unit FPGA (Xilinx KCU105)~\cite{kcu}, which is connected to the host PC. (ii) IF module: connects with baseband processing module and consists of the Mixer (Qorvo RFFC5071A~\cite{qorvo}), a High Pass Filter (Mini-Circuits ZFHP-3800ff-S+~\cite{hpf-minicircuits}) and a 15 dB LNA (Mini-Circuits ZX60-P103LN+~\cite{lna-minicircuits}). (iii) Tx/Rx module: connected with the IF module and consists of up-down converters and Tx/Rx transceivers, which are connected to Phased Array Antennas~\cite{kibaroglu201864}, and the DC beam control board. We also used a 28 GHz horn antenna (Pasternack PE9851/2F-10~\cite{horn-pasternack}) for antenna calibration and measuring beam patterns.
% % Our testbed consists of three major components (i) an 8$\times$8 phased array integrated with an RF mixer, (ii) off-the-shelf IF mixer \cite{qorvo} and (iii) FPGA baseband processing with 1Gbps ADCs/DACs \cite{kcu,fmcdaq2}. 
% We generate OFDM waveforms with 400 MHz effective bandwidth for our evaluation. A host PC handles pre/post data processing and waveform generation. A MATLAB controlled Arduino SPI platform is used to interface with the phased array and enables fast switching of beam patterns. 





% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/FPGA_block.pdf}
%     %FPGAblockDiag_crop
%     \caption{Block diagram of a mmWave node in our testbed that has 2 ADC's and 2 DAC's each sampling at 1 Gsps, which is converted to IF stage of 3.5 GHz and then signal is provided to TX module which upconverts to 28 GHz and is connected to phased array with 64 antenna. The node can configured to be transmit/receive with a switch.}
%     \label{fig:testbed}
% \end{figure}
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.44\textwidth]{figures/exptSetup.jpg}
% %     %FPGAblockDiag_crop
% %     \caption{Our experiment setup with wooden reflectors and even metal reflectors to help us study the performance}
% %     \label{fig:setup}
% % \end{figure}
 

% The components of our testbed are shown in Figure~\ref{fig:testbed_hw}.  
% % In Figure~\ref{fig:multilobebeampattern}, we show that our multi-beam patterns can be generated effectively and can be implemented on our mmWave phased arrays. We next discuss the individual components of our testbed.


% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=.95\linewidth]{figures/setup_testbed.pdf}
% %     %FPGAblockDiag_crop
% %     \caption{Shows the setup of the mmWave testbed, show base-band processing unit, IF module and the phased array Tx/Rx module.}
% %     \label{fig:testbed_hw}
% % \end{figure}

% \textbf{Baseband module:} This module is used to generate OFDM waveforms with 400 MHz effective bandwidth. The host PC handles pre/post data processing and waveform generation. The control FPGA is programmed to carry samples to and from the FMCDAQ2. It interfaces to the host PC using a PCIe interface, to take full advantage of the 1 Gsps sampling rate of the ADC/DAC. Due to the simple single-channel mixer used in the IF module, we use only the I-channel of the FMCDAQ2. We digitally encode the complex baseband conjugate symmetrically in both the upper and lower sidebands to create a real baseband signal compatible with the mixer. After the IF stage, the lower sideband is rejected using a high pass filter. Therefore, the module can generate complex baseband signals with a bandwidth of half the sampling rate. The bandwidth achieved is representative of real-life implementations like 5G-NR. In baseband reception, the module performs a digital frequency transform and then rejects negative frequencies to retrieve complex baseband information.

% \textbf{IF module:} This module converts the baseband signal to IF and vice versa since our mmWave upconverter operates on an IF of 3.4 GHz. The single-channel output from the DAC is passed into the Qorvo RFFC5071A Mixer, which upconverts the signal to 3.4GHz. The RFFC5071A is a highly customizable dual mixer with simultaneous up and down conversion capabilities. The output of the mixer is High Pass Filtered (Mini-Circuits - ZFHP-3800FF+), to reject the image caused due to single-channel upconversion. The downconversion side of the module is fed to an LNA and has no special filter.
 
% \textbf{Tx/Rx module:} The module consists of an external LO running at 12.25 GHz and a frequency doubler, producing a 24.5 GHz clock. The output of the IF stage is up/downconverted directly using the clock to generate an RF signal at 27.9 GHz of FR2. The upconverter chain drives the TX phased array antenna while the RX phased array antenna is driven by the downconverter chain. A DC board regulates the currents and voltages of the phased array and communicates with the 8x8 beamformer ICs. A MATLAB controlled Arduino SPI platform is used to interface with the DC board and enables fast switching of beam patterns. 

\review{he authors should include a more detailed description of their testbed to allow others to reproduce the same results.
}
\newtodo{We will provide a more detailed description of our testbed which is elaborated in our previous mmNets’20 paper. }

\noindent
\textbf{Hardware impairments:}
In a practical system, the unsynchronized clocks may cause CFO (Carrier frequency offset), which is eliminated using traditional methods before calculating the CSI. 
Also, SFO (Sampling frequency offset) does not change too much overtime for the super-resolution algorithm to take that into account. Note that every few seconds, the mmWave link reperforms the initial beam training and synchronizes the transceivers.

\review{One more issue is that I am not sure if the comparison is really fair. mmReliable uses a flexible phase controlled array and you can tune the phase on each antenna elements to generate arbitrary pattern. But most commerical phased array provides only a limited set of beam patterns. I think the authors might want to make this clear.
}
\newtodo{The reviewer asked how multi-beam weights can be realized using a codebook. Since multi-beam weights are a combination of two or more single beam weights, they can be quickly generated in real-time on FPGAs using a codebook of single beams. If computation is at a premium, the multi-beam patterns can be stored in the codebook. We will discuss these practical approaches in the paper. }
%Since our system relies on the complex amplitude per beam of the received signal, which is calculated using super-resolution on relative time-of-flight and not on the phase in any fashion, CFO does not impact us.

==> Makefile <==
TARGET           ?= main
TARGET_TYPE      ?= pdf
LATEXMK          ?= latexmk
LATEXDIFF        ?= latexdiff-vc

ifneq ($(V), 1)
Q                := @
LATEXMK_FLAGS    += -silent
else
Q                :=
LATEXDIFF_FLAGS  += -V
endif

UNAME_S          := $(shell uname -s)
TARGET_FILE       = $(TARGET).$(TARGET_TYPE)
TARGET_DIFF       = $(TARGET)-diff$(LATEXDIFF_BASE)

LATEXMK_FLAGS    += -$(TARGET_TYPE) -f

# Reference git branch/tag
LATEXDIFF_BASE   := submission2
LATEXDIFF_STYLE  := TRADITIONAL
# NOTE: vc-version does not take preamble
LATEXDIFF_FLAGS  += --git --flatten --force -r $(LATEXDIFF_BASE) 
LATEXDIFF_IGNORE := author,authornote,email,affiliation,institution,ccsdesc,renewcommand,section,subsecion,subsubsection
LATEXDIFF_NOENV  := (?:picture|DIFnomarkup|align|comment|CCSXML|thebibliography|figure|equation|tabular)[\w\d*@]*
LATEXDIFF_FLAGS  += --exclude-textcmd='$(LATEXDIFF_IGNORE)'

ifeq ($(shell which $(LATEXMK)), )
$(error "Please install `$(LATEXMK)`!")
endif
ifeq ($(shell which $(LATEXDIFF)), )
$(warning "Please install `latexdiff` or `latexdiff-vc` to use `make diff` function!")
endif

.PHONY: clean view check diff

$(TARGET_FILE): $(wildcard *.tex *.bib *.sty *.cls figures/*)
	@echo "Compiling..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET)

clean:
	@echo "Cleaning..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET) -C
	$(Q) rm -f $(TARGET).bbl $(TARGET_DIFF).bbl
	$(Q) if test -f $(TARGET_DIFF).tex; then $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF) -C; rm $(TARGET_DIFF).tex; fi

view: $(TARGET_FILE)
ifeq ($(OS), Windows_NT)
	$(Q) open $(TARGET_FILE)
else
ifeq ($(UNAME_S), Linux)
	$(Q) xdg-open $(TARGET_FILE) &
endif
ifeq ($(UNAME_S), Darwin)
	$(Q) open $(TARGET_FILE) &
endif
endif

check: $(TARGET_FILE)
	$(Q) grep -i -e "undefined" -e "multiply" $(TARGET).log || echo "Nothing found."

# NOTE: latexdiff will not work with IEEEtran style
diff: clean
	@echo "Compiling diff..."
	$(Q) $(LATEXDIFF) $(LATEXDIFF_FLAGS) $(TARGET).tex
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF)

